Geometric and General Relativistic Techniques for Non-relativistic Quantum Systems

This thesis explores the application of differential geometric and general relativistic techniques to deepen our understanding of quantum mechanical systems. We focus on three systems, employing these mathematical frameworks to uncover subtle features within each. First, we examine Unruh radiation in the context of an accelerated two-state atom, determining transition frequencies for a variety of accelerated trajectories via first-order perturbation theory. For harmonic motion of the atom in a vacuum, we derive transition rates with potential experimental realizations. Next, we investigate the quantum Hall effect in a spherical geometry using the Dirac operator for non-interacting fermions in a background magnetic field generated by a Wu-Yang monopole. The Atiyah-Singer index theorem constrains the degeneracy of the ground state, and the fractional quantum Hall effect is studied using the composite fermion model, where Dirac strings associated with the monopole field supply the statistical gauge field vortices. A unique, gapped ground state emerges, yielding fractions of the form $\nu = \frac{1}{2k+1}$ for large particle numbers. Finally, we examine the AdS/CMT correspondence through a bulk fermionic field in an RN-AdS$_4$ background (with a U(1) gauge field), dual to a boundary fermionic operator. Spherical and planar event horizon geometries are discussed, with the temperature of the RN black hole identified with that of the dual system on the boundary. By numerically solving for the spectral functions of the dual theory, for a spherical event horizon at zero temperature, we identify a shift in the Fermi surface from that which arises in the planar case. Preliminary evidence of a phase transition emerges upon examining these spectral functions, again for the spherical horizon, at non-zero temperature.

==> Chapter_1/Chpt_1.1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}
\label{chpt_1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Intro 1}

The field of Black Hole thermodynamics was the first significant marriage of quantum field theory and general relativity. The effect of Black Hole radiation, first investigated by S.Hawking [cite-Hawking 1975], began by considering quantum field theories in curved spaces. This  gave rise to many fields and along with those interest in string theories and higher dimensional microscopic objects in an effort to unify the known phyiscal forces was a consequence. Hawking's contribution, to express that black holes have a kind of analgous thermodynamics to thermodynamical systems we are used to in conventional physical scenarios, was just the start of the investigation into the importance of how geometric considerations impact quantum systems. This work encouraged W.G.Unruh to consider a metric where no blackhole was present. That you need only reparameterise the coordinates of flat minkowski space, such that you get the trajectory for an accelerated observer to witness what is aptly named Unruh radiation [cite-Unruh 1976]. This discovery is significant in that it affords scenarios in which this phenonomena, or variations thereof, could be experimentally verified. It is quiet difficult to locate primordial Black Holes and more difficult still to observe their radiation. Black Hole radiation aside, Unruh Radiation itself requires massive acceleration to acheive even $1\degree K$. This does not spell out a hopeless scenario though. Efforts made by [cite-Svidzinsky and Fulling papers] have looked at the possibility of extending the scheme laid out by Unruh and others to excite photons from a two-state atom (TSA). The model which formed the basis for our research was that which included a mirror that the TSA would accelerate towards (and the alternate version of an accelerated mirror), and calculating the probability of transition from an excited state in a vaccum to a ground state with a photon now present [cite-Svidzinsky]. We then looked at the possible generalisations of this scenario, a crucial point being where the relativistic accelaration was supplemented for simple harmonic motion, allowing us to look at more feasible conditions to observe this stimulation in a laboratory setting. Below I will outline the scheme for which this possible vaccum emission might be achieved. To begin with though we will proceed by reveiwing the geometry of rindler coordinates, and the quantized scalar field which gives rise to the Unruh Temperature. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Intro 2}

The study of quantum fields in curved space time has led to profound new discoveries including Hawking radiation and the Unruh \cite{Unruh1976} effect. The latter typically is discussed for the case of an uniformly accelerated observer or detector in the vacuum of flat Minkowski spacetime. The accelerated detector (which we take to be a two level system - TLS), rather than seeing the vacuum, instead experiences a thermal photon bath whose temperature $T=a\hbar/(2\pi c k_B)$, where $a$ is the proper acceleration of the TLS. One interpretation is that the virtual photons that normally dress  the internal states of such a TLS are promoted to be real excitations due to the highly non-adiabatic nature of the acceleration. Virtual photons can have measurable signatures in atomic physics, e.g. in the Lamb shift and in Raman scattering. However, experimentally observing the Unruh effect has proved challenging since to achieve $T\sim 1{}^\circ$ K, requires an extreme acceleration $a\sim 10^{20} \,{\rm m/s^2}$, and to substantially excite the TLS  the latter should have a transition frequency $\omega_0/2\pi\sim 20\,{\rm GHz}$.
The importance of the Unruh effect and its analogous effect in black holes, Hawking radiation, has led to a number of proposals over the past three decades towards an experimental test of the existence of acceleration radiation.  These proposals include detecting Unruh radiation  via electrons orbiting in storage rings \cite{Bell1983, Bell1987, Unruh1998},  in Penning traps \cite{Rogers1988}, in high atomic number nuclei \cite{Rad2012},  via shifts in accelerating Hydrogen-like atoms \cite{Pasante1998}, via   decay processes of accelerating protons or neutrons \cite{Matsas1999}, or when electrons experience ultra-intense laser acceleration \cite{Chen1999,Schutzhold2006}, by examining the Casimir-Polder coupling to an infinite plane from an accelerating two-level system \cite{Rizzuto2007}. Researchers have also investigated using cavities to enhance the effect \cite{Scully2003, Belyanin2006,Lopp2018}, and using the Berry phase or entanglement as probes of Unruh radiation \cite{Martin-Martinez2011,Hu2012,Tian2017}. With the advent of circuit QED - cQED, researchers have investigated simulations of Unruh radiation via the Dynamic Casimir Effect - DCE, \cite{Johansson2009,Wison2011, delRey2012, Lahteenmaki2013}, or by using cQED to simulate relativistically moving systems \cite{Felicetti2015,Su2017}, and also using NMR \cite{Jin2016} or by studying the interaction between pairs of accelerated atoms \cite{Rizzuto2016}, or via the dynamical Casimir effect \cite{Farias2019}. More recent work has probed  whether real motion can produce acceleration radiation and in \cite{Sanz2018,Wang2019}, the authors consider a mechanical method of modulating the electromagnetic fields in cQED DCE photon production. 


\begin{figure}[tp] 
\begin{center}
\setlength{\unitlength}{1cm}
\begin{picture}(8.5,7)
%\put(.1,-.4){\includegraphics[width=.95\columnwidth]{Figures/Fig1b}}
\put(-2,-.2){\includegraphics[width=.85\columnwidth]{Images/Shaking_Photons/Fig1}}
\end{picture}
\end{center}
\caption{We consider the generation of photons of frequency $\omega$, from a two level system (atom), with internal transition frequency $\omega_0$, mechanically oscillating at frequency $\Omega$ and amplitude $A$, and initially in the ground state with the electromagnetic field in the vacuum. a) oscillating in front of a mirror, b) oscillating inside a cavity, c) oscillating in free space.}
   \label{Fig1}
\end{figure}

In our work we instead consider a model where the centre of mass of a TLS moves in an accelerated manner   that may  be achieved in a laboratory setting e.g. oscillatory motion.  In \cite{Svidzinsky2018} the authors discussed the possibility that a TLS, uniformly accelerating away from a mirror and initially in its ground state, could experience a transition to its excited state
accompanied by the emission of a  photon.   This raises the question of what other kinds of acceleration might lead to such a process? In this paper we show that simple harmonic oscillation of the atom can also result in photon emission accompanied by an excitation from the ground  to the excited state of the TLS. 

{\color{black} Considering acceleration radiation from oscillatory motion has an advantage over continuous linear accelerated motion in that the TLS stays in a compact region and thus should be more feasible for direct experimental implementation.} In the following we derive closed compact expressions for the rate of photon production in the case of an oscillating TLS in the presence of a mirror, or within cavity, or just coupled to vacuum. For the latter we propose a cQED implementation which predicts significant rates of photon production in the microwave regime.
\vspace{.25cm}\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Rindler Coordinates}

The study of hyperbolic motion in Minkowski spacetime i.e. the case of rectilinear motion with \emph{constant} proper acceleration has been an important field arising from the study of the specific geometric properties of Minkowski spacetime. Moreover it has also crucially played a role in the understanding of general relativistic phenomena, the motion near an event horizon being of clear significance and relevance for our purposes. Here we will reveiw some of the relevant geometric properties of Rindler space and hyperbolic motion, for a more complete treatment see [cite- Socolovsky, Wald].

First we look at the familiar global coordinates for Minkowski spacetime, $x^{\mu} = (t,x,y,z)$, where we are using natural units and have set the speed of light $c=1$. The line element is given by
\begin{equation}
ds^2 = -dt^2 + dx^2 + dy^2 + dz^2
\end{equation}
and the metric is of course
\begin{equation}
g_{\mu \nu} = \eta_{\mu \nu} = \begin{pmatrix} -1 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 \\ 0 & 0 & 1 & 0 \\ 0 & 0 & 0 & 1 \end{pmatrix}.
\end{equation}
%The symmetries of this space are those of the ten-dimensional Poincar\acute{e} group. These are translations in space 
Going forward we supress the $y$ and $z$ coordinates and look only at the 1+1 dimensional Minkowski space. The line element is simply
\begin{equation}
ds^2 = -dt^2 + dx^2
\end{equation}
We can define lightcone coordinates $(u,v)$ as follows 
\begin{align}
u &= t - x \\
v &= t + x
\end{align}
where it's clear to see that in Minkowski coordinates, for constant $u$ or $v$, we get straight lines with a slope of $\pm 1$, i.e. the speed of light. To solidify this understanding we can look at the line element in these coordinates
\begin{equation}
ds^2 = dudv = \frac{1}{2}(du \otimes dv + dv \otimes du)
\end{equation}
which gives the metric as 
\begin{equation}
g_{\mu \nu} = \begin{pmatrix} 0 & \frac{1}{2} \\ \frac{1}{2} & 0\end{pmatrix}.
\end{equation}
From this we can see that the vectors $\frac{\partial}{\partial u}$ and $\frac{\partial}{\partial v}$ have length $g(\partial_{u},\partial_{u}) = g(\partial_{v},\partial_{v}) = 0 $. Thus $\frac{\partial}{\partial u}$ and $\frac{\partial}{\partial v}$ are null vectors as expected. Clearly a grid of these coordinates, in $x-t$ space, show that at the intersection of each line we have the lightcone for an obeserver at that event (see figure).  

Now when considering rectilinear motion with constant proper acceleration in Minkowski space we first look at the change of the components of the 4-velocity. Let $U^{\mu} = (\gamma, \gamma \vec{u})$ where $\vec{u}$ is the 3-velocity, where $\gamma$ is the usual Lorentz factor $\gamma = \frac{1}{\sqrt{1-u^2}}$. From this we can define a 4-acceleration by simply taking the time derivative, with respect to the proper time, of $U^{\mu}$
\begin{equation}
A^{\mu} = \frac{dU^{\mu}}{d\tau} = \gamma \frac{dU^{\mu}}{dt} = \gamma \left(\frac{d\gamma}{dt}, \frac{d(\gamma \vec{u})}{dt}\right)
\end{equation}
where the relationship between coordinate time and proper time is used, $d\tau = ds = \sqrt{-\eta_{\mu \nu}dx^{\mu}dx^{\nu}}= \sqrt{1-\left(\frac{dx}{dt}\right)^2}dt = \frac{dt}{\gamma}$. The components of the 4-acceleration can be split in to their time and spatial coordinates
\begin{equation}
A^{0} = \gamma \frac{\gamma}{dt}, \quad \vec{A} = \gamma \frac{\gamma \vec{u}}{dt}.
\end{equation}
For an instantaneously co-moving inertial reference frame, i.e. the frame in which the observer is instantaneously at rest [footnote reference to Andrew Steane p.61], $\gamma=1$ and the 4-acceleration becomes 
\begin{equation}
A^{\mu} = \left(0, \frac{d\vec{u}}{dt}\right) = (0,\vec{a}) 
\end{equation}
where $\vec{a}$ is the proper acceleration of the observer. Hyperbolic motion, as previously mentioned, is defined when the proper acceleration is constant. If again we restrict ourselves to 1+1 dimensional Minkowski space and look at the differential equation obtained for the proper acceleration we have 
\begin{equation}
a = \text{constant} = \frac{d(\gamma v)}{dt}  
\end{equation}
with $a =\lvert \vec{a} \rvert$. The first integral is immediate and, along with the initial condition that $v(0)=0$, we have
\begin{equation}
at = \frac{v(t)}{\sqrt{1-v(t)^2}}, \quad \rightarrow v(t) = \frac{at}{\sqrt{1+(at)^2}}. \label{rind.1}
\end{equation}
As $v(t) = \frac{dx}{dt}$ we can again integrate this expression with respect to $t$ to give
\begin{equation}
x(t) = a\int^{t}_{0} \frac{\tilde{t}d\tilde{t}}{\sqrt{1+(a\tilde{t})^2}}= \frac{1}{a}\sqrt{1+(at)^2} \label{rind.2}
\end{equation}
and thus the trajectory of the observer undergoing constant proper acceleration is a hyperbola
\begin{equation}
x^2 - t^2 = (1/a)^2. \label{rind.3}
\end{equation}
Note that for the equation of the trajectory \eqref{rind.2} above we are now confined to the region which is bounded by the light cone $u = 0$ for $t>0$ and $v=0$ for $t<0$, or more concretely $x \ge \vert t \vert$. This is known as the right Rindler wedge ($R$) of 1+1 dimensional Minkowski space, or Rindler space. It is also evident that the trajectories for observers with constant proper acceleration $a$ are asymptotic to these lines, the worldlines of photons. The region beyond these lines, $x \le \vert t \vert $ are inaccesible to these accelerated observers, and thus these lines are effectively event horizons for this observer. This is a motivating factor for us to look at the effect of an accelerated observer's in quantum vaccua.

First though, recall the relationship between the proper time and coordinate time $d\tau = \frac{dt}{\gamma}$. Using \eqref{rind.1} and integrating we have
\begin{equation}
\tau = \int^{t}_{0} d\tilde{t} \sqrt{1-v(\tilde{t})^2} = \int^{t}_{0} \frac{d\tilde{t}}{\sqrt{1+(a\tilde{t})^2}} = \frac{1}{a}\sinh^{-1}(at)
\end{equation} 
and thus have the coordinates for a uniformly accelrated observer in terms of their proper time
\begin{align}
t &= \frac{1}{a}\sinh(a\tau) \\
x &= \frac{1}{a}\cosh(a\tau) 
\end{align}
where we have gotten the eqaution for the $x$ coordinate from subbing our expression for $t$ in to \eqref{rind.3}. Dimensional analysis reveals the factors of $c$ that are required. 
\newpage
The equations then look like
\begin{align}
t &= \frac{c}{a}\sinh(\frac{a\tau}{c}) \\
x &= \frac{c^2}{a}\cosh(\frac{a\tau}{c}) 
\end{align}
these equations will be of particular relevance for our discussion about the acclerated two state atom. Setting $c=1$ again, more general rindler coordinates take the form 
\begin{align}
t &= \frac{e^{\alpha \xi}}{\alpha}\sinh(\alpha\eta) \label{rind.coord.1}\\
x &= \frac{e^{\alpha \xi}}{\alpha}\cosh(\alpha\eta) \label{rind.coord.2}
\end{align}
where, for constant $\xi$, we have the trajectories for accelerated observers in Minkowski space, as can be seen from \ref{fig1}.
\begin{figure}[h]
  \includegraphics[scale=0.17]{Images/Shaking_Photons/Rindler_graph.png}
  \caption{Trajectories for Rindler Coordinates}
  \label{fig1}
\end{figure} 
\newpage
The relationship between the proper acceleration and $\alpha$ is given by
\begin{equation}
a = \alpha e^{-\alpha \xi}
\end{equation}
and the proper time is related to $\eta$ via 
\begin{equation}
\tau = \frac{\alpha}{a} \eta = e^{\alpha \xi} \eta.
\end{equation}
In these coordinates the line element takes the form
\begin{equation}
ds^2 = e^{2a\xi}(-d\eta^2 + d\xi^2)
\end{equation}
which displays that this coordinate transformation is a conformal transformation of Minkowski space. This fact will be useful when looking at a massless scalar field in Rindler space.
Finally looking at one last coordinate transformation, $\rho = \frac{e^{\alpha \xi}}{\alpha}$  we recover the familiar rindler space line element 
\begin{equation}
ds^2 = -(\alpha \rho)^2 d\eta^2 + d\rho^2. \label{rind.4}
\end{equation}
This sequence of coordinate transformations has an intimate relationship with the Schwarzchild metric. There is an apparent sigularity in the inverse metric at $\rho = 0$, but this singularity is not essential but a consequence of our coordinates. If one were to work backwards through these transformations from the final equation above \eqref{rind.4} we would arrive at Minkowski space and find no such singularity. Minkowski space is thus the maximally extended space-time of Rindler space. Analogously the apparent singularity in Schwarzchild metric can too be transformed away given the correct choice of coordinates, those being Kruskal–Szekeres coordinates. These coordinates cover the entire spacetime manifold  of the maximally extended Schwarzchild solution. Therefore given the insight from Hawking to analyse the behaviour of quantum fields near the event horizon of a Schwarzchild black hole it seems natural to then attempt to apply a similar scheme to the above for an accelerated observer. This will be the task for the next section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Unruh Radiation}

There are number of ways to begin the calculations that lead to the Unruh effect. A good introduction to the thermodynamics of a black hole and a pretty neat and concise calculation can be found in [cite-A.Zee, QFT-Nut], albeit not particularly illuminating as to the origins of these effects. Interestingly the nature of the calculation is to essentially approximate the Schwarzchild metric near the horizon, which results in the above rindler metric, and to introduce imaginary time. Approximating the Schwarzchild space with Rindler space was also Unruh's motivation and what lead to the discovery of the Unruh effect. To provide a brief introduction to this effect we will begin by first looking at the solutions for a massless scalar field and then their vacua in different coordinate systems, following a similar scheme to that which can be found in [cite- B. Dolan, Group Theory Approach]. More complete treatments can be found in [cite- Unruh, Notes on BH; Socolovsky, Rind and Unruh Rad; Crispino et al., Unruh Effect and Applications]. 

The Klein-Gordon equation is often the starting point when embarking on the study of quantum field theory. It follows from varying the action
\beq
\mathbf{S} = \int d^{4}x \mathcal{L} 
\eeq
where the langrangian density $\mathbf{L}= \int d^{3}x \mathcal{L}$. For a massless, classical, scalar field theory, $\mathcal{L}$ in a curved space-time is
\beq
\mathcal{L} = -\half \sqrt{-g}\del_{\mu} \phi\del^{\mu} \phi = -\half \sqrt{-g} g^{\mu \nu}\del_{\mu} \phi\del_{\nu} \phi.
\eeq
The Euler-Lagrange equations (the equations of motion) are then
\beq
g_{\mu \nu} \del^{\nu} \del^{\mu} \phi = 0
\eeq 
where, for Minkowski space-time, the derivative operator just becomes the d'Alembertian operator. Actually, as this is a massless scalar field and our coordinates \eqref{rind.coord.1}, \eqref{rind.coord.2} are a conformal transformation of the metric, our equations of motion are both 
\beq
(\partial^{2}_{x}- \partial^{2}_{t})\phi = (\partial^{2}_{\xi}- \partial^{2}_{\eta})\phi = 0. \label{K.G._eq}
\eeq
Note again though that our coordinates $\eta$, $\xi$ are only defined in the right Rindler wedge. Now $\phi$ can be decomposed, in the Rindler coordinates, into a complete set of orthonormal solutions $u_i$, with coefficients $a_i$
\beq
\phi = \sum_i a_i u_i(\eta,\xi) + a^{*}_i u^{*}_i(\eta,\xi).
\eeq
A separate, yet equivalent set of othornormal solutions can also be found for the decomposition of $\phi$ in the Minkowski frame. We label these functions $u'_j$ and have coefficients $a'_j$ and $\phi$ can then be written
\beq
\phi = \sum_i a'_{i} u'_i(t,x) + a'^{*}_i u'^{*}_i(t,x).
\eeq
Obviously each element of these sets of functions satisfy \eqref{K.G._eq}. Looking at normalised right moving wave solutions to this equation, for the rindler observer, we have
\beq
u_i = \frac{1}{2\sqrt{\pi\omega_{i}}}e^{i\omega_{i}(\xi-\eta)}
\eeq
where the $\omega$'s are labelled by the summation variable, which we supress from here. We can find the coefficients of these functions via Fourier transforming along the world-line of the rindler observer. By this I mean; for a fixed $\xi = \xi_0$ and $\eta$ being the proper time for our rindler observer, $d\eta$ is tangent to this trajectory, integrating along it thus gives us our desired Fourier coeffiecients
\beq
a_{i} = e^{-i \omega \xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{i \omega \eta} \phi(\eta,\xi_{0})d\eta.
\eeq
The complex conjugates of the above functions and coefficients are straightforward. Now we can can relate the coefficients of these functions in these alternate coordinate systems ( with what amounts to essentially a change of basis) by
\beq
a_{i} = \sum_{j} \alpha_{ij} a'_{j} + \beta_{ij} a'_{j}
\eeq
where, upon quantizing our field, $\alpha_{ij}$ and $\beta_{ij}$ are the Bogoliubov transformation coefficients [cite-Bogoliubov]. These coefficients are found to be
\begin{align}
\alpha_{ij} =& e^{-i\omega\xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{i\omega\eta} u'_{j}(\eta,\xi_{0})d\eta \\
\beta_{ij} =& e^{i\omega\xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{-i\omega\eta} u'_{j}(\eta,\xi_{0})d\eta. \label{Unruh_1}
\end{align}
Quantizing our field, the details of which we won't go through, $\phi$ becomes an operator on the Hilbert space of quantum states and our fourier coefficients become the familiar creation and annihilation operators $\hat{a_i}^{\dagger}$, $\hat{a_i}$ respectively. These Hilbert spaces have there own vacua defined as
\beq
\hat{a_i} \ket{0_{R}} = 0
\eeq
for Rindler space and
\beq
\hat{a'_i} \ket{0_{M}} = 0
\eeq
for Minkowski space. Note that, as we have already stated that these coefficients, now operators, are related via a basis change, we can act on the Minkowski vacuum with the creation operator in the Rindler coordinates and vice versa. Moreover we can define a number operator, $\hat{N}_{i}=\hat{a_i}^{\dagger}\hat{a_i}$ in the Rindler coordinates and it is then a straightforward calculation to see that
\beq
\bra{0_{M}}\hat{N}_{i} \ket{0_{M}} = \sum_{j} \vert \beta_{ij} \vert^{2}
\eeq
or in words, the particle number is \emph{observer dependent}, provided $\beta_{ij}\neq 0$. Let us go about calculating this quantity from \eqref{Unruh_1}. Subbing in for $u'_{j}$ we have
\begin{align}
\beta_{ij} =& e^{i\omega\xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{-i\omega\eta} \left( \frac{1}{2\sqrt{\pi\omega'}}e^{i\omega'(x-t)}\right)d\eta \\
=& \frac{e^{i\omega\xi_{0}}}{2\pi}\sqrt{\frac{\omega}{\omega'}}\int_{-\infty}^{\infty} e^{-i\omega\eta} e^{(i\omega'/ \alpha) e^{\alpha(\xi_{0}-\eta)}}d\eta
\end{align}
where we have used the fact that $x-t=e^{\alpha(\xi - \eta)}/\alpha$ from \eqref{rind.coord.1}. Introducting a change in integration variable $iy = \frac{\omega'}{\alpha}e^{\alpha(\xi - \eta)}$ our integral becomes
\beq
\beta_{ij} = \frac{e^{-\frac{\pi\omega}{2\alpha}}}{2\pi\alpha}\sqrt{\frac{\omega}{\omega'}}e^{i\frac{\omega}{\alpha}\ln{(\frac{\alpha}{\omega'})}}\int_{0}^{-i\infty} y^{\frac{i\omega}{\alpha}-1} e^{-y} dy
\eeq
Which, when rotating the contour onto the real axis, we have 
\begin{align}
\beta_{ij} &= \frac{e^{-\frac{\pi\omega}{2\alpha}}}{2\pi\alpha}\sqrt{\frac{\omega}{\omega'}}e^{i\frac{\omega}{\alpha}\ln{(\frac{\alpha}{\omega'})}}\int_{0}^{\infty} y^{\frac{i\omega}{\alpha}-1} e^{-y} dy \\
&= \frac{e^{-\frac{\pi\omega}{2\alpha}}}{2\pi\alpha}\sqrt{\frac{\omega}{\omega'}}e^{i\frac{\omega}{\alpha}\ln{(\frac{\alpha}{\omega'})}} \Gamma(\frac{i\omega}{\alpha})
\end{align}
Now the quantity $\vert \beta_{ij} \vert^{2}$ is then
\beq
\vert \beta_{ij} \vert^{2} = \frac{\omega e^{-\frac{\pi\omega}{\alpha}}}{4\pi^{2}\alpha^{2}\omega'}\frac{\pi}{\frac{\omega}{\alpha}\sinh{(\frac{\pi\omega}{\alpha})}} = \frac{1}{2\pi\alpha\omega'}\frac{1}{e^{\frac{2\pi\omega}{\alpha}}-1} \label{Unruh_2}
\eeq
where we have used the fact that $\vert\Gamma(iy)\vert^{2} = \frac{\pi}{y\sinh{\pi y}}$. It is clear that we have a Bose-Einstein distribution from equation \eqref{Unruh_2}. It is then natural to associate a temperature with the factor in the exponential term to put it in this form
\beq
T = \frac{\hbar\alpha}{2\pi k_{B}}
\eeq
and this is the Unruh temperature.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Accelerated Two State Atoms}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Paper intro to work we work from}

{\color{black}\section{\it\bf Evaluating the probability to emit a photon under general non-relativistic motions:-} We now show how to derive the probability for the two-level system, moving in one dimension along a pre-set space-time trajectory, in the presence of a mirror, to become excited and emit a photon using first order perturbation theory.  Using the derived expression we first confirm that if the two level system is at rest the probability to emit a photon is zero. In the subsequent subsections we consider various other types of motions.} Following \cite{Svidzinsky2018}, we consider a two level system, or atom, coupled to the  electromagnetic field with a coupling strength $g$, and atomic transition frequency  $\omega_0$, so the excitation energy is $\Delta E=\hbar \omega_0>0$. 
For simplicity we consider motion in
one-dimension given by position $z(t)$ 
\footnote{Unlike \cite{Svidzinsky2018} our analysis will be non-relativistic and $t$ is just ordinary Newtonian time, not proper time --- the calculation can be done relativistically but there is no need for such a complication. If we assume a mechanical oscillation frequency $\Omega/2\pi \sim\, 10\, {\rm GHz}$, and a maximum amplitude of oscillation as $A\sim 10 {\rm nm}$, then the maximum velocity achieved of the atom is $v_{max}\sim 600\, {\rm m/s}\ll c$. As we show below we predict that these parameter values will yield significant acceleration radiation.}  
In the interaction picture the Hamiltonian for the interaction of the atom with the electric field
 $\phi_\omega$, is \cite{Svidzinsky2018},
%\[ H_I(t) = \hbar g\bigl\{a_\omega \phi_\omega(t,z(t))
%+ a^\dagger_\omega \phi^*_\omega(t,z(t)) \bigr\}
%\bigl(\sigma_- e^{-i\omega_0 t} + \sigma_+ e^{i\omega_0 t}  \bigr)
%\]
\begin{eqnarray}H_I(\omega,t) = \hbar g\bigl\{a_\omega \phi_\omega(t,z(t))
+ a^\dagger_\omega \phi^*_\omega(t,z(t)) \bigr\}\\\label{noSMA}
\times \bigl(\sigma_- e^{-i\omega_0 t} + \sigma_+ e^{i\omega_0 t}  \bigr)\label{Hamomega}
\end{eqnarray}
where $\sigma_+$ raises the internal atomic state and $\sigma_-$ lowers it, $a_\omega^\dagger$, $a_\omega$ are photon creation operator and annihilation operators and
$\phi_\omega$ are field modes that depend on the boundary conditions. {\color{black} We note that (\ref{Hamomega}), describes the interaction at a specific frequency $\omega$, and the full Hamiltonian is obtained by $H_I(t)\equiv \int\,H_I(\omega, t)\,d\omega$, and thus our treatment encapsulates the potential excitation of any wavelength radiation. In what follows we compute the probability to excite the atom and emit a photon of frequency $\omega$, where the latter is not taken as a fixed quantity.}
{\color{black} This interaction has been used numerous times in the literature to model the coupling between a two-level atom and a quantum field but here we do not make the rotating wave approximation and  the position of the atom is allowed to vary in time. Further, we permit the photon field mode frequency $\omega$ to be arbitrary and thus the the atom can couple to vacuum modes of any frequency. This is unlike the so-called ``single mode approximation''  (SMA), where authors consider the atom to couple preferentially to a small number of modes concentrated at a single frequency e.g. for an atom within an accelerating cavity \cite{Alsing2003, FSchuller2005, Alsing2006, Datta2009, Wang2010, Dragan2011, Hwang2012, Brown2012, Lopp2018}. Research has shown that making the SMA can lead to difficulties in superluminal propagation effects at strong couplings \cite{Sanchez2018}, and entanglement generation \cite{Bruschi2010}, however some works have  explored beyond the SMA including an NMR analogue simulation of Unruh radiation \cite{Jin2016} [2 modes].    }
If the two level system is moving on the entire real line and its position is a function of $t$, we would use right and left moving field modes
\bea \phi_\omega=e^{-i (\omega t \mp  k z(t))}, \label{eq:infinite-phi}  \eea
where $k=\omega/c>0$, is the $z$-component of the photon's wave-vector.
In the presence of a mirror fixed at $z=z_0$, we would instead use
\beq \phi_\omega=e^{-i(\omega t - k z(t) + k z_0)}- e^{-i (\omega t + k z(t) - k z_0)},\label{eq:mirror-phi}\eeq
thus ensuring that the photon field, and hence the transition amplitude,  vanishes when $z(t)$ is an integer multiple of the wavelength and the atom is at a node of the field.  In a cavity of length $L$, we would again use 
(\ref{eq:mirror-phi}), but the frequency and wave-vector would be restricted by the condition that  $k=\omega/c=2 \pi   n/L$ for some positive integer $n$.
We shall work with (\ref{eq:mirror-phi}) on the half-line for the moment,
and later adapt  the results to the case of a cavity or the entire real line as in (\ref{eq:infinite-phi}). 
In first order perturbation theory the probability of exciting the atom (via the raising operator $\sigma_+ e^{i\omega_0 t}$ in the interaction), and at the same time creating  a photon {\color{black}  of frequency $\omega$ }
via the $\hat a^\dagger \phi_\omega^*$,
%$$\hat a^\dagger \phi_\omega^*=  \bigl( e^{i(\omega t + k z(t) - k z_0)} - e^{i(\omega t - k z(t))+ k z_0} \bigr) \hat a^\dagger$$
term in the interaction potential, is given by 
\beq P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (z(t)- z_0)} -c.c. \bigr] e^{i \omega t + i \omega_0 t}
d t \right|^2 .\label{eq:phi-mirror}\eeq
{\color{black} If the atom is at rest, $z$ is constant and  the integral gives $\delta(\omega + \omega_0)$, which is zero since $\omega>0$ and $\omega_0>0$.  Thus $P=0$, and the probability to become excited and emit a photon vanishes. We now use the expression (\ref{eq:phi-mirror}), in the following to consider other types of space-time motions $z(t)$, to discover how they can give rise to non-vanishing probabilities $P$.}
\vspace{.25cm}\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Acceleration towards a mirror: Brian and My Calculations}

So here's my current understanding of 
A.A.~Svidzinsky, J.S.~Ben-Benjamin,~S.A. Fulling, and D.N. Page
{\it Phys. Rev. Lett.} {\bf 121}, 071301 (2018).

For simplicity set $c=1$ so $k=\frac{2 \pi }{\lambda}=\omega$
where $\omega$ is the angular frequency and $\lambda$ the wavelength of the emitted photon. $\omega_0$ is the angular frequency of the transition between the two internal states of the atom ($\omega$ and $\omega_0$ are both positive, Fulling an Page use $\nu$ and $\omega$ respectively).
The trajectory of the atom undergoing constant acceleration $a$ in its own instantaneous rest frame (proper acceleration) is
 $$ t(\tau) = \frac{1 }{a}\sinh(a \tau), 
\qquad z(\tau) = \frac{1 }{a}\cosh(a\tau) \eqno{(1)}. $$ 
The probability of exciting the atom (via the raising operator $\hat\sigma_+ e^{i\omega_0 t}$ in the interaction potential) and at the same time creating  a photon 
(via the 
$$\hat a^\dagger \phi_\omega^*=  \bigl( e^{i(\omega t + \omega z - \omega z_0)} - e^{i(\omega t - \omega z +\omega z_0)} \bigr) \hat a^\dagger$$
in the interaction potential) is given by 
Svidzinsky {\it et al}'s equation (2), 
$$ P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i \omega (z(\tau)-z_0)} -c.c. \bigr] e^{i \omega t(\tau) + i \omega_0 \tau}
d \tau \right|^2  ,\eqno{(2)}$$
If the atom is at rest $z$ is constant and $t=\tau$, then if there no mirror
the $c.c.$ term is missing --- the integrals give $\delta(\omega + \omega_0)$,
which is zero since $\omega>0$ and $\omega_0>0$.  

From (1) 
$$\pm z(\tau) + t(\tau) =  \pm\frac{1}{a}e^{\pm a\tau},$$
so the integral is
\begin{eqnarray*}
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau 
-&&\kern -27pt\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{-a\tau}} e^{i\omega z_0}  e^{i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau 
-\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{a\tau}} e^{i\omega z_0}  e^{- i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau -c.c.
\end{eqnarray*}
where we've changed integration variable $\tau \rightarrow -\tau$ in the second
integral.
So 
$$ P= g^2 \left|
\int_{-\infty}^\infty\bigl[e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}
 -c.c. \bigr] d \tau
\right|^2 .$$

Now change integration variables from $\tau$ to $x=\frac{\omega }{a} e^{a\tau}$, so
$d \tau = \frac{1}{a x} d x $,
$$
\int_{-\infty}^\infty e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{ i \omega_0 \tau} d\tau
=\frac{1}{a} e^{-i \bigl(\omega z_0 - \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\bigr) }
\int_0^\infty e^{i x}  x^{i\frac{\omega_0}{ a}-1 }d x.
$$
Now consider the integrals
$$I_\pm
=\int_0^\infty e^{\pm i x}  x^{\pm i\frac{\omega_0}{a}-1} d x.$$
Let $x= \pm i u = e^{\pm \frac{i\pi }{2}} u$ and $z = \pm \frac {i\omega_0}{ a}$, then
$$I_\pm =e^{-\frac {\pi \omega_0 }{2 a}}\int_0^{\mp i\infty} e^{-u}  u^{z-1} d u.$$
This is almost a $\Gamma$-function, except the integrals are along the imaginary 
axis rather than the real axis. 
Provided $\Re z>0$ (so $\omega_0 \rightarrow \omega_0 \mp  i \epsilon$ with
$\epsilon >0$) we can rotate the contour to get\footnote{Imagine doing a integral round a slice of pie with
opening angle $90^\circ$ and vertex at the origin, in the SE quadrant for the upper sign and the NE quadrant for the lower sign. There is a branch point at the origin
but this is harmless provided $\Re z>0$ as usual for $\Gamma$-functions.
The exponential kills the integral around the quarter-circle at infinity.}
$$ \int_0^{\mp i\infty} e^{-u}  u^{z-1} d u = \int_0^{\infty} e^{-u}  u^{z-1} d u = \Gamma(z), \qquad \Re z>0,$$
and
$$ I_\pm\left(\frac{\omega_0 }{a}\right) =e^{-\frac{\pi \omega_0 }{2a}}
\lim_{\epsilon\rightarrow 0^+} \Gamma\left(\pm \frac{i \omega_0 }{a} + \frac{\epsilon}{a}\right) =  e^{-\frac{\pi \omega_0 }{2a}}\Gamma\left(\pm\frac{i \omega_0 }{a}\right),$$

Write
$$ \Gamma\left(\pm\frac{i \omega_0 }{a}\right) = e^{\pm i\psi}\left|\Gamma\left(\pm\frac{i \omega_0 }{a}\right)\right|.$$
The phase $\psi$ will depend on $\frac{\omega_0 }{a}$, we don't know it's analytic form, but that doesn't matter.
What we do know is
$$ \left|\Gamma\left(\pm \frac{i \omega_0 }{a}\right)\right|^2 =\frac {a \pi }{\omega_0\sinh\left(\frac { \pi\omega_0 }{a}\right)},$$
which is all we need to write the probability as
\begin{eqnarray}
P&=&\frac{\pi g^2 e^{-\frac{\pi \omega_0 }{a}} }{a \omega_0 \sinh\left(\frac{\omega_0 }{a}\right)}
\left|e^{-i \Bigl(\omega z_0 - \frac{\omega_0}{a}\ln\bigl((\frac{a }{\omega}\bigr)\Bigr) }e^{i\psi}
- e^{i \Bigl(\omega z_0 - \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\Bigr) }e^{-i\psi} 
\right|^2   \\
&=&  
\frac{4 \pi g^2  \sin^2(\omega z_0 - \varphi) }{a \omega_0 e^{\frac{\pi \omega_0 }{a}} \sinh\left(\frac{\omega_0 }{a}\right)}=  \frac{8 \pi g^2}{a \omega_0} \frac{\sin^2(\omega z_0 - \varphi) }{e^{\frac{2\pi \omega_0 }{a}}-1}
\end{eqnarray}
where 
$$\varphi = \frac{\omega_0}{a} \ln \left(\frac{a}{\omega } \right) + \psi.$$ 

So, were confident that equation (2) is correct and we can play around with it for any trajectory. We'll use this and the paper intro to stitch 'em together. This is the work we're working from.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Probabilities from other initial states:}

From A.A.~Svidzinsky, J.S.~Ben-Benjamin,~S.A. Fulling, and D.N. Page
{\it Phys. Rev. Lett.} {\bf 121}, 071301 (2018), a probability is derived for the case in which a two state atom is excited from it's ground state via Unruh radiation and it emits a photon. From the interaction Hamiltonian given in the above paper there are four possible probabilities which can be calculated; The case mentioned above (from equation (2)), the case where the atom is in the excited state, absorbs a photon and then moves to the ground state, spontaneous emission and finally absorption of a photon. It is worth looking at each of the three cases, relativistically and for the SHO, to obtain the probabilities for these scenarios. 

The interaction Hamiltonian is given as:
$$\hat V(\tau) = {\hbar} {g} ({\hat a}{\phi_\omega} + {\hat a^\dagger}{\phi_\omega^*})({\hat \sigma}{e^{-i\omega_0\tau}} + {\hat \sigma^\dagger}{e^{i\omega_0\tau}})$$
Using this to treat each scenario we have
\subsection{The relativistic second case: Moving from the excited state to the ground state and absorbing a photon}
The probability is
$$P = g^2 \left|
\int_{-\infty}^\infty\bigl d \tau\bra{0,b}\hat V(\tau)\ket{1_\omega,a} \right|^2$$
This gives
$$P = g^2 \left|\int_{-\infty}^\infty\bigl d \tau [e^{-i \omega (z(\tau) - z_0)} - c.c.] e^{-i \omega t(\tau) - i \omega_0 \tau} \right|^2$$
Sending $\tau \rightarrow -\tau$ yields
$$P = g^2 \left|-\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{i \omega t(\tau) + i \omega_0 \tau} \right|^2$$
Which is just equation (2) with a difference in minus sign. So the probability is the same as the first case done in section 0.1.

\subsection{Relativistic third case: Spontaneous emission}
$$P = g^2 \left|
\int_{-\infty}^\infty\bigl d \tau\bra{1_\omega,b}\hat V(\tau)\ket{0,a} \right|^2$$
yields
$$P = g^2 \left|\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{i \omega t(\tau) - i \omega_0 \tau} \right|^2$$
following similar calculations as section 0.1
From (1) 
$$\pm z(\tau) + t(\tau) =  \pm\frac{1}{a}e^{\pm a\tau},$$
so the integral is
\begin{eqnarray*}
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{-i \omega_0 \tau}  d \tau 
-&&\kern -27pt\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{-a\tau}} e^{i\omega z_0}  e^{-i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau 
-\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{-a\tau}} e^{i\omega z_0}  e^{- i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau -c.c.
\end{eqnarray*}
where we've changed integration variable $\tau \rightarrow -\tau$ in the first integral. So 
$$ P= g^2 \left|
\int_{-\infty}^\infty\bigl[e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}
 -c.c. \bigr] d \tau
\right|^2 .$$

Now change integration variables from $\tau$ to $x=\frac{\omega }{a} e^{-a\tau}$, so
$d \tau = \frac{-1}{a x} d x $,
$$
\int_{-\infty}^\infty e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{ i \omega_0 \tau} d\tau
=\frac{1}{a} e^{-i \bigl(\omega z_0 + \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\bigr) }
\int_0^\infty e^{i x}  x^{-i\frac{\omega_0}{ a}-1 }d x.
$$
Now consider the integrals
$$I_\pm
=\int_0^\infty e^{\pm i x}  x^{\mp i\frac{\omega_0}{a}-1} d x.$$
Let $x= \pm i u = e^{\pm \frac{i\pi }{2}} u$ and $z = \mp \frac {i\omega_0}{ a}$, then
$$I_\pm =e^{\frac {\pi \omega_0 }{2 a}}\int_0^{\mp i\infty} e^{-u}  u^{z-1} d u.$$
This is almost a $\Gamma$-function as in section 0.1, except the integrals are along the imaginary 
axis rather than the real axis. 
Provided $\Re z>0$ (so $\omega_0 \rightarrow \omega_0 \pm  i \epsilon$ with
$\epsilon >0$) we can rotate the contour to get
$$ \int_0^{\mp i\infty} e^{-u}  u^{z-1} d u = \int_0^{\infty} e^{-u}  u^{z-1} d u = \Gamma(z), \qquad \Re z>0,$$
and
$$ I_\pm\left(\frac{\omega_0 }{a}\right) =e^{\frac{\pi \omega_0 }{2a}}
\lim_{\epsilon\rightarrow 0^+} \Gamma\left(\mp \frac{i \omega_0 }{a} + \frac{\epsilon }{a}\right) =  e^{\frac{\pi \omega_0 }{2a}}\Gamma\left(\mp\frac{i \omega_0 }{a}\right),$$
Write
$$ \Gamma\left(\mp\frac{i \omega_0 }{a}\right) = e^{\mp i\psi}\left|\Gamma\left(\mp\frac{i \omega_0 }{a}\right)\right|.$$
The phase $\psi$ will depend on $\frac{\omega_0 }{a}$, we don't know it's analytic form, but that doesn't matter.
What we do know is
$$ \left|\Gamma\left(\mp \frac{i \omega_0 }{a}\right)\right|^2 =\frac {a \pi }{\omega_0\sinh\left(\frac { \pi\omega_0 }{a}\right)},$$
the probability then is
\begin{eqnarray}
P&=&\frac{\pi g^2 e^{\frac{\pi \omega_0 }{a}} }{a \omega_0 \sinh\left(\frac{\omega_0 }{a}\right)}
\left|e^{-i \Bigl(\omega z_0 + \frac{\omega_0}{a}\ln\bigl((\frac{a }{\omega}\bigr)\Bigr) }e^{-i\psi}
- e^{i \Bigl(\omega z_0 + \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\Bigr) }e^{i\psi} 
\right|^2   \\
&=&  
\frac{4 \pi g^2  \sin^2(\omega z_0 + \varphi) }{a \omega_0 e^{\frac{-\pi \omega_0 }{a}} \sinh\left(\frac{\omega_0 }{a}\right)}=  \frac{8 \pi g^2}{a \omega_0} \frac{\sin^2(\omega z_0 + \varphi) }{1-e^{\frac{-2\pi \omega_0 }{a}}}
\end{eqnarray}
where 
$$\varphi = \frac{\omega_0}{a} \ln \left(\frac{a}{\omega } \right) + \psi.$$

So $P$ is divergent for $a \rightarrow 0$

\subsubsection{Relativistic fourth case: Absorption of a photon}

The probability is 
\begin{eqnarray}
P&=& g^{2} \left|
\int_{-\infty}^\infty\bigl d \tau\bra{0,a}\hat V(\tau)\ket{1_\omega,b} \right|^2   \\
&=&  
g^2 \left|-\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{-i \omega t(\tau) + i \omega_0 \tau} \right|^2
\end{eqnarray}
If we send $\tau \rightarrow -\tau$ $P$ becomes
$$=g^2 \left|-\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{i \omega t(\tau) - i \omega_0 \tau} \right|^2$$
Which is the same as the third case case.

\subsubsection{Second case for non-relativistic SHO:\bra{0,b}\hat V\ket{1_\omega,a}}

$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{-i k (A \sin(\Omega \tau)-z_0)} - c.c. \bigr] e^{-i \omega \tau - i \omega_0 \tau} d \tau
\right|^2. $$
sending $\tau \rightarrow -\tau$
$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau) + z_0)} -c.c. \bigr] e^{i \omega \tau + i \omega_0 \tau} d \tau
\right|^2. $$
Which is the probability for the first SHO case done in sections 0.2 and 0.3 with $z_0 \rightarrow -z_0$.

\subsubsection{Third case for non-relativistic SHO: \bra{1_\omega,b}\hat V\ket{0,a}}

$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau)-z_0)} - c.c. \bigr] e^{i \omega \tau - i \omega_0 \tau} d \tau
\right|^2. $$

this is the first case for the SHO with $\omega_0 \rightarrow -\omega_0$.

\subsubsection{Fourth case for non-relativistic SHO:\bra{0,a}\hat V\ket{1_\omega,b}}

$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{-i k (A \sin(\Omega \tau)-z_0)} - c.c. \bigr] e^{-i \omega \tau + i \omega_0 \tau} d \tau
\right|^2. $$
send $\tau \rightarrow -\tau$
$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau)+z_0)} - c.c. \bigr] e^{i \omega \tau - i \omega_0 \tau} d \tau
\right|^2. $$
again this is the first case for the SHO but now with $ \omega_0 \rightarrow -\omega_0$ and $z_0 \rightarrow -z_0$. 

The above are variations of the possible quantum states that arose from the initial setup by [cite: Svidzinsky et. al.]. This setup though now affords us a more thorough setting from which we can analse other trajectories for a particle, allowing us to more generally tackle an accelerated quantum state by simply imposing an accelerated trajectory instead of needing to specify the potential providing the energy for the acceleration. In the next sections we play around with non-relativisitic trajectories arrived at through our relativistic setup and find that we arrive at feasible probabilities that give rise to acceleration radiation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{\it\bf Oscillating 2-state atom with a mirror :-}\label{mirror}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Oscillating Atom from Paper}

%\label{sec:mirror}
We now consider an atom forced to oscillate in the presence of a stationary mirror, the latter located at $z_0$, oscillating with a motional angular frequency $\Omega$,  around $z=0$
with amplitude $0<A<z_0$ 
(so we do not hit the mirror),  and set $ z(t) = A \sin(\Omega t).$
%$$ z(t) = A \sin(\Omega t).$$
Using this in (2), the probability of creating a photon of frequency
$\omega$ from the vacuum, and at the same time exciting the atom from its ground state to its excited state is
$$P(\omega)= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega t) - z_0)} -c.c. \bigr] e^{i (\omega +  \omega_0)t} d t
\right|^2. $$
Simplify the notation by absorbing $\Omega$ into $t$ and defining dimensionless variables 
$\tau = \Omega t$, $\tilde \omega = (\omega +\omega_0)/\Omega$,
$\tilde A = k A$ and $\tilde z_0 = k z_0$, we obtain
\begin{eqnarray} P(\omega) &=& \frac{g^2}{\Omega^2} \left|
\int_{-\infty}^\infty\bigl[
e^{i (\tilde A \sin \tau - \tilde z_0)} -c.c. \bigr] e^{i \tilde \omega \tau} d \tau\right|^2 \nonumber\\ 
&=& \frac{g ^2}{\Omega^2} \left|
e^{-i\tilde z_0}\int_{-\infty}^\infty e^{i (\tilde A \sin \tau+ \tilde \omega \tau)} d \tau \right.\nonumber\\ 
& &\qquad\qquad\left.-e^{i\tilde z_0}\int_{-\infty}^\infty  e^{i (\tilde A \sin \tau - \tilde \omega \tau)} d  \tau\right|^2.
\label{totalSHO-probability} 
\end{eqnarray}

The integrals appearing in (\ref{totalSHO-probability}) 
 are related to
Anger functions \cite{Abramowitz1970} (section 12.3.1),
$$ {\bf J}_\nu(x)=\frac{1}{2\pi}\int_{-\pi}^\pi e ^{i(x \sin\theta - \nu \theta)}d \theta
= \frac{1}{\pi}\int_0^\pi \cos(x\sin\theta - \nu\theta)d \theta.$$
But Anger functions are not quite what we want since what we have in (\ref{totalSHO-probability})
, is
\begin{eqnarray}
\int_{-\infty}^\infty  e ^{i(x \sin\theta - \nu \theta)} d \theta
&=&\!\! \sum_{s=-\infty}^\infty\, \int_{-\pi}^\pi e^{i\bigl(x \sin\theta - \nu(\theta+2s\pi)\bigr)}d \theta \\
&=&\!\! \pi {\bf J}_\nu(x) \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}.
\label{eq:totalamplitude}
\end{eqnarray}
Letting $ \nu = n + \{\nu\}$, 
%$$ \nu = n + \lfloor\nu\rfloor$$
where $n$ is an integer, and $0 \le  \{\nu\}<1$, is the non-integral part of $\nu$,
then
$ \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}= \sum_{s=-\infty}^\infty  e^{-2is\{\nu\}\pi} = 1 + 2\sum_{s=0}^\infty  \cos(2s\{\nu\}\pi) = \pi \delta(\{\nu\})$
and (\ref{eq:totalamplitude}), vanishes unless $\nu$ is an integer, in which case it
diverges. This is not unexpected since when Fermi's Golden Rule says that if the transition rate is constant, integrating over all $t$ will necessarily give an infinite answer for any transition with non-zero probability.  For our periodic case its more informative to estimate a transition rate over a motional cycle rather than the accumulated  probability over all time.

\sloppy Before estimating this let us consider the case when $\nu$ is a non-zero rational number, $\nu = p/q$ with $p$ and $q$ mutually prime and positive, in the integral
$$ \int_{-\infty}^\infty e^{i(x\sin \theta -\nu \theta)} d \theta
= q \int_{-\infty}^\infty e^{i(x\sin (q \psi)  - p \psi)} d \psi 
$$
where $\psi = \theta/q$. The integrand is periodic in $\psi$
with period $2\pi$ so again the integral will diverge (unless the integral over one period vanishes).  Integrating over just one period in $\psi$, we can define
\begin{eqnarray}
{\cal J}(x;p,q) &=& 
\frac{1}{2 \pi} \int_{-\pi}^\pi e^{i(x \sin (q \psi)  - p \psi )} d \psi\\\nonumber
&=& \frac{1}{\pi} \int_0^\pi \cos\big\{x \sin (q \psi)  - p \psi \bigr\} d \psi,
\label{eq:J-def}
\end{eqnarray}
which, in terms of Anger functions, becomes
\begin{eqnarray}
{\cal J}(x;p,q) &=& 
\frac{1}{2 \pi q} \int_{-q\pi}^{q \pi} e^{i(x \sin \theta  - \frac p q  \theta )} d \theta \\\nonumber
&=&\frac{1}{q}  {\bf J}_{\frac p q }(x)\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}}.\nonumber
\end{eqnarray}
We note however that $$\sum_{s=0}^{q-1} \exp({i \pi (2 s - q + 1)p/q}) = 
\exp({-i\pi\frac{p(q-1)}{q}}) \sum_{s=0}^{q-1} \exp({2i \pi p s/q})=0,$$ 
%$$
%\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}} = 
%e^{-i\pi\frac{p(q-1)}{q}} \sum_{s=0}^{q-1} e^{\frac{2i \pi p s}{q}}=0 
%$$
since $\sum_{s=0}^{q-1} \exp(2i \pi p s/q)$,
vanishes for any two integers $p$ and $q$, provided $p/q$ is not an 
integer.
 From this observation we conclude  that the transition rate is zero unless $\tilde \omega$ is a
positive integer, that is 
\begin{equation}
\omega + \omega_0 = n\Omega,\label{eq:Omega-restriction}
\end{equation}
where $\Omega$ is the mechanical frequency, $\omega_0$ is the atomic transition frequency, $\omega$ is the frequency of the photon field and $n$ is an integer.
Since $\tilde \omega$ is  positive, $n>0$, and to obtain a closed expression for the transition probability over a mechanical cycle we can use the integral
representation of the Bessel function,  \cite{Abramowitz1970} (section 9.1.21),
$J_n (\tilde A) = \frac{1}{2 \pi}\int_{-\pi}^{\pi} 
\exp[{i(\tilde A \sin \tau - n \tau)}] d \tau = (-1)^n J_{-n}(\tilde A)$,
%\[
%J_n (\tilde A) = \frac{1}{2 \pi}\int_{-\pi}^{\pi} 
%e^{i(\tilde A \sin \tau - n \tau)} d \tau = (-1)^n J_{-n}(\tilde A)
%\]
to write  $\int_{-\pi}^{\pi} \exp [{i(\tilde A \sin \tau + \tilde z_0 -  n  \tau)} ]d \tau= 2 \pi e^{i \tilde z_0}  J_n(\tilde A)$, and $\int_{-\pi}^{\pi} \exp[{i(\tilde A \sin \tau -
 \tilde z_0 +  n \tau)} ]d  \tau
= 2 \pi e^{-i (\tilde z_0 - n \pi)}  J_n(\tilde A)$.
%\begin{eqnarray*}
%\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tau + \tilde z_0 -  n  \tau)} d \tau
%&=& 2 \pi e^{i \tilde z_0}  J_n(\tilde A)\\
%\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tau -
% \tilde z_0 +  n \tau)} d  \tau
%&=& 2 \pi e^{-i (\tilde z_0 - n \pi)}  J_n(\tilde A).
%\end{eqnarray*}
By dividing by the period of mechanical oscillation, $2\pi/\Omega$, we get a transition rate (in ${\rm Hz}$), as
\begin{eqnarray}
\overline P_{n} & = &\frac{\Omega }{2 \pi}
\frac{g^2}{ \Omega^2} \left|
 \Bigl[ 2 \pi \left(e^{-i (\tilde z_0 - n \pi)} -  e^{i \tilde z_0}\right) \Bigr]
J_n(\tilde A)\right|^2\nonumber\\
&=&
\frac{8 \pi g^2}{\Omega} \sin^2\left(\tilde z_0 -\frac{\pi n}{2}\right) J_n^2(\tilde A)\\
&=&
\frac{8 \pi g^2}{\Omega} \sin^2\left(k z_0 -\frac{\pi n}{2}\right) J_n^2(k A),\label{eq:mirror-rate}
\end{eqnarray}
where $\omega = n \Omega - \omega_0 >0$. 
\vspace{.25cm}\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\subsection{Oscillating 2-state atom}

So let's take an oscillating atom. If the motion is relativistic we can use the
anharmonic trajectory, described in 
W.~Moreau, R.~Easther and R.~Neutze, {\it American Journal of Physics} {\bf 62}, 531 (1994) in terms of elliptic integrals.  But first lest just do non-relativistic
simple harmonic motion.  So
$$ t = \tau, \qquad z(\tau) = A \sin(\Omega \tau) + z_0, $$
with angular frequency $\Omega$ and  the amplitude $0<A<z_0$ so we don't hit the mirror!  Put this in (2), with $c$ re-instated so $k c = \omega$,
$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau)-z_0)} -c.c. \bigr] e^{i \omega \tau + i \omega_0 \tau} d \tau
\right|^2. $$
Simplify the notation by absorbing $\Omega$ into $\tau$ and defining 
$\tilde \tau = \Omega \tau$, $\tilde \omega = \frac{\omega +\omega_0}{\Omega}$,
$\tilde A = k A$ and $\tilde z_0 = k z_0$.
These are all dimensionless variables, in terms of which 
$$ P = \frac{g^2}{\Omega^2} \left|
\int_{-\infty}^\infty\bigl[
e^{i (\tilde A \sin \tilde \tau-\tilde z_0)} -c.c. \bigr] e^{i \tilde \omega \tilde \tau} d \tilde \tau\right|^2 =    
\frac{4 g^2}{\Omega^2} \left|
\int_{-\infty}^\infty\sin\bigl(\tilde A \sin \tilde \tau-\tilde z_0\bigr) 
e^{i \tilde \omega \tilde \tau} d \tilde \tau\right|^2. $$
Alternatively
\begin{eqnarray} 
P(\tilde A,\tilde z_0; \tilde\omega) &=& \frac{g^2}{\Omega^2} \left|
e^{- i\tilde z_0}\int_{-\infty}^\infty
e^{i (\tilde A \sin \tilde \tau+ \tilde \omega \tilde \tau)} d \tilde \tau 
- e^{i\tilde z_0}\int_{-\infty}^\infty e^{- i (\tilde A \sin \tilde \tau - \tilde \omega \tilde \tau)} d \tilde \tau\right|^2\nonumber \\
&=& \frac{g^2}{\Omega^2} \left|
e^{- i\tilde z_0}\int_{-\infty}^\infty
e^{i (\tilde A \sin \tilde \tau+ \tilde \omega \tilde \tau)} d \tilde \tau 
- e^{i\tilde z_0}\int_{-\infty}^\infty e^{i (\tilde A \sin \tilde \tau - \tilde \omega \tilde \tau)} d \tilde \tau\right|^2\label{eq:total-SHO-probability}
\end{eqnarray}
where we have changed integration variables from $\tilde \tau$ to $-\tilde \tau$ in the 
second integral.

\subsection{Transition rates}

The integrals appearing in (\ref{eq:total-SHO-probability}) are related to
Anger functions (Abromowitz+Stegun: 12.3.1; {\tt https://dlmf.nist.gov/11.10})
$$ {\bf J}_\nu(x)=\frac{1}{2\pi}\int_{-\pi}^\pi e ^{i(x \sin\theta - \nu \theta)}d \theta
= \frac{1}{\pi}\int_0^\pi \cos(x\sin\theta - \nu\theta)d \theta.$$
Obviously
$$ {\bf J}_{-\nu}(x) =  {\bf J}_{\nu}(-x)$$
and when $\nu=n$ is an integer
$$ {\bf J}_n(x) = J_n(x),$$
a Bessel function of integer order.

Anger functions satisfy the inhomogeneous Bessel equation
$$x^2 
\frac{d^2 {\bf J}_\nu}{d^2 x} + x \frac{d {\bf J}_\nu}{d x}
+(x^2 - \nu^2) {\bf J}_\nu = (x-\nu)\frac{\sin(\nu\pi)}{\pi} 
$$
and a 3D plot as functions of $\nu$ and $x$ are shown in fig. 1.

%\begin{figure}[h]
%\includegraphics[scale=0.5]{Anger-3D}
%\caption{Anger function.}
%\end{figure}

But Anger functions are not quite what we want, what we have is
\begin{equation}
\int_{-\infty}^\infty  e ^{i(x \sin\theta - \nu \theta)} d \theta
= \sum_{s=-\infty}^\infty\left( \int_{-\pi}^\pi e^{i\bigl(x \sin\theta - \nu(\theta+2s\pi)\bigr)}d \theta \right)
= \pi {\bf J}_\nu(x) \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}.
\label{eq:total-amplitude}\end{equation}
Let
$$ \nu = n + \lfloor\nu\rfloor$$
where $n$ is an integer and $0 \le  \lfloor\nu\rfloor<1$ is the non-integral part of $\nu$. 
Then
$$ \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}= \sum_{s=-\infty}^\infty  e^{-2is[\nu]\pi} = 1 + 2\sum_{s=0}^\infty  \cos(2s\lfloor\nu\rfloor\pi) = \delta(\lfloor\nu\rfloor)$$
and (\ref{eq:total-amplitude}) vanishes unless $\nu$ is an integer, in which case it
diverges.

We can check this when $\nu$ a rational number, $\nu = \frac{p}{q}$ with $p$ and $q$ mutually prime and positive.  Then
$$ \int_{-\infty}^\infty e^{i(x\sin \theta -\nu \theta)} d \theta
= q \int_{-\infty}^\infty e^{i(x\sin (q \psi)  - p \psi)} d \psi 
$$
where $\psi = \frac{\theta}{q}$. The integrand is periodic in $\psi$
with period $2\pi$ so the integral will diverge (unless the integral over one period vanishes), so integrate over one period in $\psi$ and define
\begin{equation}
{\cal J}(x;p,q) = 
\frac{1}{2 \pi} \int_{-\pi}^\pi e^{i(x \sin (q \psi)  - p \psi )} d \psi
= \frac{1}{\pi} \int_0^\pi \cos\big\{x \sin (q \psi)  - p \psi \bigr\} d \psi.
\label{eq:J-def}
\end{equation}
In terms of Anger functions
$${\cal J}(x;p,q) = 
\frac{1}{2 \pi q} \int_{-q\pi}^{q \pi} e^{i(x \sin \theta  - \frac p q  \theta )} d \theta 
=\frac{1}{q}  {\bf J}_{\frac p q }(x)\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}}.$$
Now 
$$
\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}} = 
e^{-i\pi\frac{p(q-1)}{q}} \sum_{s=0}^{q-1} e^{\frac{2i \pi p s}{q}}=0 
$$
since $\sum_{s=0}^{q-1} e^{\frac{2i \pi p s}{q}}$ vanishes for any two positive integers $p$ and $q$.

We conclude from this that the transition rate is zero unless $\tilde \omega$ is a
positive integer, that is 
\begin{equation}
\omega + \omega_0 = n\Omega,
\end{equation}
this is a genuine quantum phenomena (though $\hbar$ does not appear
explicitly in the formula for the probability.\footnote{I guess it must be hiding in $g^2$, if this is a genuine quantum phenomenon the probability should vanish when $\hbar\rightarrow 0$.})  The divergence when $\nu=\tilde \omega$ is  presumably a consequence of Fermi's Golden Rule: in first order perturbation theory the transition rate is constant, so the total probability integrated over all time will diverge.
Better to calculate probability rate rather than a 
probability. 

Since $\tilde \omega$ is a positive integer, $n>0$, for a transition we can use the integral
representation of the Bessel function,\footnote{Abromowitz+Stegun: 9.1.21.}
\begin{eqnarray*}
J_n (\tilde A) &=& \frac{1}{2 \pi}\int_{-\pi}^{\pi} 
e^{i(\tilde A \sin \tilde \tau - n \tilde \tau)} d \tilde \tau \\
J_{-n}(\tilde A) 
&=&\frac{1}{2 \pi}\int_{-\pi}^{\pi} 
e^{i(\tilde A \sin \tilde \tau + n \tilde \tau)} d \tilde \tau
= (-1)^n J_n(\tilde A),
\end{eqnarray*}
to write
\begin{eqnarray*}
\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tilde \tau +\tilde z_0 -  n \tilde \tau)} d \tilde \tau
&=& 2 \pi e^{i \tilde z_0}  J_n(\tilde A)\\
\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tilde \tau - \tilde z_0 +  n \tilde \tau)} d \tilde \tau
&=& 2 \pi e^{-i (\tilde z_0- n \pi)}  J_n(\tilde A).
\end{eqnarray*}

Dividing by $\frac{2\pi}{\Omega}$, the period of the oscillator, we get a transition rate
\begin{eqnarray}
\overline P_n & = &\frac{\Omega }{2 \pi}
\frac{g^2}{ \Omega^2} \left|
 \Bigl[ 2 \pi \left((-1)^n e^{-i \tilde z_0} -  e^{i \tilde z_0}\right) \Bigr]
J_n(\tilde A)\right|^2\nonumber\\
&=&
\frac{8 \pi g^2}{\Omega} \sin^2\left(\tilde z_0 -\frac{\pi n}{2}\right) J_n^2(\tilde A)=
\frac{8 \pi g^2}{\Omega} \sin^2\left(k z_0 -\frac{\pi n}{2}\right) J_n^2(k A),
\end{eqnarray}
where $\omega = n \Omega - \omega_0 >0$.
Can the $\sin^2\left(k z_0 -\frac{\pi n}{2}\right)$ factor be 
interpreted as some kind of dynamical Casimir effect? 

If there's no mirror
\begin{equation}
\overline P_n  = \frac{\Omega }{2 \pi}
\frac{g^2}{\Omega^2} \left|
\int_{-\pi}^\pi e^{i \tilde A \sin \tilde \tau} e^{i \tilde \omega \tilde \tau} d \tilde \tau
\right|^2 
  = \frac{2 \pi g^2 }{\Omega} J_n^2( k A) ,\qquad n>0.
\label{eq:P_n-no-mirror}
\end{equation}
Even with no mirror you can excite an atom and emit a  photon at the same time by shaking the atom hard enough to supply energy.  
 
Some useful approximations might be (A+S refers to Abromowitz and Stegun)
\begin{eqnarray}
 J_n(x) & \approx& \frac{x^n}{2^n n!}, \qquad x \ll n    (A+S:9.1.7) \\
 J_n(x)&\approx& \sqrt\frac{2}{\pi x} \cos\left( x - \frac{(2 n +1)\pi}{4}\right), 
\qquad x \gg n  (A+S:9.2.1) \\
 J_n(n) & < & \frac{2^{\frac{1}{3}} }{3^{\frac{2}{3}}} \Gamma\left(\frac{2}{3}\right) 
n^{\frac{1}{3}}
\approx\frac{0.683 }{n^{1}{3}}, \qquad n > 0  (A+S:9.1.61). 
\end{eqnarray}
This last bound was improved to 
$$\sup_x |J_n(x)| < \frac{0.674885 }{n^{\frac{1}{3}}}$$ in L.J.~Landau, {\sl Bessel Functions: Monotonicity and Bounds}, \hfill\break
{\it Journal of the London Mathematical Society}, {\bf 61}, issue 1 (2016).
Empirically the maximum is near $x\approx n$, to less than 10\% for $n$ greater than about 25, for $n=1$ the maximum is $\approx 0.582$ at $x\approx 1.84$. 

\subsection{Atom performing SHO in free space}

The transition rate (\ref{eq:P_n-no-mirror}) with  $\omega = n\Omega - \omega_0$ is 
$$\overline P_n= \overline P(n \Omega - \omega_0)  
  = \frac{2 \pi g^2 }{\Omega} J_n^2\left(\frac { (n \Omega -\omega_0)  A }{c}\right),$$
where the speed of light has been re-instated. This is plotted on figure 2
for various values of $n$, with the factor $\frac{2 \pi g^2}{\Omega}$ omitted.

%\begin{figure}[h]
%\centerline{\includegraphics[scale=0.4]{BesselJ-squared}}
%\centerline{\includegraphics[scale=0.4]{BesselJ-100-squared}}
%\caption{Transition rate for SHO forced atom in free space to emit a photon with angular
%frequency $\omega = n\Omega - \omega_0$ and wavelength $\lambda=\frac{2\pi c}{\lambda}$ (\ref{eq:P_n-no-mirror})
%as a function of $\tilde A =\frac{2\pi}{\lambda} A$. The factor 
%$\frac{2 \pi g^2}{\Omega}$ is omitted and the upper plot just shows the first three Bessel functions,
%$J_n^2(\tilde A)$ for $n=1,2,3$.
%If $\Omega \ll\omega_0$ then $n$ must be large for $\omega>0$ and the lower
%plot shows $J_{100}^2(\tilde A)$, We see that is negligible until $\tilde A$ is of order $n$.}
%\end{figure}
%
Using (\ref{eq:P_n-no-mirror}) and the above approximations the transition rate is
\begin{equation}
\overline P = 
\begin{cases}
\frac{2 \pi g^2}{\Omega} 
\frac{(k A)^{2 n}}{2^{2n} (2n)!}, &  A \ll \frac{n \lambda }{2 \pi};\\
\frac{2 \pi g^2}{\Omega} \frac{(0.683)^2}{n^{\frac{2}{3}}}, & 
A \approx \frac{n \lambda }{2 \pi} \hbox{for} n>25;\\
 \frac{2 g^2 \lambda}{\pi \Omega A }\cos\left(k A -\frac {(2 n +1)\pi}{4 } \right),   &   A \gg \frac{n \lambda }{2 \pi}. 
\end{cases}
\end{equation} 
 
The largest value that $J_n(x)$ can take is 0.582 when $n=1$ and  $x=1.481$
and this is only achievable if $\Omega > \omega_0$, assuming this is the case
the highest transition rate is 
$$\overline P_1 = \frac{2 \pi g^2}{\Omega} (0.582)^2 \approx \frac{2.1 g^2 }{\Omega},$$ for  photons with $\omega = \Omega - \omega_0$, and this is only 
achieved by tuning the oscillation amplitude to 
$$A= \frac{1.481 \lambda }{2 \pi}= \frac{1.481 c }{(\Omega - \omega_0)}.$$


If $\Omega < \omega_0$ then the largest transition rate depends on how much less.
Let $n$ be the smallest integer for which $\omega = n \Omega - \omega_0 >0$.
Then
$$\overline P_n = \frac{2 \pi g^2 }{\Omega} \frac{(0.683)^2}{n^{\frac{2}{3}}} $$
for 
$$ A=\frac{n c }{(n \Omega - \omega_0)}.$$
 
To get an idea of numbers lets consider (5) and assume that the transition frequency of the atom $\omega_0$ and the frequency of the emitted photon $\omega$ 
are both in the optical (visible) range.
Then $\Omega = \frac{\omega + \omega_0 }{n}$, which would probably be in the ultraviolet for $n=1$, but would be in the visible for $n=2$ and is lower for larger $n$.
We can make $\Omega$ as low as we wish by taking $n$ as large as we wish. 
For $n=2$ the maximum of $J_2(x)$ is close to $x=3$, so if $\Omega$ is in the
optical the probability rate (5) is a maximum for 
$A\approx \frac{3}{k} = \frac{3 \lambda }{2 \pi}$, 
of the order of a thousand ${\buildrel _{\circ} \over {\mathrm{A}}}$, %$\AA$ 
a thousand times bigger than the atom itself.  But even if that is feasible the transition is suppressed by a
factor $\Omega \sim \omega$, which is of order $10^{15}$ Hz. 
How big can $g^2$ be
in a real experiment? ($g^2$ has dimensions of inverse time$^2$.)   

If $\Omega$ is to be much lower than optical
frequency then $n$ must be large.  As $n$ increases the first (and largest) peak in $J_n(x)$
moves out to larger $x\approx n$ and the maximum rate is for $A\approx \frac{n \lambda }{2 \pi}$.  If we want $\Omega<<\omega$ then $n>>1$ and we can
use (6) to get a maximum value for the transition rate
$$\overline P_n \approx \frac{3 \pi g^2}{\Omega n^{\frac{2}{3}}} =
\frac{3 \pi g^2 n^{\frac{1}{3}}}{(\omega + \omega_0)}  \qquad \hbox{for}\qquad A = \frac{n \lambda}{2 \pi}.$$
For fixed $\omega$ and $\omega_0$, $\overline P$ grows like $n^{\frac{1}{3}}$ and can be made large by taking $\Omega<<\omega_0$. This is not a problem,
 $n$ is large but $\omega$ also large, so $\overline P_n$ is not growing with $n$,
we can't fix $\omega$ and let $n$ grow.


\subsection{Oscillating mirror}

However, if there is a mirror we can try keeping the atom fixed and oscillating the mirror.  If we don't bother with the distinction between Rindler and
Boulware vacua for small accelerations (wouldn't know what they were for
oscillatory motion anyway!) I would naively assume that we just replace $z(\tau)-z_0$ 
with $z-z_0(\tau)$ where $z_0(\tau) = A\sin(\Omega t)$ is the position of the
mirror and $z$ (constant) the position of the stationary atom.
Also $\omega t(\tau)+\omega_0 \tau \rightarrow\omega \tau+\omega_0 t(\tau)$,
but non-relativistically  $t(\tau)=t$ so no change there.
The only effect is to replace
$z_0$ in (4) with the position of the atom, $z$, and otherwise (4) is unchanged. 

Jason said that boundary conditions mimicking an accelerating mirror can be cooked up in the lab
without having to mechanically accelerate a physical mirror.
Fulling and Wald talk about microwave transitions for $\omega_0$  ($0.3\sim 300$ GHz) and effective couplings $g_{eff}\sim 10$ MHz.
If we assume $\omega$ is also in the microwave region (so $\lambda\approx 0.1 \sim 100$ cm) then,
$\frac{ g_{eff}^2 }{(\omega + \omega_0)}\approx  10^3 \sim 10^5$ Hz.
 and transition rate is of order
For $n>10$, the Bessel function has a maximum
pretty close to $k A = n$, with $J_n(n)\approx \frac{0.675 }{n^{\frac{1}{3}}}$,
giving a transition probability
$$\overline P \approx \frac{11.5 \,g^2_{eff} }{\omega+\omega_0} n^{\frac{1}{3}}
\sin^2\left( k z - \frac{\pi n}{2}\right) \approx  10^5 \sin^2\left( \frac{2 \pi  z}{\lambda}-\frac{\pi n}{2}\right) n^{\frac{1}{3}}.$$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Generalisations and Other Setups: Stimulation from mechanical oscillation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\it\bf 2-dimensional motion}


The formalism can be applied to a 2-level atom following any closed trajectory $\vec x(t)$ in the two dimensional $y-z$ plane, with a flat mirror located at $z_0$ extending in the $y$-direction.   For an electromagnetic wave with wave-vector $(k_y,k_z)$ we simply replace $k (z(t) - z_0)$ in (\ref{eq:phi-mirror}) with
$\vec k.\vec x(t) - k_z z_0$. One cannot obtain analytic answers for a general trajectory but some simple cases are immediate:
\vspace{.25cm}\\


{\it\bf 2-level atom oscillating parallel to a mirror:-}  for oscillation in the $y$-direction replace $k (z(t) - z_0)$ in (\ref{eq:phi-mirror}) with
$ k_y A \sin(\Omega t)  - k_z z_0 $  with $A$ again a constant amplitude.
The analysis is identical and (\ref{eq:mirror-rate}) still holds, but with $k z_0$ replaced with $k_z z_0$ and $k A$ replaced with $k_y A$.
\vspace{.25cm}\\


{\it\bf Rotating 2-level atom with a mirror:-} for an atom rotating around the fixed point $(0,z_0)$ in a circle with radius $R$
and constant angular velocity $\Omega$, $\vec x(t) = R(\cos\Omega t),\sin(\Omega t)$ and
$\vec k.\vec x(t)=k_y R \cos(\Omega t) + k_z R \sin(\Omega t)$.
If we parameterize the direction of the electromagnetic wave by a phase $\delta$ with
 $k_y=k\sin\delta, \quad k_z = k\cos\delta$
then
  $k_y R \cos(\Omega t) + k_z R \sin(\Omega t) - k_z z_0  = k R \sin(\Omega t + \delta) - k z_0 \cos \delta $
and the phase $\delta$ 
in the sine function can be
absorbed into $\tau$ in (\ref{eq:phi-mirror}), which does not affect the result. We just replace the
amplitude $A$ in (\ref{eq:mirror-rate}) with the rotation radius $R$ and replace 
$k z_0$ with $k_z z_0 \cos \delta$.
\vspace{.25cm}\\


\subsection{\it\bf Oscillating 2-level atom in a cavity:-}\label{cavity}

 In a one-dimensional cavity containing no photons the transition rate to excite the atom and at the same time emit a photon of frequency $\omega$ is still given by (\ref{eq:mirror-rate}), except that the allowed values of $\omega$ are discrete, 
 $\omega = c k = \pi m c/L$,
with $m$ a positive integer and Eqn (\ref{eq:Omega-restriction}) imposes the condition
\[ \frac{\pi m c}{L} + \omega_0=n \Omega\]
on $\Omega$. The rate is enhanced however if the cavity already contains $N$ photons of 
frequency $\omega$, since then $\langle N+1|a^\dagger_\omega|N\rangle = \sqrt{N+1}$,
giving the transition rate to excite/de-excite the atom given $N$ photons in the cavity as,
\begin{equation}
\overline P_{n,m,N,\pm} = 
\frac{8 \pi \chi_\pm\, g^2}{\Omega} \sin^2\left(\frac{\pi m z_0}{L} -\frac{\pi n}{2}\right) J_n^2\left(\frac{\pi m A}{L}\right),\label{eq:cavity-rate}
\end{equation}
where $\chi_+=N+1$, to excite and emit a photon, while $\chi_-=N$ to de-excite the atom and absorb a photon, and
%With $N$ photons in the cavity there is also the possibility of exciting the atom
%and absorbing a photon, with transition rate
%\begin{equation}
%\overline P_{n,m.N,-} = 
%\frac{8 \pi N g_\omega^2}{\Omega} \sin^2\left(\frac{\pi m z_0 \cos\delta}{L} -\frac{\pi n}{2}\right) J_n^2\left(\frac{\pi m A}{L}\right)
%\end{equation}
%with the tuning
 %\begin{equation}
$n \Omega = \omega_0 - \omega = \omega_0 - \pi m c/L$. {\color{black} We note that in order to observe this phenomena one could consider one of the mirror's to be slightly imperfect and then one could perform spectroscopy on the photons leaking from the optical cavity. The signature of the photons created via (\ref{eq:cavity-rate}), will prove challenging to detect over any background of existing photon occupation within the cavity.}
%\end{equation}
\vspace{.25cm}\\

\begin{figure}[tp] 
\begin{center}
\setlength{\unitlength}{1cm}
\begin{picture}(8.5,7.5)
%\put(.1,-.4){\includegraphics[width=.95\columnwidth]{Figures/Fig1b}}
\put(-2,-.3){\includegraphics[width=.65\columnwidth]{Images/Shaking_Photons/Fig2}}
\end{picture}
\end{center}
\caption{Transition rate for SHO forced atom in free space to emit a photon with angular frequency $\omega = n\Omega - \omega_0$ and wavelength $\lambda={2\pi c}/{\omega}$, equation  (\ref{eq:P_n-no-mirror}), as a function of dimensionless oscillation amplitude $\tilde A =({2\pi}/{\lambda}) A$ and sideband index $n$. The prefactor 
${2 \pi g^2}/{\Omega}$ is omitted.  We see that transition rate is negligible until $\tilde A$ is of order $n$.}
   \label{Fig2}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experimental Scenario}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\it\bf Atom performing SHO in free space:-}\label{free} 

Repeating the analysis of previous section when there's no mirror, the transition rate to emit a   photon is,  using (\ref{eq:infinite-phi}),
\begin{equation}
\overline P_{n,\omega}  = \frac{\Omega }{2 \pi}
\frac{g^2}{\Omega^2} \left|
\int_{-\pi}^\pi e^{i \tilde A \sin \tau} e^{i \tilde \omega \tau} d \tau
\right|^2 
  = \frac{2 \pi g^2 }{\Omega} J_n^2( k A) ,
\label{eq:P_n-no-mirror}
\end{equation}
with $n>0$. Even with no mirror an atom can be excited and emit a photon at the same time by shaking the atom hard enough to supply the required energy.  
The transition rate (\ref{eq:P_n-no-mirror}), with  $\omega = n\Omega - \omega_0$ is 
\begin{equation}
\overline P_{n}
  = \frac{2 \pi g^2 }{\Omega} J_n^2\left(\frac { (n \Omega -\omega_0)  A }{c}\right),
\label{SHOfreespace}  
\end{equation}
and for a given $n$ the rate will be largest at the first peak of $J_n$. From Fig \ref{Fig2}, we observe that for a given $n$, the transition rate is negligible unless $\tilde{A}\sim n$. The maximum rate occurs when $n=1$ and $\tilde{A}\sim 1.8$, and here $\overline P_1\approx 2.1g^2/\Omega$, but to achieve this one must have a mechanical oscillation amplitude of $A\sim 1.8 c/(\Omega-\omega_0)$, which will be extremely large when compared to the highest realistically achievable values of $\Omega-\omega_0$, in an experiment. 

For a possible experimental demonstration of acceleration from a two level atom shaking in a vacuum we instead consider the case when the amplitude of oscillation $A$ is small enough so that the argument of the Bessel function in (\ref{SHOfreespace}), is small and we can use the expansion $J_1^2(x)\sim x^2/4,\; 0<x\ll 1$. To achieve a large rate we consider ultra-strong coupling $g$ of the atom to the continuum where $g=\alpha \omega_0$, with $\alpha\sim 0.2$ and above \cite{Forn-Diaz2016,  Magazzu2018, PuertasMartinez2019, FriskKockum2019, Forn-Diaz2019}. We consider a cQED setup where a two level superconducting artificial atom is placed on a vibrating cantilever/membrane which is ultra-strongly coupled via an inductive coupling to the electromagnetic vacuum of a nearby electromagnetic continuum of a superconducting co-planar waveguide. This is similar to recent experimental work \cite{Viennot2018}. By using a diamond based  nanomechanical resonator one can achieve motional frequencies in the GHz regimes \cite{Gaidarzhy2007,Rodriguez-Madrid2012}. From (\ref{SHOfreespace}),  with the approximation $J_1(x)^2 \sim x^2/4$, the rate is maximised when $\omega_0=\Omega/2$, and taking this for small amplitude oscillations we obtain $\overline P_{1}\approx(\pi A\alpha)^2\Omega^3/(32 c^2)$. Fig \ref{Fig3}, shows that the emission/transition rate for a shaken superconducting two level system can reach values of $\overline P_1\sim 10^{-4}\,{\rm Hz}$, which may be detectable in current cQED setups. {\color{black} One might also consider placing the mechanically oscillating qubit close to a mirror as discussed in Section \ref{mirror}. Oscillatory motion along an arbitrary direction in three dimensions would couple the qubit to both vacuum modes which either have the mirror as a boundary or unbounded vacuum modes (for motion parallel to the mirror). This would result in  emission of photons perpendicular to the mirror (the case treated in Section \ref{mirror}), and in directions parallel to the mirror's plane (the case treated in Section \ref{free}). Such a situation may be difficult to observe experimentally as one must achieve large couplings between the two level system and the continuum. This is possible in the above discussed cQED setup above as the electromagnetic continuum is restricted essentially to be one dimensional.}

{\color{black} We finally compare our results with recent related works. In \cite{Lo2018}, and \cite{Ferrari2019}, the authors respectively consider acceleration radiation from a mechanically oscillating two level system in free space  and the modification of spontaneous emission in a two level system adjacent to an oscillating mirror. However their studies are restricted to the case where $\Omega<\omega_0$, and only multi-photon off-resonant processes play a role in these cases. Such off-resonant processes cannot be captured via our first order perturbative analysis and thus we cannot make any clear comparison with their results. However the work of \cite{Souza2018}, which looks at the radiation emitted from a two-level atom oscillating in free-space, do consider the regime $\Omega>\omega_0$, and include resonant processes and find the  emission of photons with the frequency $\omega_1=\Omega-\omega_0$, but do not find the higher modes $\omega_n=n\Omega-\omega_0$, which we predict to also exist, though with greatly reduced probabilities. To make a more quantitative comparison we study the small photon frequency case when $\omega_1\equiv\Omega- \omega_0$, is small and $\omega_1 A/c\ll 1$.  Making the approximation $J_1(x)^2\sim x^2/4$, for $x\ll 1$, and comparing our rate (\ref{SHOfreespace}), with Eqn (5) \cite{Souza2018}, in this regime, (in the notation of \cite{Souza2018}, this is when $\omega_1\equiv\omega_{\rm cm}- \omega_0$ is small), we find that both rates scale as $\overline P_{1}\sim \Gamma_{\rm MIE}\sim A^2/\Omega$. However in our case we find $\overline P_{1}\sim \omega_1^2$, while in \cite{Souza2018}, $\Gamma_{\rm MIE}\sim \omega_1^3$, a difference which may be due to the differences between the Hamiltonians. In our study we assume the Hamiltonian (\ref{noSMA}),  a  model for coupling between two levels systems and vacuum fields used by many works and which also was used in \cite{Svidzinsky2018}, to derive the Unruh temperature for the case of uniform acceleration, while \cite{Souza2018}, Eqn (1), includes both the normal dipole coupling but also a term linear in the velocity of the two level system. }

\begin{figure}[tp] 
\begin{center}
\setlength{\unitlength}{1cm}
\begin{picture}(8.5,7.5)
%\put(.1,-.4){\includegraphics[width=.95\columnwidth]{Figures/Fig1b}}
\put(-2,-.3){\includegraphics[width=.65\columnwidth]{Images/Shaking_Photons/Fig3}}
\end{picture}
\end{center}
\caption{Transition/emission rate for an atom oscillating with simple harmonic motion in free space as a function of the amplitude of the oscillation  and ultra-strong coupling strengths $\alpha$, where $g=\alpha \omega_0$, taking a mechanical frequency $\Omega/2\pi=10\,{\rm GHz}$, and two level transition frequency $\omega_0=\Omega/2$ (\ref{SHOfreespace}).}
   \label{Fig3}
\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%












==> Chpt_1.1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}
\label{Chpt_1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Overview}

The advent of black hole thermodynamics was the first significant marriage of quantum field theory and general relativity. The microscopic origin of black Hole radiation, first investigated by S.Hawking [cite-Hawking 1975], began by considering quantum field theories in curved space time. This was just the beginning of the investigation in to how geometric considerations impact quantum systems. The success and utility of these considerations have given rise to many fields, undoubtedly the most popular of which is string theory and the effort to unify general relativity and quantum mechanics. 

One of the impacts of these considerations, with which we will be primarily concerned, was the work of W.G.Unruh \cite{Unruh1976}. Unruh considered the case of an uniformly accelerated observer or detector in the vacuum of flat Minkowski spacetime. No black hole required. Instead reparameterised coordinates of flat minkowski spacetime so that give you the trajectory for a linearly accelerated observer to witness what is aptly named Unruh radiation \cite{Unruh1976}. The accelerated detector (which later we take to be a two level system - TLS), rather than seeing the vacuum, instead experiences a thermal photon bath with temperature $T=a\hbar/(2\pi c k_B)$, where $a$ is the proper acceleration of the TLS.
One interpretation of this effect is that the virtual photons that normally dress  the internal states of such a TLS are promoted to be real excitations due to the highly non-adiabatic nature of the acceleration. Virtual photons can have measurable signatures in atomic physics, e.g. in the Lamb shift and in Raman scattering. However, experimentally observing the Unruh effect has proved challenging since to achieve $T\sim 1{}^\circ$ K, requires an extreme acceleration $a\sim 10^{20} \,{\rm m/s^2}$, and to substantially excite the TLS  the latter should have a transition frequency $\omega_0/2\pi\sim 20\,{\rm GHz}$.

Along with this, experimental verification of Hawking radiation is itself a difficult task as the temperature is inversely proportional to the mass of the black hole. Thus the thermally relevant black holes are the most unstable as they radiate away much of their energy. The expectation is that primordial black holes would be the only candidates and, them being remnants of the earlier universe, it's unlikely we will ever find one to test this hypothesis. This does not spell out a hopeless scenario though. The importance of the Unruh effect and its analogous effect in black holes, has led to a number of proposals over the past three decades towards an experimental test of the existence of acceleration radiation. These proposals include detecting Unruh radiation  via electrons orbiting in storage rings \cite{Bell1983, Bell1987, Unruh1998},  in Penning traps \cite{Rogers1988}, in high atomic number nuclei \cite{Rad2012},  via shifts in accelerating Hydrogen-like atoms \cite{Pasante1998}, via   decay processes of accelerating protons or neutrons \cite{Matsas1999}, or when electrons experience ultra-intense laser acceleration \cite{Chen1999,Schutzhold2006}, by examining the Casimir-Polder coupling to an infinite plane from an accelerating two-level system \cite{Rizzuto2007}. Researchers have also investigated using cavities to enhance the effect \cite{Scully2003, Belyanin2006,Lopp2018}, and using the Berry phase or entanglement as probes of Unruh radiation \cite{Martin-Martinez2011,Hu2012,Tian2017}. With the advent of circuit QED - cQED, researchers have investigated simulations of Unruh radiation via the Dynamic Casimir Effect - DCE, \cite{Johansson2009,Wison2011, delRey2012, Lahteenmaki2013}, or by using cQED to simulate relativistically moving systems \cite{Felicetti2015,Su2017}, and also using NMR \cite{Jin2016} or by studying the interaction between pairs of accelerated atoms \cite{Rizzuto2016}, or via the dynamical Casimir effect \cite{Farias2019}. More recent work has probed  whether real motion can produce acceleration radiation and in \cite{Sanz2018,Wang2019}, the authors consider a mechanical method of modulating the electromagnetic fields in cQED DCE photon production. 


\begin{figure}[tp] 
\begin{center}
\setlength{\unitlength}{1cm}
\begin{picture}(8.5,7)
%\put(.1,-.4){\includegraphics[width=.95\columnwidth]{Figures/Fig1b}}
\put(-2,-.2){\includegraphics[width=.85\columnwidth]{Images/Shaking_Photons/Fig1}}
\end{picture}
\end{center}
\caption{We consider the generation of photons of frequency $\omega$, from a two level system (atom), with internal transition frequency $\omega_0$, mechanically oscillating at frequency $\Omega$ and amplitude $A$, and initially in the ground state with the electromagnetic field in the vacuum. a) oscillating in front of a mirror, b) oscillating inside a cavity, c) oscillating in free space.}
   \label{Fig1}
\end{figure}

In our work we instead consider a model where the centre of mass of a TLS moves in an accelerated manner that could be more simply achieved in a laboratory setting e.g. oscillatory motion.  In \cite{Svidzinsky2018} the authors discussed the possibility that a TLS, uniformly accelerating away from a mirror and initially in its ground state, could experience a transition to its excited state accompanied by the emission of a photon. This raises the question of what other kinds of acceleration might lead to such a process? In this chapter we show that, within the same scheme as \cite{Svidzinsky2018}, we can adjust the trajectory of the TLS for different forms of accelerated motion and still stimulate photon production. We focus particularly on simple harmonic oscillation and show that this can also result in photon emission accompanied by an excitation from the ground to the excited state of the TLS. Considering acceleration radiation from oscillatory motion has an advantage over continuous linearly accelerated motion in that the TLS stays in a compact region and thus should be more feasible for direct experimental implementation.With this in mind we derive closed compact expressions for the rate of photon production in the case of an oscillating TLS in the presence of a mirror, within a cavity, and just coupled to the vacuum. For the latter we propose a cQED implementation which predicts significant rates of photon production in the microwave regime.

In the following sections though I will review the relationship between linear acceleration in a relativistic setting and the geometry of Minkowski space. After which I will derive an expression for Unruh radiation and revise the scheme set out in \cite{Svidzinsky2018}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Might use for intro}
Efforts made by [cite-Svidzinsky and Fulling papers] have looked at the possibility of extending the scheme laid out by Unruh and others to excite photons from a two-state atom (TSA). The model which formed the basis for our research was that which included a mirror that the TSA would accelerate towards (and the alternate version of an accelerated mirror), and calculating the probability of transition from an excited state in a vaccum to a ground state with a photon now present [cite-Svidzinsky]. We then looked at the possible generalisations of this scenario, a crucial point being where the relativistic accelaration was supplemented for simple harmonic motion, allowing us to look at more feasible conditions to observe this stimulation in a laboratory setting. Below I will outline the scheme for which this possible vaccum emission might be achieved. To begin with though we will proceed by reveiwing the geometry of rindler coordinates, and the quantized scalar field which gives rise to the Unruh Temperature. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Rindler Coordinates}

The study of hyperbolic motion in Minkowski spacetime i.e. the case of rectilinear motion with \emph{constant} proper acceleration has been an important field arising from the study of the specific geometric properties of Minkowski spacetime. Moreover it has also crucially played a role in the understanding of general relativistic phenomena, the motion near an event horizon being of clear significance and relevance for our purposes. Here we will reveiw some of the relevant geometric properties of Rindler space and hyperbolic motion, for a more complete treatment see [cite- Socolovsky, Wald].

First we look at the familiar global coordinates for Minkowski spacetime, $x^{\mu} = (t,x,y,z)$, where we are using natural units and have set the speed of light $c=1$. The line element is given by
\begin{equation}
ds^2 = -dt^2 + dx^2 + dy^2 + dz^2
\end{equation}
and the metric is of course
\begin{equation}
g_{\mu \nu} = \eta_{\mu \nu} = \begin{pmatrix} -1 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 \\ 0 & 0 & 1 & 0 \\ 0 & 0 & 0 & 1 \end{pmatrix}.
\end{equation}
%The symmetries of this space are those of the ten-dimensional Poincar\acute{e} group. These are translations in space 
Going forward we supress the $x$ and $y$ coordinates and look only at the 1+1 dimensional Minkowski space. The line element is simply
\begin{equation}
ds^2 = -dt^2 + dz^2
\end{equation}
We can define lightcone coordinates $(u,v)$ as follows 
\begin{align}
u &= t - z \\
v &= t + z
\end{align}
where it's clear to see that in Minkowski coordinates, for constant $u$ or $v$, we get straight lines with a slope of $\pm 1$, i.e. the speed of light. To solidify this understanding we can look at the line element in these coordinates
\begin{equation}
ds^2 = dudv = \frac{1}{2}(du \otimes dv + dv \otimes du)
\end{equation}
which gives the metric as 
\begin{equation}
g_{\mu \nu} = \begin{pmatrix} 0 & \frac{1}{2} \\ \frac{1}{2} & 0\end{pmatrix}.
\end{equation}
From this we can see that the vectors $\frac{\partial}{\partial u}$ and $\frac{\partial}{\partial v}$ have length $g(\partial_{u},\partial_{u}) = g(\partial_{v},\partial_{v}) = 0 $. Thus $\frac{\partial}{\partial u}$ and $\frac{\partial}{\partial v}$ are null vectors as expected. Clearly a grid of these coordinates, in $z-t$ space, show that at the intersection of each line we have the lightcone for an obeserver at that event (see figure).  

Now when considering rectilinear motion with constant proper acceleration in Minkowski space we first look at the change of the components of the 4-velocity. Let $U^{\mu} = (\gamma, \gamma \vec{u})$ where $\vec{u}$ is the 3-velocity, where $\gamma$ is the usual Lorentz factor $\gamma = \frac{1}{\sqrt{1-u^2}}$. From this we can define a 4-acceleration by simply taking the time derivative, with respect to the proper time, of $U^{\mu}$
\begin{equation}
A^{\mu} = \frac{dU^{\mu}}{d\tau} = \gamma \frac{dU^{\mu}}{dt} = \gamma \left(\frac{d\gamma}{dt}, \frac{d(\gamma \vec{u})}{dt}\right)
\end{equation}
where the relationship between coordinate time and proper time is used, $d\tau = ds = \sqrt{-\eta_{\mu \nu}dx^{\mu}dx^{\nu}}= \sqrt{1-\left(\frac{dz}{dt}\right)^2}dt = \frac{dt}{\gamma}$. The components of the 4-acceleration can be split in to their time and spatial coordinates
\begin{equation}
A^{0} = \gamma \frac{d\gamma}{dt}, \quad \vec{A} = \gamma \frac{\gamma \vec{u}}{dt}.
\end{equation}
For an instantaneously co-moving inertial reference frame, i.e. the frame in which the observer is instantaneously at rest [footnote reference to Andrew Steane p.61], $\gamma=1$ and the 4-acceleration becomes 
\begin{equation}
A^{\mu} = \left(0, \frac{d\vec{u}}{dt}\right) = (0,\vec{a}) 
\end{equation}
where $\vec{a}$ is the proper acceleration of the observer. Hyperbolic motion, as previously mentioned, is defined when the proper acceleration is constant. If again we restrict ourselves to 1+1 dimensional Minkowski space and look at the differential equation obtained for the proper acceleration we have 
\begin{equation}
a = \text{constant} = \frac{d(\gamma v)}{dt}  
\end{equation}
with $a =\lvert \vec{a} \rvert$. The first integral is immediate and, along with the initial condition that $v(0)=0$, we have
\begin{equation}
at = \frac{v(t)}{\sqrt{1-v(t)^2}}, \quad \rightarrow v(t) = \frac{at}{\sqrt{1+(at)^2}}. \label{rind.1}
\end{equation}
As $v(t) = \frac{dz}{dt}$ we can again integrate this expression with respect to $t$ to give
\begin{equation}
z(t) = a\int^{t}_{0} \frac{\tilde{t}d\tilde{t}}{\sqrt{1+(a\tilde{t})^2}}= \frac{1}{a}\sqrt{1+(at)^2} \label{rind.2}
\end{equation}
and thus the trajectory of the observer undergoing constant proper acceleration is a hyperbola
\begin{equation}
z^2 - t^2 = (1/a)^2. \label{rind.3}
\end{equation}
Note that for the equation of the trajectory \eqref{rind.2} above we are now confined to the region which is bounded by the light cone $u = 0$ for $t>0$ and $v=0$ for $t<0$, or more concretely $z \ge \vert t \vert$. This is known as the right Rindler wedge ($R$) of 1+1 dimensional Minkowski space, or Rindler space. It is also evident that the trajectories for observers with constant proper acceleration $a$ are asymptotic to these lines, the worldlines of photons. The region beyond these lines, $z \le \vert t \vert $ are inaccesible to these accelerated observers, and thus these lines are effectively event horizons for this observer. This is a motivating factor for us to look at the effect of an accelerated observer's in quantum vaccua.

First though, recall the relationship between the proper time and coordinate time $d\tau = \frac{dt}{\gamma}$. Using \eqref{rind.1} and integrating we have
\begin{equation}
\tau = \int^{t}_{0} d\tilde{t} \sqrt{1-v(\tilde{t})^2} = \int^{t}_{0} \frac{d\tilde{t}}{\sqrt{1+(a\tilde{t})^2}} = \frac{1}{a}\sinh^{-1}(at)
\end{equation} 
and thus have the coordinates for a uniformly accelrated observer in terms of their proper time
\begin{align}
t &= \frac{1}{a}\sinh(a\tau) \\
z &= \frac{1}{a}\cosh(a\tau) 
\end{align}
where we have gotten the eqaution for the $z$ coordinate from subbing our expression for $t$ in to \eqref{rind.3}. Dimensional analysis reveals the factors of $c$ that are required. 
\newpage
The equations then look like
\begin{align}
t &= \frac{c}{a}\sinh(\frac{a\tau}{c}) \\
z &= \frac{c^2}{a}\cosh(\frac{a\tau}{c}) 
\end{align}
these equations will be of particular relevance for our discussion about the acclerated two state atom. Setting $c=1$ again, more general rindler coordinates take the form 
\begin{align}
t &= \frac{e^{\alpha \xi}}{\alpha}\sinh(\alpha\eta) \label{rind.coord.1}\\
z &= \frac{e^{\alpha \xi}}{\alpha}\cosh(\alpha\eta) \label{rind.coord.2}
\end{align}
where, for constant $\xi$, we have the trajectories for accelerated observers in Minkowski space, as can be seen from \ref{fig1}.
\begin{figure}[h]
  \includegraphics[scale=0.17]{Images/Shaking_Photons/Rindler_graph.png}
  \caption{Trajectories for Rindler Coordinates}
  \label{fig1}
\end{figure} 
\newpage
The relationship between the proper acceleration and $\alpha$ is given by
\begin{equation}
a = \alpha e^{-\alpha \xi}
\end{equation}
and the proper time is related to $\eta$ via 
\begin{equation}
\tau = \frac{\alpha}{a} \eta = e^{\alpha \xi} \eta.
\end{equation}
In these coordinates the line element takes the form
\begin{equation}
ds^2 = e^{2a\xi}(-d\eta^2 + d\xi^2)
\end{equation}
which displays that this coordinate transformation is a conformal transformation of Minkowski space. This fact will be useful when looking at a massless scalar field in Rindler space.
Finally looking at one last coordinate transformation, $\rho = \frac{e^{\alpha \xi}}{\alpha}$  we recover the familiar rindler space line element 
\begin{equation}
ds^2 = -(\alpha \rho)^2 d\eta^2 + d\rho^2. \label{rind.4}
\end{equation}
This sequence of coordinate transformations has an intimate relationship with the Schwarzchild metric. There is an apparent sigularity in the inverse metric at $\rho = 0$, but this singularity is not essential but a consequence of our coordinates. If one were to work backwards through these transformations from the final equation above \eqref{rind.4} we would arrive at Minkowski space and find no such singularity. Minkowski space is thus the maximally extended space-time of Rindler space. Analogously the apparent singularity in Schwarzchild metric can too be transformed away given the correct choice of coordinates, those being Kruskal–Szekeres coordinates. These coordinates cover the entire spacetime manifold  of the maximally extended Schwarzchild solution. Therefore given the insight from Hawking to analyse the behaviour of quantum fields near the event horizon of a Schwarzchild black hole it seems natural to then attempt to apply a similar scheme to the above for an accelerated observer. This will be the task for the next section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Unruh Radiation}

There are number of ways to begin the calculations that lead to the Unruh effect. A good introduction to the thermodynamics of a black hole and a pretty neat and concise calculation can be found in [cite-A.Zee, QFT-Nut], albeit not particularly illuminating as to the origins of these effects. Interestingly the nature of the calculation is to essentially approximate the Schwarzchild metric near the horizon, which results in the above rindler metric, and to introduce imaginary time. Approximating the Schwarzchild space with Rindler space was also Unruh's motivation and what lead to the discovery of the Unruh effect. To provide a brief introduction to this effect we will begin by first looking at the solutions for a massless scalar field and then their vacua in different coordinate systems, following a similar scheme to that which can be found in [cite- B. Dolan, Group Theory Approach]. More complete treatments can be found in [cite- Unruh, Notes on BH; Socolovsky, Rind and Unruh Rad; Crispino et al., Unruh Effect and Applications]. 

The Klein-Gordon equation is often the starting point when embarking on the study of quantum field theory. It follows from varying the action
\beq
\mathbf{S} = \int d^{4}x \mathcal{L} 
\eeq
where the langrangian density $\mathbf{L}= \int d^{3}x \mathcal{L}$. For a massless, classical, scalar field theory, $\mathcal{L}$ in a curved space-time is
\beq
\mathcal{L} = -\half \sqrt{-g}\del_{\mu} \phi\del^{\mu} \phi = -\half \sqrt{-g} g^{\mu \nu}\del_{\mu} \phi\del_{\nu} \phi.
\eeq
The Euler-Lagrange equations (the equations of motion) are then
\beq
g_{\mu \nu} \del^{\nu} \del^{\mu} \phi = 0
\eeq 
where, for Minkowski space-time, the derivative operator just becomes the d'Alembertian operator. Actually, as this is a massless scalar field and our coordinates \eqref{rind.coord.1}, \eqref{rind.coord.2} are a conformal transformation of the metric, our equations of motion are both 
\beq
(\partial^{2}_{z}- \partial^{2}_{t})\phi = (\partial^{2}_{\xi}- \partial^{2}_{\eta})\phi = 0. \label{K.G._eq}
\eeq
Note again though that our coordinates $\eta$, $\xi$ are only defined in the right Rindler wedge. Now $\phi$ can be decomposed, in the Rindler coordinates, into a complete set of orthonormal solutions $u_i$, with coefficients $a_i$
\beq
\phi = \sum_i a_i u_i(\eta,\xi) + a^{*}_i u^{*}_i(\eta,\xi).
\eeq
A separate, yet equivalent set of othornormal solutions can also be found for the decomposition of $\phi$ in the Minkowski frame. We label these functions $u'_j$ and have coefficients $a'_j$ and $\phi$ can then be written
\beq
\phi = \sum_i a'_{i} u'_i(t,z) + a'^{*}_i u'^{*}_i(t,z).
\eeq
Obviously each element of these sets of functions satisfy \eqref{K.G._eq}. Looking at normalised right moving wave solutions to this equation, for the rindler observer, we have
\beq
u_i = \frac{1}{2\sqrt{\pi\omega_{i}}}e^{i\omega_{i}(\xi-\eta)}
\eeq
where the $\omega$'s are labelled by the summation variable, which we supress from here. We can find the coefficients of these functions via Fourier transforming along the world-line of the rindler observer. By this I mean; for a fixed $\xi = \xi_0$ and $\eta$ being the proper time for our rindler observer, $d\eta$ is tangent to this trajectory, integrating along it thus gives us our desired Fourier coeffiecients
\beq
a_{i} = e^{-i \omega \xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{i \omega \eta} \phi(\eta,\xi_{0})d\eta.
\eeq
The complex conjugates of the above functions and coefficients are straightforward. Now we can can relate the coefficients of these functions in these alternate coordinate systems ( with what amounts to essentially a change of basis) by
\beq
a_{i} = \sum_{j} \alpha_{ij} a'_{j} + \beta_{ij} a'_{j}
\eeq
where, upon quantizing our field, $\alpha_{ij}$ and $\beta_{ij}$ are the Bogoliubov transformation coefficients [cite-Bogoliubov]. These coefficients are found to be
\begin{align}
\alpha_{ij} =& e^{-i\omega\xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{i\omega\eta} u'_{j}(\eta,\xi_{0})d\eta \\
\beta_{ij} =& e^{i\omega\xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{-i\omega\eta} u'_{j}(\eta,\xi_{0})d\eta. \label{Unruh_1}
\end{align}
Quantizing our field, the details of which we won't go through, $\phi$ becomes an operator on the Hilbert space of quantum states and our fourier coefficients become the familiar creation and annihilation operators $\hat{a_i}^{\dagger}$, $\hat{a_i}$ respectively. These Hilbert spaces have there own vacua defined as
\beq
\hat{a_i} \ket{0_{R}} = 0
\eeq
for Rindler space and
\beq
\hat{a'_i} \ket{0_{M}} = 0
\eeq
for Minkowski space. Note that, as we have already stated that these coefficients, now operators, are related via a basis change, we can act on the Minkowski vacuum with the creation operator in the Rindler coordinates and vice versa. Moreover we can define a number operator, $\hat{N}_{i}=\hat{a_i}^{\dagger}\hat{a_i}$ in the Rindler coordinates and it is then a straightforward calculation to see that
\beq
\bra{0_{M}}\hat{N}_{i} \ket{0_{M}} = \sum_{j} \vert \beta_{ij} \vert^{2}
\eeq
or in words, the particle number is \emph{observer dependent}, provided $\beta_{ij}\neq 0$. Let us go about calculating this quantity from \eqref{Unruh_1}. Subbing in for $u'_{j}$ we have
\begin{align}
\beta_{ij} =& e^{i\omega\xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{-i\omega\eta} \left( \frac{1}{2\sqrt{\pi\omega'}}e^{i\omega'(z-t)}\right)d\eta \\
=& \frac{e^{i\omega\xi_{0}}}{2\pi}\sqrt{\frac{\omega}{\omega'}}\int_{-\infty}^{\infty} e^{-i\omega\eta} e^{(i\omega'/ \alpha) e^{\alpha(\xi_{0}-\eta)}}d\eta
\end{align}
where we have used the fact that $z-t=e^{\alpha(\xi - \eta)}/\alpha$ from \eqref{rind.coord.1}. Introducting a change in integration variable $iy = \frac{\omega'}{\alpha}e^{\alpha(\xi - \eta)}$ our integral becomes
\beq
\beta_{ij} = \frac{e^{-\frac{\pi\omega}{2\alpha}}}{2\pi\alpha}\sqrt{\frac{\omega}{\omega'}}e^{i\frac{\omega}{\alpha}\ln{(\frac{\alpha}{\omega'})}}\int_{0}^{-i\infty} y^{\frac{i\omega}{\alpha}-1} e^{-y} dy. \label{Unruh_2}
\eeq
This is almost a $\Gamma$-function, except the integrals are along the imaginary 
axis rather than the real axis. 
Provided $\frac{\omega}{\alpha}>0$ (so $\omega \rightarrow \omega \mp  i \epsilon$ with
$\epsilon >0$) we can rotate the contour to get\footnote{Imagine doing a integral round a slice of pie with
opening angle $90^\circ$ and vertex at the origin, in the SE quadrant for the upper sign and the NE quadrant for the lower sign. There is a branch point at the origin
but this is harmless provided $\frac{\omega}{\alpha}>0$ as usual for $\Gamma$-functions.
The exponential kills the integral around the quarter-circle at infinity.}
\begin{align}
\beta_{ij} &= \frac{e^{-\frac{\pi\omega}{2\alpha}}}{2\pi\alpha}\sqrt{\frac{\omega}{\omega'}}e^{i\frac{\omega}{\alpha}\ln{(\frac{\alpha}{\omega'})}}\int_{0}^{\infty} y^{\frac{i\omega}{\alpha}-1} e^{-y} dy \\
&= \frac{e^{-\frac{\pi\omega}{2\alpha}}}{2\pi\alpha}\sqrt{\frac{\omega}{\omega'}}e^{i\frac{\omega}{\alpha}\ln{(\frac{\alpha}{\omega'})}} \Gamma(\frac{i\omega}{\alpha}). 
\end{align}
Now the quantity $\vert \beta_{ij} \vert^{2}$ is then
\beq
\vert \beta_{ij} \vert^{2} = \frac{\omega e^{-\frac{\pi\omega}{\alpha}}}{4\pi^{2}\alpha^{2}\omega'}\frac{\pi}{\frac{\omega}{\alpha}\sinh{(\frac{\pi\omega}{\alpha})}} = \frac{1}{2\pi\alpha\omega'}\frac{1}{e^{\frac{2\pi\omega}{\alpha}}-1} \label{Unruh_2}
\eeq
where we have used the fact that $\vert\Gamma(iy)\vert^{2} = \frac{\pi}{y\sinh{\pi y}}$. It is clear that we have a Bose-Einstein distribution from equation \eqref{Unruh_2}. With this in mind it is natural to associate a temperature with the factor in the exponential. With factors of c restored throughout the above integration and $\xi_{0} = 0$, we find
\beq
T = \frac{\hbar a}{2\pi k_{B} c}
\eeq
which is the Unruh temperature.

Now that we are on sound footing with the prospect of acceleration radiation and it's origins in quantum field theory we can move to the work from \cite{Svidzinsky2018} and the setup of an accelerated two state atom with a mirror.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Accelerated Two State Atoms}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\it\bf Evaluating the probability to emit a photon under general non-relativistic motions:-} We now show how to derive the probability for the two-level system, moving in one dimension along a pre-set space-time trajectory, in the presence of a mirror, to become excited and emit a photon using first order perturbation theory.  Using the derived expression we first confirm that if the two level system is at rest the probability to emit a photon is zero. In the subsequent subsections we consider various other types of motions. Following \cite{Svidzinsky2018}, we consider a two level system, or atom, coupled to the  electromagnetic field with a coupling strength $g$, and atomic transition frequency  $\omega_0$, so the excitation energy is $\Delta E=\hbar \omega_0>0$. 
For simplicity we consider motion in
one-dimension given by position $z(t)$ 
\footnote{Our analysis will be non-relativistic and $t$ is just ordinary Newtonian time, not proper time --- the calculation can be done relativistically but there is no need for such a complication. If we assume a mechanical oscillation frequency $\Omega/2\pi \sim\, 10\, {\rm GHz}$, and a maximum amplitude of oscillation as $A\sim 10 {\rm nm}$, then the maximum velocity achieved of the atom is $v_{max}\sim 600\, {\rm m/s}\ll c$. As we show below we predict that these parameter values will yield significant acceleration radiation.}  
In the interaction picture the Hamiltonian for the interaction of the atom with the electric field
 $\phi_\omega$, is \cite{Svidzinsky2018},
%\[ H_I(t) = \hbar g\bigl\{a_\omega \phi_\omega(t,z(t))
%+ a^\dagger_\omega \phi^*_\omega(t,z(t)) \bigr\}
%\bigl(\sigma_- e^{-i\omega_0 t} + \sigma_+ e^{i\omega_0 t}  \bigr)
%\]
\begin{eqnarray}H_I(\omega,t) = \hbar g\bigl\{a_\omega \phi_\omega(t,z(t))
+ a^\dagger_\omega \phi^*_\omega(t,z(t)) \bigr\}\\\label{noSMA}
\times \bigl(\sigma_- e^{-i\omega_0 t} + \sigma_+ e^{i\omega_0 t}  \bigr)\label{Hamomega}
\end{eqnarray}
where $\sigma_+$ raises the internal atomic state and $\sigma_-$ lowers it, $a_\omega^\dagger$, $a_\omega$ are photon creation operator and annihilation operators and
$\phi_\omega$ are field modes that depend on the boundary conditions. {\color{black} We note that (\ref{Hamomega}), describes the interaction at a specific frequency $\omega$, and the full Hamiltonian is obtained by $H_I(t)\equiv \int\,H_I(\omega, t)\,d\omega$, and thus our treatment encapsulates the potential excitation of any wavelength radiation. In what follows we compute the probability to excite the atom and emit a photon of frequency $\omega$, where the latter is not taken as a fixed quantity.}
{\color{black} This interaction has been used numerous times in the literature to model the coupling between a two-level atom and a quantum field but here we do not make the rotating wave approximation and  the position of the atom is allowed to vary in time. Further, we permit the photon field mode frequency $\omega$ to be arbitrary and thus the the atom can couple to vacuum modes of any frequency. This is unlike the so-called ``single mode approximation''  (SMA), where authors consider the atom to couple preferentially to a small number of modes concentrated at a single frequency e.g. for an atom within an accelerating cavity \cite{Alsing2003, FSchuller2005, Alsing2006, Datta2009, Wang2010, Dragan2011, Hwang2012, Brown2012, Lopp2018}. Research has shown that making the SMA can lead to difficulties in superluminal propagation effects at strong couplings \cite{Sanchez2018}, and entanglement generation \cite{Bruschi2010}, however some works have  explored beyond the SMA including an NMR analogue simulation of Unruh radiation \cite{Jin2016} [2 modes].    }
If the two level system is moving on the entire real line and its position is a function of $t$, we would use right and left moving field modes
\bea \phi_\omega=e^{-i (\omega t \mp  k z(t))}, \label{eq:infinite-phi}  \eea
where $k=\omega/c>0$, is the $z$-component of the photon's wave-vector.
In the presence of a mirror fixed at $z=z_0$, we would instead use
\beq \phi_\omega=e^{-i(\omega t - k z(t) + k z_0)}- e^{-i (\omega t + k z(t) - k z_0)},\label{eq:mirror-phi}\eeq
thus ensuring that the photon field, and hence the transition amplitude,  vanishes when $z(t)$ is an integer multiple of the wavelength and the atom is at a node of the field.  In a cavity of length $L$, we would again use 
(\ref{eq:mirror-phi}), but the frequency and wave-vector would be restricted by the condition that  $k=\omega/c=2 \pi   n/L$ for some positive integer $n$.
We shall work with (\ref{eq:mirror-phi}) on the half-line for the moment,
and later adapt  the results to the case of a cavity or the entire real line as in (\ref{eq:infinite-phi}). 
In first order perturbation theory the probability of exciting the atom (via the raising operator $\sigma_+ e^{i\omega_0 t}$ in the interaction), and at the same time creating  a photon {\color{black}  of frequency $\omega$ }
via the $\hat a^\dagger \phi_\omega^*$,
%$$\hat a^\dagger \phi_\omega^*=  \bigl( e^{i(\omega t + k z(t) - k z_0)} - e^{i(\omega t - k z(t))+ k z_0} \bigr) \hat a^\dagger$$
term in the interaction potential, is given by 
\begin{align} 
P=& g^2 \left| \int_{-\infty}^\infty \bra{1_\omega,a} H_{I} \ket{0,b} dt \right| ^2 \\ 
=& g^2 \left| \int_{-\infty}^\infty\bigl[ e^{i k (z(t)- z_0)} -c.c. \bigr] e^{i \omega t + i \omega_0 t} d t \right|^2 \label{eq:phi-mirror} 
\end{align} 

where $a$ and $b$ here refer to the excited and ground states of the TLS respectively, as in \cite{Svidzinsky2018}. If the atom is at rest, $z$ is constant and  the integral gives $\delta(\omega + \omega_0)$, which is zero since $\omega>0$ and $\omega_0>0$.  Thus $P=0$, and the probability to become excited and emit a photon vanishes. We now use the expression \eqref{eq:phi-mirror}, in the following to consider various types of space-time motions $z(t)$, to discover how they can give rise to non-vanishing probabilities $P$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Acceleration towards a mirror: Brian and My Calculations}
Briefly we will review the trajectories laid out by \cite{Svidzinsky2018} to elucidate our motivations and lay the path which we will follow in subsequent sections. 

For simplicity set $c=1$ so $k=\frac{2 \pi }{\lambda}=\omega$
where $\omega$ is the angular frequency and $\lambda$ the wavelength of the emitted photon. $\omega_0$ is the angular frequency of the transition between the two internal states of the atom ($\omega$ and $\omega_0$ are both positive).
The trajectory of the atom undergoing constant acceleration $a$ in its own instantaneous rest frame (proper acceleration) we found previously to be 
\begin{equation} 
t(\tau) = \frac{1}{a}\sinh(a \tau), \qquad z(\tau) = \frac{1}{a}\cosh(a\tau) \label{eqno.1}. 
\end{equation} 
The probability from \eqref{eq:phi-mirror} above with this trajectory is
\begin{equation}
P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i \omega (z(\tau)-z_0)} -c.c. \bigr] e^{i \omega t(\tau) + i \omega_0 \tau}
d \tau \right|^2  ,\eqno{(2)}
\end{equation}
If the atom is at rest $z$ is constant and $t=\tau$, then if there is no mirror
the $c.c.$ term is missing --- the integrals give $\delta(\omega + \omega_0)$,
which is zero since $\omega>0$ and $\omega_0>0$, as above.  

From \eqref{eqno.1} 
$$\pm z(\tau) + t(\tau) =  \pm\frac{1}{a}e^{\pm a\tau},$$
so the integral is
\begin{eqnarray*}
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau 
-&&\kern -27pt\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{-a\tau}} e^{i\omega z_0}  e^{i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau 
-\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{a\tau}} e^{i\omega z_0}  e^{- i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau -c.c.
\end{eqnarray*}
where we've changed integration variable $\tau \rightarrow -\tau$ in the second
integral.
So 
$$ P= g^2 \left|
\int_{-\infty}^\infty\bigl[e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}
 -c.c. \bigr] d \tau
\right|^2 .$$

Now change integration variables from $\tau$ to $x=\frac{\omega }{a} e^{a\tau}$, so
$d \tau = \frac{1}{a x} d x $,
$$
\int_{-\infty}^\infty e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{ i \omega_0 \tau} d\tau
=\frac{1}{a} e^{-i \bigl(\omega z_0 - \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\bigr) }
\int_0^\infty e^{i x}  x^{i\frac{\omega_0}{ a}-1 }d x.
$$
Now consider the integrals
$$I_\pm
=\int_0^\infty e^{\pm i x}  x^{\pm i\frac{\omega_0}{a}-1} d x.$$
Let $x= \pm i u = e^{\pm \frac{i\pi }{2}} u$ and $z = \pm \frac {i\omega_0}{ a}$, then
$$I_\pm =e^{-\frac {\pi \omega_0 }{2 a}}\int_0^{\mp i\infty} e^{-u}  u^{z-1} d u.$$
This is almost a $\Gamma$-function, except the integrals are along the imaginary 
axis rather than the real axis. 
Provided $\Re z>0$ (so $\omega_0 \rightarrow \omega_0 \mp  i \epsilon$ with
$\epsilon >0$) we can rotate the contour to get\footnote{Imagine doing a integral round a slice of pie with
opening angle $90^\circ$ and vertex at the origin, in the SE quadrant for the upper sign and the NE quadrant for the lower sign. There is a branch point at the origin
but this is harmless provided $\Re z>0$ as usual for $\Gamma$-functions.
The exponential kills the integral around the quarter-circle at infinity.}
$$ \int_0^{\mp i\infty} e^{-u}  u^{z-1} d u = \int_0^{\infty} e^{-u}  u^{z-1} d u = \Gamma(z), \qquad \Re z>0,$$
and
$$ I_\pm\left(\frac{\omega_0 }{a}\right) =e^{-\frac{\pi \omega_0 }{2a}}
\lim_{\epsilon\rightarrow 0^+} \Gamma\left(\pm \frac{i \omega_0 }{a} + \frac{\epsilon}{a}\right) =  e^{-\frac{\pi \omega_0 }{2a}}\Gamma\left(\pm\frac{i \omega_0 }{a}\right),$$

Write
$$ \Gamma\left(\pm\frac{i \omega_0 }{a}\right) = e^{\pm i\psi}\left|\Gamma\left(\pm\frac{i \omega_0 }{a}\right)\right|.$$
The phase $\psi$ will depend on $\frac{\omega_0 }{a}$, we don't know it's analytic form, but that doesn't matter.
What we do know is
$$ \left|\Gamma\left(\pm \frac{i \omega_0 }{a}\right)\right|^2 =\frac {a \pi }{\omega_0\sinh\left(\frac { \pi\omega_0 }{a}\right)},$$
which is all we need to write the probability as
\begin{eqnarray}
P&=&\frac{\pi g^2 e^{-\frac{\pi \omega_0 }{a}} }{a \omega_0 \sinh\left(\frac{\omega_0 }{a}\right)}
\left|e^{-i \Bigl(\omega z_0 - \frac{\omega_0}{a}\ln\bigl((\frac{a }{\omega}\bigr)\Bigr) }e^{i\psi}
- e^{i \Bigl(\omega z_0 - \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\Bigr) }e^{-i\psi} 
\right|^2   \\
&=&  
\frac{4 \pi g^2  \sin^2(\omega z_0 - \varphi) }{a \omega_0 e^{\frac{\pi \omega_0 }{a}} \sinh\left(\frac{\omega_0 }{a}\right)}=  \frac{8 \pi g^2}{a \omega_0} \frac{\sin^2(\omega z_0 - \varphi) }{e^{\frac{2\pi \omega_0 }{a}}-1}
\end{eqnarray}
where 
$$\varphi = \frac{\omega_0}{a} \ln \left(\frac{a}{\omega } \right) + \psi.$$ 

So, were confident that equation (2) is correct and we can play around with it for any trajectory. We'll use this and the paper intro to stitch 'em together. This is the work we're working from.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Probabilities from other initial states:}

From A.A.~Svidzinsky, J.S.~Ben-Benjamin,~S.A. Fulling, and D.N. Page
{\it Phys. Rev. Lett.} {\bf 121}, 071301 (2018), a probability is derived for the case in which a two state atom is excited from it's ground state via Unruh radiation and it emits a photon. From the interaction Hamiltonian given in the above paper there are four possible probabilities which can be calculated; The case mentioned above (from equation (2)), the case where the atom is in the excited state, absorbs a photon and then moves to the ground state, spontaneous emission and finally absorption of a photon. It is worth looking at each of the three cases, relativistically and for the SHO, to obtain the probabilities for these scenarios. 

The interaction Hamiltonian is given as:
$$\hat V(\tau) = {\hbar} {g} ({\hat a}{\phi_\omega} + {\hat a^\dagger}{\phi_\omega^*})({\hat \sigma}{e^{-i\omega_0\tau}} + {\hat \sigma^\dagger}{e^{i\omega_0\tau}})$$
Using this to treat each scenario we have
\subsection{The relativistic second case: Moving from the excited state to the ground state and absorbing a photon}
The probability is
$$P = g^2 \left|
\int_{-\infty}^\infty\bigl d \tau\bra{0,b}\hat V(\tau)\ket{1_\omega,a} \right|^2$$
This gives
$$P = g^2 \left|\int_{-\infty}^\infty\bigl d \tau [e^{-i \omega (z(\tau) - z_0)} - c.c.] e^{-i \omega t(\tau) - i \omega_0 \tau} \right|^2$$
Sending $\tau \rightarrow -\tau$ yields
$$P = g^2 \left|-\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{i \omega t(\tau) + i \omega_0 \tau} \right|^2$$
Which is just equation (2) with a difference in minus sign. So the probability is the same as the first case done in section 0.1.

\subsection{Relativistic third case: Spontaneous emission}
$$P = g^2 \left|
\int_{-\infty}^\infty\bigl d \tau\bra{1_\omega,b}\hat V(\tau)\ket{0,a} \right|^2$$
yields
$$P = g^2 \left|\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{i \omega t(\tau) - i \omega_0 \tau} \right|^2$$
following similar calculations as section 0.1
From (1) 
$$\pm z(\tau) + t(\tau) =  \pm\frac{1}{a}e^{\pm a\tau},$$
so the integral is
\begin{eqnarray*}
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{-i \omega_0 \tau}  d \tau 
-&&\kern -27pt\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{-a\tau}} e^{i\omega z_0}  e^{-i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau 
-\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{-a\tau}} e^{i\omega z_0}  e^{- i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau -c.c.
\end{eqnarray*}
where we've changed integration variable $\tau \rightarrow -\tau$ in the first integral. So 
$$ P= g^2 \left|
\int_{-\infty}^\infty\bigl[e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}
 -c.c. \bigr] d \tau
\right|^2 .$$

Now change integration variables from $\tau$ to $x=\frac{\omega }{a} e^{-a\tau}$, so
$d \tau = \frac{-1}{a x} d x $,
$$
\int_{-\infty}^\infty e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{ i \omega_0 \tau} d\tau
=\frac{1}{a} e^{-i \bigl(\omega z_0 + \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\bigr) }
\int_0^\infty e^{i x}  x^{-i\frac{\omega_0}{ a}-1 }d x.
$$
Now consider the integrals
$$I_\pm
=\int_0^\infty e^{\pm i x}  x^{\mp i\frac{\omega_0}{a}-1} d x.$$
Let $x= \pm i u = e^{\pm \frac{i\pi }{2}} u$ and $z = \mp \frac {i\omega_0}{ a}$, then
$$I_\pm =e^{\frac {\pi \omega_0 }{2 a}}\int_0^{\mp i\infty} e^{-u}  u^{z-1} d u.$$
This is almost a $\Gamma$-function as in section 0.1, except the integrals are along the imaginary 
axis rather than the real axis. 
Provided $\Re z>0$ (so $\omega_0 \rightarrow \omega_0 \pm  i \epsilon$ with
$\epsilon >0$) we can rotate the contour to get
$$ \int_0^{\mp i\infty} e^{-u}  u^{z-1} d u = \int_0^{\infty} e^{-u}  u^{z-1} d u = \Gamma(z), \qquad \Re z>0,$$
and
$$ I_\pm\left(\frac{\omega_0 }{a}\right) =e^{\frac{\pi \omega_0 }{2a}}
\lim_{\epsilon\rightarrow 0^+} \Gamma\left(\mp \frac{i \omega_0 }{a} + \frac{\epsilon }{a}\right) =  e^{\frac{\pi \omega_0 }{2a}}\Gamma\left(\mp\frac{i \omega_0 }{a}\right),$$
Write
$$ \Gamma\left(\mp\frac{i \omega_0 }{a}\right) = e^{\mp i\psi}\left|\Gamma\left(\mp\frac{i \omega_0 }{a}\right)\right|.$$
The phase $\psi$ will depend on $\frac{\omega_0 }{a}$, we don't know it's analytic form, but that doesn't matter.
What we do know is
$$ \left|\Gamma\left(\mp \frac{i \omega_0 }{a}\right)\right|^2 =\frac {a \pi }{\omega_0\sinh\left(\frac { \pi\omega_0 }{a}\right)},$$
the probability then is
\begin{eqnarray}
P&=&\frac{\pi g^2 e^{\frac{\pi \omega_0 }{a}} }{a \omega_0 \sinh\left(\frac{\omega_0 }{a}\right)}
\left|e^{-i \Bigl(\omega z_0 + \frac{\omega_0}{a}\ln\bigl((\frac{a }{\omega}\bigr)\Bigr) }e^{-i\psi}
- e^{i \Bigl(\omega z_0 + \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\Bigr) }e^{i\psi} 
\right|^2   \\
&=&  
\frac{4 \pi g^2  \sin^2(\omega z_0 + \varphi) }{a \omega_0 e^{\frac{-\pi \omega_0 }{a}} \sinh\left(\frac{\omega_0 }{a}\right)}=  \frac{8 \pi g^2}{a \omega_0} \frac{\sin^2(\omega z_0 + \varphi) }{1-e^{\frac{-2\pi \omega_0 }{a}}}
\end{eqnarray}
where 
$$\varphi = \frac{\omega_0}{a} \ln \left(\frac{a}{\omega } \right) + \psi.$$

So $P$ is divergent for $a \rightarrow 0$

\subsubsection{Relativistic fourth case: Absorption of a photon}

The probability is 
\begin{eqnarray}
P&=& g^{2} \left|
\int_{-\infty}^\infty\bigl d \tau\bra{0,a}\hat V(\tau)\ket{1_\omega,b} \right|^2   \\
&=&  
g^2 \left|-\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{-i \omega t(\tau) + i \omega_0 \tau} \right|^2
\end{eqnarray}
If we send $\tau \rightarrow -\tau$ $P$ becomes
$$=g^2 \left|-\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{i \omega t(\tau) - i \omega_0 \tau} \right|^2$$
Which is the same as the third case case.

\subsubsection{Second case for non-relativistic SHO:\bra{0,b}\hat V\ket{1_\omega,a}}

$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{-i k (A \sin(\Omega \tau)-z_0)} - c.c. \bigr] e^{-i \omega \tau - i \omega_0 \tau} d \tau
\right|^2. $$
sending $\tau \rightarrow -\tau$
$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau) + z_0)} -c.c. \bigr] e^{i \omega \tau + i \omega_0 \tau} d \tau
\right|^2. $$
Which is the probability for the first SHO case done in sections 0.2 and 0.3 with $z_0 \rightarrow -z_0$.

\subsubsection{Third case for non-relativistic SHO: \bra{1_\omega,b}\hat V\ket{0,a}}

$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau)-z_0)} - c.c. \bigr] e^{i \omega \tau - i \omega_0 \tau} d \tau
\right|^2. $$

this is the first case for the SHO with $\omega_0 \rightarrow -\omega_0$.

\subsubsection{Fourth case for non-relativistic SHO:\bra{0,a}\hat V\ket{1_\omega,b}}

$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{-i k (A \sin(\Omega \tau)-z_0)} - c.c. \bigr] e^{-i \omega \tau + i \omega_0 \tau} d \tau
\right|^2. $$
send $\tau \rightarrow -\tau$
$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau)+z_0)} - c.c. \bigr] e^{i \omega \tau - i \omega_0 \tau} d \tau
\right|^2. $$
again this is the first case for the SHO but now with $ \omega_0 \rightarrow -\omega_0$ and $z_0 \rightarrow -z_0$. 

The above are variations of the possible quantum states that arose from the initial setup by [cite: Svidzinsky et. al.]. This setup though now affords us a more thorough setting from which we can analse other trajectories for a particle, allowing us to more generally tackle an accelerated quantum state by simply imposing an accelerated trajectory instead of needing to specify the potential providing the energy for the acceleration. In the next sections we play around with non-relativisitic trajectories arrived at through our relativistic setup and find that we arrive at feasible probabilities that give rise to acceleration radiation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{\it\bf Oscillating 2-state atom with a mirror :-}\label{mirror}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Oscillating Atom from Paper}

%\label{sec:mirror}
We now consider an atom forced to oscillate in the presence of a stationary mirror, the latter located at $z_0$, oscillating with a motional angular frequency $\Omega$,  around $z=0$
with amplitude $0<A<z_0$ 
(so we do not hit the mirror),  and set $ z(t) = A \sin(\Omega t).$
%$$ z(t) = A \sin(\Omega t).$$
Using this in (2), the probability of creating a photon of frequency
$\omega$ from the vacuum, and at the same time exciting the atom from its ground state to its excited state is
$$P(\omega)= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega t) - z_0)} -c.c. \bigr] e^{i (\omega +  \omega_0)t} d t
\right|^2. $$
Simplify the notation by absorbing $\Omega$ into $t$ and defining dimensionless variables 
$\tau = \Omega t$, $\tilde \omega = (\omega +\omega_0)/\Omega$,
$\tilde A = k A$ and $\tilde z_0 = k z_0$, we obtain
\begin{eqnarray} P(\omega) &=& \frac{g^2}{\Omega^2} \left|
\int_{-\infty}^\infty\bigl[
e^{i (\tilde A \sin \tau - \tilde z_0)} -c.c. \bigr] e^{i \tilde \omega \tau} d \tau\right|^2 \nonumber\\ 
&=& \frac{g ^2}{\Omega^2} \left|
e^{-i\tilde z_0}\int_{-\infty}^\infty e^{i (\tilde A \sin \tau+ \tilde \omega \tau)} d \tau \right.\nonumber\\ 
& &\qquad\qquad\left.-e^{i\tilde z_0}\int_{-\infty}^\infty  e^{i (\tilde A \sin \tau - \tilde \omega \tau)} d  \tau\right|^2.
\label{totalSHO-probability} 
\end{eqnarray}

The integrals appearing in (\ref{totalSHO-probability}) 
 are related to
Anger functions \cite{Abramowitz1970} (section 12.3.1),
$$ {\bf J}_\nu(x)=\frac{1}{2\pi}\int_{-\pi}^\pi e ^{i(x \sin\theta - \nu \theta)}d \theta
= \frac{1}{\pi}\int_0^\pi \cos(x\sin\theta - \nu\theta)d \theta.$$
But Anger functions are not quite what we want since what we have in (\ref{totalSHO-probability})
, is
\begin{eqnarray}
\int_{-\infty}^\infty  e ^{i(x \sin\theta - \nu \theta)} d \theta
&=&\!\! \sum_{s=-\infty}^\infty\, \int_{-\pi}^\pi e^{i\bigl(x \sin\theta - \nu(\theta+2s\pi)\bigr)}d \theta \\
&=&\!\! \pi {\bf J}_\nu(x) \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}.
\label{eq:totalamplitude}
\end{eqnarray}
Letting $ \nu = n + \{\nu\}$, 
%$$ \nu = n + \lfloor\nu\rfloor$$
where $n$ is an integer, and $0 \le  \{\nu\}<1$, is the non-integral part of $\nu$,
then
$ \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}= \sum_{s=-\infty}^\infty  e^{-2is\{\nu\}\pi} = 1 + 2\sum_{s=0}^\infty  \cos(2s\{\nu\}\pi) = \pi \delta(\{\nu\})$
and (\ref{eq:totalamplitude}), vanishes unless $\nu$ is an integer, in which case it
diverges. This is not unexpected since when Fermi's Golden Rule says that if the transition rate is constant, integrating over all $t$ will necessarily give an infinite answer for any transition with non-zero probability.  For our periodic case its more informative to estimate a transition rate over a motional cycle rather than the accumulated  probability over all time.

\sloppy Before estimating this let us consider the case when $\nu$ is a non-zero rational number, $\nu = p/q$ with $p$ and $q$ mutually prime and positive, in the integral
$$ \int_{-\infty}^\infty e^{i(x\sin \theta -\nu \theta)} d \theta
= q \int_{-\infty}^\infty e^{i(x\sin (q \psi)  - p \psi)} d \psi 
$$
where $\psi = \theta/q$. The integrand is periodic in $\psi$
with period $2\pi$ so again the integral will diverge (unless the integral over one period vanishes).  Integrating over just one period in $\psi$, we can define
\begin{eqnarray}
{\cal J}(x;p,q) &=& 
\frac{1}{2 \pi} \int_{-\pi}^\pi e^{i(x \sin (q \psi)  - p \psi )} d \psi\\\nonumber
&=& \frac{1}{\pi} \int_0^\pi \cos\big\{x \sin (q \psi)  - p \psi \bigr\} d \psi,
\label{eq:J-def}
\end{eqnarray}
which, in terms of Anger functions, becomes
\begin{eqnarray}
{\cal J}(x;p,q) &=& 
\frac{1}{2 \pi q} \int_{-q\pi}^{q \pi} e^{i(x \sin \theta  - \frac p q  \theta )} d \theta \\\nonumber
&=&\frac{1}{q}  {\bf J}_{\frac p q }(x)\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}}.\nonumber
\end{eqnarray}
We note however that $$\sum_{s=0}^{q-1} \exp({i \pi (2 s - q + 1)p/q}) = 
\exp({-i\pi\frac{p(q-1)}{q}}) \sum_{s=0}^{q-1} \exp({2i \pi p s/q})=0,$$ 
%$$
%\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}} = 
%e^{-i\pi\frac{p(q-1)}{q}} \sum_{s=0}^{q-1} e^{\frac{2i \pi p s}{q}}=0 
%$$
since $\sum_{s=0}^{q-1} \exp(2i \pi p s/q)$,
vanishes for any two integers $p$ and $q$, provided $p/q$ is not an 
integer.
 From this observation we conclude  that the transition rate is zero unless $\tilde \omega$ is a
positive integer, that is 
\begin{equation}
\omega + \omega_0 = n\Omega,\label{eq:Omega-restriction}
\end{equation}
where $\Omega$ is the mechanical frequency, $\omega_0$ is the atomic transition frequency, $\omega$ is the frequency of the photon field and $n$ is an integer.
Since $\tilde \omega$ is  positive, $n>0$, and to obtain a closed expression for the transition probability over a mechanical cycle we can use the integral
representation of the Bessel function,  \cite{Abramowitz1970} (section 9.1.21),
$J_n (\tilde A) = \frac{1}{2 \pi}\int_{-\pi}^{\pi} 
\exp[{i(\tilde A \sin \tau - n \tau)}] d \tau = (-1)^n J_{-n}(\tilde A)$,
%\[
%J_n (\tilde A) = \frac{1}{2 \pi}\int_{-\pi}^{\pi} 
%e^{i(\tilde A \sin \tau - n \tau)} d \tau = (-1)^n J_{-n}(\tilde A)
%\]
to write  $\int_{-\pi}^{\pi} \exp [{i(\tilde A \sin \tau + \tilde z_0 -  n  \tau)} ]d \tau= 2 \pi e^{i \tilde z_0}  J_n(\tilde A)$, and $\int_{-\pi}^{\pi} \exp[{i(\tilde A \sin \tau -
 \tilde z_0 +  n \tau)} ]d  \tau
= 2 \pi e^{-i (\tilde z_0 - n \pi)}  J_n(\tilde A)$.
%\begin{eqnarray*}
%\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tau + \tilde z_0 -  n  \tau)} d \tau
%&=& 2 \pi e^{i \tilde z_0}  J_n(\tilde A)\\
%\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tau -
% \tilde z_0 +  n \tau)} d  \tau
%&=& 2 \pi e^{-i (\tilde z_0 - n \pi)}  J_n(\tilde A).
%\end{eqnarray*}
By dividing by the period of mechanical oscillation, $2\pi/\Omega$, we get a transition rate (in ${\rm Hz}$), as
\begin{eqnarray}
\overline P_{n} & = &\frac{\Omega }{2 \pi}
\frac{g^2}{ \Omega^2} \left|
 \Bigl[ 2 \pi \left(e^{-i (\tilde z_0 - n \pi)} -  e^{i \tilde z_0}\right) \Bigr]
J_n(\tilde A)\right|^2\nonumber\\
&=&
\frac{8 \pi g^2}{\Omega} \sin^2\left(\tilde z_0 -\frac{\pi n}{2}\right) J_n^2(\tilde A)\\
&=&
\frac{8 \pi g^2}{\Omega} \sin^2\left(k z_0 -\frac{\pi n}{2}\right) J_n^2(k A),\label{eq:mirror-rate}
\end{eqnarray}
where $\omega = n \Omega - \omega_0 >0$. 
\vspace{.25cm}\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\subsection{Oscillating 2-state atom}

So let's take an oscillating atom. If the motion is relativistic we can use the
anharmonic trajectory, described in 
W.~Moreau, R.~Easther and R.~Neutze, {\it American Journal of Physics} {\bf 62}, 531 (1994) in terms of elliptic integrals.  But first lest just do non-relativistic
simple harmonic motion.  So
$$ t = \tau, \qquad z(\tau) = A \sin(\Omega \tau) + z_0, $$
with angular frequency $\Omega$ and  the amplitude $0<A<z_0$ so we don't hit the mirror!  Put this in (2), with $c$ re-instated so $k c = \omega$,
$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau)-z_0)} -c.c. \bigr] e^{i \omega \tau + i \omega_0 \tau} d \tau
\right|^2. $$
Simplify the notation by absorbing $\Omega$ into $\tau$ and defining 
$\tilde \tau = \Omega \tau$, $\tilde \omega = \frac{\omega +\omega_0}{\Omega}$,
$\tilde A = k A$ and $\tilde z_0 = k z_0$.
These are all dimensionless variables, in terms of which 
$$ P = \frac{g^2}{\Omega^2} \left|
\int_{-\infty}^\infty\bigl[
e^{i (\tilde A \sin \tilde \tau-\tilde z_0)} -c.c. \bigr] e^{i \tilde \omega \tilde \tau} d \tilde \tau\right|^2 =    
\frac{4 g^2}{\Omega^2} \left|
\int_{-\infty}^\infty\sin\bigl(\tilde A \sin \tilde \tau-\tilde z_0\bigr) 
e^{i \tilde \omega \tilde \tau} d \tilde \tau\right|^2. $$
Alternatively
\begin{eqnarray} 
P(\tilde A,\tilde z_0; \tilde\omega) &=& \frac{g^2}{\Omega^2} \left|
e^{- i\tilde z_0}\int_{-\infty}^\infty
e^{i (\tilde A \sin \tilde \tau+ \tilde \omega \tilde \tau)} d \tilde \tau 
- e^{i\tilde z_0}\int_{-\infty}^\infty e^{- i (\tilde A \sin \tilde \tau - \tilde \omega \tilde \tau)} d \tilde \tau\right|^2\nonumber \\
&=& \frac{g^2}{\Omega^2} \left|
e^{- i\tilde z_0}\int_{-\infty}^\infty
e^{i (\tilde A \sin \tilde \tau+ \tilde \omega \tilde \tau)} d \tilde \tau 
- e^{i\tilde z_0}\int_{-\infty}^\infty e^{i (\tilde A \sin \tilde \tau - \tilde \omega \tilde \tau)} d \tilde \tau\right|^2\label{eq:total-SHO-probability}
\end{eqnarray}
where we have changed integration variables from $\tilde \tau$ to $-\tilde \tau$ in the 
second integral.

\subsection{Transition rates}

The integrals appearing in (\ref{eq:total-SHO-probability}) are related to
Anger functions (Abromowitz+Stegun: 12.3.1; {\tt https://dlmf.nist.gov/11.10})
$$ {\bf J}_\nu(x)=\frac{1}{2\pi}\int_{-\pi}^\pi e ^{i(x \sin\theta - \nu \theta)}d \theta
= \frac{1}{\pi}\int_0^\pi \cos(x\sin\theta - \nu\theta)d \theta.$$
Obviously
$$ {\bf J}_{-\nu}(x) =  {\bf J}_{\nu}(-x)$$
and when $\nu=n$ is an integer
$$ {\bf J}_n(x) = J_n(x),$$
a Bessel function of integer order.

Anger functions satisfy the inhomogeneous Bessel equation
$$x^2 
\frac{d^2 {\bf J}_\nu}{d^2 x} + x \frac{d {\bf J}_\nu}{d x}
+(x^2 - \nu^2) {\bf J}_\nu = (x-\nu)\frac{\sin(\nu\pi)}{\pi} 
$$
and a 3D plot as functions of $\nu$ and $x$ are shown in fig. 1.

%\begin{figure}[h]
%\includegraphics[scale=0.5]{Anger-3D}
%\caption{Anger function.}
%\end{figure}

But Anger functions are not quite what we want, what we have is
\begin{equation}
\int_{-\infty}^\infty  e ^{i(x \sin\theta - \nu \theta)} d \theta
= \sum_{s=-\infty}^\infty\left( \int_{-\pi}^\pi e^{i\bigl(x \sin\theta - \nu(\theta+2s\pi)\bigr)}d \theta \right)
= \pi {\bf J}_\nu(x) \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}.
\label{eq:total-amplitude}\end{equation}
Let
$$ \nu = n + \lfloor\nu\rfloor$$
where $n$ is an integer and $0 \le  \lfloor\nu\rfloor<1$ is the non-integral part of $\nu$. 
Then
$$ \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}= \sum_{s=-\infty}^\infty  e^{-2is[\nu]\pi} = 1 + 2\sum_{s=0}^\infty  \cos(2s\lfloor\nu\rfloor\pi) = \delta(\lfloor\nu\rfloor)$$
and (\ref{eq:total-amplitude}) vanishes unless $\nu$ is an integer, in which case it
diverges.

We can check this when $\nu$ a rational number, $\nu = \frac{p}{q}$ with $p$ and $q$ mutually prime and positive.  Then
$$ \int_{-\infty}^\infty e^{i(x\sin \theta -\nu \theta)} d \theta
= q \int_{-\infty}^\infty e^{i(x\sin (q \psi)  - p \psi)} d \psi 
$$
where $\psi = \frac{\theta}{q}$. The integrand is periodic in $\psi$
with period $2\pi$ so the integral will diverge (unless the integral over one period vanishes), so integrate over one period in $\psi$ and define
\begin{equation}
{\cal J}(x;p,q) = 
\frac{1}{2 \pi} \int_{-\pi}^\pi e^{i(x \sin (q \psi)  - p \psi )} d \psi
= \frac{1}{\pi} \int_0^\pi \cos\big\{x \sin (q \psi)  - p \psi \bigr\} d \psi.
\label{eq:J-def}
\end{equation}
In terms of Anger functions
$${\cal J}(x;p,q) = 
\frac{1}{2 \pi q} \int_{-q\pi}^{q \pi} e^{i(x \sin \theta  - \frac p q  \theta )} d \theta 
=\frac{1}{q}  {\bf J}_{\frac p q }(x)\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}}.$$
Now 
$$
\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}} = 
e^{-i\pi\frac{p(q-1)}{q}} \sum_{s=0}^{q-1} e^{\frac{2i \pi p s}{q}}=0 
$$
since $\sum_{s=0}^{q-1} e^{\frac{2i \pi p s}{q}}$ vanishes for any two positive integers $p$ and $q$.

We conclude from this that the transition rate is zero unless $\tilde \omega$ is a
positive integer, that is 
\begin{equation}
\omega + \omega_0 = n\Omega,
\end{equation}
this is a genuine quantum phenomena (though $\hbar$ does not appear
explicitly in the formula for the probability.\footnote{I guess it must be hiding in $g^2$, if this is a genuine quantum phenomenon the probability should vanish when $\hbar\rightarrow 0$.})  The divergence when $\nu=\tilde \omega$ is  presumably a consequence of Fermi's Golden Rule: in first order perturbation theory the transition rate is constant, so the total probability integrated over all time will diverge.
Better to calculate probability rate rather than a 
probability. 

Since $\tilde \omega$ is a positive integer, $n>0$, for a transition we can use the integral
representation of the Bessel function,\footnote{Abromowitz+Stegun: 9.1.21.}
\begin{eqnarray*}
J_n (\tilde A) &=& \frac{1}{2 \pi}\int_{-\pi}^{\pi} 
e^{i(\tilde A \sin \tilde \tau - n \tilde \tau)} d \tilde \tau \\
J_{-n}(\tilde A) 
&=&\frac{1}{2 \pi}\int_{-\pi}^{\pi} 
e^{i(\tilde A \sin \tilde \tau + n \tilde \tau)} d \tilde \tau
= (-1)^n J_n(\tilde A),
\end{eqnarray*}
to write
\begin{eqnarray*}
\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tilde \tau +\tilde z_0 -  n \tilde \tau)} d \tilde \tau
&=& 2 \pi e^{i \tilde z_0}  J_n(\tilde A)\\
\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tilde \tau - \tilde z_0 +  n \tilde \tau)} d \tilde \tau
&=& 2 \pi e^{-i (\tilde z_0- n \pi)}  J_n(\tilde A).
\end{eqnarray*}

Dividing by $\frac{2\pi}{\Omega}$, the period of the oscillator, we get a transition rate
\begin{eqnarray}
\overline P_n & = &\frac{\Omega }{2 \pi}
\frac{g^2}{ \Omega^2} \left|
 \Bigl[ 2 \pi \left((-1)^n e^{-i \tilde z_0} -  e^{i \tilde z_0}\right) \Bigr]
J_n(\tilde A)\right|^2\nonumber\\
&=&
\frac{8 \pi g^2}{\Omega} \sin^2\left(\tilde z_0 -\frac{\pi n}{2}\right) J_n^2(\tilde A)=
\frac{8 \pi g^2}{\Omega} \sin^2\left(k z_0 -\frac{\pi n}{2}\right) J_n^2(k A),
\end{eqnarray}
where $\omega = n \Omega - \omega_0 >0$.
Can the $\sin^2\left(k z_0 -\frac{\pi n}{2}\right)$ factor be 
interpreted as some kind of dynamical Casimir effect? 

If there's no mirror
\begin{equation}
\overline P_n  = \frac{\Omega }{2 \pi}
\frac{g^2}{\Omega^2} \left|
\int_{-\pi}^\pi e^{i \tilde A \sin \tilde \tau} e^{i \tilde \omega \tilde \tau} d \tilde \tau
\right|^2 
  = \frac{2 \pi g^2 }{\Omega} J_n^2( k A) ,\qquad n>0.
\label{eq:P_n-no-mirror}
\end{equation}
Even with no mirror you can excite an atom and emit a  photon at the same time by shaking the atom hard enough to supply energy.  
 
Some useful approximations might be (A+S refers to Abromowitz and Stegun)
\begin{eqnarray}
 J_n(x) & \approx& \frac{x^n}{2^n n!}, \qquad x \ll n    (A+S:9.1.7) \\
 J_n(x)&\approx& \sqrt\frac{2}{\pi x} \cos\left( x - \frac{(2 n +1)\pi}{4}\right), 
\qquad x \gg n  (A+S:9.2.1) \\
 J_n(n) & < & \frac{2^{\frac{1}{3}} }{3^{\frac{2}{3}}} \Gamma\left(\frac{2}{3}\right) 
n^{\frac{1}{3}}
\approx\frac{0.683 }{n^{1}{3}}, \qquad n > 0  (A+S:9.1.61). 
\end{eqnarray}
This last bound was improved to 
$$\sup_x |J_n(x)| < \frac{0.674885 }{n^{\frac{1}{3}}}$$ in L.J.~Landau, {\sl Bessel Functions: Monotonicity and Bounds}, \hfill\break
{\it Journal of the London Mathematical Society}, {\bf 61}, issue 1 (2016).
Empirically the maximum is near $x\approx n$, to less than 10\% for $n$ greater than about 25, for $n=1$ the maximum is $\approx 0.582$ at $x\approx 1.84$. 

\subsection{Atom performing SHO in free space}

The transition rate (\ref{eq:P_n-no-mirror}) with  $\omega = n\Omega - \omega_0$ is 
$$\overline P_n= \overline P(n \Omega - \omega_0)  
  = \frac{2 \pi g^2 }{\Omega} J_n^2\left(\frac { (n \Omega -\omega_0)  A }{c}\right),$$
where the speed of light has been re-instated. This is plotted on figure 2
for various values of $n$, with the factor $\frac{2 \pi g^2}{\Omega}$ omitted.

%\begin{figure}[h]
%\centerline{\includegraphics[scale=0.4]{BesselJ-squared}}
%\centerline{\includegraphics[scale=0.4]{BesselJ-100-squared}}
%\caption{Transition rate for SHO forced atom in free space to emit a photon with angular
%frequency $\omega = n\Omega - \omega_0$ and wavelength $\lambda=\frac{2\pi c}{\lambda}$ (\ref{eq:P_n-no-mirror})
%as a function of $\tilde A =\frac{2\pi}{\lambda} A$. The factor 
%$\frac{2 \pi g^2}{\Omega}$ is omitted and the upper plot just shows the first three Bessel functions,
%$J_n^2(\tilde A)$ for $n=1,2,3$.
%If $\Omega \ll\omega_0$ then $n$ must be large for $\omega>0$ and the lower
%plot shows $J_{100}^2(\tilde A)$, We see that is negligible until $\tilde A$ is of order $n$.}
%\end{figure}
%
Using (\ref{eq:P_n-no-mirror}) and the above approximations the transition rate is
\begin{equation}
\overline P = 
\begin{cases}
\frac{2 \pi g^2}{\Omega} 
\frac{(k A)^{2 n}}{2^{2n} (2n)!}, &  A \ll \frac{n \lambda }{2 \pi};\\
\frac{2 \pi g^2}{\Omega} \frac{(0.683)^2}{n^{\frac{2}{3}}}, & 
A \approx \frac{n \lambda }{2 \pi} \hbox{for} n>25;\\
 \frac{2 g^2 \lambda}{\pi \Omega A }\cos\left(k A -\frac {(2 n +1)\pi}{4 } \right),   &   A \gg \frac{n \lambda }{2 \pi}. 
\end{cases}
\end{equation} 
 
The largest value that $J_n(x)$ can take is 0.582 when $n=1$ and  $x=1.481$
and this is only achievable if $\Omega > \omega_0$, assuming this is the case
the highest transition rate is 
$$\overline P_1 = \frac{2 \pi g^2}{\Omega} (0.582)^2 \approx \frac{2.1 g^2 }{\Omega},$$ for  photons with $\omega = \Omega - \omega_0$, and this is only 
achieved by tuning the oscillation amplitude to 
$$A= \frac{1.481 \lambda }{2 \pi}= \frac{1.481 c }{(\Omega - \omega_0)}.$$


If $\Omega < \omega_0$ then the largest transition rate depends on how much less.
Let $n$ be the smallest integer for which $\omega = n \Omega - \omega_0 >0$.
Then
$$\overline P_n = \frac{2 \pi g^2 }{\Omega} \frac{(0.683)^2}{n^{\frac{2}{3}}} $$
for 
$$ A=\frac{n c }{(n \Omega - \omega_0)}.$$
 
To get an idea of numbers lets consider (5) and assume that the transition frequency of the atom $\omega_0$ and the frequency of the emitted photon $\omega$ 
are both in the optical (visible) range.
Then $\Omega = \frac{\omega + \omega_0 }{n}$, which would probably be in the ultraviolet for $n=1$, but would be in the visible for $n=2$ and is lower for larger $n$.
We can make $\Omega$ as low as we wish by taking $n$ as large as we wish. 
For $n=2$ the maximum of $J_2(x)$ is close to $x=3$, so if $\Omega$ is in the
optical the probability rate (5) is a maximum for 
$A\approx \frac{3}{k} = \frac{3 \lambda }{2 \pi}$, 
of the order of a thousand ${\buildrel _{\circ} \over {\mathrm{A}}}$, %$\AA$ 
a thousand times bigger than the atom itself.  But even if that is feasible the transition is suppressed by a
factor $\Omega \sim \omega$, which is of order $10^{15}$ Hz. 
How big can $g^2$ be
in a real experiment? ($g^2$ has dimensions of inverse time$^2$.)   

If $\Omega$ is to be much lower than optical
frequency then $n$ must be large.  As $n$ increases the first (and largest) peak in $J_n(x)$
moves out to larger $x\approx n$ and the maximum rate is for $A\approx \frac{n \lambda }{2 \pi}$.  If we want $\Omega<<\omega$ then $n>>1$ and we can
use (6) to get a maximum value for the transition rate
$$\overline P_n \approx \frac{3 \pi g^2}{\Omega n^{\frac{2}{3}}} =
\frac{3 \pi g^2 n^{\frac{1}{3}}}{(\omega + \omega_0)}  \qquad \hbox{for}\qquad A = \frac{n \lambda}{2 \pi}.$$
For fixed $\omega$ and $\omega_0$, $\overline P$ grows like $n^{\frac{1}{3}}$ and can be made large by taking $\Omega<<\omega_0$. This is not a problem,
 $n$ is large but $\omega$ also large, so $\overline P_n$ is not growing with $n$,
we can't fix $\omega$ and let $n$ grow.


\subsection{Oscillating mirror}

However, if there is a mirror we can try keeping the atom fixed and oscillating the mirror.  If we don't bother with the distinction between Rindler and
Boulware vacua for small accelerations (wouldn't know what they were for
oscillatory motion anyway!) I would naively assume that we just replace $z(\tau)-z_0$ 
with $z-z_0(\tau)$ where $z_0(\tau) = A\sin(\Omega t)$ is the position of the
mirror and $z$ (constant) the position of the stationary atom.
Also $\omega t(\tau)+\omega_0 \tau \rightarrow\omega \tau+\omega_0 t(\tau)$,
but non-relativistically  $t(\tau)=t$ so no change there.
The only effect is to replace
$z_0$ in (4) with the position of the atom, $z$, and otherwise (4) is unchanged. 

Jason said that boundary conditions mimicking an accelerating mirror can be cooked up in the lab
without having to mechanically accelerate a physical mirror.
Fulling and Wald talk about microwave transitions for $\omega_0$  ($0.3\sim 300$ GHz) and effective couplings $g_{eff}\sim 10$ MHz.
If we assume $\omega$ is also in the microwave region (so $\lambda\approx 0.1 \sim 100$ cm) then,
$\frac{ g_{eff}^2 }{(\omega + \omega_0)}\approx  10^3 \sim 10^5$ Hz.
 and transition rate is of order
For $n>10$, the Bessel function has a maximum
pretty close to $k A = n$, with $J_n(n)\approx \frac{0.675 }{n^{\frac{1}{3}}}$,
giving a transition probability
$$\overline P \approx \frac{11.5 \,g^2_{eff} }{\omega+\omega_0} n^{\frac{1}{3}}
\sin^2\left( k z - \frac{\pi n}{2}\right) \approx  10^5 \sin^2\left( \frac{2 \pi  z}{\lambda}-\frac{\pi n}{2}\right) n^{\frac{1}{3}}.$$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Generalisations and Other Setups: Stimulation from mechanical oscillation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\it\bf 2-dimensional motion}


The formalism can be applied to a 2-level atom following any closed trajectory $\vec x(t)$ in the two dimensional $y-z$ plane, with a flat mirror located at $z_0$ extending in the $y$-direction.   For an electromagnetic wave with wave-vector $(k_y,k_z)$ we simply replace $k (z(t) - z_0)$ in (\ref{eq:phi-mirror}) with
$\vec k.\vec x(t) - k_z z_0$. One cannot obtain analytic answers for a general trajectory but some simple cases are immediate:
\vspace{.25cm}\\


{\it\bf 2-level atom oscillating parallel to a mirror:-}  for oscillation in the $y$-direction replace $k (z(t) - z_0)$ in (\ref{eq:phi-mirror}) with
$ k_y A \sin(\Omega t)  - k_z z_0 $  with $A$ again a constant amplitude.
The analysis is identical and (\ref{eq:mirror-rate}) still holds, but with $k z_0$ replaced with $k_z z_0$ and $k A$ replaced with $k_y A$.
\vspace{.25cm}\\


{\it\bf Rotating 2-level atom with a mirror:-} for an atom rotating around the fixed point $(0,z_0)$ in a circle with radius $R$
and constant angular velocity $\Omega$, $\vec x(t) = R(\cos\Omega t),\sin(\Omega t)$ and
$\vec k.\vec x(t)=k_y R \cos(\Omega t) + k_z R \sin(\Omega t)$.
If we parameterize the direction of the electromagnetic wave by a phase $\delta$ with
 $k_y=k\sin\delta, \quad k_z = k\cos\delta$
then
  $k_y R \cos(\Omega t) + k_z R \sin(\Omega t) - k_z z_0  = k R \sin(\Omega t + \delta) - k z_0 \cos \delta $
and the phase $\delta$ 
in the sine function can be
absorbed into $\tau$ in (\ref{eq:phi-mirror}), which does not affect the result. We just replace the
amplitude $A$ in (\ref{eq:mirror-rate}) with the rotation radius $R$ and replace 
$k z_0$ with $k_z z_0 \cos \delta$.
\vspace{.25cm}\\


\subsection{\it\bf Oscillating 2-level atom in a cavity:-}\label{cavity}

 In a one-dimensional cavity containing no photons the transition rate to excite the atom and at the same time emit a photon of frequency $\omega$ is still given by (\ref{eq:mirror-rate}), except that the allowed values of $\omega$ are discrete, 
 $\omega = c k = \pi m c/L$,
with $m$ a positive integer and Eqn (\ref{eq:Omega-restriction}) imposes the condition
\[ \frac{\pi m c}{L} + \omega_0=n \Omega\]
on $\Omega$. The rate is enhanced however if the cavity already contains $N$ photons of 
frequency $\omega$, since then $\langle N+1|a^\dagger_\omega|N\rangle = \sqrt{N+1}$,
giving the transition rate to excite/de-excite the atom given $N$ photons in the cavity as,
\begin{equation}
\overline P_{n,m,N,\pm} = 
\frac{8 \pi \chi_\pm\, g^2}{\Omega} \sin^2\left(\frac{\pi m z_0}{L} -\frac{\pi n}{2}\right) J_n^2\left(\frac{\pi m A}{L}\right),\label{eq:cavity-rate}
\end{equation}
where $\chi_+=N+1$, to excite and emit a photon, while $\chi_-=N$ to de-excite the atom and absorb a photon, and
%With $N$ photons in the cavity there is also the possibility of exciting the atom
%and absorbing a photon, with transition rate
%\begin{equation}
%\overline P_{n,m.N,-} = 
%\frac{8 \pi N g_\omega^2}{\Omega} \sin^2\left(\frac{\pi m z_0 \cos\delta}{L} -\frac{\pi n}{2}\right) J_n^2\left(\frac{\pi m A}{L}\right)
%\end{equation}
%with the tuning
 %\begin{equation}
$n \Omega = \omega_0 - \omega = \omega_0 - \pi m c/L$. {\color{black} We note that in order to observe this phenomena one could consider one of the mirror's to be slightly imperfect and then one could perform spectroscopy on the photons leaking from the optical cavity. The signature of the photons created via (\ref{eq:cavity-rate}), will prove challenging to detect over any background of existing photon occupation within the cavity.}
%\end{equation}
\vspace{.25cm}\\

\begin{figure}[tp] 
\begin{center}
\setlength{\unitlength}{1cm}
\begin{picture}(8.5,7.5)
%\put(.1,-.4){\includegraphics[width=.95\columnwidth]{Figures/Fig1b}}
\put(-2,-.3){\includegraphics[width=.65\columnwidth]{Images/Shaking_Photons/Fig2}}
\end{picture}
\end{center}
\caption{Transition rate for SHO forced atom in free space to emit a photon with angular frequency $\omega = n\Omega - \omega_0$ and wavelength $\lambda={2\pi c}/{\omega}$, equation  (\ref{eq:P_n-no-mirror}), as a function of dimensionless oscillation amplitude $\tilde A =({2\pi}/{\lambda}) A$ and sideband index $n$. The prefactor 
${2 \pi g^2}/{\Omega}$ is omitted.  We see that transition rate is negligible until $\tilde A$ is of order $n$.}
   \label{Fig2}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experimental Scenario}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\it\bf Atom performing SHO in free space:-}\label{free} 

Repeating the analysis of previous section when there's no mirror, the transition rate to emit a   photon is,  using (\ref{eq:infinite-phi}),
\begin{equation}
\overline P_{n,\omega}  = \frac{\Omega }{2 \pi}
\frac{g^2}{\Omega^2} \left|
\int_{-\pi}^\pi e^{i \tilde A \sin \tau} e^{i \tilde \omega \tau} d \tau
\right|^2 
  = \frac{2 \pi g^2 }{\Omega} J_n^2( k A) ,
\label{eq:P_n-no-mirror}
\end{equation}
with $n>0$. Even with no mirror an atom can be excited and emit a photon at the same time by shaking the atom hard enough to supply the required energy.  
The transition rate (\ref{eq:P_n-no-mirror}), with  $\omega = n\Omega - \omega_0$ is 
\begin{equation}
\overline P_{n}
  = \frac{2 \pi g^2 }{\Omega} J_n^2\left(\frac { (n \Omega -\omega_0)  A }{c}\right),
\label{SHOfreespace}  
\end{equation}
and for a given $n$ the rate will be largest at the first peak of $J_n$. From Fig \ref{Fig2}, we observe that for a given $n$, the transition rate is negligible unless $\tilde{A}\sim n$. The maximum rate occurs when $n=1$ and $\tilde{A}\sim 1.8$, and here $\overline P_1\approx 2.1g^2/\Omega$, but to achieve this one must have a mechanical oscillation amplitude of $A\sim 1.8 c/(\Omega-\omega_0)$, which will be extremely large when compared to the highest realistically achievable values of $\Omega-\omega_0$, in an experiment. 

For a possible experimental demonstration of acceleration from a two level atom shaking in a vacuum we instead consider the case when the amplitude of oscillation $A$ is small enough so that the argument of the Bessel function in (\ref{SHOfreespace}), is small and we can use the expansion $J_1^2(x)\sim x^2/4,\; 0<x\ll 1$. To achieve a large rate we consider ultra-strong coupling $g$ of the atom to the continuum where $g=\alpha \omega_0$, with $\alpha\sim 0.2$ and above \cite{Forn-Diaz2016,  Magazzu2018, PuertasMartinez2019, FriskKockum2019, Forn-Diaz2019}. We consider a cQED setup where a two level superconducting artificial atom is placed on a vibrating cantilever/membrane which is ultra-strongly coupled via an inductive coupling to the electromagnetic vacuum of a nearby electromagnetic continuum of a superconducting co-planar waveguide. This is similar to recent experimental work \cite{Viennot2018}. By using a diamond based  nanomechanical resonator one can achieve motional frequencies in the GHz regimes \cite{Gaidarzhy2007,Rodriguez-Madrid2012}. From (\ref{SHOfreespace}),  with the approximation $J_1(x)^2 \sim x^2/4$, the rate is maximised when $\omega_0=\Omega/2$, and taking this for small amplitude oscillations we obtain $\overline P_{1}\approx(\pi A\alpha)^2\Omega^3/(32 c^2)$. Fig \ref{Fig3}, shows that the emission/transition rate for a shaken superconducting two level system can reach values of $\overline P_1\sim 10^{-4}\,{\rm Hz}$, which may be detectable in current cQED setups. {\color{black} One might also consider placing the mechanically oscillating qubit close to a mirror as discussed in Section \ref{mirror}. Oscillatory motion along an arbitrary direction in three dimensions would couple the qubit to both vacuum modes which either have the mirror as a boundary or unbounded vacuum modes (for motion parallel to the mirror). This would result in  emission of photons perpendicular to the mirror (the case treated in Section \ref{mirror}), and in directions parallel to the mirror's plane (the case treated in Section \ref{free}). Such a situation may be difficult to observe experimentally as one must achieve large couplings between the two level system and the continuum. This is possible in the above discussed cQED setup above as the electromagnetic continuum is restricted essentially to be one dimensional.}

{\color{black} We finally compare our results with recent related works. In \cite{Lo2018}, and \cite{Ferrari2019}, the authors respectively consider acceleration radiation from a mechanically oscillating two level system in free space  and the modification of spontaneous emission in a two level system adjacent to an oscillating mirror. However their studies are restricted to the case where $\Omega<\omega_0$, and only multi-photon off-resonant processes play a role in these cases. Such off-resonant processes cannot be captured via our first order perturbative analysis and thus we cannot make any clear comparison with their results. However the work of \cite{Souza2018}, which looks at the radiation emitted from a two-level atom oscillating in free-space, do consider the regime $\Omega>\omega_0$, and include resonant processes and find the  emission of photons with the frequency $\omega_1=\Omega-\omega_0$, but do not find the higher modes $\omega_n=n\Omega-\omega_0$, which we predict to also exist, though with greatly reduced probabilities. To make a more quantitative comparison we study the small photon frequency case when $\omega_1\equiv\Omega- \omega_0$, is small and $\omega_1 A/c\ll 1$.  Making the approximation $J_1(x)^2\sim x^2/4$, for $x\ll 1$, and comparing our rate (\ref{SHOfreespace}), with Eqn (5) \cite{Souza2018}, in this regime, (in the notation of \cite{Souza2018}, this is when $\omega_1\equiv\omega_{\rm cm}- \omega_0$ is small), we find that both rates scale as $\overline P_{1}\sim \Gamma_{\rm MIE}\sim A^2/\Omega$. However in our case we find $\overline P_{1}\sim \omega_1^2$, while in \cite{Souza2018}, $\Gamma_{\rm MIE}\sim \omega_1^3$, a difference which may be due to the differences between the Hamiltonians. In our study we assume the Hamiltonian (\ref{noSMA}),  a  model for coupling between two levels systems and vacuum fields used by many works and which also was used in \cite{Svidzinsky2018}, to derive the Unruh temperature for the case of uniform acceleration, while \cite{Souza2018}, Eqn (1), includes both the normal dipole coupling but also a term linear in the velocity of the two level system. }

\begin{figure}[tp] 
\begin{center}
\setlength{\unitlength}{1cm}
\begin{picture}(8.5,7.5)
%\put(.1,-.4){\includegraphics[width=.95\columnwidth]{Figures/Fig1b}}
\put(-2,-.3){\includegraphics[width=.65\columnwidth]{Images/Shaking_Photons/Fig3}}
\end{picture}
\end{center}
\caption{Transition/emission rate for an atom oscillating with simple harmonic motion in free space as a function of the amplitude of the oscillation  and ultra-strong coupling strengths $\alpha$, where $g=\alpha \omega_0$, taking a mechanical frequency $\Omega/2\pi=10\,{\rm GHz}$, and two level transition frequency $\omega_0=\Omega/2$ (\ref{SHOfreespace}).}
   \label{Fig3}
\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%












==> Chpt_1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}
\label{Chpt_1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Overview}

The advent of black hole thermodynamics was the first significant marriage of quantum field theory and general relativity. The microscopic origin of black Hole radiation, first investigated by S.Hawking [cite-Hawking 1975], began by considering quantum field theories in curved space time. This was just the beginning of the investigation in to how geometric considerations impact quantum systems. The success and utility of these considerations have given rise to many fields, undoubtedly the most popular of which is string theory and the effort to unify general relativity and quantum mechanics. 

One of the impacts of these considerations, with which we will be primarily concerned, was the work of W.G.Unruh \cite{Unruh1976}. Unruh considered the case of an uniformly accelerated observer or detector in the vacuum of flat Minkowski spacetime. No black hole required. Instead reparameterised coordinates of flat minkowski spacetime so that give you the trajectory for a linearly accelerated observer to witness what is aptly named Unruh radiation \cite{Unruh1976}. The accelerated detector (which later we take to be a two level system - TLS), rather than seeing the vacuum, instead experiences a thermal photon bath with temperature $T=a\hbar/(2\pi c k_B)$, where $a$ is the proper acceleration of the TLS.
One interpretation of this effect is that the virtual photons that normally dress  the internal states of such a TLS are promoted to be real excitations due to the highly non-adiabatic nature of the acceleration. Virtual photons can have measurable signatures in atomic physics, e.g. in the Lamb shift and in Raman scattering. However, experimentally observing the Unruh effect has proved challenging since to achieve $T\sim 1{}^\circ$ K, requires an extreme acceleration $a\sim 10^{20} \,{\rm m/s^2}$, and to substantially excite the TLS  the latter should have a transition frequency $\omega_0/2\pi\sim 20\,{\rm GHz}$.

Along with this, experimental verification of Hawking radiation is itself a difficult task as the temperature is inversely proportional to the mass of the black hole. Thus the thermally relevant black holes are the most unstable as they radiate away much of their energy. The expectation is that primordial black holes would be the only candidates and, them being remnants of the earlier universe, it's unlikely we will ever find one to test this hypothesis. This does not spell out a hopeless scenario though. The importance of the Unruh effect and its analogous effect in black holes, has led to a number of proposals over the past three decades towards an experimental test of the existence of acceleration radiation. These proposals include detecting Unruh radiation  via electrons orbiting in storage rings \cite{Bell1983, Bell1987, Unruh1998},  in Penning traps \cite{Rogers1988}, in high atomic number nuclei \cite{Rad2012},  via shifts in accelerating Hydrogen-like atoms \cite{Pasante1998}, via   decay processes of accelerating protons or neutrons \cite{Matsas1999}, or when electrons experience ultra-intense laser acceleration \cite{Chen1999,Schutzhold2006}, by examining the Casimir-Polder coupling to an infinite plane from an accelerating two-level system \cite{Rizzuto2007}. Researchers have also investigated using cavities to enhance the effect \cite{Scully2003, Belyanin2006,Lopp2018}, and using the Berry phase or entanglement as probes of Unruh radiation \cite{Martin-Martinez2011,Hu2012,Tian2017}. With the advent of circuit QED - cQED, researchers have investigated simulations of Unruh radiation via the Dynamic Casimir Effect - DCE, \cite{Johansson2009,Wison2011, delRey2012, Lahteenmaki2013}, or by using cQED to simulate relativistically moving systems \cite{Felicetti2015,Su2017}, and also using NMR \cite{Jin2016} or by studying the interaction between pairs of accelerated atoms \cite{Rizzuto2016}, or via the dynamical Casimir effect \cite{Farias2019}. More recent work has probed  whether real motion can produce acceleration radiation and in \cite{Sanz2018,Wang2019}, the authors consider a mechanical method of modulating the electromagnetic fields in cQED DCE photon production. 


\begin{figure}[tp] 
\begin{center}
\setlength{\unitlength}{1cm}
\begin{picture}(8.5,7)
%\put(.1,-.4){\includegraphics[width=.95\columnwidth]{Figures/Fig1b}}
\put(-2,-.2){\includegraphics[width=.85\columnwidth]{Images/Shaking_Photons/Fig1}}
\end{picture}
\end{center}
\caption{We consider the generation of photons of frequency $\omega$, from a two level system (atom), with internal transition frequency $\omega_0$, mechanically oscillating at frequency $\Omega$ and amplitude $A$, and initially in the ground state with the electromagnetic field in the vacuum. a) oscillating in front of a mirror, b) oscillating inside a cavity, c) oscillating in free space.}
   \label{Fig1}
\end{figure}

In our work we instead consider a model where the centre of mass of a TLS moves in an accelerated manner that could be more simply achieved in a laboratory setting e.g. oscillatory motion.  In \cite{Svidzinsky2018} the authors discussed the possibility that a TLS, uniformly accelerating away from a mirror and initially in its ground state, could experience a transition to its excited state accompanied by the emission of a photon. This raises the question of what other kinds of acceleration might lead to such a process? In this chapter we show that, within the same scheme as \cite{Svidzinsky2018}, we can adjust the trajectory of the TLS for different forms of accelerated motion and still stimulate photon production. We focus particularly on simple harmonic oscillation and show that this can also result in photon emission accompanied by an excitation from the ground to the excited state of the TLS. Considering acceleration radiation from oscillatory motion has an advantage over continuous linearly accelerated motion in that the TLS stays in a compact region and thus should be more feasible for direct experimental implementation.With this in mind we derive closed compact expressions for the rate of photon production in the case of an oscillating TLS in the presence of a mirror, within a cavity, and just coupled to the vacuum. For the latter we propose a cQED implementation which predicts significant rates of photon production in the microwave regime.

In the following sections though I will review the relationship between linear acceleration in a relativistic setting and the geometry of Minkowski space. After which I will derive an expression for Unruh radiation and revise the scheme set out in \cite{Svidzinsky2018}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Might use for intro}
Efforts made by [cite-Svidzinsky and Fulling papers] have looked at the possibility of extending the scheme laid out by Unruh and others to excite photons from a two-state atom (TSA). The model which formed the basis for our research was that which included a mirror that the TSA would accelerate towards (and the alternate version of an accelerated mirror), and calculating the probability of transition from an excited state in a vaccum to a ground state with a photon now present [cite-Svidzinsky]. We then looked at the possible generalisations of this scenario, a crucial point being where the relativistic accelaration was supplemented for simple harmonic motion, allowing us to look at more feasible conditions to observe this stimulation in a laboratory setting. Below I will outline the scheme for which this possible vaccum emission might be achieved. To begin with though we will proceed by reveiwing the geometry of rindler coordinates, and the quantized scalar field which gives rise to the Unruh Temperature. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Rindler Coordinates}

The study of hyperbolic motion in Minkowski spacetime i.e. the case of rectilinear motion with \emph{constant} proper acceleration has been an important field arising from the study of the specific geometric properties of Minkowski spacetime. Moreover it has also crucially played a role in the understanding of general relativistic phenomena, the motion near an event horizon being of clear significance and relevance for our purposes. Here we will reveiw some of the relevant geometric properties of Rindler space and hyperbolic motion, for a more complete treatment see [cite- Socolovsky, Wald].

First we look at the familiar global coordinates for Minkowski spacetime, $x^{\mu} = (t,x,y,z)$, where we are using natural units and have set the speed of light $c=1$. The line element is given by
\begin{equation}
ds^2 = -dt^2 + dx^2 + dy^2 + dz^2
\end{equation}
and the metric is of course
\begin{equation}
g_{\mu \nu} = \eta_{\mu \nu} = \begin{pmatrix} -1 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 \\ 0 & 0 & 1 & 0 \\ 0 & 0 & 0 & 1 \end{pmatrix}.
\end{equation}
%The symmetries of this space are those of the ten-dimensional Poincar\acute{e} group. These are translations in space 
Going forward we supress the $x$ and $y$ coordinates and look only at the 1+1 dimensional Minkowski space. The line element is simply
\begin{equation}
ds^2 = -dt^2 + dz^2
\end{equation}
We can define lightcone coordinates $(u,v)$ as follows 
\begin{align}
u &= t - z \\
v &= t + z
\end{align}
where it's clear to see that in Minkowski coordinates, for constant $u$ or $v$, we get straight lines with a slope of $\pm 1$, i.e. the speed of light. To solidify this understanding we can look at the line element in these coordinates
\begin{equation}
ds^2 = dudv = \frac{1}{2}(du \otimes dv + dv \otimes du)
\end{equation}
which gives the metric as 
\begin{equation}
g_{\mu \nu} = \begin{pmatrix} 0 & \frac{1}{2} \\ \frac{1}{2} & 0\end{pmatrix}.
\end{equation}
From this we can see that the vectors $\frac{\partial}{\partial u}$ and $\frac{\partial}{\partial v}$ have length $g(\partial_{u},\partial_{u}) = g(\partial_{v},\partial_{v}) = 0 $. Thus $\frac{\partial}{\partial u}$ and $\frac{\partial}{\partial v}$ are null vectors as expected. Clearly a grid of these coordinates, in $z-t$ space, show that at the intersection of each line we have the lightcone for an obeserver at that event (see figure).  

Now when considering rectilinear motion with constant proper acceleration in Minkowski space we first look at the change of the components of the 4-velocity. Let $U^{\mu} = (\gamma, \gamma \vec{u})$ where $\vec{u}$ is the 3-velocity, where $\gamma$ is the usual Lorentz factor $\gamma = \frac{1}{\sqrt{1-u^2}}$. From this we can define a 4-acceleration by simply taking the time derivative, with respect to the proper time, of $U^{\mu}$
\begin{equation}
A^{\mu} = \frac{dU^{\mu}}{d\tau} = \gamma \frac{dU^{\mu}}{dt} = \gamma \left(\frac{d\gamma}{dt}, \frac{d(\gamma \vec{u})}{dt}\right)
\end{equation}
where the relationship between coordinate time and proper time is used, $d\tau = ds = \sqrt{-\eta_{\mu \nu}dx^{\mu}dx^{\nu}}= \sqrt{1-\left(\frac{dz}{dt}\right)^2}dt = \frac{dt}{\gamma}$. The components of the 4-acceleration can be split in to their time and spatial coordinates
\begin{equation}
A^{0} = \gamma \frac{d\gamma}{dt}, \quad \vec{A} = \gamma \frac{\gamma \vec{u}}{dt}.
\end{equation}
For an instantaneously co-moving inertial reference frame, i.e. the frame in which the observer is instantaneously at rest [footnote reference to Andrew Steane p.61], $\gamma=1$ and the 4-acceleration becomes 
\begin{equation}
A^{\mu} = \left(0, \frac{d\vec{u}}{dt}\right) = (0,\vec{a}) 
\end{equation}
where $\vec{a}$ is the proper acceleration of the observer. Hyperbolic motion, as previously mentioned, is defined when the proper acceleration is constant. If again we restrict ourselves to 1+1 dimensional Minkowski space and look at the differential equation obtained for the proper acceleration we have 
\begin{equation}
a = \text{constant} = \frac{d(\gamma v)}{dt}  
\end{equation}
with $a =\lvert \vec{a} \rvert$. The first integral is immediate and, along with the initial condition that $v(0)=0$, we have
\begin{equation}
at = \frac{v(t)}{\sqrt{1-v(t)^2}}, \quad \rightarrow v(t) = \frac{at}{\sqrt{1+(at)^2}}. \label{rind.1}
\end{equation}
As $v(t) = \frac{dz}{dt}$ we can again integrate this expression with respect to $t$ to give
\begin{equation}
z(t) = a\int^{t}_{0} \frac{\tilde{t}d\tilde{t}}{\sqrt{1+(a\tilde{t})^2}}= \frac{1}{a}\sqrt{1+(at)^2} \label{rind.2}
\end{equation}
and thus the trajectory of the observer undergoing constant proper acceleration is a hyperbola
\begin{equation}
z^2 - t^2 = (1/a)^2. \label{rind.3}
\end{equation}
Note that for the equation of the trajectory \eqref{rind.2} above we are now confined to the region which is bounded by the light cone $u = 0$ for $t>0$ and $v=0$ for $t<0$, or more concretely $z \ge \vert t \vert$. This is known as the right Rindler wedge ($R$) of 1+1 dimensional Minkowski space, or Rindler space. It is also evident that the trajectories for observers with constant proper acceleration $a$ are asymptotic to these lines, the worldlines of photons. The region beyond these lines, $z \le \vert t \vert $ are inaccesible to these accelerated observers, and thus these lines are effectively event horizons for this observer. This is a motivating factor for us to look at the effect of an accelerated observer's in quantum vaccua.

First though, recall the relationship between the proper time and coordinate time $d\tau = \frac{dt}{\gamma}$. Using \eqref{rind.1} and integrating we have
\begin{equation}
\tau = \int^{t}_{0} d\tilde{t} \sqrt{1-v(\tilde{t})^2} = \int^{t}_{0} \frac{d\tilde{t}}{\sqrt{1+(a\tilde{t})^2}} = \frac{1}{a}\sinh^{-1}(at)
\end{equation} 
and thus have the coordinates for a uniformly accelrated observer in terms of their proper time
\begin{align}
t &= \frac{1}{a}\sinh(a\tau) \\
z &= \frac{1}{a}\cosh(a\tau) 
\end{align}
where we have gotten the eqaution for the $z$ coordinate from subbing our expression for $t$ in to \eqref{rind.3}. Dimensional analysis reveals the factors of $c$ that are required. 
\newpage
The equations then look like
\begin{align}
t &= \frac{c}{a}\sinh(\frac{a\tau}{c}) \\
z &= \frac{c^2}{a}\cosh(\frac{a\tau}{c}) 
\end{align}
these equations will be of particular relevance for our discussion about the acclerated two state atom. Setting $c=1$ again, more general rindler coordinates take the form 
\begin{align}
t &= \frac{e^{\alpha \xi}}{\alpha}\sinh(\alpha\eta) \label{rind.coord.1}\\
z &= \frac{e^{\alpha \xi}}{\alpha}\cosh(\alpha\eta) \label{rind.coord.2}
\end{align}
where, for constant $\xi$, we have the trajectories for accelerated observers in Minkowski space, as can be seen from \ref{fig1}.
\begin{figure}[h]
  \includegraphics[scale=0.17]{Images/Shaking_Photons/Rindler_graph.png}
  \caption{Trajectories for Rindler Coordinates}
  \label{fig1}
\end{figure} 
\newpage
The relationship between the proper acceleration and $\alpha$ is given by
\begin{equation}
a = \alpha e^{-\alpha \xi}
\end{equation}
and the proper time is related to $\eta$ via 
\begin{equation}
\tau = \frac{\alpha}{a} \eta = e^{\alpha \xi} \eta.
\end{equation}
In these coordinates the line element takes the form
\begin{equation}
ds^2 = e^{2\alpha\xi}(-d\eta^2 + d\xi^2)
\end{equation}
which displays that this coordinate transformation is a conformal transformation of Minkowski space. This fact will be useful when looking at a massless scalar field in Rindler space.
Finally looking at one last coordinate transformation, $\rho = \frac{e^{\alpha \xi}}{\alpha}$  we recover the familiar rindler space line element 
\begin{equation}
ds^2 = -(\alpha \rho)^2 d\eta^2 + d\rho^2. \label{rind.4}
\end{equation}
This sequence of coordinate transformations has an intimate relationship with the Schwarzchild metric. There is an apparent sigularity in the inverse metric at $\rho = 0$, but this singularity is not essential but a consequence of our coordinates. If one were to work backwards through these transformations from the final equation above \eqref{rind.4} we would arrive at Minkowski space and find no such singularity. Minkowski space is thus the maximally extended space-time of Rindler space. Analogously the apparent singularity in Schwarzchild metric can too be transformed away given the correct choice of coordinates, those being Kruskal–Szekeres coordinates. These coordinates cover the entire spacetime manifold  of the maximally extended Schwarzchild solution. Therefore given the insight from Hawking to analyse the behaviour of quantum fields near the event horizon of a Schwarzchild black hole it seems natural to then attempt to apply a similar scheme to the above for an accelerated observer. This will be the task for the next section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Unruh Radiation}

There are number of ways to begin the calculations that lead to the Unruh effect. A good introduction to the thermodynamics of a black hole and a pretty neat and concise calculation can be found in [cite-A.Zee, QFT-Nut], albeit not particularly illuminating as to the origins of these effects. Interestingly the nature of the calculation is to essentially approximate the Schwarzchild metric near the horizon, which results in the above rindler metric, and to introduce imaginary time. Approximating the Schwarzchild space with Rindler space was also Unruh's motivation and what lead to the discovery of the Unruh effect. To provide a brief introduction to this effect we will begin by first looking at the solutions for a massless scalar field and then their vacua in different coordinate systems, following a similar scheme to that which can be found in [cite- B. Dolan, Group Theory Approach]. More complete treatments can be found in [cite- Unruh, Notes on BH; Socolovsky, Rind and Unruh Rad; Crispino et al., Unruh Effect and Applications]. 

The Klein-Gordon equation is often the starting point when embarking on the study of quantum field theory. It follows from varying the action
\beq
\mathbf{S} = \int d^{4}x \mathcal{L} 
\eeq
where the langrangian density $\mathbf{L}= \int d^{3}x \mathcal{L}$. For a massless, classical, scalar field theory, $\mathcal{L}$ in a curved space-time is
\beq
\mathcal{L} = -\half \sqrt{-g}\del_{\mu} \phi\del^{\mu} \phi = -\half \sqrt{-g} g^{\mu \nu}\del_{\mu} \phi\del_{\nu} \phi.
\eeq
The Euler-Lagrange equations (the equations of motion) are then
\beq
g_{\mu \nu} \del^{\nu} \del^{\mu} \phi = 0
\eeq 
where, for Minkowski space-time, the derivative operator just becomes the d'Alembertian operator. Actually, as this is a massless scalar field and our coordinates \eqref{rind.coord.1}, \eqref{rind.coord.2} are a conformal transformation of the metric, our equations of motion are both 
\beq
(\partial^{2}_{z}- \partial^{2}_{t})\phi = (\partial^{2}_{\xi}- \partial^{2}_{\eta})\phi = 0. \label{K.G._eq}
\eeq
Note again though that our coordinates $\eta$, $\xi$ are only defined in the right Rindler wedge. Now $\phi$ can be decomposed, in the Rindler coordinates, into a complete set of orthonormal solutions $u_i$, with coefficients $a_i$
\beq
\phi = \sum_i a_i u_i(\eta,\xi) + a^{*}_i u^{*}_i(\eta,\xi).
\eeq
A separate, yet equivalent set of othornormal solutions can also be found for the decomposition of $\phi$ in the Minkowski frame. We label these functions $u'_j$ and have coefficients $a'_j$ and $\phi$ can then be written
\beq
\phi = \sum_i a'_{i} u'_i(t,z) + a'^{*}_i u'^{*}_i(t,z).
\eeq
Obviously each element of these sets of functions satisfy \eqref{K.G._eq}. Looking at normalised right moving wave solutions to this equation, for the rindler observer, we have
\beq
u_i = \frac{1}{2\sqrt{\pi\omega_{i}}}e^{i\omega_{i}(\xi-\eta)}
\eeq
where the $\omega$'s are labelled by the summation variable, which we supress from here. We can find the coefficients of these functions via Fourier transforming along the world-line of the rindler observer. By this I mean; for a fixed $\xi = \xi_0$ and $\eta$ being the proper time for our rindler observer, $d\eta$ is tangent to this trajectory, integrating along it thus gives us our desired Fourier coeffiecients
\beq
a_{i} = e^{-i \omega \xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{i \omega \eta} \phi(\eta,\xi_{0})d\eta.
\eeq
The complex conjugates of the above functions and coefficients are straightforward. Now we can can relate the coefficients of these functions in these alternate coordinate systems ( with what amounts to essentially a change of basis) by
\beq
a_{i} = \sum_{j} \alpha_{ij} a'_{j} + \beta_{ij} a'_{j}
\eeq
where, upon quantizing our field, $\alpha_{ij}$ and $\beta_{ij}$ are the Bogoliubov transformation coefficients [cite-Bogoliubov]. These coefficients are found to be
\begin{align}
\alpha_{ij} =& e^{-i\omega\xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{i\omega\eta} u'_{j}(\eta,\xi_{0})d\eta \\
\beta_{ij} =& e^{i\omega\xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{-i\omega\eta} u'_{j}(\eta,\xi_{0})d\eta. \label{Unruh_1}
\end{align}
Quantizing our field, the details of which we won't go through, $\phi$ becomes an operator on the Hilbert space of quantum states and our fourier coefficients become the familiar creation and annihilation operators $\hat{a_i}^{\dagger}$, $\hat{a_i}$ respectively. These Hilbert spaces have there own vacua defined as
\beq
\hat{a_i} \ket{0_{R}} = 0
\eeq
for Rindler space and
\beq
\hat{a'_i} \ket{0_{M}} = 0
\eeq
for Minkowski space. Note that, as we have already stated that these coefficients, now operators, are related via a basis change, we can act on the Minkowski vacuum with the creation operator in the Rindler coordinates and vice versa. Moreover we can define a number operator, $\hat{N}_{i}=\hat{a_i}^{\dagger}\hat{a_i}$ in the Rindler coordinates and it is then a straightforward calculation to see that
\beq
\bra{0_{M}}\hat{N}_{i} \ket{0_{M}} = \sum_{j} \vert \beta_{ij} \vert^{2}
\eeq
or in words, the particle number is \emph{observer dependent}, provided $\beta_{ij}\neq 0$. Let us go about calculating this quantity from \eqref{Unruh_1}. Subbing in for $u'_{j}$ we have
\begin{align}
\beta_{ij} =& e^{i\omega\xi_{0}}\sqrt{\frac{\omega}{\pi}}\int_{-\infty}^{\infty} e^{-i\omega\eta} \left( \frac{1}{2\sqrt{\pi\omega'}}e^{i\omega'(z-t)}\right)d\eta \\
=& \frac{e^{i\omega\xi_{0}}}{2\pi}\sqrt{\frac{\omega}{\omega'}}\int_{-\infty}^{\infty} e^{-i\omega\eta} e^{(i\omega'/ \alpha) e^{\alpha(\xi_{0}-\eta)}}d\eta
\end{align}
where we have used the fact that $z-t=e^{\alpha(\xi - \eta)}/\alpha$ from \eqref{rind.coord.1}. Introducting a change in integration variable $iy = \frac{\omega'}{\alpha}e^{\alpha(\xi - \eta)}$ our integral becomes
\beq
\beta_{ij} = \frac{e^{-\frac{\pi\omega}{2\alpha}}}{2\pi\alpha}\sqrt{\frac{\omega}{\omega'}}e^{i\frac{\omega}{\alpha}\ln{(\frac{\alpha}{\omega'})}}\int_{0}^{-i\infty} y^{\frac{i\omega}{\alpha}-1} e^{-y} dy. \label{Unruh_2}
\eeq
This is almost a $\Gamma$-function, except the integrals are along the imaginary 
axis rather than the real axis. 
Provided $\frac{\omega}{\alpha}>0$ (so $\omega \rightarrow \omega \mp  i \epsilon$ with
$\epsilon >0$) we can rotate the contour to get\footnote{Imagine doing a integral round a slice of pie with
opening angle $90^\circ$ and vertex at the origin, in the SE quadrant for the upper sign and the NE quadrant for the lower sign. There is a branch point at the origin
but this is harmless provided $\frac{\omega}{\alpha}>0$ as usual for $\Gamma$-functions.
The exponential kills the integral around the quarter-circle at infinity.}
\begin{align}
\beta_{ij} &= \frac{e^{-\frac{\pi\omega}{2\alpha}}}{2\pi\alpha}\sqrt{\frac{\omega}{\omega'}}e^{i\frac{\omega}{\alpha}\ln{(\frac{\alpha}{\omega'})}}\int_{0}^{\infty} y^{\frac{i\omega}{\alpha}-1} e^{-y} dy \\
&= \frac{e^{-\frac{\pi\omega}{2\alpha}}}{2\pi\alpha}\sqrt{\frac{\omega}{\omega'}}e^{i\frac{\omega}{\alpha}\ln{(\frac{\alpha}{\omega'})}} \Gamma(\frac{i\omega}{\alpha}). 
\end{align}
Now the quantity $\vert \beta_{ij} \vert^{2}$ is then
\beq
\vert \beta_{ij} \vert^{2} = \frac{\omega e^{-\frac{\pi\omega}{\alpha}}}{4\pi^{2}\alpha^{2}\omega'}\frac{\pi}{\frac{\omega}{\alpha}\sinh{(\frac{\pi\omega}{\alpha})}} = \frac{1}{2\pi\alpha\omega'}\frac{1}{e^{\frac{2\pi\omega}{\alpha}}-1} \label{Unruh_2}
\eeq
where we have used the fact that $\vert\Gamma(iy)\vert^{2} = \frac{\pi}{y\sinh{\pi y}}$. It is clear that we have a Bose-Einstein distribution from equation \eqref{Unruh_2}. With this in mind it is natural to associate a temperature with the factor in the exponential. With factors of c restored throughout the above integration and $\xi_{0} = 0$, we find
\beq
T = \frac{\hbar a}{2\pi k_{B} c}
\eeq
which is the Unruh temperature.

Now that we are on sound footing with the prospect of acceleration radiation and it's origins in quantum field theory we can move to the work from \cite{Svidzinsky2018} and the setup of an accelerated two state atom with a mirror.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Accelerated Two State Atoms}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\it\bf Evaluating the probability to emit a photon under general non-relativistic motions:-} We now show how to derive the probability for the two-level system, moving in one dimension along a pre-set space-time trajectory, in the presence of a mirror, to become excited and emit a photon using first order perturbation theory.  Using the derived expression we first confirm that if the two level system is at rest the probability to emit a photon is zero. In the subsequent subsections we consider various other types of motions. Following \cite{Svidzinsky2018}, we consider a two level system, or atom, coupled to the  electromagnetic field with a coupling strength $g$, and atomic transition frequency  $\omega_0$, so the excitation energy is $\Delta E=\hbar \omega_0>0$. 
For simplicity we consider motion in
one-dimension given by position $z(t)$ 
\footnote{Our analysis will be non-relativistic and $t$ is just ordinary Newtonian time, not proper time --- the calculation can be done relativistically but there is no need for such a complication. If we assume a mechanical oscillation frequency $\Omega/2\pi \sim\, 10\, {\rm GHz}$, and a maximum amplitude of oscillation as $A\sim 10 {\rm nm}$, then the maximum velocity achieved of the atom is $v_{max}\sim 600\, {\rm m/s}\ll c$. As we show below we predict that these parameter values will yield significant acceleration radiation.}  
In the interaction picture the Hamiltonian for the interaction of the atom with the electric field
 $\phi_\omega$, is \cite{Svidzinsky2018},
%\[ H_I(t) = \hbar g\bigl\{a_\omega \phi_\omega(t,z(t))
%+ a^\dagger_\omega \phi^*_\omega(t,z(t)) \bigr\}
%\bigl(\sigma_- e^{-i\omega_0 t} + \sigma_+ e^{i\omega_0 t}  \bigr)
%\]
\begin{eqnarray}H_I(\omega,t) = \hbar g\bigl\{a_\omega \phi_\omega(t,z(t))
+ a^\dagger_\omega \phi^*_\omega(t,z(t)) \bigr\}\\\label{noSMA}
\times \bigl(\sigma_- e^{-i\omega_0 t} + \sigma_+ e^{i\omega_0 t}  \bigr)\label{Hamomega}
\end{eqnarray}
where $\sigma_+$ raises the internal atomic state and $\sigma_-$ lowers it, $a_\omega^\dagger$, $a_\omega$ are photon creation operator and annihilation operators and
$\phi_\omega$ are field modes that depend on the boundary conditions. {\color{black} We note that (\ref{Hamomega}), describes the interaction at a specific frequency $\omega$, and the full Hamiltonian is obtained by $H_I(t)\equiv \int\,H_I(\omega, t)\,d\omega$, and thus our treatment encapsulates the potential excitation of any wavelength radiation. In what follows we compute the probability to excite the atom and emit a photon of frequency $\omega$, where the latter is not taken as a fixed quantity.}
{\color{black} This interaction has been used numerous times in the literature to model the coupling between a two-level atom and a quantum field but here we do not make the rotating wave approximation and  the position of the atom is allowed to vary in time. Further, we permit the photon field mode frequency $\omega$ to be arbitrary and thus the the atom can couple to vacuum modes of any frequency. This is unlike the so-called ``single mode approximation''  (SMA), where authors consider the atom to couple preferentially to a small number of modes concentrated at a single frequency e.g. for an atom within an accelerating cavity \cite{Alsing2003, FSchuller2005, Alsing2006, Datta2009, Wang2010, Dragan2011, Hwang2012, Brown2012, Lopp2018}. Research has shown that making the SMA can lead to difficulties in superluminal propagation effects at strong couplings \cite{Sanchez2018}, and entanglement generation \cite{Bruschi2010}, however some works have  explored beyond the SMA including an NMR analogue simulation of Unruh radiation \cite{Jin2016} [2 modes].    }
If the two level system is moving on the entire real line and its position is a function of $t$, we would use right and left moving field modes
\bea \phi_\omega=e^{-i (\omega t \mp  k z(t))}, \label{eq:infinite-phi}  \eea
where $k=\omega/c>0$, is the $z$-component of the photon's wave-vector.
In the presence of a mirror fixed at $z=z_0$, we would instead use
\beq \phi_\omega=e^{-i(\omega t - k z(t) + k z_0)}- e^{-i (\omega t + k z(t) - k z_0)},\label{eq:mirror-phi}\eeq
thus ensuring that the photon field, and hence the transition amplitude,  vanishes when $z(t)$ is an integer multiple of the wavelength and the atom is at a node of the field.  In a cavity of length $L$, we would again use 
(\ref{eq:mirror-phi}), but the frequency and wave-vector would be restricted by the condition that  $k=\omega/c=2 \pi   n/L$ for some positive integer $n$.
We shall work with (\ref{eq:mirror-phi}) on the half-line for the moment,
and later adapt  the results to the case of a cavity or the entire real line as in (\ref{eq:infinite-phi}). 
In first order perturbation theory the probability of exciting the atom (via the raising operator $\sigma_+ e^{i\omega_0 t}$ in the interaction), and at the same time creating  a photon {\color{black}  of frequency $\omega$ }
via the $\hat a^\dagger \phi_\omega^*$,
%$$\hat a^\dagger \phi_\omega^*=  \bigl( e^{i(\omega t + k z(t) - k z_0)} - e^{i(\omega t - k z(t))+ k z_0} \bigr) \hat a^\dagger$$
term in the interaction potential, is given by 
\begin{align} 
P=& g^2 \left| \int_{-\infty}^\infty \bra{1_\omega,a} H_{I} \ket{0,b} dt \right| ^2 \\ 
=& g^2 \left| \int_{-\infty}^\infty\bigl[ e^{i k (z(t)- z_0)} -c.c. \bigr] e^{i \omega t + i \omega_0 t} d t \right|^2 \label{eq:phi-mirror} 
\end{align} 

where $a$ and $b$ here refer to the excited and ground states of the TLS respectively, as in \cite{Svidzinsky2018}. If the atom is at rest, $z$ is constant and  the integral gives $\delta(\omega + \omega_0)$, which is zero since $\omega>0$ and $\omega_0>0$.  Thus $P=0$, and the probability to become excited and emit a photon vanishes. We now use the expression \eqref{eq:phi-mirror}, in the following to consider various types of space-time motions $z(t)$, to discover how they can give rise to non-vanishing probabilities $P$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Acceleration towards a mirror: Brian and My Calculations}
Briefly we will review the trajectories laid out by \cite{Svidzinsky2018} to elucidate our motivations and lay the path which we will follow in subsequent sections. 

For simplicity set $c=1$ so $k=\frac{2 \pi }{\lambda}=\omega$
where $\omega$ is the angular frequency and $\lambda$ the wavelength of the emitted photon. $\omega_0$ is the angular frequency of the transition between the two internal states of the atom ($\omega$ and $\omega_0$ are both positive).
The trajectory of the atom undergoing constant acceleration $a$ in its own instantaneous rest frame (proper acceleration) we found previously to be 
\begin{equation} 
t(\tau) = \frac{1}{a}\sinh(a \tau), \qquad z(\tau) = \frac{1}{a}\cosh(a\tau) \label{eqno.1}. 
\end{equation} 
The probability from \eqref{eq:phi-mirror} above with this trajectory is
\begin{equation}
P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i \omega (z(\tau)-z_0)} -c.c. \bigr] e^{i \omega t(\tau) + i \omega_0 \tau}
d \tau \right|^2  ,\eqno{(2)}
\end{equation}
If the atom is at rest $z$ is constant and $t=\tau$, then if there is no mirror
the $c.c.$ term is missing --- the integrals give $\delta(\omega + \omega_0)$,
which is zero since $\omega>0$ and $\omega_0>0$, as above.  

From \eqref{eqno.1} 
$$\pm z(\tau) + t(\tau) =  \pm\frac{1}{a}e^{\pm a\tau},$$
so the integral is
\begin{eqnarray*}
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau 
-&&\kern -27pt\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{-a\tau}} e^{i\omega z_0}  e^{i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau 
-\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{a\tau}} e^{i\omega z_0}  e^{- i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau -c.c.
\end{eqnarray*}
where we've changed integration variable $\tau \rightarrow -\tau$ in the second
integral.
So 
$$ P= g^2 \left|
\int_{-\infty}^\infty\bigl[e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}
 -c.c. \bigr] d \tau
\right|^2 .$$

Now change integration variables from $\tau$ to $x=\frac{\omega }{a} e^{a\tau}$, so
$d \tau = \frac{1}{a x} d x $,
$$
\int_{-\infty}^\infty e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{ i \omega_0 \tau} d\tau
=\frac{1}{a} e^{-i \bigl(\omega z_0 - \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\bigr) }
\int_0^\infty e^{i x}  x^{i\frac{\omega_0}{ a}-1 }d x.
$$
Now consider the integrals
$$I_\pm
=\int_0^\infty e^{\pm i x}  x^{\pm i\frac{\omega_0}{a}-1} d x.$$
Let $x= \pm i u = e^{\pm \frac{i\pi }{2}} u$ and $z = \pm \frac {i\omega_0}{ a}$, then
$$I_\pm =e^{-\frac {\pi \omega_0 }{2 a}}\int_0^{\mp i\infty} e^{-u}  u^{z-1} d u.$$
This is almost a $\Gamma$-function, except the integrals are along the imaginary 
axis rather than the real axis. 
Provided $\Re z>0$ (so $\omega_0 \rightarrow \omega_0 \mp  i \epsilon$ with
$\epsilon >0$) we can rotate the contour to get\footnote{Imagine doing a integral round a slice of pie with
opening angle $90^\circ$ and vertex at the origin, in the SE quadrant for the upper sign and the NE quadrant for the lower sign. There is a branch point at the origin
but this is harmless provided $\Re z>0$ as usual for $\Gamma$-functions.
The exponential kills the integral around the quarter-circle at infinity.}
$$ \int_0^{\mp i\infty} e^{-u}  u^{z-1} d u = \int_0^{\infty} e^{-u}  u^{z-1} d u = \Gamma(z), \qquad \Re z>0,$$
and
$$ I_\pm\left(\frac{\omega_0 }{a}\right) =e^{-\frac{\pi \omega_0 }{2a}}
\lim_{\epsilon\rightarrow 0^+} \Gamma\left(\pm \frac{i \omega_0 }{a} + \frac{\epsilon}{a}\right) =  e^{-\frac{\pi \omega_0 }{2a}}\Gamma\left(\pm\frac{i \omega_0 }{a}\right),$$

Write
$$ \Gamma\left(\pm\frac{i \omega_0 }{a}\right) = e^{\pm i\psi}\left|\Gamma\left(\pm\frac{i \omega_0 }{a}\right)\right|.$$
The phase $\psi$ will depend on $\frac{\omega_0 }{a}$, we don't know it's analytic form, but that doesn't matter.
What we do know is
$$ \left|\Gamma\left(\pm \frac{i \omega_0 }{a}\right)\right|^2 =\frac {a \pi }{\omega_0\sinh\left(\frac { \pi\omega_0 }{a}\right)},$$
which is all we need to write the probability as
\begin{eqnarray}
P&=&\frac{\pi g^2 e^{-\frac{\pi \omega_0 }{a}} }{a \omega_0 \sinh\left(\frac{\omega_0 }{a}\right)}
\left|e^{-i \Bigl(\omega z_0 - \frac{\omega_0}{a}\ln\bigl((\frac{a }{\omega}\bigr)\Bigr) }e^{i\psi}
- e^{i \Bigl(\omega z_0 - \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\Bigr) }e^{-i\psi} 
\right|^2   \\
&=&  
\frac{4 \pi g^2  \sin^2(\omega z_0 - \varphi) }{a \omega_0 e^{\frac{\pi \omega_0 }{a}} \sinh\left(\frac{\omega_0 }{a}\right)}=  \frac{8 \pi g^2}{a \omega_0} \frac{\sin^2(\omega z_0 - \varphi) }{e^{\frac{2\pi \omega_0 }{a}}-1}
\end{eqnarray}
where 
$$\varphi = \frac{\omega_0}{a} \ln \left(\frac{a}{\omega } \right) + \psi.$$ 

So, were confident that equation (2) is correct and we can play around with it for any trajectory. We'll use this and the paper intro to stitch 'em together. This is the work we're working from.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Probabilities from other initial states:}

From A.A.~Svidzinsky, J.S.~Ben-Benjamin,~S.A. Fulling, and D.N. Page
{\it Phys. Rev. Lett.} {\bf 121}, 071301 (2018), a probability is derived for the case in which a two state atom is excited from it's ground state via Unruh radiation and it emits a photon. From the interaction Hamiltonian given in the above paper there are four possible probabilities which can be calculated; The case mentioned above (from equation (2)), the case where the atom is in the excited state, absorbs a photon and then moves to the ground state, spontaneous emission and finally absorption of a photon. It is worth looking at each of the three cases, relativistically and for the SHO, to obtain the probabilities for these scenarios. 

The interaction Hamiltonian is given as:
$$\hat V(\tau) = {\hbar} {g} ({\hat a}{\phi_\omega} + {\hat a^\dagger}{\phi_\omega^*})({\hat \sigma}{e^{-i\omega_0\tau}} + {\hat \sigma^\dagger}{e^{i\omega_0\tau}})$$
Using this to treat each scenario we have
\subsection{The relativistic second case: Moving from the excited state to the ground state and absorbing a photon}
The probability is
$$P = g^2 \left|
\int_{-\infty}^\infty\bigl d \tau\bra{0,b}\hat V(\tau)\ket{1_\omega,a} \right|^2$$
This gives
$$P = g^2 \left|\int_{-\infty}^\infty\bigl d \tau [e^{-i \omega (z(\tau) - z_0)} - c.c.] e^{-i \omega t(\tau) - i \omega_0 \tau} \right|^2$$
Sending $\tau \rightarrow -\tau$ yields
$$P = g^2 \left|-\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{i \omega t(\tau) + i \omega_0 \tau} \right|^2$$
Which is just equation (2) with a difference in minus sign. So the probability is the same as the first case done in section 0.1.

\subsection{Relativistic third case: Spontaneous emission}
$$P = g^2 \left|
\int_{-\infty}^\infty\bigl d \tau\bra{1_\omega,b}\hat V(\tau)\ket{0,a} \right|^2$$
yields
$$P = g^2 \left|\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{i \omega t(\tau) - i \omega_0 \tau} \right|^2$$
following similar calculations as section 0.1
From (1) 
$$\pm z(\tau) + t(\tau) =  \pm\frac{1}{a}e^{\pm a\tau},$$
so the integral is
\begin{eqnarray*}
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{a\tau}} e^{-i\omega z_0}  e^{-i \omega_0 \tau}  d \tau 
-&&\kern -27pt\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{-a\tau}} e^{i\omega z_0}  e^{-i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau 
-\int_{-\infty}^\infty 
e^{-i \frac{\omega}{a} e^{-a\tau}} e^{i\omega z_0}  e^{- i \omega_0 \tau}  d \tau \\
&=&
\int_{-\infty}^\infty 
e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}  d \tau -c.c.
\end{eqnarray*}
where we've changed integration variable $\tau \rightarrow -\tau$ in the first integral. So 
$$ P= g^2 \left|
\int_{-\infty}^\infty\bigl[e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{i \omega_0 \tau}
 -c.c. \bigr] d \tau
\right|^2 .$$

Now change integration variables from $\tau$ to $x=\frac{\omega }{a} e^{-a\tau}$, so
$d \tau = \frac{-1}{a x} d x $,
$$
\int_{-\infty}^\infty e^{i \frac{\omega}{a} e^{-a\tau}} e^{-i\omega z_0}  e^{ i \omega_0 \tau} d\tau
=\frac{1}{a} e^{-i \bigl(\omega z_0 + \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\bigr) }
\int_0^\infty e^{i x}  x^{-i\frac{\omega_0}{ a}-1 }d x.
$$
Now consider the integrals
$$I_\pm
=\int_0^\infty e^{\pm i x}  x^{\mp i\frac{\omega_0}{a}-1} d x.$$
Let $x= \pm i u = e^{\pm \frac{i\pi }{2}} u$ and $z = \mp \frac {i\omega_0}{ a}$, then
$$I_\pm =e^{\frac {\pi \omega_0 }{2 a}}\int_0^{\mp i\infty} e^{-u}  u^{z-1} d u.$$
This is almost a $\Gamma$-function as in section 0.1, except the integrals are along the imaginary 
axis rather than the real axis. 
Provided $\Re z>0$ (so $\omega_0 \rightarrow \omega_0 \pm  i \epsilon$ with
$\epsilon >0$) we can rotate the contour to get
$$ \int_0^{\mp i\infty} e^{-u}  u^{z-1} d u = \int_0^{\infty} e^{-u}  u^{z-1} d u = \Gamma(z), \qquad \Re z>0,$$
and
$$ I_\pm\left(\frac{\omega_0 }{a}\right) =e^{\frac{\pi \omega_0 }{2a}}
\lim_{\epsilon\rightarrow 0^+} \Gamma\left(\mp \frac{i \omega_0 }{a} + \frac{\epsilon }{a}\right) =  e^{\frac{\pi \omega_0 }{2a}}\Gamma\left(\mp\frac{i \omega_0 }{a}\right),$$
Write
$$ \Gamma\left(\mp\frac{i \omega_0 }{a}\right) = e^{\mp i\psi}\left|\Gamma\left(\mp\frac{i \omega_0 }{a}\right)\right|.$$
The phase $\psi$ will depend on $\frac{\omega_0 }{a}$, we don't know it's analytic form, but that doesn't matter.
What we do know is
$$ \left|\Gamma\left(\mp \frac{i \omega_0 }{a}\right)\right|^2 =\frac {a \pi }{\omega_0\sinh\left(\frac { \pi\omega_0 }{a}\right)},$$
the probability then is
\begin{eqnarray}
P&=&\frac{\pi g^2 e^{\frac{\pi \omega_0 }{a}} }{a \omega_0 \sinh\left(\frac{\omega_0 }{a}\right)}
\left|e^{-i \Bigl(\omega z_0 + \frac{\omega_0}{a}\ln\bigl((\frac{a }{\omega}\bigr)\Bigr) }e^{-i\psi}
- e^{i \Bigl(\omega z_0 + \frac{\omega_0}{a}\ln\bigl(\frac{a }{\omega}\bigr)\Bigr) }e^{i\psi} 
\right|^2   \\
&=&  
\frac{4 \pi g^2  \sin^2(\omega z_0 + \varphi) }{a \omega_0 e^{\frac{-\pi \omega_0 }{a}} \sinh\left(\frac{\omega_0 }{a}\right)}=  \frac{8 \pi g^2}{a \omega_0} \frac{\sin^2(\omega z_0 + \varphi) }{1-e^{\frac{-2\pi \omega_0 }{a}}}
\end{eqnarray}
where 
$$\varphi = \frac{\omega_0}{a} \ln \left(\frac{a}{\omega } \right) + \psi.$$

So $P$ is divergent for $a \rightarrow 0$

\subsubsection{Relativistic fourth case: Absorption of a photon}

The probability is 
\begin{eqnarray}
P&=& g^{2} \left|
\int_{-\infty}^\infty\bigl d \tau\bra{0,a}\hat V(\tau)\ket{1_\omega,b} \right|^2   \\
&=&  
g^2 \left|-\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{-i \omega t(\tau) + i \omega_0 \tau} \right|^2
\end{eqnarray}
If we send $\tau \rightarrow -\tau$ $P$ becomes
$$=g^2 \left|-\int_{-\infty}^\infty\bigl d \tau [e^{i \omega (z(\tau) - z_0)} - c.c.] e^{i \omega t(\tau) - i \omega_0 \tau} \right|^2$$
Which is the same as the third case case.

\subsubsection{Second case for non-relativistic SHO:\bra{0,b}\hat V\ket{1_\omega,a}}

$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{-i k (A \sin(\Omega \tau)-z_0)} - c.c. \bigr] e^{-i \omega \tau - i \omega_0 \tau} d \tau
\right|^2. $$
sending $\tau \rightarrow -\tau$
$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau) + z_0)} -c.c. \bigr] e^{i \omega \tau + i \omega_0 \tau} d \tau
\right|^2. $$
Which is the probability for the first SHO case done in sections 0.2 and 0.3 with $z_0 \rightarrow -z_0$.

\subsubsection{Third case for non-relativistic SHO: \bra{1_\omega,b}\hat V\ket{0,a}}

$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau)-z_0)} - c.c. \bigr] e^{i \omega \tau - i \omega_0 \tau} d \tau
\right|^2. $$

this is the first case for the SHO with $\omega_0 \rightarrow -\omega_0$.

\subsubsection{Fourth case for non-relativistic SHO:\bra{0,a}\hat V\ket{1_\omega,b}}

$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{-i k (A \sin(\Omega \tau)-z_0)} - c.c. \bigr] e^{-i \omega \tau + i \omega_0 \tau} d \tau
\right|^2. $$
send $\tau \rightarrow -\tau$
$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau)+z_0)} - c.c. \bigr] e^{i \omega \tau - i \omega_0 \tau} d \tau
\right|^2. $$
again this is the first case for the SHO but now with $ \omega_0 \rightarrow -\omega_0$ and $z_0 \rightarrow -z_0$. 

The above are variations of the possible quantum states that arose from the initial setup by [cite: Svidzinsky et. al.]. This setup though now affords us a more thorough setting from which we can analse other trajectories for a particle, allowing us to more generally tackle an accelerated quantum state by simply imposing an accelerated trajectory instead of needing to specify the potential providing the energy for the acceleration. In the next sections we play around with non-relativisitic trajectories arrived at through our relativistic setup and find that we arrive at feasible probabilities that give rise to acceleration radiation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{\it\bf Oscillating 2-state atom with a mirror :-}\label{mirror}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Oscillating Atom from Paper}

%\label{sec:mirror}
We now consider an atom forced to oscillate in the presence of a stationary mirror, the latter located at $z_0$, oscillating with a motional angular frequency $\Omega$,  around $z=0$
with amplitude $0<A<z_0$ 
(so we do not hit the mirror),  and set $ z(t) = A \sin(\Omega t).$
%$$ z(t) = A \sin(\Omega t).$$
Using this in (2), the probability of creating a photon of frequency
$\omega$ from the vacuum, and at the same time exciting the atom from its ground state to its excited state is
$$P(\omega)= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega t) - z_0)} -c.c. \bigr] e^{i (\omega +  \omega_0)t} d t
\right|^2. $$
Simplify the notation by absorbing $\Omega$ into $t$ and defining dimensionless variables 
$\tau = \Omega t$, $\tilde \omega = (\omega +\omega_0)/\Omega$,
$\tilde A = k A$ and $\tilde z_0 = k z_0$, we obtain
\begin{eqnarray} P(\omega) &=& \frac{g^2}{\Omega^2} \left|
\int_{-\infty}^\infty\bigl[
e^{i (\tilde A \sin \tau - \tilde z_0)} -c.c. \bigr] e^{i \tilde \omega \tau} d \tau\right|^2 \nonumber\\ 
&=& \frac{g ^2}{\Omega^2} \left|
e^{-i\tilde z_0}\int_{-\infty}^\infty e^{i (\tilde A \sin \tau+ \tilde \omega \tau)} d \tau \right.\nonumber\\ 
& &\qquad\qquad\left.-e^{i\tilde z_0}\int_{-\infty}^\infty  e^{i (\tilde A \sin \tau - \tilde \omega \tau)} d  \tau\right|^2.
\label{totalSHO-probability} 
\end{eqnarray}

The integrals appearing in (\ref{totalSHO-probability}) 
 are related to
Anger functions \cite{Abramowitz1970} (section 12.3.1),
$$ {\bf J}_\nu(x)=\frac{1}{2\pi}\int_{-\pi}^\pi e ^{i(x \sin\theta - \nu \theta)}d \theta
= \frac{1}{\pi}\int_0^\pi \cos(x\sin\theta - \nu\theta)d \theta.$$
But Anger functions are not quite what we want since what we have in (\ref{totalSHO-probability})
, is
\begin{eqnarray}
\int_{-\infty}^\infty  e ^{i(x \sin\theta - \nu \theta)} d \theta
&=&\!\! \sum_{s=-\infty}^\infty\, \int_{-\pi}^\pi e^{i\bigl(x \sin\theta - \nu(\theta+2s\pi)\bigr)}d \theta \\
&=&\!\! \pi {\bf J}_\nu(x) \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}.
\label{eq:totalamplitude}
\end{eqnarray}
Letting $ \nu = n + \{\nu\}$, 
%$$ \nu = n + \lfloor\nu\rfloor$$
where $n$ is an integer, and $0 \le  \{\nu\}<1$, is the non-integral part of $\nu$,
then
$ \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}= \sum_{s=-\infty}^\infty  e^{-2is\{\nu\}\pi} = 1 + 2\sum_{s=0}^\infty  \cos(2s\{\nu\}\pi) = \pi \delta(\{\nu\})$
and (\ref{eq:totalamplitude}), vanishes unless $\nu$ is an integer, in which case it
diverges. This is not unexpected since when Fermi's Golden Rule says that if the transition rate is constant, integrating over all $t$ will necessarily give an infinite answer for any transition with non-zero probability.  For our periodic case its more informative to estimate a transition rate over a motional cycle rather than the accumulated  probability over all time.

\sloppy Before estimating this let us consider the case when $\nu$ is a non-zero rational number, $\nu = p/q$ with $p$ and $q$ mutually prime and positive, in the integral
$$ \int_{-\infty}^\infty e^{i(x\sin \theta -\nu \theta)} d \theta
= q \int_{-\infty}^\infty e^{i(x\sin (q \psi)  - p \psi)} d \psi 
$$
where $\psi = \theta/q$. The integrand is periodic in $\psi$
with period $2\pi$ so again the integral will diverge (unless the integral over one period vanishes).  Integrating over just one period in $\psi$, we can define
\begin{eqnarray}
{\cal J}(x;p,q) &=& 
\frac{1}{2 \pi} \int_{-\pi}^\pi e^{i(x \sin (q \psi)  - p \psi )} d \psi\\\nonumber
&=& \frac{1}{\pi} \int_0^\pi \cos\big\{x \sin (q \psi)  - p \psi \bigr\} d \psi,
\label{eq:J-def}
\end{eqnarray}
which, in terms of Anger functions, becomes
\begin{eqnarray}
{\cal J}(x;p,q) &=& 
\frac{1}{2 \pi q} \int_{-q\pi}^{q \pi} e^{i(x \sin \theta  - \frac p q  \theta )} d \theta \\\nonumber
&=&\frac{1}{q}  {\bf J}_{\frac p q }(x)\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}}.\nonumber
\end{eqnarray}
We note however that $$\sum_{s=0}^{q-1} \exp({i \pi (2 s - q + 1)p/q}) = 
\exp({-i\pi\frac{p(q-1)}{q}}) \sum_{s=0}^{q-1} \exp({2i \pi p s/q})=0,$$ 
%$$
%\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}} = 
%e^{-i\pi\frac{p(q-1)}{q}} \sum_{s=0}^{q-1} e^{\frac{2i \pi p s}{q}}=0 
%$$
since $\sum_{s=0}^{q-1} \exp(2i \pi p s/q)$,
vanishes for any two integers $p$ and $q$, provided $p/q$ is not an 
integer.
 From this observation we conclude  that the transition rate is zero unless $\tilde \omega$ is a
positive integer, that is 
\begin{equation}
\omega + \omega_0 = n\Omega,\label{eq:Omega-restriction}
\end{equation}
where $\Omega$ is the mechanical frequency, $\omega_0$ is the atomic transition frequency, $\omega$ is the frequency of the photon field and $n$ is an integer.
Since $\tilde \omega$ is  positive, $n>0$, and to obtain a closed expression for the transition probability over a mechanical cycle we can use the integral
representation of the Bessel function,  \cite{Abramowitz1970} (section 9.1.21),
$J_n (\tilde A) = \frac{1}{2 \pi}\int_{-\pi}^{\pi} 
\exp[{i(\tilde A \sin \tau - n \tau)}] d \tau = (-1)^n J_{-n}(\tilde A)$,
%\[
%J_n (\tilde A) = \frac{1}{2 \pi}\int_{-\pi}^{\pi} 
%e^{i(\tilde A \sin \tau - n \tau)} d \tau = (-1)^n J_{-n}(\tilde A)
%\]
to write  $\int_{-\pi}^{\pi} \exp [{i(\tilde A \sin \tau + \tilde z_0 -  n  \tau)} ]d \tau= 2 \pi e^{i \tilde z_0}  J_n(\tilde A)$, and $\int_{-\pi}^{\pi} \exp[{i(\tilde A \sin \tau -
 \tilde z_0 +  n \tau)} ]d  \tau
= 2 \pi e^{-i (\tilde z_0 - n \pi)}  J_n(\tilde A)$.
%\begin{eqnarray*}
%\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tau + \tilde z_0 -  n  \tau)} d \tau
%&=& 2 \pi e^{i \tilde z_0}  J_n(\tilde A)\\
%\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tau -
% \tilde z_0 +  n \tau)} d  \tau
%&=& 2 \pi e^{-i (\tilde z_0 - n \pi)}  J_n(\tilde A).
%\end{eqnarray*}
By dividing by the period of mechanical oscillation, $2\pi/\Omega$, we get a transition rate (in ${\rm Hz}$), as
\begin{eqnarray}
\overline P_{n} & = &\frac{\Omega }{2 \pi}
\frac{g^2}{ \Omega^2} \left|
 \Bigl[ 2 \pi \left(e^{-i (\tilde z_0 - n \pi)} -  e^{i \tilde z_0}\right) \Bigr]
J_n(\tilde A)\right|^2\nonumber\\
&=&
\frac{8 \pi g^2}{\Omega} \sin^2\left(\tilde z_0 -\frac{\pi n}{2}\right) J_n^2(\tilde A)\\
&=&
\frac{8 \pi g^2}{\Omega} \sin^2\left(k z_0 -\frac{\pi n}{2}\right) J_n^2(k A),\label{eq:mirror-rate}
\end{eqnarray}
where $\omega = n \Omega - \omega_0 >0$. 
\vspace{.25cm}\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\subsection{Oscillating 2-state atom}

So let's take an oscillating atom. If the motion is relativistic we can use the
anharmonic trajectory, described in 
W.~Moreau, R.~Easther and R.~Neutze, {\it American Journal of Physics} {\bf 62}, 531 (1994) in terms of elliptic integrals.  But first lest just do non-relativistic
simple harmonic motion.  So
$$ t = \tau, \qquad z(\tau) = A \sin(\Omega \tau) + z_0, $$
with angular frequency $\Omega$ and  the amplitude $0<A<z_0$ so we don't hit the mirror!  Put this in (2), with $c$ re-instated so $k c = \omega$,
$$P= g^2 \left|
\int_{-\infty}^\infty\bigl[
e^{i k (A \sin(\Omega \tau)-z_0)} -c.c. \bigr] e^{i \omega \tau + i \omega_0 \tau} d \tau
\right|^2. $$
Simplify the notation by absorbing $\Omega$ into $\tau$ and defining 
$\tilde \tau = \Omega \tau$, $\tilde \omega = \frac{\omega +\omega_0}{\Omega}$,
$\tilde A = k A$ and $\tilde z_0 = k z_0$.
These are all dimensionless variables, in terms of which 
$$ P = \frac{g^2}{\Omega^2} \left|
\int_{-\infty}^\infty\bigl[
e^{i (\tilde A \sin \tilde \tau-\tilde z_0)} -c.c. \bigr] e^{i \tilde \omega \tilde \tau} d \tilde \tau\right|^2 =    
\frac{4 g^2}{\Omega^2} \left|
\int_{-\infty}^\infty\sin\bigl(\tilde A \sin \tilde \tau-\tilde z_0\bigr) 
e^{i \tilde \omega \tilde \tau} d \tilde \tau\right|^2. $$
Alternatively
\begin{eqnarray} 
P(\tilde A,\tilde z_0; \tilde\omega) &=& \frac{g^2}{\Omega^2} \left|
e^{- i\tilde z_0}\int_{-\infty}^\infty
e^{i (\tilde A \sin \tilde \tau+ \tilde \omega \tilde \tau)} d \tilde \tau 
- e^{i\tilde z_0}\int_{-\infty}^\infty e^{- i (\tilde A \sin \tilde \tau - \tilde \omega \tilde \tau)} d \tilde \tau\right|^2\nonumber \\
&=& \frac{g^2}{\Omega^2} \left|
e^{- i\tilde z_0}\int_{-\infty}^\infty
e^{i (\tilde A \sin \tilde \tau+ \tilde \omega \tilde \tau)} d \tilde \tau 
- e^{i\tilde z_0}\int_{-\infty}^\infty e^{i (\tilde A \sin \tilde \tau - \tilde \omega \tilde \tau)} d \tilde \tau\right|^2\label{eq:total-SHO-probability}
\end{eqnarray}
where we have changed integration variables from $\tilde \tau$ to $-\tilde \tau$ in the 
second integral.

\subsection{Transition rates}

The integrals appearing in (\ref{eq:total-SHO-probability}) are related to
Anger functions (Abromowitz+Stegun: 12.3.1; {\tt https://dlmf.nist.gov/11.10})
$$ {\bf J}_\nu(x)=\frac{1}{2\pi}\int_{-\pi}^\pi e ^{i(x \sin\theta - \nu \theta)}d \theta
= \frac{1}{\pi}\int_0^\pi \cos(x\sin\theta - \nu\theta)d \theta.$$
Obviously
$$ {\bf J}_{-\nu}(x) =  {\bf J}_{\nu}(-x)$$
and when $\nu=n$ is an integer
$$ {\bf J}_n(x) = J_n(x),$$
a Bessel function of integer order.

Anger functions satisfy the inhomogeneous Bessel equation
$$x^2 
\frac{d^2 {\bf J}_\nu}{d^2 x} + x \frac{d {\bf J}_\nu}{d x}
+(x^2 - \nu^2) {\bf J}_\nu = (x-\nu)\frac{\sin(\nu\pi)}{\pi} 
$$
and a 3D plot as functions of $\nu$ and $x$ are shown in fig. 1.

%\begin{figure}[h]
%\includegraphics[scale=0.5]{Anger-3D}
%\caption{Anger function.}
%\end{figure}

But Anger functions are not quite what we want, what we have is
\begin{equation}
\int_{-\infty}^\infty  e ^{i(x \sin\theta - \nu \theta)} d \theta
= \sum_{s=-\infty}^\infty\left( \int_{-\pi}^\pi e^{i\bigl(x \sin\theta - \nu(\theta+2s\pi)\bigr)}d \theta \right)
= \pi {\bf J}_\nu(x) \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}.
\label{eq:total-amplitude}\end{equation}
Let
$$ \nu = n + \lfloor\nu\rfloor$$
where $n$ is an integer and $0 \le  \lfloor\nu\rfloor<1$ is the non-integral part of $\nu$. 
Then
$$ \sum_{s=-\infty}^\infty  e^{-2is\nu\pi}= \sum_{s=-\infty}^\infty  e^{-2is[\nu]\pi} = 1 + 2\sum_{s=0}^\infty  \cos(2s\lfloor\nu\rfloor\pi) = \delta(\lfloor\nu\rfloor)$$
and (\ref{eq:total-amplitude}) vanishes unless $\nu$ is an integer, in which case it
diverges.

We can check this when $\nu$ a rational number, $\nu = \frac{p}{q}$ with $p$ and $q$ mutually prime and positive.  Then
$$ \int_{-\infty}^\infty e^{i(x\sin \theta -\nu \theta)} d \theta
= q \int_{-\infty}^\infty e^{i(x\sin (q \psi)  - p \psi)} d \psi 
$$
where $\psi = \frac{\theta}{q}$. The integrand is periodic in $\psi$
with period $2\pi$ so the integral will diverge (unless the integral over one period vanishes), so integrate over one period in $\psi$ and define
\begin{equation}
{\cal J}(x;p,q) = 
\frac{1}{2 \pi} \int_{-\pi}^\pi e^{i(x \sin (q \psi)  - p \psi )} d \psi
= \frac{1}{\pi} \int_0^\pi \cos\big\{x \sin (q \psi)  - p \psi \bigr\} d \psi.
\label{eq:J-def}
\end{equation}
In terms of Anger functions
$${\cal J}(x;p,q) = 
\frac{1}{2 \pi q} \int_{-q\pi}^{q \pi} e^{i(x \sin \theta  - \frac p q  \theta )} d \theta 
=\frac{1}{q}  {\bf J}_{\frac p q }(x)\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}}.$$
Now 
$$
\sum_{s=0}^{q-1} e^{i \pi (2 s - q + 1)\frac{p}{q}} = 
e^{-i\pi\frac{p(q-1)}{q}} \sum_{s=0}^{q-1} e^{\frac{2i \pi p s}{q}}=0 
$$
since $\sum_{s=0}^{q-1} e^{\frac{2i \pi p s}{q}}$ vanishes for any two positive integers $p$ and $q$.

We conclude from this that the transition rate is zero unless $\tilde \omega$ is a
positive integer, that is 
\begin{equation}
\omega + \omega_0 = n\Omega,
\end{equation}
this is a genuine quantum phenomena (though $\hbar$ does not appear
explicitly in the formula for the probability.\footnote{I guess it must be hiding in $g^2$, if this is a genuine quantum phenomenon the probability should vanish when $\hbar\rightarrow 0$.})  The divergence when $\nu=\tilde \omega$ is  presumably a consequence of Fermi's Golden Rule: in first order perturbation theory the transition rate is constant, so the total probability integrated over all time will diverge.
Better to calculate probability rate rather than a 
probability. 

Since $\tilde \omega$ is a positive integer, $n>0$, for a transition we can use the integral
representation of the Bessel function,\footnote{Abromowitz+Stegun: 9.1.21.}
\begin{eqnarray*}
J_n (\tilde A) &=& \frac{1}{2 \pi}\int_{-\pi}^{\pi} 
e^{i(\tilde A \sin \tilde \tau - n \tilde \tau)} d \tilde \tau \\
J_{-n}(\tilde A) 
&=&\frac{1}{2 \pi}\int_{-\pi}^{\pi} 
e^{i(\tilde A \sin \tilde \tau + n \tilde \tau)} d \tilde \tau
= (-1)^n J_n(\tilde A),
\end{eqnarray*}
to write
\begin{eqnarray*}
\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tilde \tau +\tilde z_0 -  n \tilde \tau)} d \tilde \tau
&=& 2 \pi e^{i \tilde z_0}  J_n(\tilde A)\\
\int_{-\pi}^{\pi} e^{i(\tilde A \sin \tilde \tau - \tilde z_0 +  n \tilde \tau)} d \tilde \tau
&=& 2 \pi e^{-i (\tilde z_0- n \pi)}  J_n(\tilde A).
\end{eqnarray*}

Dividing by $\frac{2\pi}{\Omega}$, the period of the oscillator, we get a transition rate
\begin{eqnarray}
\overline P_n & = &\frac{\Omega }{2 \pi}
\frac{g^2}{ \Omega^2} \left|
 \Bigl[ 2 \pi \left((-1)^n e^{-i \tilde z_0} -  e^{i \tilde z_0}\right) \Bigr]
J_n(\tilde A)\right|^2\nonumber\\
&=&
\frac{8 \pi g^2}{\Omega} \sin^2\left(\tilde z_0 -\frac{\pi n}{2}\right) J_n^2(\tilde A)=
\frac{8 \pi g^2}{\Omega} \sin^2\left(k z_0 -\frac{\pi n}{2}\right) J_n^2(k A),
\end{eqnarray}
where $\omega = n \Omega - \omega_0 >0$.
Can the $\sin^2\left(k z_0 -\frac{\pi n}{2}\right)$ factor be 
interpreted as some kind of dynamical Casimir effect? 

If there's no mirror
\begin{equation}
\overline P_n  = \frac{\Omega }{2 \pi}
\frac{g^2}{\Omega^2} \left|
\int_{-\pi}^\pi e^{i \tilde A \sin \tilde \tau} e^{i \tilde \omega \tilde \tau} d \tilde \tau
\right|^2 
  = \frac{2 \pi g^2 }{\Omega} J_n^2( k A) ,\qquad n>0.
\label{eq:P_n-no-mirror}
\end{equation}
Even with no mirror you can excite an atom and emit a  photon at the same time by shaking the atom hard enough to supply energy.  
 
Some useful approximations might be (A+S refers to Abromowitz and Stegun)
\begin{eqnarray}
 J_n(x) & \approx& \frac{x^n}{2^n n!}, \qquad x \ll n    (A+S:9.1.7) \\
 J_n(x)&\approx& \sqrt\frac{2}{\pi x} \cos\left( x - \frac{(2 n +1)\pi}{4}\right), 
\qquad x \gg n  (A+S:9.2.1) \\
 J_n(n) & < & \frac{2^{\frac{1}{3}} }{3^{\frac{2}{3}}} \Gamma\left(\frac{2}{3}\right) 
n^{\frac{1}{3}}
\approx\frac{0.683 }{n^{1}{3}}, \qquad n > 0  (A+S:9.1.61). 
\end{eqnarray}
This last bound was improved to 
$$\sup_x |J_n(x)| < \frac{0.674885 }{n^{\frac{1}{3}}}$$ in L.J.~Landau, {\sl Bessel Functions: Monotonicity and Bounds}, \hfill\break
{\it Journal of the London Mathematical Society}, {\bf 61}, issue 1 (2016).
Empirically the maximum is near $x\approx n$, to less than 10\% for $n$ greater than about 25, for $n=1$ the maximum is $\approx 0.582$ at $x\approx 1.84$. 

\subsection{Atom performing SHO in free space}

The transition rate (\ref{eq:P_n-no-mirror}) with  $\omega = n\Omega - \omega_0$ is 
$$\overline P_n= \overline P(n \Omega - \omega_0)  
  = \frac{2 \pi g^2 }{\Omega} J_n^2\left(\frac { (n \Omega -\omega_0)  A }{c}\right),$$
where the speed of light has been re-instated. This is plotted on figure 2
for various values of $n$, with the factor $\frac{2 \pi g^2}{\Omega}$ omitted.

%\begin{figure}[h]
%\centerline{\includegraphics[scale=0.4]{BesselJ-squared}}
%\centerline{\includegraphics[scale=0.4]{BesselJ-100-squared}}
%\caption{Transition rate for SHO forced atom in free space to emit a photon with angular
%frequency $\omega = n\Omega - \omega_0$ and wavelength $\lambda=\frac{2\pi c}{\lambda}$ (\ref{eq:P_n-no-mirror})
%as a function of $\tilde A =\frac{2\pi}{\lambda} A$. The factor 
%$\frac{2 \pi g^2}{\Omega}$ is omitted and the upper plot just shows the first three Bessel functions,
%$J_n^2(\tilde A)$ for $n=1,2,3$.
%If $\Omega \ll\omega_0$ then $n$ must be large for $\omega>0$ and the lower
%plot shows $J_{100}^2(\tilde A)$, We see that is negligible until $\tilde A$ is of order $n$.}
%\end{figure}
%
Using (\ref{eq:P_n-no-mirror}) and the above approximations the transition rate is
\begin{equation}
\overline P = 
\begin{cases}
\frac{2 \pi g^2}{\Omega} 
\frac{(k A)^{2 n}}{2^{2n} (2n)!}, &  A \ll \frac{n \lambda }{2 \pi};\\
\frac{2 \pi g^2}{\Omega} \frac{(0.683)^2}{n^{\frac{2}{3}}}, & 
A \approx \frac{n \lambda }{2 \pi} \hbox{for} n>25;\\
 \frac{2 g^2 \lambda}{\pi \Omega A }\cos\left(k A -\frac {(2 n +1)\pi}{4 } \right),   &   A \gg \frac{n \lambda }{2 \pi}. 
\end{cases}
\end{equation} 
 
The largest value that $J_n(x)$ can take is 0.582 when $n=1$ and  $x=1.481$
and this is only achievable if $\Omega > \omega_0$, assuming this is the case
the highest transition rate is 
$$\overline P_1 = \frac{2 \pi g^2}{\Omega} (0.582)^2 \approx \frac{2.1 g^2 }{\Omega},$$ for  photons with $\omega = \Omega - \omega_0$, and this is only 
achieved by tuning the oscillation amplitude to 
$$A= \frac{1.481 \lambda }{2 \pi}= \frac{1.481 c }{(\Omega - \omega_0)}.$$


If $\Omega < \omega_0$ then the largest transition rate depends on how much less.
Let $n$ be the smallest integer for which $\omega = n \Omega - \omega_0 >0$.
Then
$$\overline P_n = \frac{2 \pi g^2 }{\Omega} \frac{(0.683)^2}{n^{\frac{2}{3}}} $$
for 
$$ A=\frac{n c }{(n \Omega - \omega_0)}.$$
 
To get an idea of numbers lets consider (5) and assume that the transition frequency of the atom $\omega_0$ and the frequency of the emitted photon $\omega$ 
are both in the optical (visible) range.
Then $\Omega = \frac{\omega + \omega_0 }{n}$, which would probably be in the ultraviolet for $n=1$, but would be in the visible for $n=2$ and is lower for larger $n$.
We can make $\Omega$ as low as we wish by taking $n$ as large as we wish. 
For $n=2$ the maximum of $J_2(x)$ is close to $x=3$, so if $\Omega$ is in the
optical the probability rate (5) is a maximum for 
$A\approx \frac{3}{k} = \frac{3 \lambda }{2 \pi}$, 
of the order of a thousand ${\buildrel _{\circ} \over {\mathrm{A}}}$, %$\AA$ 
a thousand times bigger than the atom itself.  But even if that is feasible the transition is suppressed by a
factor $\Omega \sim \omega$, which is of order $10^{15}$ Hz. 
How big can $g^2$ be
in a real experiment? ($g^2$ has dimensions of inverse time$^2$.)   

If $\Omega$ is to be much lower than optical
frequency then $n$ must be large.  As $n$ increases the first (and largest) peak in $J_n(x)$
moves out to larger $x\approx n$ and the maximum rate is for $A\approx \frac{n \lambda }{2 \pi}$.  If we want $\Omega<<\omega$ then $n>>1$ and we can
use (6) to get a maximum value for the transition rate
$$\overline P_n \approx \frac{3 \pi g^2}{\Omega n^{\frac{2}{3}}} =
\frac{3 \pi g^2 n^{\frac{1}{3}}}{(\omega + \omega_0)}  \qquad \hbox{for}\qquad A = \frac{n \lambda}{2 \pi}.$$
For fixed $\omega$ and $\omega_0$, $\overline P$ grows like $n^{\frac{1}{3}}$ and can be made large by taking $\Omega<<\omega_0$. This is not a problem,
 $n$ is large but $\omega$ also large, so $\overline P_n$ is not growing with $n$,
we can't fix $\omega$ and let $n$ grow.


\subsection{Oscillating mirror}

However, if there is a mirror we can try keeping the atom fixed and oscillating the mirror.  If we don't bother with the distinction between Rindler and
Boulware vacua for small accelerations (wouldn't know what they were for
oscillatory motion anyway!) I would naively assume that we just replace $z(\tau)-z_0$ 
with $z-z_0(\tau)$ where $z_0(\tau) = A\sin(\Omega t)$ is the position of the
mirror and $z$ (constant) the position of the stationary atom.
Also $\omega t(\tau)+\omega_0 \tau \rightarrow\omega \tau+\omega_0 t(\tau)$,
but non-relativistically  $t(\tau)=t$ so no change there.
The only effect is to replace
$z_0$ in (4) with the position of the atom, $z$, and otherwise (4) is unchanged. 

Jason said that boundary conditions mimicking an accelerating mirror can be cooked up in the lab
without having to mechanically accelerate a physical mirror.
Fulling and Wald talk about microwave transitions for $\omega_0$  ($0.3\sim 300$ GHz) and effective couplings $g_{eff}\sim 10$ MHz.
If we assume $\omega$ is also in the microwave region (so $\lambda\approx 0.1 \sim 100$ cm) then,
$\frac{ g_{eff}^2 }{(\omega + \omega_0)}\approx  10^3 \sim 10^5$ Hz.
 and transition rate is of order
For $n>10$, the Bessel function has a maximum
pretty close to $k A = n$, with $J_n(n)\approx \frac{0.675 }{n^{\frac{1}{3}}}$,
giving a transition probability
$$\overline P \approx \frac{11.5 \,g^2_{eff} }{\omega+\omega_0} n^{\frac{1}{3}}
\sin^2\left( k z - \frac{\pi n}{2}\right) \approx  10^5 \sin^2\left( \frac{2 \pi  z}{\lambda}-\frac{\pi n}{2}\right) n^{\frac{1}{3}}.$$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Generalisations and Other Setups: Stimulation from mechanical oscillation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\it\bf 2-dimensional motion}


The formalism can be applied to a 2-level atom following any closed trajectory $\vec x(t)$ in the two dimensional $y-z$ plane, with a flat mirror located at $z_0$ extending in the $y$-direction.   For an electromagnetic wave with wave-vector $(k_y,k_z)$ we simply replace $k (z(t) - z_0)$ in (\ref{eq:phi-mirror}) with
$\vec k.\vec x(t) - k_z z_0$. One cannot obtain analytic answers for a general trajectory but some simple cases are immediate:
\vspace{.25cm}\\


{\it\bf 2-level atom oscillating parallel to a mirror:-}  for oscillation in the $y$-direction replace $k (z(t) - z_0)$ in (\ref{eq:phi-mirror}) with
$ k_y A \sin(\Omega t)  - k_z z_0 $  with $A$ again a constant amplitude.
The analysis is identical and (\ref{eq:mirror-rate}) still holds, but with $k z_0$ replaced with $k_z z_0$ and $k A$ replaced with $k_y A$.
\vspace{.25cm}\\


{\it\bf Rotating 2-level atom with a mirror:-} for an atom rotating around the fixed point $(0,z_0)$ in a circle with radius $R$
and constant angular velocity $\Omega$, $\vec x(t) = R(\cos\Omega t),\sin(\Omega t)$ and
$\vec k.\vec x(t)=k_y R \cos(\Omega t) + k_z R \sin(\Omega t)$.
If we parameterize the direction of the electromagnetic wave by a phase $\delta$ with
 $k_y=k\sin\delta, \quad k_z = k\cos\delta$
then
  $k_y R \cos(\Omega t) + k_z R \sin(\Omega t) - k_z z_0  = k R \sin(\Omega t + \delta) - k z_0 \cos \delta $
and the phase $\delta$ 
in the sine function can be
absorbed into $\tau$ in (\ref{eq:phi-mirror}), which does not affect the result. We just replace the
amplitude $A$ in (\ref{eq:mirror-rate}) with the rotation radius $R$ and replace 
$k z_0$ with $k_z z_0 \cos \delta$.
\vspace{.25cm}\\


\subsection{\it\bf Oscillating 2-level atom in a cavity:-}\label{cavity}

 In a one-dimensional cavity containing no photons the transition rate to excite the atom and at the same time emit a photon of frequency $\omega$ is still given by (\ref{eq:mirror-rate}), except that the allowed values of $\omega$ are discrete, 
 $\omega = c k = \pi m c/L$,
with $m$ a positive integer and Eqn (\ref{eq:Omega-restriction}) imposes the condition
\[ \frac{\pi m c}{L} + \omega_0=n \Omega\]
on $\Omega$. The rate is enhanced however if the cavity already contains $N$ photons of 
frequency $\omega$, since then $\langle N+1|a^\dagger_\omega|N\rangle = \sqrt{N+1}$,
giving the transition rate to excite/de-excite the atom given $N$ photons in the cavity as,
\begin{equation}
\overline P_{n,m,N,\pm} = 
\frac{8 \pi \chi_\pm\, g^2}{\Omega} \sin^2\left(\frac{\pi m z_0}{L} -\frac{\pi n}{2}\right) J_n^2\left(\frac{\pi m A}{L}\right),\label{eq:cavity-rate}
\end{equation}
where $\chi_+=N+1$, to excite and emit a photon, while $\chi_-=N$ to de-excite the atom and absorb a photon, and
%With $N$ photons in the cavity there is also the possibility of exciting the atom
%and absorbing a photon, with transition rate
%\begin{equation}
%\overline P_{n,m.N,-} = 
%\frac{8 \pi N g_\omega^2}{\Omega} \sin^2\left(\frac{\pi m z_0 \cos\delta}{L} -\frac{\pi n}{2}\right) J_n^2\left(\frac{\pi m A}{L}\right)
%\end{equation}
%with the tuning
 %\begin{equation}
$n \Omega = \omega_0 - \omega = \omega_0 - \pi m c/L$. {\color{black} We note that in order to observe this phenomena one could consider one of the mirror's to be slightly imperfect and then one could perform spectroscopy on the photons leaking from the optical cavity. The signature of the photons created via (\ref{eq:cavity-rate}), will prove challenging to detect over any background of existing photon occupation within the cavity.}
%\end{equation}
\vspace{.25cm}\\

\begin{figure}[tp] 
\begin{center}
\setlength{\unitlength}{1cm}
\begin{picture}(8.5,7.5)
%\put(.1,-.4){\includegraphics[width=.95\columnwidth]{Figures/Fig1b}}
\put(-2,-.3){\includegraphics[width=.65\columnwidth]{Images/Shaking_Photons/Fig2}}
\end{picture}
\end{center}
\caption{Transition rate for SHO forced atom in free space to emit a photon with angular frequency $\omega = n\Omega - \omega_0$ and wavelength $\lambda={2\pi c}/{\omega}$, equation  (\ref{eq:P_n-no-mirror}), as a function of dimensionless oscillation amplitude $\tilde A =({2\pi}/{\lambda}) A$ and sideband index $n$. The prefactor 
${2 \pi g^2}/{\Omega}$ is omitted.  We see that transition rate is negligible until $\tilde A$ is of order $n$.}
   \label{Fig2}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experimental Scenario}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\it\bf Atom performing SHO in free space:-}\label{free} 

Repeating the analysis of previous section when there's no mirror, the transition rate to emit a   photon is,  using (\ref{eq:infinite-phi}),
\begin{equation}
\overline P_{n,\omega}  = \frac{\Omega }{2 \pi}
\frac{g^2}{\Omega^2} \left|
\int_{-\pi}^\pi e^{i \tilde A \sin \tau} e^{i \tilde \omega \tau} d \tau
\right|^2 
  = \frac{2 \pi g^2 }{\Omega} J_n^2( k A) ,
\label{eq:P_n-no-mirror}
\end{equation}
with $n>0$. Even with no mirror an atom can be excited and emit a photon at the same time by shaking the atom hard enough to supply the required energy.  
The transition rate (\ref{eq:P_n-no-mirror}), with  $\omega = n\Omega - \omega_0$ is 
\begin{equation}
\overline P_{n}
  = \frac{2 \pi g^2 }{\Omega} J_n^2\left(\frac { (n \Omega -\omega_0)  A }{c}\right),
\label{SHOfreespace}  
\end{equation}
and for a given $n$ the rate will be largest at the first peak of $J_n$. From Fig \ref{Fig2}, we observe that for a given $n$, the transition rate is negligible unless $\tilde{A}\sim n$. The maximum rate occurs when $n=1$ and $\tilde{A}\sim 1.8$, and here $\overline P_1\approx 2.1g^2/\Omega$, but to achieve this one must have a mechanical oscillation amplitude of $A\sim 1.8 c/(\Omega-\omega_0)$, which will be extremely large when compared to the highest realistically achievable values of $\Omega-\omega_0$, in an experiment. 

For a possible experimental demonstration of acceleration from a two level atom shaking in a vacuum we instead consider the case when the amplitude of oscillation $A$ is small enough so that the argument of the Bessel function in (\ref{SHOfreespace}), is small and we can use the expansion $J_1^2(x)\sim x^2/4,\; 0<x\ll 1$. To achieve a large rate we consider ultra-strong coupling $g$ of the atom to the continuum where $g=\alpha \omega_0$, with $\alpha\sim 0.2$ and above \cite{Forn-Diaz2016,  Magazzu2018, PuertasMartinez2019, FriskKockum2019, Forn-Diaz2019}. We consider a cQED setup where a two level superconducting artificial atom is placed on a vibrating cantilever/membrane which is ultra-strongly coupled via an inductive coupling to the electromagnetic vacuum of a nearby electromagnetic continuum of a superconducting co-planar waveguide. This is similar to recent experimental work \cite{Viennot2018}. By using a diamond based  nanomechanical resonator one can achieve motional frequencies in the GHz regimes \cite{Gaidarzhy2007,Rodriguez-Madrid2012}. From (\ref{SHOfreespace}),  with the approximation $J_1(x)^2 \sim x^2/4$, the rate is maximised when $\omega_0=\Omega/2$, and taking this for small amplitude oscillations we obtain $\overline P_{1}\approx(\pi A\alpha)^2\Omega^3/(32 c^2)$. Fig \ref{Fig3}, shows that the emission/transition rate for a shaken superconducting two level system can reach values of $\overline P_1\sim 10^{-4}\,{\rm Hz}$, which may be detectable in current cQED setups. {\color{black} One might also consider placing the mechanically oscillating qubit close to a mirror as discussed in Section \ref{mirror}. Oscillatory motion along an arbitrary direction in three dimensions would couple the qubit to both vacuum modes which either have the mirror as a boundary or unbounded vacuum modes (for motion parallel to the mirror). This would result in  emission of photons perpendicular to the mirror (the case treated in Section \ref{mirror}), and in directions parallel to the mirror's plane (the case treated in Section \ref{free}). Such a situation may be difficult to observe experimentally as one must achieve large couplings between the two level system and the continuum. This is possible in the above discussed cQED setup above as the electromagnetic continuum is restricted essentially to be one dimensional.}

{\color{black} We finally compare our results with recent related works. In \cite{Lo2018}, and \cite{Ferrari2019}, the authors respectively consider acceleration radiation from a mechanically oscillating two level system in free space  and the modification of spontaneous emission in a two level system adjacent to an oscillating mirror. However their studies are restricted to the case where $\Omega<\omega_0$, and only multi-photon off-resonant processes play a role in these cases. Such off-resonant processes cannot be captured via our first order perturbative analysis and thus we cannot make any clear comparison with their results. However the work of \cite{Souza2018}, which looks at the radiation emitted from a two-level atom oscillating in free-space, do consider the regime $\Omega>\omega_0$, and include resonant processes and find the  emission of photons with the frequency $\omega_1=\Omega-\omega_0$, but do not find the higher modes $\omega_n=n\Omega-\omega_0$, which we predict to also exist, though with greatly reduced probabilities. To make a more quantitative comparison we study the small photon frequency case when $\omega_1\equiv\Omega- \omega_0$, is small and $\omega_1 A/c\ll 1$.  Making the approximation $J_1(x)^2\sim x^2/4$, for $x\ll 1$, and comparing our rate (\ref{SHOfreespace}), with Eqn (5) \cite{Souza2018}, in this regime, (in the notation of \cite{Souza2018}, this is when $\omega_1\equiv\omega_{\rm cm}- \omega_0$ is small), we find that both rates scale as $\overline P_{1}\sim \Gamma_{\rm MIE}\sim A^2/\Omega$. However in our case we find $\overline P_{1}\sim \omega_1^2$, while in \cite{Souza2018}, $\Gamma_{\rm MIE}\sim \omega_1^3$, a difference which may be due to the differences between the Hamiltonians. In our study we assume the Hamiltonian (\ref{noSMA}),  a  model for coupling between two levels systems and vacuum fields used by many works and which also was used in \cite{Svidzinsky2018}, to derive the Unruh temperature for the case of uniform acceleration, while \cite{Souza2018}, Eqn (1), includes both the normal dipole coupling but also a term linear in the velocity of the two level system. }

\begin{figure}[tp] 
\begin{center}
\setlength{\unitlength}{1cm}
\begin{picture}(8.5,7.5)
%\put(.1,-.4){\includegraphics[width=.95\columnwidth]{Figures/Fig1b}}
\put(-2,-.3){\includegraphics[width=.65\columnwidth]{Images/Shaking_Photons/Fig3}}
\end{picture}
\end{center}
\caption{Transition/emission rate for an atom oscillating with simple harmonic motion in free space as a function of the amplitude of the oscillation  and ultra-strong coupling strengths $\alpha$, where $g=\alpha \omega_0$, taking a mechanical frequency $\Omega/2\pi=10\,{\rm GHz}$, and two level transition frequency $\omega_0=\Omega/2$ (\ref{SHOfreespace}).}
   \label{Fig3}
\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%












==> Chpt_2_Notes.tex <==

\section{Vortices on a sphere} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A vortex of strength $v$ at the N-pole of the sphere, $z=0$, with flux $2\pi v$ out of the sphere, is described by a magnetic potential
\begin{equation}
a=\frac{v}{2 i} \left[ \frac{d z}{z} 
- \frac{d \bar z}{\bar z}\right].\label{eq:vortex-N}
\end{equation}
Then $d a=0$ provided $z\ne 0$ but, if we isolate the N-pole by surrounding it by a small circle $S^1_\epsilon$ of radius $\epsilon$ 
centred on $z=0$, 
\begin{equation}
\int_{S^1_\epsilon} a =
 \frac{v}{2 i}\int_{S^1_\epsilon} \frac{d z}{ z} 
-\frac{v}{2 i}\int_{S^1_\epsilon} \frac{d \bar z}{\bar z}
=   \pi  v  - \pi (- v)= 2\pi v.\label{eq:vortex-S1}
\end{equation}
Thus (\ref{eq:vortex-N}) describes a point vortex of strength $v$ at the N-pole,
$f = da$ is a $\delta$-function at $z=0$,
which can be represented by
\[\partial_{\bar z}\left(\frac{1}{z}\right)=
  \partial_{z}\left(\frac{1}{\bar z}\right) = 2\pi \delta(z).\] 
However this potential also gives an anti-vortex, of strength $-v$, at the S pole:
the anti-podal point is given by $z \rightarrow \frac{1}{\bar z}$, which sends $a\rightarrow -a$. This is perhaps clearer using polar co-ordinates, $(\theta,\phi)$, 
in which 
\[ a = v d \phi\]
which represents an infinite straight flux tube in 3-dimensions, threading through both the N-pole and the S-pole of the sphere.  The total flux through the sphere 
arising from $f = da$ is zero.

The position of the vortex through the N-pole can be moved around by using
\begin{equation}
a=\frac{v}{2 i} \left[ \frac{d z}{(z-z_1)} 
- \frac{d \bar z}{(\bar z - \bar z_1)}\right],\label{eq:vortex-A}
\end{equation}
representing a vortex of strength $v$ through the point $z_1$, but there is still
an anti-vortex through the S-pole for any finite $z_1$.
However the vortex at the S-pole can be removed by adding a uniform magnetic field with a semi-infinite solenoid threading the S pole and terminating at the centre of the sphere,
\begin{equation}
a=\frac{v}{2 i} \left[ \frac{d z}{(z-z_1)} 
- \frac{d \bar z}{(\bar z - \bar z_1)}\right] 
+\frac{v}{2 i}\left(\frac{z d \bar z - \bar z d z}{1+z \bar z}\right),\label{eq:solenoid}
\end{equation}
giving the field strength
\[ f=d a = i\left(2 \pi  v \delta(z_1)  + \frac{v}{2}\frac{1}{(1+ z \bar z)^2}\right) d z \wedge d \bar z \] 
This is perfectly regular at the S pole and represents a magnetic monopole of charge $-v$ at the centre of the sphere together with a point vortex of strength $v$ at $z_1$,
the total flux is zero (figure 1). It is actually like a Dirac monopole with it's accompanying
string threading the sphere at $z_1$, but a Dirac string is a gauge artifact, a vortex is not.

\begin{figure}[h]
\centerline{\includegraphics{Images/QH_Sphere/Vortex}}
\caption{A vortex threading the sphere. (a) shows the simple vortex in (\ref{eq:vortex-N}) piercing the sphere at the north and south poles; 
(b) shows the vortex in (\ref{eq:vortex-A}), piercing the sphere at $z_1$ and the south pole; (c) shows the combination of the vortex in (b) combined with a Dirac monopole of charge $-1$ uniformly distributed on the sphere together with its accompanying string through the south pole; (d) the Dirac string and the vortex through the south pole cancel leaving a uniform monopole field with a vortex at $z_1$.  The total flux through the sphere in (d) is zero --- the Dirac string has been moved  from the south pole to the point $z_1$.}
\end{figure}

If there are $N-1$ vortices all of the same strength $v$ positioned at $z_j$ then the fields are simply added:
\begin{equation}a=\frac{v}{2 i} \sum_{j=1}^{N-1}\left( \frac{d z }{z-z_j}
-  \frac{d \bar z}{\bar z-\bar z_j}\right)
-\frac{i (N-1) v}{2}\left(\frac{z d \bar z - \bar z d z}{1+z \bar z}\right).\label{eq:a}
\end{equation}
The corresponding field strength is
\[ f = d a =i\left( 2 \pi v \sum_{j=1}^{N-1}\delta(z-z_j) -
\frac{(N-1)v}{(1 + z \bar z)^2} \right)  dz \wedge \bar dz\]
and
\[ \int_{S^2} f =0.\]
If in addition a background monopole field with charge $m'$ is present then the total gauge potential on the northern hemisphere is
\begin{equation} A^{(+)}  = \frac{v}{2 i} \sum_{j=1}^{N-1}\left( \frac{d z }{z-z_j}
-  \frac{d \bar z}{\bar z-\bar z_j}\right)
+ \frac{i m}{2}\left(\frac{z d \bar z - \bar z d z}{1+z \bar z}\right),\label{eq:A+}
\end{equation}
where $m=m' - (N-1)v$,
and the field strength is
\[ F = d A^{(+)} = i\left(2 \pi v \sum_{j=1}^{N-1} \delta(z-z_j) + 
\frac{m}{2 (1+z \bar z)^2}\right)dz \wedge d \bar z.\]
On the southern hemisphere we take the potential to be
\begin{align} A^{(-)} 
&= \frac{v}{2 i} \sum_{j=1}^{N-1}\left( \frac{d z }{z-z_j}
-  \frac{d \bar z}{\bar z-\bar z_j}\right)
- \frac{i (N-1)v (z d \bar z - \bar z d z)}{2(1+z \bar z)}
+\frac{i m'}{2} \frac{1}{(1+ z \bar z)}  \left( \frac{d z}{z} - \frac{d \bar z}{\bar z} \right)\nonumber\\
&= \frac{v}{2 i} \sum_{j=1}^{N-1}\left( \frac{d z }{z-z_j}
-  \frac{d \bar z}{\bar z-\bar z_j}\right)
+ \frac{i}{2} \left( \frac{m}{(1+ z \bar z)}  +  (N-1) v \right) 
  \left( \frac{d z}{z} - \frac{d \bar z}{\bar z} \right),\label{eq:A-}
\end{align}
which is perfectly well defined as $|z|\rightarrow \infty$. Again
\[ F = d A^{(-)} = i\left(2 \pi v \sum_{j=1}^{N-1} \delta(z-z_j) + 
\frac{m}{2 (1+z \bar z)^2} \right)dz \wedge d \bar z.\]
The total flux is
\[ \int_{S^2} F= 2\pi \bigl[m + (N-1)v \bigr],\]
see figure 2.

\begin{figure}[h]
\centerline{\includegraphics{Images/QH_Sphere/Composite-fermions}}
\caption{Composite fermions. (a) represents three electrons in a uniform background flux with total magnetic charge $m=-9$, giving filling factor $\frac{1}{3}$;
(b) six Dirac strings are promoted to be real vortices and attached to the electrons in pairs; (c) the total magnetic flux is now $m'=-3$; (d) the resulting configuration consists of three composite fermions in a field of strength $-3$ giving an effective filling factor 1.}
\end{figure}

What we have done here is taken $|m|$ monopoles each of charge $\pm 1$
(depending on the sign of $m$) and promoted the Dirac strings on 
$N-1$ of them to be real vortices at $z_i$, but leaving $|m'|$ of them as Wu-Yang monopoles, for which the Dirac string is a gauge artifact.
The configuration is indistinguishable from that of a monopole of charge $m$
together with $N-1$ vortices.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Dirac Operator}

Gauge potential for radial magnetic field
\begin{equation*}A^{(\pm)}=\frac{m}{2} (\pm 1-\cos\theta) d \phi \qquad \Rightarrow \qquad
F=dA=\frac{m}{2}\sin\theta d\theta \wedge d\phi\label{eq:Apm}\end{equation*}
and
\begin{equation*}\frac{1}{2\pi}\int_{S^2} F =m,\end{equation*}
with integral $m$ (monopole charge).
The upper (lower) sign is for the upper (lower) hemisphere.
\newpage
We shall use a complex co-ordinate on $S^2$. As a way to visualise how we might arrive at complex coordinates on the sphere one can take the stereographic projection of a circle with radius $R$, centred at the origin, on to the horizontal axis like so
\begin{figure}
\begin{tikzpicture}
  \draw [thick](0,0) circle (3cm);
  \draw [->](0,-4) -- (0,4);
  \draw [->](-4,0) -- (4,0);
  \draw [thick](0,-3) -- (2.4,1.8);
  \draw [thick](0,0) -- (2.4,1.8);
  \draw [shift={(0,0)}, gray, fill, fill opacity=0.5] (0,0) -- (36.86:0.4) arc (36.86:90.:0.4) -- cycle;
  \draw (0.07,0.9) node[anchor=north west] {$\theta$};
  \fill[fill=black] (1.5,0) circle (1pt);
  \draw (1.5,0.02) node[anchor=north west] {$p$};
  \draw (1.15,1.6) node[anchor=north west] {$R$};
  \draw [shift={(0,-3)}, gray, fill, fill opacity=0.5] (0,0) -- (65:0.7) arc (65:90.:0.7) -- cycle;
  \draw (0.02,-1.7) node[anchor=north west] {$\alpha$};
  \draw (0.02,4) node[anchor=north west] {$x_{3}$};
  \draw (4,0.02) node[anchor=north west] {$x_{1}$};
  \draw (2.4,2.2) node[anchor=north west] {$(x_{1},x_{3})$};
  \fill[fill=black] (2.4,1.8) circle (1pt);
\end{tikzpicture}
\label{fig:Stereo}
\end{figure}
where $\theta$ is the standard polar angle in spherical coordinates. It is clear from this picture that $\frac{p}{R} = \tan{(\alpha)}$ and with some elementary geometry that $\alpha = \frac{\theta}{2}$. Multiplying by a complex phase dependent on the azimuthal angle we get our complex coordinates, with the complex plane now projected on to the $x_{1} - x_{2}$ plane. 
\begin{equation*}z= R\left(\tan\frac{\theta}{2}\right) e^{i\phi}=\frac{v}{u},\end{equation*}
{\it e.g.} with $v=\sin\frac{\theta}{2} e^{i(\phi+\delta)}$ and $u=\cos\frac{\theta}{2}e^{i\delta}$.
Then we have
\begin{align*}
1+ z \bar z &= \frac{1}{\cos^{2}\frac{\theta}{2}},\\
\frac{d\left(\tan\frac{\theta}{2}\right)}{d\theta} &= \frac{1}{2}\left( 1+ \tan^{2}\frac{\theta}{2}\right) = \frac{1}{\cos^{2}\frac{\theta}{2}},\\
dz &= \frac{1}{2\cos^{2}\frac{\theta}{2}} e^{i\phi} d\theta + izd\phi = \frac{(1+z\bar z)}{2}e^{i\phi} d\theta + i z d\phi,\\
d\bar{z} & = \frac{(1+z \bar z)}{2} e^{-i\phi} d\theta -i\bar{z}d\phi,\\
d\bar{z} \wedge dz &= i\tan\frac{\theta}{2}\left(1+\tan^{2}\frac{\theta}{2}\right) d\theta \wedge d \phi,\\
\Rightarrow \qquad \frac{d\bar{z}\wedge dz}{(1+ z\bar{z})^2} & = \frac{i}{2} \sin\theta d\theta \wedge d\phi.
\end{align*}
In terms of $z$ and $\bar{z}$
\begin{align}
A^{(+)} &= \frac{im}{2} \frac{(zd\bar{z} - \bar{z}dz)}{(1+ z \bar z)}
 =\frac{im}{2}  \frac{z \bar z}{(1+ z \bar z)} d \ln\left(\frac{\bar{z}}{z}\right) ,\nonumber \\
A^{(-)} &=\frac{im}{2}  \frac{1}{(1+ z \bar z)}
d \ln\left(\frac{z}{\bar z}\right) ,\label{eq:A+A-}\\
F &= i m\frac{dz \wedge d\bar{z}}{(1 + z \bar z)^2}. \nonumber
\end{align}
In particular $A^{(-)}(z) =  A^{(+)}(1/z) =A^{(+)}(z)+i e^{-i m \phi}d( e^{i m \phi}) .$

Define complex orthonormal 1-forms
\begin{equation*} e^1 = \frac{dz}{1 + z\bar{z}}, \qquad e^{\bar 1} = \frac{d\bar{z}}{1 + z\bar{z}}\end{equation*}
and metric
\begin{equation*} d s^2 = e^1 \otimes e^{\bar 1} + e^{\bar 1} \otimes e^1 = \frac{2 d z d\bar{z}}{(1 + z \bar{z})^2}
=\frac{1}{4}(d ^2\theta + \sin^2\theta d^2 \phi),\end{equation*}
corresponding to the metric on  sphere of radius $\frac{1}{2}$.

Indices are raised and lowered with
\begin{equation*}\delta_{1 \bar 1} \qquad \hbox{and} \qquad \delta^{1 \bar 1}.\end{equation*}

Complex connection 1-forms  (really only one complex connection 1-form)
are determined from
\begin{align*}
d e^1 + \omega^{1 \bar 1} \wedge e_{\bar 1} &= - \frac{z d \bar z \wedge d z}{(1 + z \bar z)^2} + \omega^{1\bar 1}\wedge e^1=0\\
\Rightarrow \qquad \omega^{1 \bar 1} &= \frac{z d \bar z }{ (1+ z \bar z)} + f dz,\\
\omega^{\bar 1  1} &= \frac{\bar z d z }{ (1+ z \bar z)} + g d \bar z,
\end{align*}
where $f(z,\bar z)$ and $g(z,\bar z)$ are functions. It is consistent to take $f=g=0$ and
\begin{equation*}\omega^{1 \bar 1}= \frac{z d \bar z - \bar z d z}{ (1+ z \bar z)}.\end{equation*}
Note that 
\begin{equation*}\omega_{1\bar 1}= -\omega_{\bar 1 1}=-\omega^{1 \bar 1}. \end{equation*}
The curvature 2-forms are
\[R_{1 \bar 1} = d \omega_{1 \bar 1} = \frac{2 d z \wedge d \bar z}{(1+ \bar z z)^2}= 2 e^1 \wedge e^{\bar 1}.\]


Spin-$\frac{1}{2}$ co-variant derivatives, for a Fermion with charge $e=-1$, are\footnote{In terms of the more usual $e^1 = d\theta$ and $e^2=\sin\theta d \phi$, with $\omega^{12}=-\cos\theta d\theta \wedge d \phi$ (or better still $\omega^{12}=(\pm1-\cos\theta) d\theta \wedge d \phi$ on the northern/southern hemisphere, so it is well defined at the north/south pole), the co-variant derivative in  the Dirac operator (for an electrically neutral fermion) would be \begin{equation*} D_\mu=\partial_\mu + \omega^{a b}_{\mu} \frac{[\sigma_a,\sigma_b]}{ 8} = \partial_\mu + \omega^{1 2}{}_\mu \frac{[\sigma^1,\sigma^2]}{ 4  } = \partial_\mu + \frac{i}{ 2} \omega^{1 2}{}_\mu \sigma^3,\end{equation*} consistent with spin $s=\frac{1}{2}$.}
\begin{align}D_z &= \partial_z + \frac{1}{ 2}\omega_{1 \bar 1,z}\gamma^{1 \bar 1} + i A_z \nonumber \\
& = \partial_z + \frac{1}{ 2}\frac{\bar z \sigma_3}{ (1+ z \bar z)} + \frac{m}{ 2} \frac{\bar z }{ (1+ z \bar z)} 
= \partial_z + \frac{(m+\sigma_3)}{ 2} \frac{\bar z }{ (1+ z \bar z)},\label{eq:Dz}\\
D_{\bar z} &= \partial_{\bar z} + \frac{1}{ 2}\omega_{\bar 1 1, \bar z} \gamma^{\bar 1 1} + i A_{\bar z}\nonumber \\
                 & = \partial_{\bar z} - \frac{1}{ 2} \frac{z \sigma_3}{ (1+ z \bar z)} -\frac{m}{2}\frac{z}{(1+ z \bar z)} 
= \partial_{\bar z} - \frac{(m+\sigma_3)}{ 2} \frac{z }{ (1+ z \bar z)},\label{eq:Dbarz}
\end{align},
where $\gamma^1 = \sigma_1 + i \sigma_2$ and $\gamma^{\bar 1} = \sigma_1 - i \sigma_2$ so
\[ \gamma^{1 \bar 1} = \frac 1 2 (\gamma^1 \gamma^{\bar 1} - \gamma^{\bar 1} \gamma^1) = \sigma_3.\]
The commutator is
\[ [D_z,D_{\bar z}] = i F_{z \bar z}= -\frac{(m+\sigma_3)}{(1+ \bar z z)^2}.\]

The Dirac operator is
\begin{align} 
i\Dslash 
& = i(1+z \bar z) \bigl(\sigma_+ D_z + \sigma_- D_{\bar z} \bigr) \nonumber \\
&= i(1+z \bar{z})\begin{pmatrix}
0 & \partial_{z} + \frac{(m-1)}{2}\frac{\bar{z}}{(1 + z \bar{z})} \nonumber\\
\partial_{\bar{z}} - \frac{(m+1)}{2}\frac{z}{(1 + z \bar{z})} & 0
\end{pmatrix}\\
&= i\begin{pmatrix}0 & (1 + z \bar z)\partial_{z} + \frac{(m-1)}{ 2} \bar z  \\ 
(1 + z \bar z)\partial_{\bar z} - \frac{(m+1)}{ 2} z  & 0
\end{pmatrix}.\label{eq:Dirac0}
\end{align}

In terms of $\theta$ and $\phi$ the Dirac operator is
\begin{align*}i\Dslash = \hskip 14cm& \\
i\begin{pmatrix}
0 & e^{-i\phi} \left\{\partial_\theta +\frac{1}{\sin\theta}
\left[\frac{(m-1)}{2}(\pm 1 -\cos\theta) -i\partial_\phi\right]\right\}\\
e^{i\phi} \left\{\partial_\theta -\frac{1}{\sin\theta}
\left[\frac{(m+1)}{2}(\pm 1 -\cos\theta) -i\partial_\phi\right]\right\}& 0\\
\end{pmatrix}, \end{align*}
so
\[ \Dslash \psi = \Dslash'\bigl( e^{i \sigma_3 \phi}\psi\bigr) \]
with
\[
\Dslash' = 
\begin{pmatrix}
0 & \partial_\theta +\frac{1}{\sin\theta}
\left[\frac{(m+1)}{2}(\pm 1 -\cos\theta) -i\partial_\phi\right]\\
\partial_\theta -\frac{1}{\sin\theta}
\left[\frac{(m-1)}{2}(\pm 1 -\cos\theta) -i\partial_\phi\right]& 0\\
\end{pmatrix}. \]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Angular momentum}

In the presence of a magnetic field the orbital angular momentum generators
are naturally modified to
\[ L_a =  \epsilon_{a b c} x_b (p_c + e  A_c)=-i\epsilon_{a b c} x_b (\partial_c + i e A_c),\]
where $x_b$ are Cartesian co-ordinates in 3-dimensions.  But these do not close,  
\[  [L_a , L_b]=i \epsilon_{a b c}  \bigl( L_c  + e   x_c({\bf r}.{\bm B})\bigr).\] 
If ${\bm B} = {\bm \nabla}\times {\bm A}$ is radial, ${\bm B} = B \hat {\bm r}$, then
\[ [L_a , L_b]=i \epsilon_{a b c} ( L_c - e  B  r x_c) \]
So we define, \cite{Fierz},
\[ J_a =  L_a - e B r x_a\]
in terms of which
\begin{equation}
  [J_a , J_b ]=i \epsilon_{a b c} J_c
  + i e r^2\Bigl( x_a (L_b B) - x_b (L_a B)\Bigr).\label{eq:JJB}
\end{equation}
Then if $B=B(r)$ is spherically symmetric $L_a B(r)=0$ and the algebra closes
\[ [J_a , J_b]=i \epsilon_{a b c} J_c.\]
In particular for a monopole field $ B = \frac{1}{2}\frac{m} {r^2}$ and
\[  J_a =  L_a -   \frac{e m}{2} \frac{x_a}{r}.\]
In terms of ladder operators
\begin{align*} J_{\pm} & = J_1 \pm i J_2 = L_1 \pm i L_2  - \frac{e m}{2} \sin\theta e^{\pm i \phi}
  = \pm  e^{\pm i\phi} \left( \partial_\theta \pm i \cot \theta
      \partial_\phi\right) -  \frac{e m}{2} \sin\theta e^{\pm i \phi}\\
  J_3 & = L_3 -  \frac{e m}{2} \cos\theta = -i\partial_\phi
- \frac{e m}{2} \cos\theta. \end{align*}

Converting from $(\theta,\phi)$ to $(z,\bar z)$
\begin{align*} \frac{x_1 + i x_2}{r} = \sin\theta e^{ i\phi} & = \frac{2 z}{1+ z \bar z},\\
   \frac{x_1 - i x_2}{r} = \sin\theta e^{-i\phi}& = \frac{2 \bar z}{1+ z \bar z},\\
   \frac{x_3} {r}  = \cos \theta& = \frac{1-z \bar z} { 1+ z \bar z}
  \end{align*}
and (with $e=-1$)
\begin{align}
  J_+ &= z^2 \bigl(\partial_z + i A_z\bigr) +
        \bigl(\partial_{\bar z} + i A_{\bar z}\bigr) + \frac{m z}{1+ z \bar z}\nonumber \\
  J_- &= -{\bar z^2} \bigl (\partial_{\bar z}  + i A_{\bar z}\bigr ) - \bigl(\partial_z + i A_z \bigr)+ \frac{m \bar z}{1+ z \bar z}\\
  J_3 & = z\bigl(\partial_z +iA_z\bigr)
        - \bar z \bigl( \partial_{\bar z} + i A_{\bar z}\bigr )
        + \frac{m}{2} \left( \frac{1-z \bar z}{1 + z \bar z} \right).\nonumber 
\end{align}
Using the monopole potential (\ref{eq:A+A-}) 
\begin{align}
  J_+ & = z^2 \partial_z + \partial_{\bar z}
        +\frac{m z}{2}
        \nonumber \\
 J_- & = -{\bar z}^2 \partial_{\bar z} - \partial_z
 + \frac{m \bar z}{2}
       \\  
  J_3 &= z \partial_z - \bar z \partial_{\bar z}
        + \frac{m}{2},
        \nonumber \end{align} 
      and
      \begin{equation}[J_+,J_-] = 2 J_3, \qquad [J_3,J_\pm] = \pm J_\pm,\label{eq:J-algebra} \end{equation}
with\footnote{When $m=0$,  \[L_a L_a =- (1 + z \bar z)^2 \partial_z \partial_{\bar z} =-\left(\partial_\theta^2 + \cot\theta\partial_\theta + \frac{1}{\sin^2\theta}\partial_\phi^2\right)\] is just the usual scalar Laplacian.}
\[ J^2 = \frac{1}{2}(J_+ J_- + J_- J_+)  + J_3^2 = - (1 + z \bar z)^2 \partial_z \partial_{\bar z}+ \frac{m}{2} (1+ z \bar z) J_3.\]

Of course (\ref{eq:J-algebra}) is just the orbital angular momentum, to this must be added the intrinsic angular momentum
of the electrons. This requires adding terms proportional to $\gamma^1 \gamma^{\bar 1} -\gamma^1 \gamma^{\bar 1} = \sigma_3$. There is a well defined procedure for doing this: Lie 
derivatives on spinors arising from a vector field $\vec X = X^\mu \partial_\mu$ will cause dragging of the orthonormal frames and this can be accounted for by defining \cite{SpinorLie}
\begin{equation}
 {\cal L}_{\vec X} = X^\mu D_\mu + \frac 1 4 (d X)_{i j} \gamma^{i j} \label{eq:LieK}\end{equation}
where $X$ is the one-form metric dual to the vector ${\vec X}$ and 
$d X_{i j} = -d x_{j i}$ are the components of $d X$ in an orthonormal basis.
For the three rotation  generators
\[ \vec L_+ = z^2 \partial_z + \partial_{\bar z}, \qquad
\vec L_- = -\bar z^2 \partial_z - \partial_z,\qquad
\vec L_3  = z \partial_z - \bar z \partial_{\bar z},\]
the corresponding one-forms are
\[ L_+ = \frac{d z + z^2 d \bar z}{(1+\bar z z)^2}, \qquad
L_- = -\frac{d \bar z + \bar z^2 d z}{(1+\bar z z)^2},\quad
 L_3  = \frac{z d \bar z -\bar z d z}{(1+\bar z z)^2},\]
giving
\begin{align*}
d L_+ &= \frac{4 z}{1+ \bar z z} e^{1 \bar 1}= - 4 L_3 \wedge L_+,\\
d L_- &= \frac{4 \bar z}{1+ \bar z z} e^{1 \bar 1}=4 L_3 \wedge L_-\\
d L_3 &= 2\left(\frac{1- \bar z z}{1+ \bar z z} \right)e^{1 \bar 1}=-2 L_+ \wedge L_-.
\end{align*}
Following the prescription (\ref{eq:LieK}) we define the Lie derivatives
\begin{align}
 {\bm J}_+ &= z^2 \bigl(\partial_z + i A_z + \frac 1 2 \omega_{1 \bar 1, z}\sigma_3\bigr) +
        \bigl(\partial_{\bar z}  +i A_{\bar z} + \frac 1 2 \omega_{1 {\bar 1}, {\bar z}} \sigma_3\bigr) + \frac{(m + \sigma_3) z}{1+ z \bar z}\nonumber \\
 & = z^2 \partial_z + \partial_{\bar z}
        +\frac{(m + \sigma_3)z}{2}
        \nonumber \\
 {\bm J}_- &= -{\bar z^2} \bigl (\partial_{\bar z}  + i A_{\bar z} 
+ \frac 1 2 \omega_{1 \bar 1, \bar{z}} \sigma_3\bigr) - \bigl(\partial_z + i A_z +\frac 1 2 \omega_{1 \bar 1, z}\sigma_3\bigr)+ \frac{(m+\sigma_3) \bar z}{1+ z \bar z}\nonumber\\
  & = -{\bar z}^2 \partial_{\bar z} - \partial_z
 + \frac{(m+\sigma_3) \bar z}{2} \label{eq:J-def} \\  
{\bm J}_3 & = z\bigl(\partial_z +iA_z + \frac 1 2 \omega_{1 \bar 1, z}\sigma_3\bigr)
        - \bar z \bigl( \partial_{\bar z} + i A_{\bar z} + \frac 1 2 \omega_{1 {\bar 1}, {\bar z}} \sigma_3\bigr )
        + \frac{(m+\sigma_3)}{2} \left( \frac{1-z \bar z}{1 + z \bar z} \right)\nonumber \\
&= z \partial_z - \bar z \partial_{\bar z}
        + \frac{(m+\sigma_3)}{2}.
        \nonumber
\end{align} 
The commutation relations are
\begin{equation}
[{\bm J}_+,{\bm J}_-] = 2 {\bm J}_3, \qquad [{\bm J}_3,{\bm J}_\pm] = \pm {\bm J}_\pm.\label{eq:J_T-albegra} 
\end{equation}
and
\[ 
{\bm J}^2 = \frac{1}{2}({\bm J}_+ {\bm J}_- + {\bm J}_- {\bm J}_+)  + {\bm J}_3^2 
= - (1 + z \bar z)^2 \partial_z \partial_{\bar z} + \frac 1 2(m + \sigma_3) (1+ z \bar z) {\bm J_3}.
\]
We find
\[
[{\bm J}_3, D_z]=-D_z,\qquad  [{\bm J}_3, D_{\bar z}]=D_{\bar z} \]
from which
\begin{align*}
 [{\bm J}_3,\Dslash]&=[{\bm J}_3,\sigma_+] D_z + \sigma_+[{\bm J}_3,D_z]
+ [{\bm J}_3,\sigma_-] D_{\bar z} + \sigma_-[{\bm J}_3,D_{\bar z}]\\
&= \frac 1 2 [\sigma_3,\sigma_+] D_z - D_z + \frac 1 2 [\sigma_3,\sigma_-] + D_{\bar z}=0.
\end{align*}

Also
\[ [{\bm J}^2,\Dslash] =0,\]
as we expect from $SU(2)$ symmetry.

The Dirac operator (\ref{eq:Dirac0}) squares to
\begin{align}(i\Dslash)^2 & = \nonumber  \\ 
& \kern -10pt  -(1+\bar z z)^2 \partial_z \partial_{\bar z} 
+\frac{m}{2}(1+\bar z z) \left(J_3+\frac{1}{2} \sigma_3\right)  
+ \frac {\bar z z} {4} - \frac {m^2}{4}+ \frac 1 2  +\frac{1}{2} (1+ \bar z z) J_3  \sigma_3\nonumber \\
& \kern -19pt = -(1+\bar z z)^2 \partial_z \partial_{\bar z} 
+\frac{m}{2}(1+\bar z z) {\bm J_3}
+ \frac {\bar z z} {4} - \frac {m^2}{4}+ \frac 1 2  +\frac{1}{2} (1+ \bar z z) {\bm J_3}\sigma_3 - \frac{(1+ \bar z z)}{4} \nonumber \\
& \kern -19pt = {\bm J}^2 +\frac 1 4(1-m^2). \label{eq:Dslash2}
\nonumber\end{align}
We know that the eigenvalues of $(i\Dslash)^2$ are $n(n+|m|)$ 
and the eigenvalues of ${\bm J}^2$ are $J(J+1)$, for some $J$ labelling irreps of $SU(2)$,
so the relation between $J$ and $n$ is
\begin{align*}
J(J+1) + \frac{1-m^2}{4} & = n(n+|m|)\\
\Rightarrow \qquad J(J+1) + \frac 1 4 & = n^2 + n|m| + \frac{m^2}{4}\\
\Rightarrow \left(J+\frac 1 2\right)^2 & = \left(n + \frac{|m|}{2}\right)^2 \\
\Rightarrow J+\frac 1 2 & = n + \frac{|m|}{2}.
\end{align*}
If $m=0$ then it is not possible to have $n=0$: there are no zero modes when there is no magnetic field.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Zero Modes}

Spinors can be decomposed in terms of chiral eigenstates
\begin{equation*}\Psi = \begin{pmatrix}\chi_{+} \\ \chi_{-}\end{pmatrix}\end{equation*}
with $\sigma_3 \chi_{\pm} = \pm \chi_{\pm}$.
Eigenspinors must satisfy
\begin{equation*}i\Dslash \Psi = \lambda \Psi.\end{equation*}
Zero modes can be obtained from the ansatz
\begin{equation}\chi_+ = \frac{z^p}{(1+ z \bar z)^{\frac{q}{ 2}}}=\left( \sin\frac{\theta}{2} \right)^p \left( \cos\frac{\theta}{2} \right)^{q-p} e^{i p \phi},\label{eq:chi-plus}\end{equation}
with constant exponents $p$ and $q$,
satisfying
\begin{align*}
D_{\bar z} \chi_+ &= -\frac{q}{ 2} \frac{z^{p+1}}{(1+z \bar z)^{\frac{q}{ 2}+1}} -\frac{(m+1)}{ 2} \frac{z^{p+1}}{ (1+ z \bar z)^{\frac{q}{ 2}+1}}\\
&= -\frac{(q+m+1)}{ 2}\frac{z^{p+1}}{(1+z \bar z)^{\frac{q}{ 2}+1}}
\end{align*}
hence $D_{\bar z} \chi_+ =0$ if $q=-m-1$ for any $p$. 

A good quantum number for labelling these different states is their angular momentum
\[ {\bm J}_3 = z \frac{\partial}{\partial z} - \bar z \frac{\partial}{\partial \bar z}
+\frac 1 2 (m + \sigma_3).\]
Since ${\bm J}_3(z \bar z)=0$ 
\[{\bm J}_3 \chi_+ = \left(p + \frac{m+1}{2}\right)\chi_+\] 
and the angular momentum of (\ref{eq:chi-plus}) is $p+\frac 1 2 (m+1)$.


However for $\chi_+$ to be non-singular near $\theta=0$,
we must constrain $p\ge 0$. For finiteness near $\theta=\pi$, where $|z| \rightarrow \infty$ we must have $p\le q$ thus
\[0 \le -m-1 \]
and positive chirality zero modes can only exist if $m \le -1$, in which case
$q=|m|-1$. But this is not sufficient, if we put $q=p$ in there is a singularity in the phase at $\theta=\pi$.
To check the behaviour of $\chi_+$ near the south pole more carefully we should perform a gauge transformation transformation between
the northern and southern hemisphere. $\chi_+$ is a positive chirality spinor on the northern hemisphere, more explicitly written 
$\chi_+^{(+)}$.  From the form of $(1+\bar z z) D_{\bar z}$, with $-\frac{(m+1)}{2} \bar z = \frac{(|m|-1)}{2} \bar z$, it would seem that we
should perform a gauge transformation involving both the gauge field and the tangent bundle, and use
\[ \chi_+^{(-)} = 
e^{i(m+1) \phi } \chi_+^{(+)}
= \left( \sin\frac{\theta}{2} \right)^p \left( \cos\frac{\theta}{2} \right)^{|m|-1-p} e^{i (-|m|+1+p) \phi} \]
on the southern hemisphere, which is perfectly well behaved for $p=|m|-1$.

Thus for a monopole 
with charge $m=-1,-2,\ldots$ there are $|m|$ linearly independent positive chirality zero modes
labelled by the positive integer  $p=0,1,\cdots,|m|-1$,
\begin{equation*}\chi_+^{(+)} = \frac{z^p}{ (1+z \bar z)^\frac{|m|-1}{2}}=\left(\sin\frac{\theta}{2}\right)^p
\left(\cos\frac{\theta}{2}\right)^{|m|-1-p} e^{i p \phi},\qquad \chi_-=0.\end{equation*}


Similarly negative chirality zero modes are obtained from
\begin{align*}\chi_-^{(+)} = \frac{\bar z^{\bar p}}{ (1+ z \bar z)^{\frac{\bar q}{ 2}}}=\left( \sin\frac{\theta}{2} \right)^{\bar p} \left( \cos\frac{\theta}{2} \right)^{\bar p-\bar q} e^{-i \bar p \phi}, \end{align*}
with constant exponents $\bar p$ and $\bar q$,
satisfying
\begin{align*}
D_z \chi_-^{(+)} &= -\frac{\bar q}{ 2} \frac{\bar z^{\bar p+1}}{(1+z \bar z)^{\frac{\bar q}{ 2}+1}} + \frac{(m-1)}{ 2} \frac{\bar z^{\bar p+1}}{ (1+ z \bar z)^{\frac{\bar q}{ 2}+1}}\\
&= -\frac{(\bar q-m+1)}{ 2}\frac{\bar z^{\bar p+1}}{(1+z \bar z)^{\frac{\bar q}{ 2}+1}},
\end{align*}
hence $D_z \chi_-0$ if $\bar q=m-1$ for any $\bar p$. 
The angular momentum of $\chi_-$ is $-\bar p$.

Again, for $\chi_-$ to be finite near $\theta=0$,
we must constrain $\bar p\ge 0$ and, for $\chi_-$ to be finite near $\theta=\pi$, we must constrain $\bar p\le \bar q$. Hence finite $\chi_+$ requires $0\le \bar p \le m-1$,
so the integer $m\ge 1$ for a non-trivial zero-mode.  Also, for $\chi_-$ to be single valued in $\phi$ we must constrain $\bar p$ to be an integer.  Thus for a monopole 
with charge $m=1,2,\ldots$ there are $m$ linearly independent negative chirality zero modes
labelled by the positive integer  $\bar p=0,1,\cdots,m-1$,
\begin{equation*}\chi_+ = 0,\qquad \chi_-= \frac{\bar z^{\bar p}}{ (1+z \bar z)^\frac{m+1}{ 2}}=\left(\sin\frac{\theta}{2}\right)^{\bar p}
\left(\cos\frac{\theta}{2}\right)^{m-1-\bar p} e^{-i \bar p \phi}.\end{equation*}

We can summarize all the chiral zero modes by stating that for any integer monopole charge $m$
there are $|m|$ linearly independent zero modes, labelled by an integer $p =0,1,\ldots,|m|-1$ (we drop the bar on $\bar p$ for the negative chirality zero modes),
\begin{equation*}\chi^p_{\pm} 
:= \frac{\stackrel{\hbox{\tiny (--)}}{z}\kern -3pt {}^p}{ (1+z \bar z)^\frac{|m|-1}{ 2}}
=\left(\sin\frac{\theta}{2}\right)^p
\left(\cos\frac{\theta}{2}\right)^{|m|-1-p} e^{\pm i p \phi},\qquad \chi_\mp=0\end{equation*}
where the upper sign is for $m<0$ and the lower sign for $m>0$.
Since both $-\Dslash_1^2$ and $-\Dslash_2^2$ are non-negative operators the energy
cannot go below zero and if we can find a state with zero energy then it is a ground state.

Let us focus on negative $m$, the case $m>0$ is much the same.
A general zero mode for fixed $m<0$ is a linear combination of the $\chi^p_+$,
\begin{equation*}\chi_+(z) = \sum_{p=0}^{|m|-1} a_p\chi^p_+(z)=\frac{1 }{ (1+ z \bar z)^\frac{|m|-1}{ 2}}    \sum_{p=0}^{|m|-1} a_p z^p,\end{equation*}
with constant (complex) co-efficients $a_p$.\footnote{For simplicity we omit the $\bar z$ from the argument of $\chi_+(z,\bar z)$ --- the notation is not meant to imply that $\chi_+(z)$ is holomorphic, but it only differs from a holomorphic function by a simple overall factor.}

Now suppose we have two identical charged particles of mass $M$ on the sphere with co-ordinates $z_1$ and $z_2$. The Hamiltonian is
\begin{equation*}H = -\frac{\hbar^2 }{ 2 M} (\Dslash_1^2 + \Dslash_2^2)\end{equation*}
which, being a sum of two non-negative operators is itself a non-negative operator.
The most general zero mode of $-\Dslash_1^2$ is
\begin{equation*}\chi_+(z_1,z_2)= \frac{1 }{ (1+ z_1 \bar z_1)^{\frac{|m|-1}{2}}} \sum_{p_1=0}^{|m|-1} a_{p_1}(z_2) z_1^{p_1}.\end{equation*}
$\chi_-(z_1,z_2)$ will be a zero mode, and hence a ground state, of $H$ if $a_{p_1}(z_2)$
is a zero mode of $-\Dslash_2^2$ for each $p_1$,
\begin{equation*}a_{p_1}(z_2) = \frac{1 }{ (1+ z_2 \bar z_2)^{\frac{|m|-1}{ 2}}} \sum_{p_2=0}^{|m|-1} a_{p_1,p_2} z_2^{p_2}.\end{equation*}
The most general ground state of $H$ is thus
\begin{equation*}\chi_+(z_1,z_2)=\frac{1}{ [(1+ z_1 \bar z_1)(1+ z_2 \bar z_2)]^\frac{|m|-1}{ 2}}
\sum_{p_1,p_2=0}^{|m|-1} a_{p_1,p_2} z_1^{p_1} z_2^{p_2}\end{equation*}
where $a_{p_1,p_2}$ are $m^2$ arbitrary (complex) constants.  When we take into account that the particles are fermions and $\chi_-(z_1,z_2)$ should be anti-symmetric under  interchange of the two particles then $a_{p_1,p_2}$ must be anti-symmetric 
in its two indices.  

Generalising this to $N$ identical particles with co-ordinates $z_i$, $i=1,\ldots,N$, the most general zero mode of the Hamiltonian
\begin{equation} H= -\frac{\hbar^2}{ 2M}\sum_{i=1}^N \Dslash_i^2
\label{eq:Hamiltonian}\end{equation}
is
\begin{equation*} \chi_+(z_1,\cdots,z_N) =  \left[\prod_{i=1}^N \frac{1}{ (1+ z_i \bar z_i)}\right]^{\frac{|m|-1}{ 2}}
\sum_{p_1,\cdots,p_N=0}^{|m|-1} a_{p_1,\cdots,p_N} z_1^{p_1}\cdots  z_n^{p_N}\end{equation*}
where $a_{p_1,\cdots,p_N}$ is completely anti-symmetric in all its indices (in particular no two $p_i$ are the same).
The number of independent $c$'s, namely
$\frac{|m|!}{ N! (|m|-N)!}$, is the degeneracy of the ground state and $n$ cannot be greater than $|m|$ for this state to have
zero energy --- if $N>|m|$ at least one of the particles is forced into a higher energy state.  In particular in $N=|m|$ the ground state is unique (up to a trivial 
normalisation).  In fact $\nu = \frac{N}{ |m|}$ is the filling factor and for $\nu=1$
the ground state 
\begin{equation*} \chi_+(z_1,\cdots,z_N) =  \left[\prod_{i=1}^N \frac{1}{ (1+ z_i \bar z_i)}\right]^{\frac{|m|-1}{ 2}}
\prod_{j<k}(z_k-z_j)\end{equation*}
is unique, up to an overall constant normalisation.

The total angular momentum of $\chi_+$ is
\[ {\bm J}_{3,Tot}\chi_+ = \sum_{i=1}^N {\bm J}_{3,i}\chi_+ 
=\sum_{i=1}^N \left(z_i\frac{\partial}{\partial z_i} + \frac{m+1}{2}\right)\chi_+=\frac{N(m+1)}{2}.\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Full Spectrum}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

More generally the eigenvalues are labelled by a non-negative integer $n$ and
\begin{equation*}\lambda_n = \pm \sqrt{n(n+|m|)}\end{equation*}
with degeneracy $2n+|m|$, \cite{Dolan}.
A generic eigenspinor looks like
\begin{equation*}\Psi = \begin{pmatrix} \phi_1 \\ \phi_2 \end{pmatrix}\end{equation*}
hitting this with the Dirac operator results in a set of coupled of partial differential equations
\begin{align}
(1 + z \bar z)\partial_z \phi_2 + \frac{(m-1)}{ 2} \bar z \phi_2 &= -i\lambda \phi_1, \label{d1}\\
(1 + z \bar z)\partial_{\bar z} \phi_1 - \frac{(m+1)}{ 2} z \phi_1 &= -i\lambda \phi_2 \label{d2}
\end{align}
squaring the Dirac operator will separate these
\begin{align*}
{\Dslash}^2 \Psi &= -{\lambda}^2 \Psi \\
&={(1+z \bar z) \begin{pmatrix} 0 & D_z \\ D_{\bar z} & 0 \end{pmatrix}} {(1+z \bar z) \begin{pmatrix} D_z \phi_2 \\ D_{\bar z} \phi_1 \end{pmatrix}} = -{\lambda}^2 \begin{pmatrix} \phi_1 \\ \phi_2 \end{pmatrix} \\
&=(1+z \bar z)\begin{pmatrix} \bar z D_{\bar z} \phi_1 + (1+z \bar z) D_z D_{\bar z} \phi_1 \\ z D_z \phi_2 + (1+z \bar z) D_{\bar z} D_z \phi_2 \end{pmatrix} \\
\end{align*}
This gives two second-order partial differential equations
\begin{align*}
(1+z\bar z)^2 {\partial_{z} \partial_{\bar z} \phi_1} + \alpha (1+z \bar z)(\bar z\partial_{\bar z} - z\partial_z) \phi_1 +({\lambda}^2 -\alpha(1+z\bar z) -\alpha(\alpha-1)z\bar z)\phi_1 &= 0 \\
(1+z\bar z)^2 {\partial_{z} \partial_{\bar z} \phi_2} + (1-\alpha) (1+z \bar z)(z\partial_z - \bar z\partial_{\bar z}) \phi_2 +({\lambda}^2 -(1-\alpha)(1+z\bar z) -\alpha(\alpha-1)z\bar z)\phi_2 &= 0
\end{align*}
Where $\alpha= \frac{(1+m)}{2}$ and $(1-\alpha) = \frac {1-m}{2}$. We can simplify this expression with the ansatz
\begin{equation*}\phi_1 = \frac {z^p \bar z^{\bar p}}{(1+z\bar z)^q} f(z\bar z).\end{equation*}
Such a state has angular momentum $p-\bar p$.

Letting $x=z\bar z$ and denote derivatives with respect to $x$ with primes we obtain 
\begin{align*}\partial_z \phi_1 &= \frac {z^p \bar z^{\bar p}}{(1+x)^q} (\frac{p}{z}f -\frac{q\bar z}{1+x}f +\bar z f')  \\
\partial_{\bar z} \phi_1 &= \frac {z^p {\bar z}^{\bar p}}{(1+x)^q} (\frac{\bar p}{\bar z}f -\frac{qz}{1+x}f + z f')\\
(\bar z\partial_{\bar z} - z\partial_z) \phi_1 &= \frac {z^p {\bar z}^{\bar p}}{(1+x)^q}({\bar p}-p)f \\
\partial_{z}\partial_{\bar z} {\phi_1} = \frac {z^p {\bar z}^{\bar p}}{(1+x)^q} &\Big[(\frac{p}{z} -\frac{q\bar z}{1+x})(\frac{\bar p}{\bar z}f -\frac{qz}{1+x}f + z f') \\ &+({\bar p}f'-\frac{q}{(1+x)}f+\frac{qx}{(1+x)^2}f-\frac{qx}{(1+x)}f'+f'+xf'')\Big] \\
\end{align*}
With this expression for $\phi_1$ we have a common factor of $\frac {z^p \bar z^{\bar p}}{(1+z\bar z)^q}$ in our differential equation, which becomes a second order ODE in $f$. Dividing out the common factor and collecting like terms gives
\begin{align*} &x{(1+x)^2} f'' + (1+x)\Big[(p+{\bar p}+1)(1+x)-2qx\Big]f'\\ &+\Big[p{\bar p}\frac{(1+x)^2}{x}+(1+x)[\alpha({\bar p}-p)-q(p+{\bar p}+1)]+x(q(q+1)-{\alpha}^2)\Big]f +({\lambda}^2-\alpha)f=0
\end{align*} 
With the substitution $x=\frac{u}{(1-u)}$, and denoting derivatives with respect to $u$ with dots ($\dot f$) we have 
\begin{align*}
(1+x)^{2} f' &= \dot f \\
x(1+x)f' &= u\dot f \\
x(1+x)^{2} f'' &= u(1-u) \ddot{f} -2u\dot f
\end{align*}
Which when substituted in nearly gives us a the hyper-geometric differential equation
\begin{align*}
  &u(1-u)\ddot{f} +\Big[(p+{\bar p}+1)-2u(q+1)\Big]\dot{f}+ \frac{1}{1-u}\Big[\frac{p{\bar p}}{u}+\alpha({\bar p}-p)-q(p+{\bar p}+1)\\ & \hskip 3cm +u(q(q+1)-{\alpha}^2)\Big]f+({\lambda}^2-\alpha)f=0 \\
\end{align*}
Now using the fact that $\frac{1}{1-u} = 1 + \frac{u}{1-u}$ to rewrite our differential equation
\begin{align*}
&u(1-u)\ddot{f} +\Big[(p+{\bar p}+1)-2u(q+1)\Big]\dot{f}+ \frac{1}{1-u}\Big[\frac{p{\bar p}}{u}+u(\alpha({\bar p}-p)-q(p+{\bar p}-q)-{\alpha}^2)\Big]f\\ &+({\lambda}^2+\alpha({\bar p}-p-1)-q(p+{\bar p}+1))f=0 \\
\end{align*}
This equation becomes the hypergeometric equation by setting the $\frac{1}{1-u}$ coefficients of $f$ to zero. So now we have 2 constraints.
\begin{align*}
p{\bar p} &=0 \\
(q-\alpha)(q+\alpha)-{\bar p}(q-\alpha)-p(q+\alpha) &= 0 \\
\end{align*}
So either $p$ or $\bar p$ is zero or both, which results in 4 separate possible relations for these constants.
\begin{align*}
\bar p &= 0, \quad q= p + \alpha \quad \text{ or } \quad q= -\alpha, \quad p \text{ is arbitrary}, \\
p &= 0, \quad q= {\bar p} - \alpha \quad \text{ or }\quad q= \alpha, \quad \bar{p} \text{ is arbitrary} \\
\end{align*}
Now we have 4 hypergeometric equations with these values substituted in;
\begin{align}
\intertext{With $\bar p=0$ we have}
q = -\alpha: \quad &u(1-u)\ddot{f} +\big(p+1-u(2-2\alpha)\big)\dot{f}+({\lambda}^2)f=0 \label{eq:1}\\
q = p+ \alpha: \quad &u(1-u)\ddot{f} +\big(p+1-u(2p+2\alpha+2)\big)\dot{f}+({\lambda}^2-(2\alpha+p)(p+1))f=0 \label{eq:2}\\
\intertext{or $p=0$ and}
q= \alpha: \quad &u(1-u)\ddot{f} +\big(\bar{p}+1-u(2\alpha+2)\big)\dot{f}+({\lambda}^2-2\alpha)f=0, \label{eq:3}\\
q= \bar{p} -\alpha: \quad &u(1-u)\ddot{f} +\big(\bar{p}+1-u(2{\bar p}-2\alpha+2)\big)\dot{f}+({\lambda}^2-{\bar p}({\bar p}+1-2\alpha))f=0 \label{eq:4}
\end{align}
The solutions for the hypergeometric differential equation, which have paramenters $a,b,c$, i.e.
\begin{equation*}u(1-u)\ddot{f} +\big(c-u(a+b+1)\big)\dot{f}-(ab)f=0, \\\end{equation*}
around $u=0$ are of the form \begin{equation*}F(a,b;c;u) = \sum_{n=o}^{\infty} \frac{{(a)_n}{(b)_n}}{(c)_n}{\frac{u^n}{n!}}.\\\end{equation*}
The equations \eqref{eq:1},\eqref{eq:2},\eqref{eq:3} and \eqref{eq:4} can be tidied up somewhat by substituting for alpha $2\alpha=m+1$. Our equations then become
\begin{align*}
&u(1-u)\ddot{f} +\big(p+1-u(1-m)\big)\dot{f}+({\lambda}^2)f=0\\
&u(1-u)\ddot{f} +\big(p+1-u(2p+m+2+1)\big)\dot{f}+({\lambda}^2-(m+1+p)(p+1))f=0\\
&u(1-u)\ddot{f} +\big(\bar{p}+1-u(m+2+1)\big)\dot{f}+({\lambda}^2-m-1)f=0\\
&u(1-u)\ddot{f} +\big(\bar{p}+1-u(2{\bar p}-m+1)\big)\dot{f}+({\lambda}^2-{\bar p}({\bar p}-m))f=0\\
\intertext{Our parameters in each case then are}
&\eqref{eq:1}: \quad F(a,b;c;u) = F(\frac{-m}{2}+\sqrt{\frac{m^2}{4}+\lambda^2},\frac{-m}{2}-\sqrt{\frac{m^2}{4}+\lambda^2};p+1,u)\\
&\eqref{eq:2}: \quad F(a,b;c;u) = F(p+\frac{m}{2}+1+\sqrt{\frac{m^2}{4}+\lambda^2},p+\frac{m}{2}+1-\sqrt{\frac{m^2}{4}+\lambda^2};p+1,u)\\
&\eqref{eq:3}: \quad F(a,b;c;u) = F(\frac{m}{2}+1+\sqrt{\frac{m^2}{4}+\lambda^2}, \frac{m}{2}+1-\sqrt{\frac{m^2}{4}+\lambda^2};\bar{p}+1,u)\\
&\eqref{eq:4}: \quad F(a,b;c;u) = F(\bar{p}-\frac{m}{2}+\sqrt{\frac{m^2}{4}+\lambda^2},\bar{p}-\frac{m}{2}-\sqrt{\frac{m^2}{4}+\lambda^2};\bar{p}+1,u)\\
\end{align*}
This gives us the parameters for the hypergeometric equation. The factor of $\sqrt{\frac{m^2}{4}+\lambda^2}$  is common to all 4 expressions, I'm not sure what the significance of this is, if any. The solution to equations \eqref{eq:1} and \eqref{eq:2} are related by adding $p+m+1$ to the parameters in \eqref{eq:1}. Similarly the solutions to \eqref{eq:3} and \eqref{eq:4} are related by adding $\bar{p}-m-1$ to the parameters in \eqref{eq:3}.The hypergeometric functions given above are only one solution to the second order ODE, the second is of the form
\begin{equation}
u^{1-c}(1-u)^{c-a-b}F(1-a,1-b;2-c;u).\label{eq:second-solution}
\end{equation}
These are solutions around zero. These are the only solutions considered in the paper we have been following \cite{Villalba}. Should we consider solutions around $u=1$. As $u=\sin^{2}(\frac{\theta}{2})$ , $u=0$ is around the north pole of our sphere and $u=1$ is around the south pole. Should the solutions be similar or the same? I think it is reasonable to ignore solutions for $u$ at infinity as $u=\sin^{2}(\frac{\theta}{2})$ always lies between 0 and 1. Also in \cite{Villalba} the author justifies truncating the hypergeometric series, reducing it to finite polynomials, as ``we are looking for normalizable solutions according to the product''
\begin{align}
2\pi \int_{0}^{2\pi}{\Phi_k^{{\mu}\dagger}}{\Phi_{k'}^{\mu}}d\theta = \delta_{kk'}
\end{align}
I'm not sure why this product implies we should truncate the hypergeometric series. It does not appear to be a sufficient motivation. We will however continue with this thought and set one of the parameters equal to a negative integer for each of our four equations. For each we set $b= -n, \quad n \ \in \ \mathbb{Z^+}$ and we can find the form of the eigenvalues $\lambda$ with
\begin{align*}
&\eqref{eq:1}: \quad a=n-m, \quad b=-n, \quad c=p+1 \\
&\eqref{eq:2}: \quad a=n+2p+m+2, \quad b=-n, \quad c=p+1\\
&\eqref{eq:3}: \quad a=n+m+2, \quad  b=-n, \quad, c=\bar{p}+1\\
&\eqref{eq:4}: \quad a=n+2\bar{p}-m, \quad b=-n, \quad c=\bar{p}+1\\
\intertext{For (1) we have}
-ab &= n(n+m+2) \quad \text{and} \quad -ab= \lambda^2-m-1 \\
\lambda &= \pm \sqrt{n(n+m+2)+m+1} \\
\intertext{with a little rearranging we can show that}
\lambda &= \pm \sqrt{(n+1)(n+1+m)}
\intertext{which agrees with the results from \cite{Dolan}. Identical steps can be followed to show that the eigenvalues for all four equations are}
&\eqref{eq:1}: \quad \lambda_{n} = \pm \sqrt{(n)(n-m)} \\
&\eqref{eq:2}: \quad \lambda_{n+p+1} = \pm \sqrt{(n+1+p)(n+1+p+m)} \\
&\eqref{eq:3}: \quad \lambda_{n+1} = \pm \sqrt{(n+1)(n+1+m)} \\
&\eqref{eq:4}: \quad \lambda_{n+\bar{p}} = \pm \sqrt{(n+\bar{p})(n+\bar{p}-m)} 
\end{align*}
Now that we have set one of the parameters to a negative integer we can get the explicit form of the finit polynomial. They turn out to be Jacobi's polynomials, of the form \begin{equation*}F(\alpha+1+\beta+n, -n; \ \alpha+1; u)= \frac{n!}{(\alpha+1)_n}P^{(\alpha,\beta)}_{n}(1-2u) \end{equation*}
and for our four cases we have
\begin{align}
&F_1(n-m,-n;1+p;u), \ \alpha=p,\ \beta=-(m+p+1)\label{eq:F_1}\\
&F_2(2p+2+n+m,-n;1+p;u),\ \alpha=p, \ \beta=m+p+1\label{eq:F_2}\\
&F_3(n+m+2,-n;1+\bar{p};u), \ \alpha=\bar{p}, \ \beta=m+1-\bar{p}\label{eq:F_3}\\
&F_4(n+2\bar{p}-m,-n;1+\bar{p};u), \ \alpha=\bar{p}, \ \beta=\bar{p}-m-1
\label{eq:F_4}
\end{align}
                                                                    
Where I have introduced the subscript in the above functions to correspond with the number of our equations. We should also check the behaviour of our initial functions, now with the parameters set, around the north and south poles to ensure we avoid any singular points. Our functions for $\phi_1$ are
\begin{align*}
&\eqref{eq:1}:\ \frac{z^{p}}{(1+z\bar{z})^{-(\frac{m+1}{2})}}F_1,\quad &\eqref{eq:2}:\ \frac{z^{p}}{(1+z\bar{z})^{p+(\frac{m+1}{2})}}F_2\\
&\eqref{eq:3}:\ \frac{\bar{z}^{\bar{p}}}{(1+z\bar{z})^{(\frac{m+1}{2})}}F_3, \quad &\eqref{eq:4}:\ \frac{\bar{z}^{\bar{p}}}{(1+z\bar{z})^{\bar{p}-(\frac{m+1}{2})}}F_4\\
\intertext{If we substitute in for $z=\tan(\frac{\theta}{2})e^{i\phi}$, $\bar{z}=\tan(\frac{\theta}{2})e^-{i\phi}$ and $\frac{1}{1+ z\bar{z}} = \cos^2({\frac{\theta}{2}})$, and with some we have}
\eqref{eq:1}&:\quad (\sin(\frac{\theta}{2}))^{p}(\cos(\frac{\theta}{2}))^{-(p+m+1)}e^{ip\phi}F_1\\
\eqref{eq:2}&:\quad (\sin(\frac{\theta}{2}))^{p}(\cos(\frac{\theta}{2}))^{(p+m+1)}e^{ip\phi}F_2\\
\eqref{eq:3}&:\quad (\sin(\frac{\theta}{2}))^{\bar{p}}(\cos(\frac{\theta}{2}))^{(m+1-\bar{p})}e^{-{i\bar{p}\phi}}F_3\\
\eqref{eq:4}&:\quad (\sin(\frac{\theta}{2}))^{\bar{p}}(\cos(\frac{\theta}{2}))^{(\bar{p}-m-1)}e^{-{i\bar{p}\phi}}F_4\\
\intertext{From this form of $\phi_1$ we can see that there is a fixed range for p where it is well behaved at the poles. All four equations vanish at the poles (for $\theta=0$ and $\theta=\pi$) provided $p$ and $\bar{p}$ are positive in each case and }
\eqref{eq:1}&:\  0\leq p \leq -m-1\\
\eqref{eq:2}&:\  p \geq -m-1\\
\eqref{eq:3}&:\  0\leq \bar{p}\leq m+1\\
\eqref{eq:4}&:\  \bar{p} \geq m+1 
\end{align*}
With these boundaries for $p$ we also avoid the coordinate $\phi$ being singular at the poles as the $\sin$ and $\cos$ vanish there. It also seems that the powers of the $\sin$ and $\cos$ are the parameters for the Jacobi polynomials such that $\phi_1$ takes the form \begin{equation*}\phi_1 = (\sin(\frac{\theta}{2}))^{\alpha}(\cos(\frac{\theta}{2}))^{\beta}e^{(\pm)i\alpha\phi} \frac{n!}{(\alpha+1)_n}P^{(\alpha,\beta)}_{n}(1-2u), \end{equation*} where the sign of the coordinate $\phi$ is determined if its a $p$ or $\bar{p}$, I'm not sure if this surprising or to be expected.
The next step we need to take is to ensure that our solutions, which are solutions to the squared dirac operator, are solutions to our initial coupled differential equations \eqref{d1} and \eqref{d2}. To do so we must find solutions for the second component of the eigenspinor
\begin{equation*} \phi_2 = \frac{z^{s}\bar{z}^{\bar{s}}}{(1+z\bar{z})^r} g(z\bar z). \end{equation*} The steps are virtually identical to the case of $\phi_1$ and the resulting set of hyper geometric functions looks like
\begin{align}
&G_1(k-m+2,-k;1+s;u), \ \alpha=s,\ \beta=-(s+m-1), \ \bar{s} = 0, \ r=\alpha', \  \text{$s$ arbitary}\label{eq:G_1}\\
&G_2(2s+k+m,-k;1+s;u),\ \alpha=s, \ \beta=s+m-1, \ \bar{s} = 0, \ r=s-\alpha'\label{eq:G_2}\\
&G_3(k+m,-k;1+\bar{s};u), \ \alpha=\bar{s}, \ \beta=m-1-\bar{s}, \ s=0, \ r=-\alpha', \ \text{$\bar s $ arbitrary}\label{eq:G_3} \\
&G_4(k+2(\bar{s}+1)-m,-k;1+\bar{s};u), \ \alpha=\bar{s}, \ \beta=\bar{s}-m+1, \ s=0, \ r=\bar{s} + \alpha',\label{eq:G_4}
\end{align}
with $\alpha'=\frac{1-m}{2}$. A comparison of the eigenvalues from each solution gives us a hint as to how $n$, $k$, $p$, $s$, $\bar p$ and $\bar s$ are related.
\begin{center}
\begin{tabular}{ c|c|c|c }
  $F_1$ & $\lambda_{n} = \pm \sqrt{(n)(n-m)}$ & $G_1$ &  $\lambda_{k+1} = \pm \sqrt{(k+1)(k+1-m)}$\\ \cline{1-1} \cline {3-3}
  $F_2$ & $\lambda_{n+p+1} = \pm \sqrt{(n+1+p)(n+1+p+m)}$ & $G_2$ & $\lambda_{k+p} = \pm \sqrt{(k+s)(k+s+m)}$\\ \cline{1-1} \cline {3-3}
  $F_3$ & $\lambda_{n+1} = \pm \sqrt{(n+1)(n+1+m)}$ & $G_3$ & $\lambda_{k} = \pm \sqrt{(k)(k+m)}$\\ \cline{1-1} \cline {3-3}
  $F_4$ & $\lambda_{n+\bar{p}} = \pm \sqrt{(n+\bar{p})(n+\bar{p}-m)}$ & $G_4$ & $\lambda_{k+\bar{s}+1} = \pm \sqrt{(k+\bar{s}+1)(k+\bar{s}+1-m)}$.
\end{tabular}
\end{center}
This can be made more concrete by subbing (\ref{eq:G_1})-(\ref{eq:G_4}), along with our $F$'s
in (\ref{eq:F_1})-(\ref{eq:F_4}), into \eqref{d1} and \eqref{d2}: we have
\begin{align*}
(1 + z \bar z)\partial_z \left(\frac{z^{s}\bar{z}^{\bar{s}}}{(1+z\bar{z})^r} g(z\bar z)\right) + \frac{(m-1)}{ 2} \bar z \left(\frac{z^{s}\bar{z}^{\bar{s}}}{(1+z\bar{z})^r} g(z\bar z)\right) &= -i\lambda \left(\frac{z^{p}\bar{z}^{\bar{p}}}{(1+z\bar{z})^q} f(z\bar z)\right)\\
(1 + z \bar z)\partial_{\bar z} \left(\frac{z^{p}\bar{z}^{\bar{p}}}{(1+z\bar{z})^q} f(z\bar z)\right) - \frac{(m+1)}{ 2} z \left(\frac{z^{p}\bar{z}^{\bar{p}}}{(1+z\bar{z})^q} f(z\bar z)\right) &= -i\lambda \left(\frac{z^{s}\bar{z}^{\bar{s}}}{(1+z\bar{z})^r} g(z\bar z)\right)
\end{align*}
Looking at the allowed values for $s$ and $\bar{s}$ and how they are constrained, in a similar way to $p$ and $\bar{p}$, by the form of $\phi_2$ we find that the natural choice of $G$ and $F$ is for $F_1$ and $G_1$, $F_2$ and $G_2$ etc. to be related via the above equation. This gives us 4 pairs of coupled equations. \\
For $F_1$ and $G_1$, up to a proportionality constant, we have
\begin{align*}
\eqref{d1}&: \ (1 + z \bar z)\partial_z \left(\frac{z^{s}}{(1+z\bar{z})^{\alpha'}} G_1\right) + \frac{(m-1)}{ 2} \bar z \left(\frac{z^{s}}{(1+z\bar{z})^{\alpha'}} G_1\right) = -i\lambda c_1 \left(\frac{z^{p}}{(1+z\bar{z})^{-\alpha}} F_1\right)\\
\eqref{d2}&: \ (1 + z \bar z)\partial_{\bar z} \left(\frac{z^{p}}{(1+z\bar{z})^{-\alpha}} F_1\right) - \frac{(m+1)}{ 2} z \left(\frac{z^{p}}{(1+z\bar{z})^{-\alpha}} F_1\right) = \frac{-i\lambda}{c_1} \left(\frac{z^{s}}{(1+z\bar{z})^{\alpha'}} G_1\right)
\end{align*}
and doing the differentiation in \eqref{d1} we have
\begin{equation*}
    (1 + z \bar z)\left(\frac{z^{s}}{(1+z\bar{z})^{\alpha'}} \left( \frac{s}{z}G_1 - \frac{2\alpha' \bar{z}}{(1+z\bar{z})}G_1 + \frac{\partial u}{\partial z}\frac{dG_1}{du} \right)\right) = -i\lambda c_1 \left(\frac{z^{p}}{(1+z\bar{z})^{-\alpha}} F_1\right)
\end{equation*}
with $\alpha'= 1-\alpha = \frac{1-m}{2}$, $u= \frac{z \bar z}{(1+z\bar z)}$ and $\frac{\partial u}{\partial z} = \frac{\bar z}{(1+z\bar z)^2} $ we can rearrange this equation in to the form
\begin{equation*}
    z^{s}\left( sG_1 - 2\alpha' u G_1 + u(1-u)\frac{dG_1}{du} \right) = -i\lambda c_1 z^{p+1}F_1.
\end{equation*}
Rewriting this in terms of the parameters of $G_1(a,b;c;u)$ hypergeomtric functions gives
\begin{equation*}
    z^{s}\left( (c-1)G_1 - (a+b-1) u G_1 + u(1-u)\frac{dG_1}{du} \right) = -i\lambda c_1 z^{p+1}F_1
\end{equation*}
which, with a bit of work, we find the l.h.s. is this identity 15.2.9 from \cite{abramowitz+stegun} in chapter 15
\begin{align*}
     &\frac{d}{du} [u^{c-1}(1-u)^{a+b-c}F(a,b;c;u)] = (c-1)u^{c-2}(1-u)^{a+b-c-1}F(a-1,b-1;c-1;u) \\
\intertext{fleshing out the differentiation on the left gives}
    &(c-1)u^{c-2}(1-u)^{a+b-c}F(a,b;c;u)-(a+b-c)u^{c-1}(1-u)^{a+b-c-1}F(a,b;c;u)+ \\
    &u^{c-1}(1-u)^{a+b-c}\frac{dF}{du} = (c-1)u^{c-2}(1-u)^{a+b-c-1}F(a-1,b-1;c-1;u)\\
\intertext{then dividing through the factors of $u$ (ommitting the parameters in $F$ on the r.h.s)}
    & (c-1)(1-u)F - (a+b-c)uF + u(1-u)\frac{dF}{du} = (c-1) F(a-1,b-1;c-1;u) \\
    & (c-1)F -(a+b-1)uF + u(1-u) \frac{dF}{du} = (c-1)F(a-1,b-1;c-1;u)
\end{align*}
Thus our above subbing $G_1$ and $F_1$ into \eqref{d1} yields 
\begin{equation*}
    sz^{s}G_1(k+1-m,-(k+1);s;u) = -i\lambda c_1 z^{p+1}F_1(n-m,-n;1+p;u).
\end{equation*}
with $n=k+1$, $p+1=s$ and $c_1=\frac{i(p+1)}{\lambda}$. Following similar steps for $F_1$ in \eqref{d2} and using the differentiation identity 15.2.1 in \cite{abramowitz+stegun} we find the same relation as above between $F_1$ and $G_1$. Following similar steps for the 3 remaining pairs of coupled differential equations, and using the differentiation identities from \cite{abramowitz+stegun} here listed;
\begin{center}
\begin{tabular}{|c|c|}
    \hline For $G_2$ in \eqref{d1} use 15.2.4 & For $F_2$ in \eqref{d2} use 15.2.6 \\
    \hline For $G_3$ in \eqref{d1} use 15.2.1 & For $F_3$ in \eqref{d2} use 15.2.3 \\
    \hline For $G_4$ in \eqref{d1} use 15.2.6 & For $F_4$ in \eqref{d2} use 15.2.4 \\ 
    \hline
\end{tabular}
\end{center}
we arrive at the relations between the $G$'s and $F$'s
\begin{align*}
  &G_1=c_1F_1, \quad n=k+1, \ n\geq1,   \ p=s-1\\
  &G_2=c_2F_2, \quad n=k, \ k\geq0, \ p=s-1\\
  &G_3=c_3F_3, \quad n=k-1, \ k\geq1, \ \bar{p} = \bar{s} +1 \\
  &G_4=c_4F_4, \quad n=k, \ k\geq0, \ \bar{p} = \bar{s} +1,
\end{align*}
with our complex proportionality constants, $\{c_i,i=1,2,3,4\} $ being
\begin{align}
  &c_{1}= \frac{i(p+1)}{\lambda_{n}}\\
  &c_{2}= \frac{i(p+1)}{\lambda_{n+p+1}}\\
  &c_{3}= \frac{\lambda_{n+1}}{i\bar{p}}\\
  &c_{4}= \frac{\lambda_{n+\bar{p}}}{i\bar{p}}\label{eq:c_i}
\end{align}
(I think the factors of $p$ and $p+1$ are different if we use Jacobi polynomials rather than hypergeometric functions, the normalisations differ).

Thus the solutions we have for the squared Dirac operator are valid for our initial Dirac equation. Also it is worth noting that in each case we have that 
\begin{align*}
    &\phi_1= \frac{z^{p}}{(1+z\bar{z})^{-\alpha}}F_1, \quad \phi_2 = \frac{z^{s}}{(1+z\bar{z})^{1-\alpha}}G_1 \\
    &\Rightarrow \phi_2 =\frac{c_1z}{(1+z\bar z)}\phi_1
    \intertext{And for $F_2$,$F_3$ and $F_4$}
    F_2 \text{ \&} \ G_2 &\Rightarrow \ \phi_2 = c_2z\phi_1 \\
    F_3 \text{ \&} \ G_3 &\Rightarrow \ \phi_1 = \frac{\bar z}{c_3(1+z\bar z)} \phi_2\\
    F_4 \text{ \&} \ G_4 &\Rightarrow \ \phi_1 = \frac{\bar z}{c_4}\phi_2.
\end{align*}
I think given the way $n$ and $k$ are related, which are the degree's of the polynomials from the hypergeometric functions, this should be how the components of the eigenspinor are related.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Jacobi Polynomials}

To get a deeper understanding of the spectrum we should arrange the
eigenspinors into irreducible representations of $SU(2)$.
To this end we shift the integer $n$ in (\ref{eq:1})-(\ref{eq:4})
and re-express $F_1 - F_4$ in (\ref{eq:F_1}) - (\ref{eq:F_4}), and their associated eigenvalues, as 
\begin{align*}
&F_1(n-m,-n;1+p;u),&\qquad \lambda = n(n-m)\\
&F_2(n+p+1+m,p+1-n;1+p;u),&\qquad \lambda = n(n+m)\\
&F_3(n+m+1,-n+1;1+\bar{p};u),&\qquad \lambda = n(n+m)\\
&F_4(n+\bar{p}-m,\bar{p}-n;1+\bar{p};u),& \qquad \lambda = n(n-m).
\end{align*}
The associated $\phi_1$'s are
\begin{align}
&\phi_1=e^{i p \phi} u^{\frac p 2} (1-u)^{-\frac{m+1+p}{2}} F_1(n-m,-n;1+p;u),\label{eq:phi_1-F_1}\\
&\phi_1=e^{i p \phi} u^{\frac p 2} (1-u)^{\frac{m+1+p}{2}} F_2(n+p+1+m,p+1-n;1+p;u),\label{eq:phi_1-F_2}\\
&\phi_1=e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{m+1-\bar{p}}{2}} F_3(n+m+1,-n+1;1+\bar{p};u)\label{eq:phi_1-F_3}\\
&\phi_1=e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{\bar{p} -m-1}{2}} F_4(n+\bar{p}-m,\bar{p}-n;1+\bar{p};u).\label{eq:phi_1-F_4}
\end{align}
We might worry that $\phi_1$ in (\ref{eq:phi_1-F_1}) looks as though it diverges at $u=1$ if $m$ and $p$ are positive, but $F_1$ will have $(1-u)$ factors in it if $F_1(1)=0$. Using the identity (Abromowitz and Stegun: 15.3.3)
\[ F(a,b;c;u) = (1-u)^{a+b-c} F(c-a, c-b; c; u) \]
we have
\begin{align}
  \phi_1&=e^{i p \phi} u^{\frac p 2} (1-u)^{-\frac{m+1+p}{2}} F_1(n-m,-n;1+p;u),\label{eq:F_1a}\\
  &=e^{i p \phi} u^{\frac p 2} (1-u)^{\frac{m+1+p}{2}} F_1(p+1+m -n,p+1+n;1+p;u),\label{eq:F_1b}\\
        \phi_1&=e^{i p \phi} u^{\frac p 2} (1-u)^{\frac{m+1+p}{2}} F_2(n+p+1+m,p+1-n;1+p;u),\label{eq:F_2a}\\
  &=e^{i p \phi} u^{\frac p 2} (1-u)^{-\frac{m+1+p}{2}} F_2(-n-m,n;1+p;u),\label{eq:F_2b}\\
  \phi_1&=e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{m+1-\bar{p}}{2}} F_3(n+m+1,-n+1;1+\bar{p};u)\label{eq:F_3a}\\
  &=e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{\bar{p}-m-1}{2}} F_3(\bar p -m -n,\bar p +n ;1+\bar{p};u)\label{eq:F_3b}\\
  \phi_1&=e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{\bar{p} -m-1}{2}} F_4(n+\bar{p}-m,\bar{p}-n;1+\bar{p};u),\label{eq:F_4a}\\
  &=e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{m+1-\bar{p}}{2}} F_4(1+m-n,n+1;1+\bar{p};u).\label{eq:F_4b}
\end{align}
There is clearly a redundancy here, for example (\ref{eq:F_1a})
and (\ref{eq:F_2b}) are the same except $n$ in (\ref{eq:F_1a})
is replaced with $-n$ in (\ref{eq:F_2b}). Removing this redundancy a complete set is  
\begin{align}
        \phi_1&=e^{i p \phi} u^{\frac p 2} (1-u)^{\frac{m+1+p}{2}} F_2(n+p+1+m,p+1-n;1+p;u),\label{eq:F2a}\\
  &=e^{i p \phi} u^{\frac p 2} (1-u)^{-\frac{m+1+p}{2}} F_2(-n-m,n;1+p;u),\label{eq:F2b}\\
  \phi_1&=e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{m+1-\bar{p}}{2}} F_3(n+m+1,-n+1;1+\bar{p};u)\label{eq:F3a}\\
  &=e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{\bar{p}-m-1}{2}} F_3(\bar p -m -n,\bar p +n ;1+\bar{p};u)\label{eq:F3b}.\end{align}
Both of these have eigenvalue squared
\[ \lambda^2 = n(n+m),\]
with $n\ge 0$ for positive $m$ and $n\le 0$ for negative $m$.
Indeed from (\ref{eq:second-solution}) we see that, with $\bar p = -p$,
(\ref{eq:F3b}) is the second solution associated with (\ref{eq:F2a})
and
(\ref{eq:F3a}) is the second solution associated with (\ref{eq:F2b}).

Thus (\ref{eq:F2a})--(\ref{eq:F3b}) are all we need.
These give Jacobi polynomials whenever $a$ or $b$ in the hypergeometric function $F(a,b;c;u)$ is either zero or a negative integer. The details depend on the sign of $m$:
\begin{itemize}
\item $m>0$:
    \begin{align}
      \hbox{(\ref{eq:F2a})}  \ \Rightarrow \ 
      \phi_1
      &= e^{i p \phi} u^{\frac p 2} (1-u)^{\frac{m+1+p}{2}} P_{n-p-1}^{(p,p+m+1)}(1-2 u), \quad 0\le p \le n-1,\label{eq:phi_1-2a}\\
       \hbox{(\ref{eq:F3a})}  \ \Rightarrow \ 
      \phi_1
      &= e^{-i \bar{p} \phi} u^{\frac {\bar p} {2}} (1-u)^{\frac{m+1 - {\bar p}}{2}} P_{n-1}^{(\bar p,m+1-\bar p)}(1-2 u), \quad 0 < \bar p < m+1,\label{eq:phi_1-3a}\\
       \hbox{(\ref{eq:F3b})}  \ \Rightarrow \ 
      \phi_1
      &= e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{\bar p -m-1}{2}} P_{m+n - \bar p}^{(\bar p,\bar p-m-1)}(1-2 u), \label{eq:phi_1-3b} \\
 & \hskip 5.7cm  m+1\le \bar p \le m+n. \nonumber
      \end{align}
      We do not need (\ref{eq:F2b}) as (\ref{eq:phi_1-2a}) exhausts the $\bar p=0$ possibilities.  There are precisely $2n+m$ different solutions here all with $\lambda =n(n+m)$. We use strict inequalities in (\ref{eq:phi_1-3a}) because $\bar p=0$ in 
      (\ref{eq:phi_1-3a}) is the same as $p=0$ in (\ref{eq:phi_1-2a}) and
      $\bar p = m+1$ in (\ref{eq:phi_1-3a}) is the same as
            $\bar p = m+1$ in (\ref{eq:phi_1-3b}).
      
          \item $m<0$ (with $n'=-n \ge 0$):
             \begin{align}
      \hbox{(\ref{eq:F2a})}  \ \Rightarrow \ 
      \phi_1
      &= e^{i p \phi} u^{\frac p 2} (1-u)^{\frac{p-|m|+1}{2}} P_{n'+|m|-p-1}^{(p,p-|m|+1)}(1-2 u),  \label{eq:phi_1-2a-}\\
  & \hskip 5.5cm |m|-1 < p \le n'+|m|-1,\nonumber \\
       \hbox{(\ref{eq:F2b})}  \ \Rightarrow \ 
      \phi_1
      &= e^{i  p \phi} u^{\frac {p} {2}} (1-u)^{\frac{|m|-1-p}{2}} P_{n'}^{(p,|m|-1-p)}(1-2 u), \quad 0 \le  p \le |m|-1,\label{eq:phi_1-2b-}\\
       \hbox{(\ref{eq:F3b})}  \ \Rightarrow \ 
      \phi_1
      &= e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{\bar p +|m|-1}{2}} P_{n' - \bar p}^{(\bar p,\bar p+|m|-1)}(1-2 u), \quad
1\le \bar p \le n'. \label{eq:phi_1-3b-}
      \end{align}
  We do not need (\ref{eq:F3a}) as (\ref{eq:F3b}) exhausts the $p=0$ possibilities.  There are precisely $2n+m$ different solutions here all with $\lambda =n'(n'+|m|)$. We use a strict inequality for the lower bound in in (\ref{eq:phi_1-2a-}) because $p=|m|-1$ in 
      (\ref{eq:phi_1-2a-}) is the same as $p=|m|-1$ in (\ref{eq:phi_1-2b-}) and
we do not include $\bar p=0$ in (\ref{eq:phi_1-3b-})
because that would replicate $p=0$ in (\ref{eq:phi_1-3b-}).
         \end{itemize}

    A similar analysis involving $G_1$-$G_4$ in (\ref{eq:G_1})-(\ref{eq:G_4})
    gives $\phi_2$, analogues of (\ref{eq:phi_1-F_1})-(\ref{eq:phi_1-F_4}), 
\begin{align}
        \phi_2&=e^{i s \phi} u^{\frac s 2} (1-u)^{\frac{s+m-1}{2}} G_2(s+n+m,s-n;1+s;u),\label{eq:G2a}\\
  &=e^{i s \phi} u^{\frac s 2} (1-u)^{\frac{1-m-s}{2}} G_2(-n-m+1,n+1;1+s;u),\label{eq:G2b}\\
  \phi_2&=e^{-i \bar s \phi} u^{\frac {\bar s} 2} (1-u)^{\frac{m-1-\bar{s}}{2}} G_3(n+m,-n;1+\bar{s};u)\label{eq:G3a}\\
              &=e^{-i \bar s \phi} u^{\frac {\bar s} 2} (1-u)^{\frac{1+\bar{s}-m}{2}} G_3(1+\bar s -n- m,n+\bar s+1 ;1+\bar{s};u)\label{eq:G3b},\end{align}
            both of which have
            \[ \lambda^2 = n(n+m)\]
            with $n\ge 0$   when $m>0$ and $n\le 0$ when $m<0$.   Again we treat positive and negative $m$ separately
\begin{itemize}
\item $m>0$, $n\ge 0$,
 $\lambda^2 =n(n+m)$:
    \begin{align}
      \hbox{(\ref{eq:G2a})}  \ \Rightarrow \ 
      \phi_2
      &= e^{i s \phi} u^{\frac s 2} (1-u)^{\frac{s+m-1}{2}} P_{n-s}^{(s,s+m-1)}(1-2 u), \quad 1\le s \le n,\label{eq:phi_2-2a}\\
       \hbox{(\ref{eq:G3a})}  \ \Rightarrow \ 
      \phi_2
      &= e^{-i \bar{s} \phi} u^{\frac {\bar s} {2}} (1-u)^{\frac{m-1 - {\bar s}}{2}} P_n^{(\bar s,m-1-\bar s)}(1-2 u), \quad 0 \le \bar s \le m-1,\label{eq:phi_2-3a}\\
       \hbox{(\ref{eq:G3b})}  \ \Rightarrow \ 
      \phi_2
      &= e^{-i \bar s \phi} u^{\frac {\bar s} 2} (1-u)^{\frac{\bar s -m+1}{2}}
        P_{m+n - \bar s-1}^{(\bar s,\bar s -m+1)}(1-2 u), \quad m \le \bar s \le m+n-1.\label{eq:phi_2-3b} 
      \end{align}
      Again there is a total of $2n+m$ linearly independent eigenfunctions here, all with the same eigenvalue. We do not need (\ref{eq:G2b}) as (\ref{eq:phi_2-2a}) exhausts the $\bar s=0$ possibilities. We do not include  $\bar s=m-1$ in
      (\ref{eq:phi_2-3b}) because $\bar s=m-1$ in 
      (\ref{eq:phi_2-3b}) is the same as $\bar s=m-1$ in (\ref{eq:phi_2-3a}).
      Also we do not include $s=0$ in (\ref{eq:phi_2-2a}) as that is the same
      as $\bar s=0$ in (\ref{eq:phi_2-3a}).
          \item $m<0$ (with $n'=-n \ge 0$), $\lambda^2=n'(n'+|m|)$:
             \begin{align}
      \hbox{(\ref{eq:G2a})}  \ \Rightarrow \ 
      \phi_2
      &= e^{i s \phi} u^{\frac s 2} (1-u)^{\frac{s-|m|-1}{2}} P_{n'+|m|-s}^{(s,s-|m|-1)}(1-2 u), \quad |m|+1 \le s \le n'+|m|,\label{eq:phi_2-2a-}\\
       \hbox{(\ref{eq:G2b})}  \ \Rightarrow \ 
      \phi_2
      &= e^{i  s \phi} u^{\frac {s} {2}} (1-u)^{\frac{|m|+1-s}{2}} P_{n'-1}^{(s,|m|+1-s)}(1-2 u), \quad 1 \le  s \le |m|,\label{eq:phi_2-2b-}\\
           \phi_2
      &= e^{-i \bar s \phi} u^{\frac {\bar s} 2} (1-u)^{\frac{\bar s +|m|+1}{2}} P_{n' - \bar s -1}^{(\bar s,\bar s+|m|+1)}(1-2 u), \quad 0\le \bar s \le n'-1.\label{eq:phi_2-3b-} 
      \end{align}
      We do not need (\ref{eq:G3a}) as (\ref{eq:G3b}) exhausts the $s=0$ possibilities.  There are precisely $2n+m$ different solutions here all with
      $\lambda =n'(n'+|m|)$. We do not include $s=0$ in (\ref{eq:phi_2-2b-})
      as that is the same as $\bar s=0$ in (\ref{eq:phi_2-3b-}) and we do not include $s=|m|+1$ in (\ref{eq:phi_2-2b-}) as that is the same as $s=|m|+1$ in (\ref{eq:phi_2-2a-}).
         \end{itemize}

         To recap, the eigenfunctions with $\lambda^2=n(n+|m|)$ are
         \begin{itemize}
         \item $m>0$:
           \begin{align}
      \phi_1
      &= e^{i p \phi} u^{\frac p 2} (1-u)^{\frac{m+1+p}{2}} P_{n-p-1}^{(p,p+m+1)}(1-2 u), \quad 0\le p \le n-1,\label{eq:phi_1-1}\\
      \phi_1
      &= e^{-i \bar{p} \phi} u^{\frac {\bar p} {2}} (1-u)^{\frac{m+1 - {\bar p}}{2}} P_{n-1}^{(\bar p,m+1-\bar p)}(1-2 u), \quad 0 < \bar p < m+1,\label{eq:phi_1-2}\\
      \phi_1
             &= e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{\bar p -m-1}{2}} P_{m+n - \bar p}^{(\bar p,\bar p-m-1)}(1-2 u), \quad m+1\le \bar p \le m+n.\label{eq:phi_1-3}\\
      \phi_2
      &= e^{i s \phi} u^{\frac s 2} (1-u)^{\frac{s+m-1}{2}} P_{n-s}^{(s,s+m-1)}(1-2 u), \quad 1\le s \le n,\label{eq:phi_2-1}\\
      \phi_2
      &= e^{-i \bar{s} \phi} u^{\frac {\bar s} {2}} (1-u)^{\frac{m-1 - {\bar s}}{2}} P_n^{(\bar s,m-1-\bar s)}(1-2 u), \quad 0 \le \bar s \le m-1,\label{eq:phi_2-2}\\
            \phi_2
      &= e^{-i \bar s \phi} u^{\frac {\bar s} 2} (1-u)^{\frac{\bar s -m+1}{2}}
        P_{m+n - \bar s-1}^{(\bar s,\bar s -m+1)}(1-2 u), \quad m \le \bar s \le m+n-1.\label{eq:phi_2-3} 
           \end{align}
         \item $m<0$:
           \begin{align}
 \phi_1
      &= e^{i p \phi} u^{\frac p 2} (1-u)^{\frac{p-|m|+1}{2}} P_{n+|m|-p-1}^{(p,p-|m|+1)}(1-2 u), \quad |m|-1 < p \le n+|m|-1,\label{eq:-phi_1-1}\\
      \phi_1
      &= e^{i  p \phi} u^{\frac {p} {2}} (1-u)^{\frac{|m|-1-p}{2}} P_{n}^{(p,|m|-1-p)}(1-2 u), \quad 0 \le  p \le |m|-1,\label{eq:-phi_1-2}\\
      \phi_1
      &= e^{-i \bar p \phi} u^{\frac {\bar p} 2} (1-u)^{\frac{\bar p +|m|-1}{2}} P_{n - \bar p}^{(\bar p,\bar p+|m|-1)}(1-2 u), \quad 1\le \bar p \le n.\label{eq:-phi_1-3} \\
&\nonumber\\
             \phi_2
      &= e^{i s \phi} u^{\frac s 2} (1-u)^{\frac{s-|m|-1}{2}} P_{n+|m|-s}^{(s,s-|m|-1)}(1-2 u), \quad |m|+1 \le s \le n+|m|,\label{eq:-phi_2-1}\\
      \phi_2
      &= e^{i  s \phi} u^{\frac {s} {2}} (1-u)^{\frac{|m|+1-s}{2}} P_{n-1}^{(s,|m|+1-s)}(1-2 u), \quad 1 \le  s \le |m|,\label{eq:-phi_2-2}\\
           \phi_2
      &= e^{-i \bar s \phi} u^{\frac {\bar s} 2} (1-u)^{\frac{\bar s +|m|+1}{2}} P_{n - \bar s -1}^{(\bar s,\bar s+|m|+1)}(1-2 u), \quad 0\le \bar s \le n-1.\label{eq:-phi_2-3} 
                \end{align}
              \end{itemize}
These formula can be made much neater using the identities in Appendix B of \cite{Wu+Yang},
\begin{align}
P^{(-\alpha,\beta)}_{n+\alpha}(1-2u)&=(-1)^\alpha \frac{n!(n+\alpha+\beta)!}{(n+\alpha)!(n+\beta)!}u^\alpha P_n^{(\alpha,\beta)}(1-2u), \\
P^{(\alpha,-\beta)}_{n+\beta}(1-2u)&= \frac{n!(n+\alpha+\beta)!}{(n+\alpha)!(n+\beta)!}(1-u)^\beta P_n^{(\alpha,\beta)}(1-2u), \label{eq:P-beta}\\
P^{(-\alpha,-\beta)}_{n+\alpha+\beta}(1-2u)&=(-1)^{\alpha}(u)^\alpha (1-u)^ \beta  P_n^{(\alpha,\beta)}(1-2u). 
\end{align}
Then, up to normalisations,
\begin{itemize}
\item $m>0$, with $p=-\bar p$ and $s=-\bar s$:
\begin{align}
\phi_1 & = e^{-i \bar{p} \phi} u^{\frac {\bar p} {2}} (1-u)^{\frac{m+1 - {\bar p}}{2}} P_{n-1}^{(\bar p,m+1-\bar p)}(1-2 u), \quad -n+1 \le \bar p \le n+m ,\label{eq:phi_1+}\\
\phi_2 & = e^{-i \bar{s} \phi} u^{\frac {\bar s} {2}} (1-u)^{\frac{m-1 - {\bar s}}{2}} P_n^{(\bar s,m-1-\bar s)}(1-2 u), \quad -n \le \bar s \le n+m-1.\label{eq:phi_2+}
\end{align}
\item $m<0$ with $\bar p = -p$ and $\bar s = -s$:
\begin{align}
\phi_1 & = e^{i  p \phi} u^{\frac {p} {2}} (1-u)^{\frac{|m|-1-p}{2}} P_{n}^{(p,|m|-1-p)}(1-2 u), \quad -n \le  p \le n+|m|-1,\label{eq:-phi_1-}\\
\phi_2 & = e^{i  s \phi} u^{\frac {s} {2}} (1-u)^{\frac{|m|+1-s}{2}} P_{n-1}^{(s,|m|+1-s)}(1-2 u), \quad -n+1 \le  s \le n+|m|.\label{eq:-phi_2-}
\end{align}
\end{itemize}

The eigenspinors can be more succinctly written by defining $y=\frac{1-x}{1+x}=1-2u = \cos\theta$, $\alpha = p$ and $\beta = |m|-1-p$.  In terms of which the un-normalised components for $m<0$ are
\begin{align}
\phi_1 & = z^\alpha \left(\frac{1+y}{2} \right)^{\frac{\alpha+\beta}{2}} P_n^{(\alpha,\beta)}(y)\label{eq:phi_1}\\ 
\phi_2 & = z^{\alpha+1} \left(\frac{1+y}{2} \right)^{\frac{\alpha+\beta}{2}+1} P_{n-1}^{(\alpha+1,\beta+1)}(y),\label{eq:phi_2}
\end{align}
with $-n\le \alpha \le n + |m| +1$ and $\lambda = \pm\sqrt{n(n+|m|)}$.
If we use $|m|$ everywhere in the polynomials then the $m<0$ case is obtained from the $m>0$ case simply by interchanging $\phi_1$ and $\phi_2$ and complex conjugating.  The disadvantage of these forms is that it is not a priori obvious, given the
ranges of $p$, $s$, $\bar p$ and $\bar s$, that they are finite at $u=0$ and $u=1$, but they are!

The overall normalisation of the eigenspinors is arbitrary, but the relative normalisation is fixed  by the Dirac equation. We can obtain the relative normalisations of $\phi_1$ and $\phi_2$ from
\begin{align} \left\{(1+ \bar z z)\partial_z +\left(\frac{m-1}2\right) \bar z \right\} \phi_2 & = - i \frac \lambda c \phi_1,\label{eq:D_z-phi_2}\\
\left\{(1+ \bar z z)\partial_{\bar z} - \left(\frac{m+1}2\right)z\right\}  \phi_1 & 
= - i \lambda c \phi_2\label{eq:D_zbar-phi_1} \end{align} 
where $c$ is a constant to be determined.
Using (\ref{eq:phi_1}) with 
$\bar z z= x=\frac{1-y}{1+y}$ and $\alpha+\beta = -m-1=|m|-1$,
\begin{align*}
\left\{(1+ \bar z z)\partial_{\bar z} - \left(\frac{m+1}2\right)z\right\}  \phi_1&=
z^{\alpha+1}\left\{(1+x)\frac{d y}{d x}\frac{d}{d y}  - \left( \frac{m+1}{2} \right)  \right\}
\left\{\left(\frac{1+y}{2}\right)^{\frac{\alpha + \beta}{2}}  P_n^{(\alpha,\beta)}(y)\right\}\\
&=z^{\alpha+1}\left\{-(1+y) \frac{d}{d y}  + \left( \frac{\alpha + \beta}{2} \right)  \right\}
\left\{\left(\frac{1+y}{2}\right)^{\frac{\alpha + \beta}{2}}  P_n^{(\alpha,\beta)}(y)\right\}\\
&=-2 z^{\alpha+1}\left(\frac{1+y}{2}\right)^{\frac{\alpha + \beta}{2}+1} 
\frac{d P_n^{(\alpha,\beta)}(y)}{d y}.  \\
\end{align*}
Now we use\footnote{https://en.wikipedia.org/wiki/Jacobi\_polynomials.}
\[ \frac{d P_n^{(\alpha,\beta)}}{d y} = \frac{1}{2} (n+\alpha + \beta+1) P_{n-1}^{(\alpha+1,\beta+1)}=  \frac{1}{2} (n-m) P_{n-1}^{(\alpha+1,\beta+1)},\]
put this into in (\ref{eq:D_zbar-phi_1}) with $\lambda = \pm \sqrt{n(n+|m|)}$ 
and compare with (\ref{eq:phi_2}) to obtain
\begin{equation}
 c=\mp i\sqrt{\frac{n+|m|}{n}}.\label{eq:c-value}\end{equation}

As a check we should
 confirm (\ref{eq:D_z-phi_2}) with (\ref{eq:c-value}).
We can do this using Rodrigues' 
formula%\cite{JacobiPolynomials}
\footnote{https://en.wikipedia.org/wiki/Jacobi\_polynomials.}
\begin{equation}
P_n^{(\alpha,\beta)}(y)  = \frac{(-1)^n}{2^n n!}(1-y)^{-\alpha} (1+y)^{-\beta} \frac{d^n}{d y^n}
\Bigl\{ (1-y)^\alpha (1+y)^\beta (1-y^2)^n \Bigr\},\label{eq:Rodrigues-P}
\end{equation}
which can be used to show that
\begin{equation} \frac{d}{d y} \left\{ (1-y)^{\alpha +1}(1+y)^{\beta +1}
P_{n-1}^{(\alpha+1,\beta+1)}(y) \right\} = - 2 n  (1-y)^\alpha(1+y)^\beta
P_n^{(\alpha,\beta)}(y).\label{eq:R-2}\end{equation}
Now
\begin{align*}
\left\{  (1 \vline width 0pt height 14pt depth 9pt \right.  & \left. +\bar z z) \partial_z   +\left( \frac{m-1}{2} \right) \bar z  \right\} \phi_2\\
&= z^\alpha 
\left\{
(1+x) (\alpha+1) +(1+x) x \frac{d}{d x} -\left(\frac{\alpha+\beta+2}{2}\right) x  
\right\}
\left\{ \left(\frac{1+y}{2} \right)^{\frac {\alpha + \beta}{2} +1} P_{n-1}^{(\alpha+1,\beta+1)}(y) \right\}\\
&= z^\alpha \left\{ 2\left(\frac{\alpha+1}{1+y}\right)
-(1-y) \frac{d}{d y} -\left(\frac{\alpha+\beta+2}{2}\right) \left(\frac{1-y}{1+y}  \right)
\right\}
\left\{ \left(\frac{1+y}{2} \right)^{\frac {\alpha + \beta}{2} +1} P_{n-1}^{(\alpha+1,\beta+1)}(y) \right\}\\
&= -\frac{z^\alpha }{2^{\frac{\alpha+\beta}{2}+1}}
(1-y)^{-\alpha} (1+y)^{\frac{\alpha - \beta}{2}}  \frac{d}{d y} 
\left\{
 (1-y)^{\alpha+1}  (1+y)^{\beta+1} 
P_{n-1}^{(\alpha+1,\beta+1)}(y) \right\} \\
&= \frac{n z^\alpha }{2^{\frac{\alpha+\beta}{2}}}
(1-y)^{-\alpha} (1+y)^{\frac{\alpha - \beta}{2}} 
\left\{  (1-y)^{\alpha}  (1+y)^{\beta}  P_n^{(\alpha,\beta)}(y) \right\}
\hskip 3cm \hbox{(using (\ref{eq:R-2}))}\\
& = n z^\alpha \left( \frac{1+y}{2}\right)^{\frac{\alpha + \beta}{2}} P_n^{(\alpha,\beta)}(y).  
\end{align*}
Equating this with $-i \frac{\lambda}{c} \phi_1=\mp i \frac{\sqrt{n(n+|m|)}}{c} \phi_1$, as in (\ref{eq:D_z-phi_2}) reproduces (\ref{eq:c-value}), so everything is consistent.

In summary, the eigenspinors with  $\lambda = \pm \sqrt{n(n+|m|)}$ are, for $m<0$,
\begin{empheq}[box=\fbox]{equation}
\psi_{\lambda,\alpha} = {\cal N} 
 z^\alpha \left(\frac{1+y}{2} \right)^{\frac{\alpha+\beta}{2}}\begin{pmatrix}
 P_n^{(\alpha,\beta)}(y)\\ 
\mp i \sqrt{\frac{n+|m|}{n}} z \left(\frac{1+y}{2}\right)  P_{n-1}^{(\alpha+1,\beta+1)}(y)
\end{pmatrix}\label{eq:sphere-eigenspinors}
\end{empheq}
with $\alpha =-n,\ldots n+|m|$, $\alpha+\beta = |m|-1$ and ${\cal N}$ 
an overall constant that will depend on $n$, $\alpha$ and $\beta$. 
The normalisation can be fixed using
\[\int_{-1}^1 (1-y)^\alpha (1+y)^\beta P^{(\alpha,\beta)}_n(y) P^{(\alpha,\beta)}_{n'}(y) d y
= \frac{2^{\alpha+\beta+1}}{(2 n + \alpha +\beta +1)} 
\frac{\Gamma(n+\alpha+1)\Gamma(n+\beta+1)}{\Gamma(n+1)\Gamma(n+\alpha+\beta+1)}
\delta_{n n'}.
\] 
For $m>0$ interchange the two components and complex conjugate. 
In calculating the normalisation we want 
\begin{equation}
  \int_{-1}^{1} dy \ |\psi_{\lambda, \alpha}(y)|^{2} ~=~ \frac{1}{2\pi}.
\end{equation}
Where we integrate from $-1 \rightarrow 1$ as $dy = -\sin{\theta}d\theta$.
Rewriting the eigenspinors as
\begin{align}
&\psi_{\lambda,\alpha} = \mathcal{N} z^{\alpha} \left(\frac{1+y}{2}\right)^{\frac{\alpha + \beta}{2}} \begin{pmatrix}
\Tilde{\phi_{1}} \\ \Tilde{\phi_{2}}
\end{pmatrix} \\
\intertext{The above integral becomes;}
&\int_{-1}^{1} \mathcal{N}^2 (z\bar{z})^{\alpha}\left(\frac{1+y}{2}\right)^{\alpha + \beta}\left(|\Tilde{\phi_{1}}|^2 + |\Tilde{\phi_{2}}|^2 \right) \\
&= \int_{-1}^{1}\frac{\mathcal{N}^2}{2^{\alpha +\beta}}(1-y)^\alpha (1+y)^\beta \left(|\Tilde{\phi_{1}}|^2 + |\Tilde{\phi_{2}}|^2 \right)\\
&= \frac{\mathcal{N}^2}{2^{\alpha +\beta}} \int_{-1}^1  (1-y)^\alpha (1+y)^\beta \left(P^{(\alpha,\beta)}_n(y)\right)^2 +  (1-y)^{\alpha+1} (1+y)^{\beta+1}\left(\frac{n+|m|}{4n}\right) \left(P^{(\alpha+1,\beta+1)}_{n-1}(y)\right)^2 \ dy \\
\intertext{Using the above definition from \cite{abramowitz+stegun} along with $\alpha + \beta = |m| -1$ we have}
&= \frac{\mathcal{N}^2}{2^{|m|-1}} \left(\frac{2^{|m|}}{(2 n + |m|)} 
\frac{\Gamma(n+\alpha+1)\Gamma(n+\beta+1)}{\Gamma(n+1)\Gamma(n+|m|)} +  \frac{n+|m|}{4n}\frac{2^{|m|+2}}{(2 n + |m|)} 
\frac{\Gamma(n+\alpha+1)\Gamma(n+\beta+1)}{\Gamma(n)\Gamma(n+|m|+1)}\right) \label{eq.N1}\\
&= \frac{4\mathcal{N}^2}{2n+|m|}\left(\frac{\Gamma(n+\alpha+1)\Gamma(n+\beta+1)}{\Gamma(n+1)\Gamma(n+|m|)}\right) \label{eq.N2}
\end{align}
Where we have used the fact that $\Gamma (n+1) = n\Gamma(n)$ between \eqref{eq.N1} and \eqref{eq.N2}. Thus our normalisation coefficient , for $\alpha, \ \beta > -1$ is \begin{equation}
    \mathcal{N}= \frac{\pm \sqrt{2n+|m|}}{2\sqrt{2\pi}}\left(\frac{\Gamma(n+1)\Gamma(n+|m|)}{\Gamma(n+\alpha+1)\Gamma(n+\beta+1)}\right)^\frac{1}{2}
\end{equation}
For the case where $\alpha < -1$ and $\beta >-1$ we need only modify the integrand above
\begin{align*}
&= \frac{\mathcal{N}^2}{2^{\alpha +\beta}} \int_{-1}^1  (1-y)^\alpha (1+y)^\beta \left(P^{(\alpha,\beta)}_n(y)\right)^2 +  (1-y)^{\alpha+1} (1+y)^{\beta+1}\left(\frac{n+|m|}{4n}\right) \left(P^{(\alpha+1,\beta+1)}_{n-1}(y)\right)^2 \ dy \\
\intertext{Using the definitions in appendix B of \cite{Wu+Yang}}
&= \frac{\mathcal{N}^2}{2^{\alpha +\beta}} \int_{-1}^1  (1-y)^\alpha (1+y)^\beta \left(2^{\alpha} (y-1)^{-\alpha}C_{1}P^{(-\alpha,\beta)}_{n+\alpha}(y)\right)^2 \\ 
&~+~ (1-y)^{\alpha+1} (1+y)^{\beta+1}\left(\frac{n+|m|}{4n}\right) \left(2^{\alpha+1} (y-1)^{-(\alpha+1)}C_{2}P^{(-(\alpha+1),\beta+1)}_{n+\alpha}(y)\right)^2 \ dy \\
&= \frac{\mathcal{N}^2}{2^{-\alpha +\beta}} \int_{-1}^1  (1-y)^{-\alpha} (1+y)^\beta C_{1}^{2}\left(P^{(-\alpha,\beta)}_{n+\alpha}(y)\right)^2 \\  
& ~+~ (1-y)^{-(\alpha+1)} (1+y)^{\beta+1}\left(\frac{n+|m|}{n}\right)C_{2}^{2} \left(P^{(-(\alpha+1),\beta+1)}_{n+\alpha}(y)\right)^2 \ dy \\
\intertext{Where $C_1$ and $C_2$ are the constants dependent on $\alpha$ and $\beta$ from appendix B of \cite{Wu+Yang}. The relation between $C_1$ and $C_2$ is}
&C_{2} = \frac{n}{n+\alpha+\beta+1}C_1 = \frac{n}{n+|m|}C_1\\
\intertext{combining this with the orthogonality condition above gives}
&= \frac{\mathcal{N}^2}{2^{-\alpha +\beta}} {C_{1}^{2}} \left(\frac{2^{-\alpha +\beta+1}}{(2 n + |m|)} 
\frac{\Gamma(n+1)\Gamma(n+|m|)}{\Gamma(n+\alpha+1)\Gamma(n+\beta + 1)} +  \frac{2^{-\alpha +\beta+1}}{(2 n + |m|)}\frac{n}{(n+|m|)}
\frac{\Gamma(n)\Gamma(n+|m|+1)}{\Gamma(n+\alpha + 1)\Gamma(n+\beta+1)}\right) \\
&= \frac{4\mathcal{N}^2}{2n+|m|}\left(\frac{\Gamma(n+\alpha+1)\Gamma(n+\beta+1)}{\Gamma(n+1)\Gamma(n+|m|)}\right)^{2} \frac{\Gamma(n+1)\Gamma(n+|m|)}{\Gamma(n+\alpha+1)\Gamma(n+\beta + 1)} \label{eq.N2}
\end{align*}
Again using the fact that $\Gamma (n+1) = n\Gamma(n)$ and that $C_1$ is the gamma function part of the orthogonality relation. Our normalisation coefficient is the same as the case for $\alpha>-1$ \begin{equation}
    \mathcal{N}= \frac{\pm \sqrt{2n+|m|}}{2\sqrt{2\pi}}\left(\frac{\Gamma(n+1)\Gamma(n+|m|)}{\Gamma(n+\alpha+1)\Gamma(n+\beta+1)}\right)^\frac{1}{2}
\end{equation}
The case in which $\beta < -1$ and $\alpha$ and  $\beta < -1$ is nearly identical to the above process, and we recover the same normalisation.  


As a concrete example consider $n=1$ with $m<0$.  We first write Rodrigues' formula (\ref{eq:Rodrigues-P}) in terms of $u$, with $y=\frac{1-x}{1+x}=1-2u$, 
\[P_n^{(\alpha,\beta)}(1-2u)  = \frac{1}{n!} u^{-\alpha} (1-u)^{-\beta} \frac{d^n}{d u^n}
\Bigl\{ u^{n+\alpha} (1-u)^{(n+\beta)} \Bigr\}.\]
In particular for $n=1$
\[ P_1^{(p,|m|-1-p)}(y)= \frac{p+1 - (|m|-p) x}{1+x},\qquad p=0,\ldots,|m|-1.\]
Including the other two states (\ref{eq:-phi_1-1}) and (\ref{eq:-phi_1-3}), with $p=|m|$ and $\bar p = 1$, the most
general $n=1$ positive chirality state is
\begin{align} \phi_1(z) &= 
\left(\frac{1}{1+\bar z z}\right)^{\frac{|m|+1}{2}} \left\{ 
 a_{\bar 1} \bar z + \sum_{p=0}^{|m|} \left(\frac{p+1 -(|m|-p) x}{|m|+1} \right)
 a_p z^p\right\}\\
&= 
\left(\frac{1}{1+\bar z z}\right)^{\frac{|m|+1}{2}} \sum_{p=-1}^{|m|} \left(\frac{p+1 -(|m|-p) x}{|m|+1} \right)
 a_p z^p\\
&= \left(\frac{1}{1+\bar z z}\right)^{\frac{|m|+1}{2}} 
 \left(
a_{\bar 1} \bar z +  \sum_{p=0}^{|m|} a_p z^p\right)
-\left(\frac{1}{1+\bar z z}\right)^{\frac{|m|-1}{2}}  
\sum_{p=0}^{|m|-1} \left(\frac{|m|-p}{|m|+1}\right) a_p   z^p, \label{eq:phi1_n=1a}
 \end{align}
where $a_{-1}=-a_{\bar 1}$ in (\ref{eq:phi1_n=1a}).  

 The second term on the right hand side of (\ref{eq:phi1_n=1a}) is of precisely the same form as the
 zero mode $n=0$ state and is therefore annihilated by the Dirac operator. 
Using this it is easy to check that $i(1+z \bar z) D_z \phi_1 = \sqrt{|m|+1}\, \phi_2$ implies
\[ \phi_2(z) = -\frac{i}{\sqrt{|m|+1}} \left(\frac{1}{1+\bar z z}\right)^{\frac{|m|+1}{2}}
\sum_{s=0}^{|m|+1} a_{s-1} z^s,\]
the structure of which is of course compatible with (\ref{eq:-phi_2-1}) -- (\ref{eq:-phi_2-3}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Relation to scalar wave-functions}

Our Dirac eigenspinors (\ref{eq:phi_1+})-(\ref{eq:-phi_2-}) are simply related to the scalar eigenfunctions (strictly cross-sections of a $U(1)$ bundle) in equation (28) of reference \cite{Wu+Yang},  
\[ \phi_0 =  e^{-i\bar s \phi} u^{\frac{\bar s}{2}}(1-u)^{\frac{m-\bar s}{2}} P^{(\bar s,m-\bar s)}_n (1-2u),\qquad -n \le \bar s \le n+m,\]
which is $\phi_2$ above for $m>0$, with $m-1$ replaced by $m$, equivalent to
throwing away the contribution from the spin connection in $D_{\bar z}$.\footnote{To relate this to the notation in \cite{Wu+Yang} use (\ref{eq:P-beta}) to write
\[e^{-i\bar s \phi} u^{\frac{\bar s}{2}}(1-u)^{\frac{m-\bar s}{2}} P^{(\bar s,m-\bar s)}_n  \propto  e^{-i\bar s \phi} u^{\frac{\bar s}{2}}(1-u)^{\frac{\bar s-m}{2}} P^{(\bar s,\bar s-m)}_{n-\bar s +m}
= e^{i(\bm q + \bm m)\phi} u^{-\frac{\bm{q}+ \bm {m}}{2}} (1-u)^{\frac{\bm{q} - \bm{m}}{2}} 
P^{(-\bm q - \bm m , \bm q - \bm m)}_{\bm n},\]
where boldface letters represent the notation in \cite{Wu+Yang}:
\[
\bm q  = -\frac{m}{2},\qquad \bm m  = \frac{m}{2} - \bar s,\qquad
\bm n  = n -\bar s + m, \qquad \bm l = n + \frac {m}{2}, \qquad
\bm m = -\bm l,-\bm l + 1,\ldots,\bm l - 1,\bm l.\]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Relation to Wigner $D$-matrices}

              The Jacobi polynomials $P_K^{(\alpha,\beta)}$ are related to Wigner $D$-matrices for $SU(2)$,%\cite{WignerDmatrix}
\footnote{https://en.wikipedia.org/wiki/Wigner\_D-matrix.}
              \begin{equation}
                D^J_{M',M}(\theta,\psi,\phi)=e^{- i M' \psi}d^J_{M',M}(\theta) e^{-i M \phi},\label{eq:DJM}\end{equation}
              as follows: let \[ K= \min \{J\pm M, J\pm M' \},\]
then 
\begin{equation} \hbox{if}\ K = \begin{cases}
    J+M, \quad \alpha= M'-M, & i)\\
    J-M, \quad \alpha= M-M',  & ii) \\
    J+M', \quad \alpha= M-M', & iii)\\
    J-M', \quad \alpha= M'-M,  & iv)\\
  \end{cases}\label{eq:dJM}\end{equation}
and $\beta + \alpha = 2 J - 2 K$, then
\begin{align*} d^J_{M',M}(\theta) &={\cal N}\left( \sin \frac \theta 2 \right)^\alpha
\kern -5pt    \left( \cos \frac \theta 2 \right)^\beta \kern -5pt P_K^{(\alpha,\beta)}(\cos\theta)\\
&={\cal N}u^{\frac{\alpha}{2}}(1-u)^{\frac{\beta}{2}} P_K^{(\alpha,\beta)}(1-2u)
\end{align*}
where 
\begin{equation*}
{\cal N}= (-1)^\eta {2 J -K \choose K+\alpha}^{\frac 1 2} {K+\beta \choose \beta}^{-\frac 1 2}
\end{equation*}
is a normalisation ($\eta$ gives is a case dependent sign).\footnote{\[\eta=\begin{cases} 
M'-M & \hbox{in} \ (i)\ \&\ (iv) \\ 0 & \hbox{in} \ (ii)\ \& \ (iii). \end{cases}\]} Applying this to (\ref{eq:phi_1-1})-(\ref{eq:-phi_2-3}) we see that in every case
\begin{equation}
   J=n + \frac{|m|-1}{2} \label{j.1} 
\end{equation} 
and the Dirac operator has eigenvalue squared
\[ \lambda^2 = J(J+1) - \frac{(m^2-1)}{4} =\frac{1}{4}  \bigl\{(2 J+1)^2 - m^2\bigr\},\]
as expected from \cite{Dolan}.

                For (\ref{eq:phi_1-1}) - (\ref{eq:phi_1-3}) and (\ref{eq:-phi_1-1}) - (\ref{eq:-phi_1-3})  there is a choice of $i) - iv)$ in (\ref{eq:dJM}) that sets $M=\frac{m+1}{2}$ in $\phi_1$, namely
\begin{itemize}
\item $m>0$:                \begin{align*}
                  (\ref{eq:phi_1-1}) \quad iv) \qquad & \Rightarrow \qquad M=\frac{m+1}{2}, \quad M' = p +\frac{m+1}{2}, \quad & 0\le p \le n-1,\\
                  (\ref{eq:phi_1-2})\ \quad ii) \qquad & \Rightarrow \qquad M=\frac{m+1}{2}, \quad M' = -\bar p +\frac{m+1}{2}, \quad & 1\le p \le m,\\
                  (\ref{eq:phi_1-3}) \quad iii) \qquad & \Rightarrow \qquad M=\frac{m+1}{2}, \quad M' = - \bar p +\frac{m+1}{2}, \quad & m+1\le p \le m+n,\\
\end{align*}
\item $m<0$:
\begin{align*}
                  (\ref{eq:-phi_1-1}) \quad iv) \qquad & \Rightarrow \qquad M=\frac{m+1}{2}, \quad M' = p +\frac{m+1}{2}, \quad & |m| \le  p \le |m|+n-1,\\
                  (\ref{eq:-phi_1-2})\ \quad i) \qquad & \Rightarrow \qquad M=\frac{m+1}{2}, \quad M' = p +\frac{m+1}{2}, \quad & 0\le p \le |m|-1,\\
                  (\ref{eq:-phi_1-3}) \quad iii) \qquad & \Rightarrow \qquad M=\frac{m+1}{2}, \quad M' = - \bar p +\frac{m+1}{2}, & \quad  1\le \bar p \le n.\\
\end{align*}
\end{itemize}
If we choose $\psi = -\phi$ in (\ref{eq:DJM}) we have
\[D^J_{M',M}(\theta,-\phi,\phi)=e^{i (M'-M) \phi}d^J_{M',M}(\theta),\]
and in all the cases listed above $-J \le M' \le J$ with $J= n+\frac{m-1}{2}$.
In addition $M'-M =p$ or $-\bar p$ giving just the right power of $e^{i\phi}$ for us to conclude
that, for either sign of $m$, the complete set of $\phi_1$ eigenspinors is precisely equivalent to
the $M=\frac{m+1}{2}$ column of $D^J_{M',M}(\theta,-\phi,\phi)$.

For $\phi_2$ a parallel analysis yields
\begin{itemize} 
\item $m>0$:
 \begin{align*}
                  (\ref{eq:phi_2-1}) \quad iv) \qquad & \Rightarrow \qquad M=\frac{m-1}{2}, \quad M' = s +\frac{m-1}{2}, \quad & 1\le s \le n\\
                  (\ref{eq:phi_2-2})\ \quad ii) \qquad & \Rightarrow \qquad M=\frac{m-1}{2}, \quad M' = -\bar s +\frac{m-1}{2}, \quad & 0\le \bar s \le m-1,\\
                  (\ref{eq:phi_2-3}) \quad iii) \qquad & \Rightarrow \qquad M=\frac{m-1}{2}, \quad M' = - \bar s +\frac{m-1}{2}, \quad & m\le \bar s \le m+n-1,\\
\end{align*}
\item $m<0$:
\begin{align*}
                  (\ref{eq:-phi_2-1}) \quad iv) \qquad & \Rightarrow \qquad M=\frac{m-1}{2}, \quad M' = s +\frac{m+1}{2}, \quad & |m|+1 \le  s \le |m|+n,\\
                  (\ref{eq:-phi_2-2})\ \quad i) \qquad & \Rightarrow \qquad M=\frac{m-1}{2}, \quad M' = s +\frac{m+1}{2}, \quad & 1\le s \le |m|,\\
                  (\ref{eq:-phi_2-3}) \quad iii) \qquad & \Rightarrow \qquad M=\frac{m-1}{2}, \quad M' = - \bar s +\frac{m+1}{2}, & \quad  0\le \bar s \le n-1.\\
\end{align*}
\end{itemize}
Again the choice $\psi = -\phi$ in (\ref{eq:DJM}) gives
\[D^J_{M',M}(\theta,-\phi,\phi)=e^{i (M'-M) \phi}d^J_{M',M}(\theta),\]
and in all the cases listed above $-J \le M' \le J$ with $J= n+\frac{|m|-1}{2}$.
In addition $M'-M =s$ or $-\bar s$ again giving just the right power of $e^{i\phi}$ for us to conclude
that, for either sign of $m$, the complete set of $\phi_2$ eigenspinors is precisely equivalent to
the $M=\frac{m-1}{2}$ column of $D^J_{M',M}(\theta,-\phi,\phi)$.
 
This is a consequence of the Harish-Chandra theorem for harmonic analysis on symmetric spaces.

In conclusion the eigenspinors for Landau level $n$, with degeneracy $d_n=|m|+2n$
and  $\lambda^2 = n(n+|m|)$,  are obtained by setting 
\[ J= n +\frac{|m|-1}{2}, \qquad M=\frac{m\pm 1}{2}, \qquad M'=k-n-\frac{|m|+1}{2},\qquad l=M' -M\]
in
\[ \phi^J_{\pm,k}(z) = e^{i l \phi} d^J_{l+\frac{m}{2}\pm \frac{1}{2},\frac{m}{2}\pm \frac{1}{2}}(\theta),\]
with $k=1,\cdots,d_n$ and the upper (lower) sign for $\phi_1$ ($\phi_2$).
The range of $l$ is
\[ l=\begin{cases}
-n-m, \ldots, n-1, & m>0, \qquad \phi_1;\\
-n-m+1, \ldots, n, & m>0,  \qquad \phi_2;\\
-n, \ldots, n+|m|-1, & m<0,  \qquad \phi_1;\\
-n+1, \ldots, n+|m|, & m<0,  \qquad \phi_2.\\
\end{cases}\]

We can focus on one spin by adding an extra Zeeman splitting, over and above that contained in the Dirac operator itself.
To focus on the positive chirality component, $\phi_1$, add

\[ H_Z =  \mu B (\bm 1 - \sigma_3) = \frac{\mu |m|}{2 \pi}  (\bm 1 - \sigma_3)\] 
to the Hamiltonian (\ref{eq:Hamiltonian}).
When the magnetic moment  $\mu>0$ is large, all negative chirality modes are pushed to high energy and the positive chirality modes are unaffected.   

We can now write down the wave function for $N$ spin-split particles filling Landau level $n$ when $m<0$.
The degeneracy of Landau level $\widetilde n$, with $0\le \widetilde n \le n$, is  
\[\widetilde d=|m| + 2\widetilde n\]      
and the total number of particles is
\[N= |m| + (|m|+2) + \cdots + (|m| + 2n) = (n+1)(|m|+n). \]                 
The total number of particles filling all the Landau levels up to, but not including,  $\widetilde n$
is 
\[ \widetilde s =\sum_{\widetilde n'=0}^{\widetilde n-1}=\widetilde n(|m|+\widetilde n-1).\]
The state filling Landau level $\widetilde n$ is                 
\[ \Phi_+^{\widetilde n}(z_{\widetilde s+1},\ldots,z_{\widetilde s + \widetilde n})
=\phi_{+,1}^{\widetilde J}(z_{\widetilde s+i_1}) \cdots 
\phi_{+,\widetilde n}^{\widetilde J}(z_{\widetilde s + i_{\widetilde n}}) 
\epsilon^{i_1 \cdots i_{\widetilde n}},\]
with $\widetilde J = \widetilde n+\frac{|m|-1}{2}$

The total wave function is then
\[ \Psi_+
(z_1,\cdots,z_N)=\prod_{\widetilde n=0}^n \Phi_+^{\widetilde n}.\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Fractional filling fractions}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In Jain's composite fermion picture there are vortex fluxes of statistical gauge field $a$ attached to the charge carriers.
The spectrum of the Dirac operator can be determined when there are magnetic vortices threading through the surface of the sphere in addition to a monopole at the centre. A vortex of strength $v$ at the N-pole, with flux $2\pi v$ out of the sphere, is described by a magnetic potential
\begin{equation}
a=-\frac{i v}{2} \left[ \frac{d z}{z} 
- \frac{d \bar z}{\bar z}\right].\label{eq:vortex-N}
\end{equation}
Then $d a=0$ provided $z\ne 0$ but, if we isolate the N-pole by surrounding it by a small circle $S^1_\epsilon$ of radius $\epsilon$ 
centred on $z=0$, 
\begin{equation}
\int_{S^1_\epsilon} a =
- \frac{i v}{2}\int_{S^1_\epsilon} \frac{d z}{ z} 
+ \frac{i v}{2}\int_{S^1_\epsilon} \frac{d \bar z}{\bar z}
=   \pi  v  - \pi (- v)= 2\pi v.\label{eq:vortex-S1}
\end{equation}

However this potential also gives an anti-vortex, of strength $-v$, at the S pole:
the anti-podal point is given by $z \rightarrow \frac{1}{\bar z}$, which sends $a\rightarrow -a$. This is perhaps clearer using polar co-ordinates, $(\theta,\phi)$, 
in which 
\[ a = v d \phi\]
which represents an infinite straight flux tube in 3-dimensions, threading through both the N-pole and the S-pole of the sphere.  The total flux through the sphere is zero.

We can move the position of the vortex through the N-pole around by using
\begin{equation}
a=-\frac{i v}{2} \left[ \frac{d z}{(z-z_0)} 
- \frac{d \bar z}{(\bar z - \bar z_0)}\right],\label{eq:vortex-A}
\end{equation}
representing a vortex of strength $v$ through the point $z_0$, but there is still
an anti-vortex through the S-pole for any finite $z_0$.

We can remove the vortex at the S-pole using the potential due to a semi-infinite solenoid threading the S pole and terminating at the centre of the sphere
\begin{equation}
a=-\frac{i v}{2} \left[ \frac{d z}{(z-z_0)} 
- \frac{d \bar z}{(\bar z - \bar z_0)}\right] 
-\frac{i v}{2}\left(\frac{z d \bar z - \bar z d z}{1+z \bar z}\right).\label{eq:solenoid}
\end{equation}
This vanishes at the S-pole. What this does is remove the vortex of strength $-2 \pi v$ at the S-pole replace it with a constant flux $-\frac{v}{2}$ over the whole surface of the sphere.

If there are $N-1$ vortices all of the same strength $v$ positioned at $z_i$ then these can be represented by $(N-1)$ semi-infinite solenoids terminating at the centre of the sphere plus a constant flux:
\begin{equation}a=-\frac{i v}{2} \sum_{i=1}^{N-1}\left( \frac{d z }{z-z_i}
-  \frac{d \bar z}{\bar z-\bar z_i}\right)
-\frac{i (N-1) v}{2}\left(\frac{z d \bar z - \bar z d z}{1+z \bar z}\right).\label{eq:a}
\end{equation}
The corresponding field strength is
\[ f = d a =i\left( 2 \pi v \sum_{i=1}^{N-1}\delta(z-z_i) -
\frac{(N-1)v}{(1 + z \bar z)^2} \right)  dz \wedge \bar dz\]
and
\[ \int_{S^2} f =0.\]

  Omitting the self-energy of a composite fermions with its own vortex, and assuming all the vortices have the same strength $v_i=v$, the Dirac operator in (\ref{eq:Dirac0}) then involves covariant derivatives
\begin{align}
D_z & = \partial_z
+ \frac v 2 \sum_{j=1}^{N-1}\frac{1}{z - z_j}
+ \frac{(\widetilde m +\sigma_3)}{2} \frac{\bar z}{1+z \bar z }
,\label{eq:Dzv}\\
    D_{\bar z} 
& = \partial_{\bar z}
- \frac v 2 \sum_{j=1}^{N-1}\frac{1}{\bar z - \bar z_j}
- \frac{(\widetilde m+\sigma_3)}{2} \frac{ z}{1+z \bar z },\label{eq:Dbarzv}
\end{align}
where $\widetilde m = m -(N-1)v$.


Except at the vortices the spinor Lie derivatives corresponding to angular momentum (\ref{eq:J-def}) are modified to
\begin{align}
 {\bm J}_+   & = z^2 \partial_z + \partial_{\bar z} + 
\frac v 2 \sum_{j=1}^{N-1} \left( \frac{z^2}{z - z_j}  +  \frac{1}{\bar z - \bar z_j}\right)
        +\frac{(\widetilde m+ \sigma_3)z}{2}
        \nonumber \\
 {\bm J}_-   & = -{\bar z}^2 \partial_{\bar z} - \partial_z + \frac v 2 \sum_{j=1}^{N-1}\left( \frac{\bar z^2}{\bar z - \bar z_j}  +  \frac{1}{z - z_j}\right)
 + \frac{(\widetilde m + \sigma_3) \bar z}{2} \label{eq:J-def-vortices} \\  
{\bm J}_3  &= z \partial_z - \bar z \partial_{\bar z}+
 \frac v 2 \sum_{j=1}^{N-1}\left( \frac{z}{z - z_j}  +  \frac{\bar z}{\bar z - \bar z_j}\right)       
+ \frac{(\widetilde m +\sigma_3)}{2}.
        \nonumber
\end{align} 
From (\ref{eq:JJB}) we know that these will close at any point on the sphere where $B$ is radial and uniform, that is the algebra
closes at all points away from the vortices, but not at the vortices themselves. Thus the algebra is well defined and closes on the
sphere with $N-1$ points removed.

We still have
We find
\[
[{\bm J}_3, D_z]=-D_z,\qquad  [{\bm J}_3, D_{\bar z}]=D_{\bar z} \]
from which
\[ [{\bm J}_3,\Dslash]=0.\]
{\bf I haven't checked $ [{\bm J}^2,\Dslash] =?$}

The composite fermion scenario requires that the vortices partially cancel the background gauge field: if $m$ is positive $v$ is negative and vice versa.  Thus paradoxically we see from the third terms on the right hand side of (\ref{eq:Dzv}) and (\ref{eq:Dbarzv}) that the uniform part of the statistical gauge field actually has the apparent effect of enhancing the background field.

The the background gauge field and the uniform part of the statistical gauge field appear on an equal footing in the Dirac operator, they cannot be picked apart in the co-variant derivatives (\ref{eq:Dzv}) and (\ref{eq:Dbarzv}).\footnote{They do however have different gauge transformation properties: $m$ transforms according to (\ref{eq:A+A-}), it is a Wu-Yang monopole, while $v$ is global and does not change between the two hemispheres, it is a Dirac monopole with a string.
The charge $\widetilde m$ is partly Wu-Yang monopole and partly Dirac. But this is not evident on any single co-ordinate patch.}

Defining $\widetilde m = m - (N-1) v$ we can interpret the whole magnetic field as arising from a uniform background magnetic field of charge $\widetilde m$, with $|\widetilde m| > |m|$,  and $N-1$ vortices at the points $z_i$. 
The Atiyah-Singer index theorem now tells us to expect
\[n_+ - n_- = -\frac{1}{2\pi} \int_{S^2} (F + f) = -m=-\widetilde m -(N-1)v.\]

The zero modes of $D_z$, with $m>0$, can have the general form
\[ \chi_- = 
\frac{\bar z^{\bar s}}{(1+ z \bar z)^{\frac{m-1-(N-1) v}{2}}} 
\prod_{i=1}^{N-1} \frac{ (z-z_i)^{-\frac{v}{2}}}{(\bar z-\bar z_i)^{\bar l}}\]
(there are no positive chirality zero modes which are regular when $m>0$).
$\bar s$ and $\bar l$ are not independent in the above expression, we could take linear combinations of zero modes with this form, using $\bar z_i$ dependent co-efficients, to give factors of $(\bar z - \bar z_i)$ in the numerator which could cancel powers of $\bar l$ in the denominator. 
We can remove this redundancy choosing states that are eigenspinors of ${\bm J}_3$:
\[ {\bm J}_3 \chi_- = \left(-\bar s - \frac v 2 \sum_{i=1}^{N-1} \frac{z}{z-z_i} 
+ \bar l \sum_{i=1}^{N-1} \frac{\bar z}{\bar z -\bar z_i}  
+ \frac{v}{2} \sum_{i=1}^{N-1} \left( \frac{z}{z-z_i}+\frac{\bar z}{\bar z - \bar z_i}\right) 
+\frac{\widetilde m -1}{2} \right) \chi_.\]
Thus $\chi_-$ is an eigenspinor of ${\bm J}_3$ if and only if $\bar l = - \frac v 2$, so
\[ \chi_- = 
\frac{\bar z^{\bar s}}{(1+ z \bar z)^{\frac{m-1-(N-1) v}{2}}} 
\prod_{i=1}^{N-1}  |z-z_i|^{- v}.\]

To avoid branch cuts and singularities at $z=0$ we must have ${\bar s}\ge 0$.
To avoid branch cuts and singularities at $z=z_i$ we assume $v$ is an even integer
(which is negative $v=-2k$ when $m$ is positive) and $k - {\bar l} \ge 0$.
For finiteness as $|z|\rightarrow \infty$, 
\[\bar s + 2 (N-1) \le m-1 + 2 (N-1)k,\]
so
\[ 0 \le \bar s \le m-1= \widetilde m - 2k(N-1)-1,\]
giving $m=\widetilde m - 2k(N-1)$ linearly independent zero modes, as required by the index theorem. 
Thus
\[ \chi_- = 
\frac{\bar z^{\bar s}}{(1+ z \bar z)^{\frac{\widetilde m-1}{2}} }
\prod_{i=1}^{N-1} |z-z_i|^{2k}.\]


If we have $N$ composite fermions at points $z_i$ with $i=1,\ldots,N$ the most  general zero mode for positive $m$ is
\[  \chi_-(z_i) = \frac{ \prod_{i < j} |z_i - z_j|^{2  k}}{\prod_{i-1}^N(1+z_i \bar z_i)^{\frac {\widetilde m - 1} 2}}\left( \sum_{\bar s_1,\ldots,\bar s_N=0}^{\widetilde m-1- 2 k (N-1)} a_{\bar s_1,\cdots,\bar s_N}\bar z_1^{\bar s_1} \cdots \bar z_N^{\bar s_N}\right).\]
Then for $\chi_-$ to be anti-symmetric in its arguments, $a_{\bar s_1,\ldots,\bar s_N}$ must be
anti-symmetric in its indices.  The ground state is then unique
if an only if $k$ is a positive integer and $a_{\bar s_1 \cdots \bar s_N}$ is the 
$\widetilde m - 2 k(N-1)$ dimensional
$\epsilon$-tensor, which requires
\[N = \widetilde m - 2 k(N-1) =m\qquad \Leftrightarrow \qquad
  \widetilde m = (2 k+1) N - 2k.\]
We are led to  the unique ground state
\begin{equation} \chi_-(z_1,\ldots,z_n) =  \prod_{i=1}^N\frac{1}{(1+|z_i|^2)^{\frac {\widetilde m - 1} 2}}  \prod_{i <  j}(\bar z_i - \bar z_j )
  |z_i - z_j|^{2 k}
\label{eq:Laughlin-}\end{equation}
with an energy gap $\sim 1/M$.

Interpreting the uniform field as arising from a charge $\widetilde m$ the filling factor is then
\[ \frac{N}{\widetilde m} = \frac{N}{(2 k +1) N -2k}
  \qquad \mathop{\longrightarrow}_{N \rightarrow \infty} \qquad
  \frac{1}{2 k+1}\]

A similar analysis with $m<0$ requires $v=2k>0$ and $\widetilde m = m -2(N-1)k <0$.  There is a unique positive chirality zero mode when  $|\widetilde m| = (2 k+1) N - 2k$,
\begin{equation} \chi_+(z_1,\ldots,z_n) =  \prod_{i=1}^N\frac{1}{(1+|z_i|^2)^{\frac {|\widetilde m| - 1} 2}}  \prod_{i <  j}(z_i - z_j )
  |\bar z_i - \bar z_j|^{2 k}.\label{eq:Laughlin+}\end{equation}

To relate (\ref{eq:Laughlin+}) to the Laughlin ground state wave-function we write, for $m<0$ and $v= 2k>0$, 
\[ \chi_+(z_1,\ldots,z_n) =  \prod_{i=1}^N\frac{1}{(1+|z_i|^2)^{\frac {|\widetilde m| - 1} 2}}  \prod_{i <  j}(z_i - z_j )^{2 k+1}
  \left(\frac {\bar z_i - \bar z_j}{z_i - z_j}\right)^k.\]
The last factor
\[  \prod_{i <  j}\left(\frac {\bar z_i - \bar z_j}{z_i - z_j}\right)^k
  = \exp\left({k \sum_{i<j} \Bigl\{ \log(\bar z_i - \bar z_j ) -  \log(z_i - z_j )\Bigr\}}\right)\]
is a phase and can be removed by the singular gauge transformation
\[ a \rightarrow a' = a -i 
  k \sum_{i<j} \left(
    \frac{1}{\bar z_i - \bar z_j } -  \frac{1}{z_i - z_j }\right).\]
Comparing with (\ref{eq:a}) we see that the vortices have been completely gauged away.
In this gauge
\[ \chi_+(z_1,\ldots,z_n) =  \prod_{i=1}^N\frac{1}{(1+|z_i|^2)^{\frac {|\widetilde m| - 1} 2}}  \prod_{i <  j}(z_i - z_j )^{2 k+1},\]
which is the Laughlin wave function, up to the factor
$\prod_{i=1}^N\left(\frac{1}{1+|z_i|^2}\right)^{\frac {|\widetilde m| - 1} 2}$
which on the sphere is analogous to the factor 
$\prod_{i=1}^N e^{- |z_i|^2/4 l_B^2}$,
with $\frac{1}{4 l_B^2} = \frac{1}{2}\left(\frac{e B}{2 \hbar c}\right)$,
on the plane. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Dirac operator on the plane}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

On the flat 2-dimensional plane with complex co-ordinate $z=\frac{1}{\sqrt{2}} (x+i y)$
and constant perpendicular magnetic field we use
\[  A= \frac{i B}{2} (z d \bar z - \bar z dz) \ \Rightarrow \ F=d A = i B\, (dz \wedge \bar d z) = B\, (d x \wedge d y).\]

The Dirac operator is
\begin{equation} 
i\Dslash   = i(\sigma_+ D_z + \sigma_- D_{\bar z} \bigr) 
= i \begin{pmatrix}
0 & \partial_{z} - b \bar z  \\ 
\partial_{\bar{z}} +b z & 0
\end{pmatrix}.\label{eq:Dirac-Plane}
\end{equation}
where $b=\frac{ e B}{\hbar} = \frac{1}{l_B^2}$ with $l_B$ is the magnetic length.
The square is
\[(i\Dslash)^2 = \left( 
-\partial_z \partial_{\bar z} -\frac{b}{2}L_3
 + \frac{b^2}{4} \bar z z\right) - \frac{b}{2} \sigma_3 ,\] 
Eigenspinors 
\[ \psi = \begin{pmatrix} 
\phi_+ \\ \phi_- 
\end{pmatrix} \]
satisfy
\[ \left(
\partial_z \partial_{\bar z} +\frac{b}{2}(z\partial_z - \bar z \partial_{\bar z})
\pm \frac{b}{2} - \frac{b^2}{4} \bar z z\right)\phi_\pm = -\lambda^2 \phi_\pm \]
and are given in \cite{Jellaletal} in terms of associated Laguerre polynomials $L_n^{(\alpha)}(y)$. 
We have
\[
[D_z, D_{\bar z}] = 2b, \qquad [L_3,D_z]=-D_z, \qquad [L_3,D_{\bar z}]=D_{\bar z}, \qquad [L_3,\Dslash^2]=0, \qquad [L_3,\Dslash]=-\sigma_3 \Dslash.
\]

Eigenspinors can be constructed using either of the forms
\begin{align*} 
\phi_\pm = z^{p_\pm} f_{\pm}(x)  \qquad &\qquad   \qquad  \qquad \hbox{(1)} \\
\phi_\pm = \bar{z}^{\bar p_\pm} g_{\pm}(x) \qquad &  \qquad  \qquad  \qquad  \hbox{(2)}  
\end{align*}
with $x= \bar z z$.

We shall treat these separately, with $b>0$.
\begin{enumerate}

\item With $f'_\pm = \frac{ d f_\pm}{d x}$ we have
\begin{align*}
\partial_z \phi_\pm & = p_\pm  z^{p_\pm -1} f_{\pm} + z^{p_\pm} \bar z f'_\pm
=z^{p_\pm -1} ( p_\pm f_\pm + x f'_\pm)\\
\partial_{\bar z} \partial_z \phi_\pm & 
=z^{p_\pm} \bigl\{x f''_\pm +(p_\pm+1)f'_\pm\bigr\}\\
\end{align*}
and
\[ (z \partial_z - \bar z \partial_{\bar z}) \phi_\pm = p_\pm \phi_\pm\]
giving
\[ x f''_\pm +(p_\pm +1) f'_\pm + \left( \frac{b}{2}(p_\pm \pm 1) - \frac{b^2 x}{4}\right) f_\pm  = -\lambda^2 f_\pm. \]
We get Laguerre's equation by writing $f_\pm = e^{-b \bar z z/2} h_\pm $ leading to
 \[ x h''_\pm +(p_\pm + 1 - b x) h'_\pm  -\frac{b}{2}(1\mp 1)h_\pm = -\lambda^2 h _\pm. \]
In terms of the dimensionless variable $y= b \bar z z$
 \begin{align*} 
y \ddot h_+ + (p_+ + 1 - y) \dot h_+   & = -\widetilde \lambda^2 h _+ \\ 
y \ddot h_- + (p_- + 1 - y) \dot h_-   & = -(\widetilde \lambda^2-1 )h _- 
\end{align*}
where $\dot h_\pm = \frac{d h_\pm}{d y}$ and $\widetilde \lambda^2 = \frac{\lambda^2}{b}$.
These are associated Laguerre equations: the eigenvalues are 
$\widetilde \lambda^2 = n =0,1,2,\ldots$ and  and $h_{\pm} = L_{n_\pm}^{(p_\pm)}(y)$ are associated Laguerre polynomials of order 
$n_\pm$ ($n_+ = n_-+1 =n$).
Obviously $p_\pm=0,1,2,\ldots$ is a non-negative integer for the solution to be regular.

Thus
\[ \phi_+ \propto z^{p_+} e^{-y/2} L_n^{(p_+)}(y), \qquad \phi_- \propto z^{p_-} e^{-y/2} L_{n-1}^{(p_-)}(y).\]
Since $\lambda = \pm \sqrt{b n}$ we have
\[\left(\partial_{\bar z} + \frac{b}{2} z\right) \phi_+ = \mp i \lambda \phi_- = \mp i \sqrt{b n}\, \phi_- \] 
we can take $\phi_+ = z^{p_+} e^{-y/2} L_n^{(p_+)}(y)$ and 
\[ \phi_- = \pm \frac{i}{\sqrt{ b n}}  \left( b z^{p_+ +1} \frac{d L_n^{(p_+)}}{d y}\right)e^{-y/2}. 
\]
Now using the identity (see Wikipedia: https://en.wikipedia.org/wiki/Laguerre\_polynomials)
\[\frac{d L_n^{(\alpha)}} {d y}=- L_{n-1}^{(\alpha+1)}, \]  
for $n\ge 1$, so
\[ \phi_- =  \mp i\sqrt{ \frac b n} z^{p_+ +1} L_{n-1}^{(p_++1)} e^{-y/2}
\]
and $p_ - = p_+ +1$.
Thus, for $n\ge 1$ our un-normalised eigenspinor is 
\begin{equation}
\psi_{n,p} = z^p e^{-y/2}\begin{pmatrix}
L_n^{(p)}(y) \\ \mp i \sqrt{\frac{b}{n}}z L_{n-1}^{(p+1)}(y)
\end{pmatrix} \label{eq:Lzp-spinor}\end{equation}
with eigenvalue $\lambda = \sqrt{b n}$  and $p=0,1,2,\ldots$.
Note that there is no upper bound to $p$, in the infinite flat plane the degeneracy is infinite. 
For $n=0$, $\phi_-=0$ and the zero-mode chiral spinors are $\phi_+= z^p e^{-y/2}$. 

For consistency we should check that
\[\left(\partial_{z} - \frac{b}{2} \bar z\right) \phi_- = -i \lambda \phi_+.\] 
Again ignoring normalisations let 
\[\phi_- = z^{p_-} e^{-y/2} L_{n-1}^{(p_-)}(y).\]
Then
\[ \left(\partial_{z} - \frac{b}{2} \bar z\right) \phi_- = 
z^{p_- - 1} \left\{ (p_- - y)L_{n-1}^{(p_-)}\bigr) -y L_{n-2}^{(p_- +1)}\right\}e^{-y/2}
\]
and the recurrence relation
\[n L_n^{(p-1)} = (p-y)L_{n-1}^{(p)}-y L_{n-2}^{(p+1)} \]
gives 
\[ \left(\partial_{z} - \frac{b}{2} \bar z\right) \phi_- = z^{p_- - 1} n L_n^{(p_--1)} e^{-y/2}
= \mp i \sqrt{b n} \,\phi_+\]
so indeed, with $p_- = p_+ +1$,
 \[ \phi_+ = \pm i \sqrt{\frac{n}{b}} z^{p_+} L_n^{(p_+)} e^{-y/2}, 
\]
is in agreement with (\ref{eq:Lzp-spinor}), up to a constant normalisation.

\item Let $\phi_\pm = \bar z^{\bar p_\pm} g_\pm(x)$. In this case we get
\begin{align*}
 x g''_\pm +(\bar p_\pm +1) g'_\pm - \left( \frac{b}{2}(\bar p_\pm \mp 1) + \frac{b^2}{4}\right) g_\pm  = -\lambda^2 g_\pm. \end{align*}
Again let $g_\pm = e^{-b \bar z z/2} h_\pm $ leading to
 \begin{align*} 
y \ddot h_+ + (\bar p_+ + 1 - y) \dot h_+ & = -(\widetilde \lambda^2-\bar p_+) h _+ \\ 
y \ddot h_- + (\bar p_- + 1 - y) \dot h_-   & = -(\widetilde \lambda^2-\bar p_--1 )h _-.
\end{align*}

Thus
\[ \phi_+ \propto z^{\bar p_+} e^{-y/2} L_{n_+}^{(\bar p_+)}(y), 
\qquad \phi_- \propto z^{\bar p_-} e^{-y/2} L_{n_-}^{(\bar p_-)}(y)\]
with $n_+ = n - \bar p_+$ and $n_- = n  -\bar p_- -1$.

We have
\[\left(\partial_{\bar z} + \frac{b}{2} z\right) \phi_+ = - i \lambda \phi_- = \mp i \sqrt{b n}\, \phi_- \] 
we can take $\phi_+ = z^{\bar p_+} e^{-y/2} L_{n_+}^{(\bar p_+)}(y)$ and
\begin{align*}
 \phi_- & = \pm \frac{i \bar z^{\bar p_+-1}}{\sqrt{ b n}}  \left(\bar p_+ L_{n_+}^{(\bar p_+)} +y \frac{d L_{n_+}^{(\bar p_+)}}{d y}\right)e^{-y/2}\\
 & = \pm \frac{i \bar z^{\bar p_+-1}}{\sqrt{ b n}}  \left(\bar p_+ L_{n_+}^{(\bar p_+)}  - y L_{n_+-1 }^{(\bar p_++1)} \right)e^{-y/2}. 
\end{align*}
Now using the identity (Abramowitz and Stegun 22.7.31)
\[y L_{n_+-1}^{(\bar p_+ +1)} = (n_++\bar p_+) L_{n_+-1}^{(\bar p_+)}  - n_+ L_{n_+}^{(\bar p_+)} \]  
gives
\begin{align*}
 \phi_- & = \pm \frac{i z^{\bar p_+ - 1}}{\sqrt{ b n}} (n_+ +\bar p_+)\bigl(L_{n_+}^{(\bar p_+)}-  L_{n_+-1}^{(\bar p_+)} \bigr)e^{-y/2}\\
&=\pm \frac{i z^{\bar p_+ - 1}}{\sqrt{ b n}} (n_+ +\bar p_+) L_{n_+}^{(\bar p_+-1)} e^{-y/2} \\
& = \pm i \sqrt{\frac{n}{b}}  z^{\bar p_+ - 1} L_{n_+}^{(\bar p_+-1)} e^{-y/2} \\,
\end{align*}
where we have used Abromowitz and Stegun 22.7.30,
\[  L_{n_+}^{(\bar p_+-1)} = L_{n_+}^{(\bar p_+)}-  L_{n_+-1}^{(\bar p_+)}.\]
Thus, for $n\ge 1$ our un-normalised eigenspinor is, with $\bar p =\bar p_+ = \bar p_- + 1$ and $n_+ = n - \bar p_+$,
\begin{equation}
\psi_{n,\bar p} = \bar z^{\bar p-1} e^{-y/2}\begin{pmatrix}
  \bar z L_{n-\bar p}^{(\bar p)}(y) \\ \pm i \sqrt{\frac{n}{b}} L_{n-\bar p}^{(\bar p-1)}(y)
\end{pmatrix}. \label{eq:Lzpbar-spinor}\end{equation}
Note that the degeneracy of this class of eigenspinors is finite, since 
\hbox{$\bar p \le n$}.

Again we should check 
\[\left(\partial_{z} - \frac{b}{2} \bar z\right) \phi_- = -i \lambda \phi_+\] 
for consistency.
Let 
\[\phi_- = \bar z^{\bar p_-} e^{-y/2} L_{n_-}^{(\bar p_-)}(y).\]
Then
\begin{align*} 
\left(\partial_{z} - \frac{b}{2} \bar z\right) \phi_- & = 
b \bar z^{\bar p_- + 1} \left( -L_{n_-}^{(\bar p_-)}  + \frac{d L_{n_-}^{(\bar p_-)}}{d y}\right)e^{-y/2}\\
& = -b \bar z^{\bar p_- + 1} \left( L_{n_-}^{(\bar p_-)}  + L_{n_--1}^{(\bar p_-+1 )} \right)e^{-y/2}\\
& = -b \bar z^{\bar p_- + 1} L_{n_-}^{(\bar p_-+1)} e^{-y/2}\\
& = \mp i \sqrt{b n} \phi_+
\end{align*}
leading to
\[\phi_+ = \mp i \sqrt{\frac b n} z^{\bar p} L_{n - \bar p}^{(\bar p)} e^{-y/2}, \]
where $\bar p_- = \bar p -1$ and $n_- = n - \bar p$
in agreement with (\ref{eq:Lzpbar-spinor}), up to a constant normalisation.

\end{enumerate}

In summary the eigenspinors are
\begin{empheq}[box=\fbox]{align}
\psi_{n,p} & = {\cal N} z^p e^{-y/2}\begin{pmatrix}
L_n^{(p)}(y) \\ \mp i \sqrt{\frac{b}{n}}z L_{n-1}^{(p+1)}(y)
\end{pmatrix}\nonumber\\
\psi_{n,\bar p} & = \overline{\cal N} \bar z^{\bar p-1} e^{-y/2}\begin{pmatrix}
  \bar z L_{n-\bar p}^{(\bar p)}(y) \\ \pm i \sqrt{\frac{n}{b}} L_{n-\bar p}^{(\bar p-1)}(y)
\end{pmatrix},\label{eq:plane-eigenspinors}
\end{empheq}
satisfying
\[  i\Dslash \psi_{n,p} = \lambda \psi_{n,p}, \qquad  i\Dslash \psi_{n,\bar p} = \lambda \psi_{n,\bar p}\]
with eigenvalues $\lambda = \pm \sqrt{b n}$ (${\cal N}$ and $\overline{\cal N}$ are normalisation constants depending on n and, respectively, $p$ and $\bar p$). 
Note that
\[\left(L_3 + \frac 1 2 \sigma_3\right) \psi_{n,p}= \left(p + \frac 1 2 \right)\psi_{n,p},
\qquad \left(L_3 - \frac 1 2 \sigma_3\right) \psi_{n,\bar p}= \left(\bar p - \frac 1 2 \right)\psi_{n,\bar p}.\] 
Thus  $n$ and $p$ ($\bar p$) are good quantum numbers.
If $b<0$ use $y=|b|x$, $\lambda=\pm\sqrt{|b|n}$, interchange the two spinor components and complex conjugate them .

The eigenspinors (\ref{eq:plane-eigenspinors}) should reduce to ordinary plane waves as $b\rightarrow 0$ and this follows from  Abramowitz and Stegun (A+S) 22.15.2,
\[\lim_{n\rightarrow\infty} \left\{ \frac{1}{n^p} L_n^{(p)}\left( \frac {x}{n} \right)\right\} = x^{-p/2} J_p(2\sqrt{x}).\] 
Let $|b| n =\frac{k^2}{4} $, so $\lambda^2=\pm \frac{k^2}{4}$ 
and $y=|b| r^2 =\frac{k^2 r^2}{4 n}$, then\footnote{The factor of $\frac 1 4$ is because $z= x+ i y$
gives
\[ \partial_z \partial_{\bar z} = \frac 1 4 (\partial_x^2 + \partial_y^2).\]}
\[\lim_{n\rightarrow\infty} \left\{ \frac{1}{n^p} L_n^{(p)} (y)\right\} = 
\left(\frac{k r}{2}\right)^{-p} J_p(k r)\] 
Then, as $n\rightarrow \infty$,
\[ \psi_{n,p} \approx \begin{pmatrix}
e^{-i p \phi} J_p(k r)\\
0
\end{pmatrix},
\] 
which is a plane wave in 2-d polar co-ordinates.

Of course (\ref{eq:sphere-eigenspinors}) should also reduce to (\ref{eq:plane-eigenspinors}) in the limit of the radius $R$ of the sphere tending to infinity. This will involve an interplay with the limit $|m|\rightarrow\infty$, because the magnetic flux is $b=\frac{m}{2 \pi R^2}$, and is probably related to 
22.15.5 in Abramowitz and Stegun,
\[ \lim_{\beta\rightarrow\infty} P_n^{(\alpha,\beta)}\left(1 - \frac{2 x}{\beta}\right) = L_n^{(\alpha)}(x),\]
To investigate the planar limit we first make the substitution $z=\frac{z'}{R}$, with $R=2r$ i.e. twice the radius of the sphere (due to our initial setup being a sphere of radius $2$). Making this substitution in the metric gives \begin{align*} &ds^2=\frac{2 d z d\bar{z}}{(1 + z \bar{z})^2} = \frac{2 d z' d\bar{z'}}{R^2(1 + \frac{z' \bar{z'}}{R^2})^2}
~=~\frac{(ds')^2}{R^2}\\
& (ds')^2 = R^2 ds^2,
\end{align*}
which gives us the metric on a sphere with Radius $R$. So we can proceed with this substitution. A good initial check is that in the $R \rightarrow \infty$ limit we should find that equation \eqref{d1} and \eqref{d2} reduce to the eigenvalue equation for the Dirac operator in the plane. 

First we find that partial derivatives with respect to $z$ and $\bar{z}$ become \begin{equation*}
    \partial_z = R\partial_{z'}
\end{equation*}
and equations \eqref{d1} and \eqref{d2} in terms of $z'$ are
\begin{align*}
(1 +\frac{z' \bar{z'}}{R^2})(R)\partial_{z'} \phi_2 + \frac{(m-1)}{ 2} (\frac{\bar z'}{R}) \phi_2 &= -i\lambda \phi_1, \\
(1 +\frac{z' \bar{z'}}{R^2})(R)\partial_{\bar{z'}} \phi_1 - \frac{(m+1)}{ 2} \frac{ z'}{R} \phi_1 &= -i\lambda \phi_2 \\
\intertext{dividing through by $R$} 
(1 +\frac{z' \bar{z'}}{R^2})\partial_{z'} \phi_2 + \frac{(m-1)}{ 2} (\frac{\bar z'}{R^2}) \phi_2 &= \frac{-i\lambda}{R} \phi_1, \\
(1 +\frac{z' \bar{z'}}{R^2})\partial_{\bar{z'}} \phi_1 - \frac{(m+1)}{ 2} \frac{ z'}{R^2} \phi_1 &= \frac{-i\lambda}{R} \phi_2 \\
\end{align*}
Taking the limit as $R \rightarrow \infty$, defining $b= -\frac{m}{R^2}$ and $\lambda_P= \lim_{R\to\infty} \frac{\lambda}{R}$ we get
\begin{align*}
    \left(\partial_{z'} - \frac{b}{2} \bar {z}'\right) \phi_2 &= -i \lambda_P \phi_1\\
    \left(\partial_{\bar{z}'} + \frac{b}{2} z'\right) \phi_1 &= -i \lambda_P \phi_2
\end{align*}
Which is the eigenvalue equation for the Dirac operator in the plane. 

Now we check that the eigen-spinors on the sphere go to the eigen-spinors on the plane in the $R \rightarrow \infty$ limit. This can be done by rewriting the eigen-spinors on the sphere in terms of $x=\frac{x'}{R^2}$.

\begin{align*}
\psi_{\lambda,\alpha} &= \mathcal{N} 
 ({\frac{z'}{R}})^\alpha \left(\frac{1}{1+\frac{x'}{R^2}} \right)^{\frac{\alpha+\beta}{2}}\begin{pmatrix}
 P_n^{(\alpha,\beta)}\left(\frac{1-\frac{x'}{R^2}}{1+\frac{x'}{R^2}}\right)\\ 
\mp i \sqrt{\frac{n+|m|}{n}} \frac{z'}{R} \left(\frac{1}{1+\frac{x'}{R^2}} \right) P_{n-1}^{(\alpha+1,\beta+1)}\left(\frac{1-\frac{x'}{R^2}}{1+\frac{x'}{R^2}}\right)
\end{pmatrix}\\
\intertext{Using the expansion $\frac{1}{1+x}= 1-x+x^2-x^3+...$ and omitting terms higher than $\mathcal{O}(R^4)$ we have}
\psi_{\lambda,\alpha} &= \mathcal{N} 
 (z')^\alpha \left(\frac{1}{R^2+x'} \right)^{\frac{\alpha}{2}}\left(1-\frac{x'}{R^2}\right)^{\frac{\beta}{2}}\begin{pmatrix}
 P_n^{(\alpha,\beta)}\left(1-\frac{2x'}{R^2}\right)\\ 
\mp i \sqrt{\frac{1}{R^2}+\frac{|m|}{nR^2}} z' \left(1-\frac{x'}{R^2}\right) P_{n-1}^{(\alpha+1,\beta+1)}\left(1-\frac{2x'}{R^2}\right).\\
\end{pmatrix}\\
\intertext{Now using $\beta = bR^2$, for large $R$, we have}
\psi_{\lambda,\alpha} &= \mathcal{N} 
 (z')^\alpha \left(\frac{1}{R^2+x'} \right)^{\frac{\alpha}{2}}\left(1-\frac{bx'}{\beta}\right)^{\frac{\beta}{2}}\begin{pmatrix}
 P_n^{(\alpha,\beta)}\left(1-\frac{2bx'}{\beta}\right)\\ 
\mp i \sqrt{\frac{1}{R^2}+\frac{|m|}{nR^2}} z' \left(1-\frac{x'}{R^2}\right) P_{n-1}^{(\alpha+1,\beta+1)}\left(1-\frac{2bx'}{\beta}\right).\\
\end{pmatrix}\\
\intertext{Which in the limit as $R \rightarrow \infty$, and utilising 22.15.5 from Abramowitz and Stegun, is} 
\psi_{n,p} &= (z')^\alpha e^{-y'/2}\begin{pmatrix}
L_n^{(\alpha)}(y') \\ \mp i \sqrt{\frac{b}{n}}z' L_{n-1}^{(\alpha+1)}(y')
\end{pmatrix}
\end{align*}
With $y'=bx'$. Except I am uncertain what happens with the $\alpha$ term in front?


==> Chpt_3.tex <==
\chapter{Holographic Duality with a Dyonic Reissner-Nordstr\"om Black Hole}
\label{chp3_ADS-CFT_for_Reissner_Nordstrom_BH}

\section{Introduction}

The proposition of the Holographic principle by 't Hooft in [cite: 't Hooft 1993], and it's formulation in string theory by Susskind [cite: Susskind 1995], has led to an abundance of research into theories that utilise the principle to tackle otherwise mathematically intractable problems using geometric techniques. The most shining example of which has been the Anti de Sitter- conformal field theory correspondence (AdS/CFT), first proposed by Maldacena in [cite: Maldacena 1997]. In the two and half decades since Maldacena's conjecture of the correspondence a flood of research has followed and the applications have expanded to a broad range of topics. A comprehensive introduction to the general topic of this Gauge/Gravity duality can be found in [cite: Ammon, Gauge-Grav Duality 2015]. The success of this correspondence in giving an avenue to examine strongly coupled conformal field theories has motivated the extension of these techniques to condensed matter systems. 

As yet there is no analytic proof of the AdS/CFT correspondence and thus the broader topic of Guage/Gravity duality does not admit a rigorous way in which to apply it's techniques to condensed matter systems. There is however a collection of prescriptive approaches which have been devised. In this chapter we will focus primarily on those methods formulated in [Cite: Son and Starinets 2002, Iqbal and Liu 2008, 2009] and their applications by Liu et al. in [cite: Liu, McGreevy, Vegh 2009] where they used the correspondence to look for signatures of non-Fermi liquids.


Specifically we consider an asymptotically AdS space with a charged black hole, a Reissner-Nordstr\"om (RN-AdS$_{4}$) black hole with a dyonic charge, i.e. electric and magnetic charges. This is an extension of the work done in [cite: liu et al.] but with the modification that we use a spherical event horizon, as opposed to a planar one, and due to the inclusion of a magentic monopole we utilise the eigen-functions and eigen-values found in chapter 2 [ref:Chpt2] in our analysis here. Liu et al. [Cite: Liu 2009] mainly consider zero temperature systems for the boundary quantum field theory of their paper. We are instead interested in looking at non-zero temperature and specifically looking at the critical temperature for a black hole where the Hawking-Page phase transition [cite: Hawking, Page] occurs. This phase transition only occurs with a spherical event horizon. Work on fermionic bulk fields in RN-AdS$_{4}$ to examine holographic condensed matter systems has been looked at in [cite: Ren and Herzog 2012] where they examine the Green's functions for the boundary theory at nonzero temperatures and densities, and find Rashba like dispersion relations but do not include a magnetic charge nor examine the behaviour of the boundary theory at the Hawking-Page phase transition. In [cite: Dias et al. 2020] they use the AdS/CFT correspondence to look at fermionic instabilities for RN-AdS$_{4}$ black-holes and find that their are no linear mode instabilities for fermionic fields in this space, but again their work does not include a magnetic charge nor examine the behaviour of the Green's functions for the boundary theory at the aforementioned critical temperature.

We replicate the results found in [cite: Liu] and then find resonance behaviour for the same system of quasiparticle peaks with our spherical event horizon. We then consider non-zero tempreature and specifically look at the behaviour of the Green's functions at the critical temperature $T= T_{c}$. The behaviour of the Green's functions at this temperature, which is a phase transition for the black-hole in the bulk theory, may be indicitive of a phase transition in the dual theory. We present numerical results which we believe are consistent with this understanding.[?]

This chapter then will proceed as follows. Firstly I will give a broad introduction to the general topic of holographic duality, drawing a thread between the concepts on which it relies in \S \ref{Holog}. This will give us some intuition as to why the prescriptions we will utilise throughout the remainder of this chapter are reasonable. In \S \ref{Hol.Q.M} we will look at the applications of this approach to condensed matter systems, what is known as holographic quantum matter, and discuss the relevance of the Hawking-Page phase transition. We will review the prescription from [Cite:Iqbal and Liu] and it's applications to non-Fermi liquids in [Cite: Liu, Mcgreevy] \S \ref{Holo.Spinors}. In \S \ref{Results} we will present our findings.

\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Background to Holographic Duality} \label{Holog}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Duality}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The concept of duality exists across mathematics and physics. Though it's specific usage depends on the context there is an essential character of physical theories being dual to one another that is neatly outlined in [Cite: Castellani.]. The particular type of duality we are concerned with is that of strongly coupled theories dual to weakly coupled ones. This is known as an S-duality in the language of string theory. 

An elementary example of a duality in a physical model is the relationship between the electric and magnetic fields in a vacuum. This duality arises from a symmetry of the source free Maxwell's equations
\begin{align}
\nabla \cdot \mathbf{E} &= 0 \ , \quad \nabla \times \mathbf{E}= -\frac{\partial \mathbf{B}}{\partial t} \\
\nabla \cdot \mathbf{B} &= 0 \ , \quad \nabla \times \mathbf{B}= \mu_{0}\epsilon_{0}\frac{\partial \mathbf{E}}{\partial t}.
\end{align}
The symmetry is straightforward, sending $\mathbf{E} \rightarrow \mathbf{B}$ and $\mathbf{B} \rightarrow -\mu_{0}\epsilon_{0} \mathbf{E}$ leaves Maxwell's equations invariant. This is the duality in the theory. The electric and magnetic fields are dual to one another in this model. There is a more general form of this duality which was derived by [Cite: Gibbons and Rasheed] and reveals even further the symmetry in this theory , a concise introduction to this can be found here [B. Dolan, Bayntun]. If a source charge for the electric field is reintroduced this symmetry is broken, unless we also introduce a magnetic charge. As was covered in Chapter 2 [Ref:chapt2] introducting a magnetic monopole leads to Dirac's quantization condition
\begin{equation}
\frac{qm}{2\pi\hbar} = N \label{dirac.quant}
\end{equation}
where $q,m$ are the electric and magnetic charges respectively and $N \in \mathbb{Z}$. From this equation one can see \eqref{dirac.quant} that the strength of the magnetic charge is inversely proportional to the strength of the electric charge. In this way the strong coupling of the magnetic field is "dual" to the weak coupling of the electric field and vice versa. This is the most straight forward example of a duality in a theory that displays this connection between dual fields and their coupling strengths, an S-duality.

There are many systems that exhibit duality between weakly coupled and strongly coupled theories. One of the first examples was discovered by Krammers and Wannier in 1941 [cite: Kramers-Wannier 1941]. This duality exists between the free energy of a two-dimensional Ising model at low temperature and one at high temperature. The temperature here plays the role of the coupling in the theory and the high and low temperatures are the strong and weak couplings. This duality is explicit and there is an analytic transformation to go from one theory to the other [cite: Kramers-Wannier 1941]. 

Another strong-weak duality can be found between the massive Thirring model and the sine-Gordon scalar theory. This was first discovered by Coleman [Cite: S. Coleman 1975] between a fermionic field in one spatial dimension and a scalar field from the sine-Gordon equation. His method of calculation involved showing that the Green's functions for both theories gave equivalent spectra. There is a concise derivation of this duality in [Juricic et.al.] which shows explicitly how the lagrangians are equivalant and how the couplings display the strong-weak duality. This particular duality sheds light on the process of bosonization of fermionic particles in 1+1 dimensions. Note there is not a dimensional reduction here, nor in the previous two examples. Thus these dualities are of a different character to the AdS/CFT correspondence, which is still an S-duality but also relies on the CFT being one dimension lower than the AdS space it is dual to.

The duality at the heart of the AdS/CFT correspondence, and the first realisation of the holographic principle in [Cite: Maldacena 1997], is the relationship between a type IIB string theory in AdS$_{5} \times \mathbf{S}^{5}$ and an $\mathcal{N} = 4$, SU($N$) supersymmetric Yang-Mills theory in four spacetime dimensions, where $\mathcal{N}$ is the number of independent supersymmetries and $N$ the degree of the symmetry for the gauge fields. This is the dual CFT on the boundary of the string theory in the background AdS$_5$ space. The relevant coupling parameters for this duality on the AdS side are $l_{s}$ and $L$ , the string length and radius of curvature, and on the CFT side is the 't Hooft coupling $\lambda = g^{2}_{YM}$ and $N$. These parameters are realted via 
\begin{equation}
\left(\frac{L}{l_s}\right)^4 \propto \lambda, \quad  \left(\frac{L}{l_p}\right)^4 \propto N
\end{equation}
The strongest statement we have of the AdS/CFT correspondence is that the generating functional of the field theory is equivalent to the partition function for the string theory on the boundary of the AdS space
\begin{equation}
Z_{CFT_4} = Z_{ADS_5}. \label{ADSCFT}
\end{equation}
A proof of this duality would require a complete non-perturbative description of quantised string theory in a curved space, which we do not have. Instead we must consider the limit as $\lambda \rightarrow \infty$ and $N \rightarrow \infty$ where the strings are weakly coupled and the AdS side of the duality is effectively a classical gravity theory. Equation \eqref{ADSCFT} can then be given by 
\begin{equation}
Z_{CFT_4}[{\bf{A}}] \approx e^{-S_{AdS}} \label{ADSCFT1}
\end{equation} 
Where $\bf{A}$ here are source fields for the CFT that will depend on the behaviour of the dual bulk fields in the AdS space on the boundary and $S_{AdS}$ is the classical gravity action. This correspondence, following a similar line of reasoning for the specific case of AdS$_5$/CFT$_4$ generalises to AdS$_{d+1}$/CFT$_{d}$. A more precise statement can be given for example for a bulk field $\phi(x)$ that on the boundary takes on the value $\phi_{0}(x)$ 
\begin{equation}
\left\langle \exp\left[i \int d^dx\;\phi_0 (x) \mathcal{O} (x) \right]\right\rangle_{\mathrm{CFT}} = e^{-S_{\mathrm{grav}}[\phi|_{\partial \mathcal{M}}= \phi_0]} \label{ADSCFT2}
\end{equation} 
with $\mathcal{M}$ the AdS$_{d+1}$ space. The value of the bulk field on the boundary then acts as the source to the operator $\mathcal{O}(x)$ for the boundary CFT. Equation \eqref{ADSCFT2} and the equivalent expression for a ferminioc field we will use in our review in \S \ref{Holo.Spinors} allows us to compute correlation functions for strongly coupled field theories in $d$ dimensions on the boundary of a $d+1$ dimensional space time.
For a detailed introduction to these arguments and the evidence for it's veracity see [Cite: Ammon, Erdminger 2015].

The dimensional reduction in this duality, between AdS in $d+1$ dimensions and a CFT in $d$ dimensions is the realisation of the holographic principle. In the next section then we will try elucidate what this principle is. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Holographic Principle}\label{HoloPrinc} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The holographic principle is a direct consequence of the work done on black hole thermodynamics. As was mentioned in the first chapter of this thesis, one of the most successful marriages of quantum field theory (QFT) and general relativity (GR) has been within the regime of the microscopic understanding of black hole thermodynamics. From Chapter 1 [Ref: Chpt1] we discussed that the temperature of a black hole is given by it's Hawking temperature. For a metric in $d$ dimensions of the form 
\begin{equation}
ds^2 = -f(r) dt^2 + \frac{dr^2}{f(r)} + r^2 d\Omega^{2}_{d-2}
\end{equation} 
with an event horizon at $r=r_{h}$ the temperature of the blackhole is given by 
\begin{equation}
T_{H} = \frac{|f'(r_{h})|}{4\pi}. \label{Hawk_Rad}
\end{equation}
where we are working in units of $\hbar= c=G =1$. A natural next quantity to consider next, once you have a relation between particular qualities of the system and it's temperature, is entropy. How does the entropy of this system relate to geometric and physical qualities of the black hole? Bekenstein [cite: Bekenstein] had first proposed a proportionality relation between the area of the event horizon, for a Schwarzchild black hole, $A$ and the entropy of the black hole $S_{BH}$, motivated by the fact that a black hole's event horizon hides information and that clasically it does not decrease. Once Hawking had explained the temperature of a blackhole quantum mechanically, the constants of proportionality were worked out giving
\begin{equation}
S_{BH} = \frac{k_{B}A}{4 {l_{p}}^{2}}.
\end{equation}
This relationship highlights something particular about the nature of spacetime in the presence of a black hole. If we take a particular interpretation of the entropy as a measure of the information contained within a system, then this equation is telling us that what we know about the space is not proportional to the volume, as we could reasonably expect. Instead it is saying that the information about the space is contained on a two-dimensional surface in the space. 'T Hooft had precisely this interpretation in [Cite:'t Hooft, 1993] and considered that the information in a space was indeed encoded on the horizon of the blackhole. He took inspiration from the developments of lattice quantum field theory and proposed a two dimensional system of spins on a lattice, with lattice spacing $l_{p}$. This lattice of 2 spin-like degrees of freedom, which at each site could be spin-up or spin-down, played the role of a binary structure in which all of the information of the space was encoded. In [Cite:Susskind 1995] Susskind developed this notion even further within the context of string theory. He imagined a screen at the boundary of this space, which again featured as the binary system that encoded the infromation about the space. This "screen" was composed of illuminable dots which were also spaced a distance $l_{p}$ apart. If a particular dot was illuminated it would be considered 'on', and the unlit dots were considered to be in the 'off' position. Developing an image of the space seems tractable from this setup but determining distances between objects in the space was more complicated. The argument Susskind puts forward to explain this is beyond what we require for this introduction, but can be found in [Cite: Susskind 1995]. The fundamental contribution Susskind makes here is to extend the understanding about the relationship between the information about the space and the event horizon. Instead of the information being \emph{on} the event horizon, it is actually encoded on the boundary of the space, like a hologram. This is the holographic principle: the details and physical information in the space is related to a holographic "image" on the boundary of the space. Holographic duality then, which the ADS/CFT correspondence is the most succesful realisation of, is the relationship between a general relativistic theory in the bulk related to an inherently quantum mechanical system on the boundary.
With this in mind we should review the geometric properties of AdS and it's boundary.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Geometry of AdS Spacetime} \label{ADS_Geom} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The General Relativistic origins for de Sitter (dS) and AdS spacetime is in the search for solutions to the Einstein field equations that included a cosmological constant in the Einstein-Hilbert action in a vacuum, again with $G$ and $c$ set to $1$,
\begin{equation}
S = \frac{1}{16\pi}\int d^d x \sqrt{-det(g)} \left( R - 2\Lambda \right)
\end{equation} 
where the dS and AdS solutions correspond to negative and positive cosmological constant $\Lambda$, respectively and $d$ is the dimension of the spacetime. The metrics for these spacetime's are the solutions to the Einstein field equation that arises from varying this action with respect to the metric, giving
\begin{equation}
R_{\mu \nu} -\frac{1}{2} g_{\mu \nu} R + \Lambda g_{\mu \nu} = 0.
\end{equation}
Taking the trace of this equation with the inverse-metric one finds
\begin{align}
g^{\mu \nu} R_{\mu \nu} -\frac{1}{2} g^{\mu \nu} g_{\mu \nu} R + \Lambda g^{\mu \nu}g_{\mu \nu} &= 0 \\
R -\frac{d}{2}R + d\Lambda &= 0 \\
R &= \frac{2d}{d-2} \Lambda \label{ADS.1}
\end{align}
It's clear from \eqref{ADS.1} that the metric that would satisfy these equations would be one of constant scalar curvature. From a geometric perspective, considering spaces of constant curvature, the familiar examples are that of embeddings of surfaces in euclidian space. The plane, sphere and hyperboloid are the typical examples of embedded surfaces in 3-dimensional euclidian space with constant vanishing, positive and negative curvatures respectively. These however are all riemannian manifolds. When considering spacetime manifolds we are looking at lorentzian manifolds (or pseudo-riemannian manifolds). Within this framework then Minkowski, dS and AdS spacetime can be thought of precisely along these lines, they are the equivalent examples with vanishing, positive and negative scalar curvatures, respectively. Thus the space we are interested in, AdS, is that which has a negative cosmological constant and a constant, negative, scalar curvature. Though if this is the lorentzian analog of a hyperbolic plane embedded in euclidian space we don't imagine that there is a boundary of this plane. It extends off to infinity. How then is there a boundary for our AdS space, on which we expect to find our dual CFT? If we consider, in a similar way to our euclidan examples, that the ADS space is actually a hyperbolic hypersurface embbeded in a higher-dimensional space we can more clearly display the geometric properties of this manifold. A more in-depth treatment of this can be found in [L. Sokolowski]. 

As in this chapter we are considering AdS$_{4}$, we will begin with an ambient 5-dimensional (2+3) flat lorentzian manifold with coordinates $(X_0 ,X_1 ,X_2 ,X_3, X_4)$, with two timelike coordinates $X_0, \ X_1$. The metric on this is given by
\begin{equation}
ds^2 = -dX_{0}^2  -dX_{1}^2 + dX_{2}^2 + dX_{3}^2 + dX_{4}^2. \label{ADS.2}
\end{equation}  
Consider a 4-dimensional hyperbolic hypersurface in this space given by the equation
\begin{equation}
X_{2}^2 + X_{3}^2 + X_{4}^2 - X_{0}^2  -X_{1}^2 = -L^2 \label{ADS.3}
\end{equation}
where $L$ is a constant and, given the above metric, all the points on this hypersurface are equidistant from the origin. Thus sometimes the term pseudosphere is used to refer to such hypersurfaces, and $L$ is known as the radius of curvature. This is also why this particular 4-dimensional spacetime is considered maximally symmetric. A suitable parameterisation is given by
\begin{align}
X_0 &= L\sin(\frac{t}{L})\cosh(\frac{\rho}{L}) \\
X_1 &= L\cos(\frac{t}{L})\cosh(\frac{\rho}{L}) \\
X_2 &= L\sinh(\frac{\rho}{L})\sin{\theta}\cos{\phi} \\
X_3 &= L\sinh(\frac{\rho}{L})\sin{\theta}\sin{\phi} \\
X_4 &= L\sinh(\frac{\rho}{L})\cos{\theta}
\end{align} 
where the coordinates take the values $-\pi L < t < \pi L$,  $\rho \ge 0$ and $\theta ,\ \phi$ are the usual spherical coordinates with $0 \le \theta \le \pi$ and $0 \le \phi \le 2\pi$. It's straightforward to check that these coordinates satisfy \eqref{ADS.3}. Now subbing them in to \eqref{ADS.2} the metric on our hypersurface is given by
\begin{equation}
ds^2 =  -\cosh^{2}(\frac{\rho}{L})dt^2 +d\rho^2 + L^2\sinh^2(\frac{\rho}{L})(d\theta^2 + \sin^{2}\theta d\phi^2) 
\end{equation}
and upon noticing the hyperbolic sine function infront of what looks like the metric on a unit 2-sphere we can spot a natural redefinition for $\rho$. Setting $r := L\sinh(\frac{\rho}{L})$ gives
\begin{equation}
ds^2 =  -\left(1 + \frac{r^2}{L^2} \right)dt^2 + \frac{1}{\left(1 + \frac{r^2}{L^2} \right)}dr^2 + r^2(d\theta^2 + \sin^{2}\theta d\phi^2) \label{ADS.5.1}
\end{equation}
and we arrive at the familiar metric, with global coordinates for AdS$_{4}$. To display the relationship between the cosmological constant and $L$ we move to what are known as Poincare coordinates. They are given by the following equations 
\begin{align}
X_0 &= \frac{1}{2z}(L^2 + |\vec{r}|^2 - t^2) \\
X_1 &= L\frac{t}{z} \\
X_2 &= L\frac{x}{z} \\
X_3 &= L\frac{y}{z} \\
X_4 &= L\frac{1}{2z}(L^2 - |\vec{r}|^2 + t^2)
\end{align}
where $|\vec{r}|^2 = x^2 +y^2 + z^2$. The metric then becomes
\begin{equation}
ds^2 = \frac{L^2}{z^2}(-dt^2 + dx^2 + dy^2 + dz^2) \label{ADS.4}
\end{equation}
with an obvious coordinate singularity at $z=0$, where the metric is not defined. The above form of the metric generalises to a $d$-dimensional AdS space so working through the christoffel symbols to calculate the Ricci scalar from the metric in $d$ dimensions one finds
\begin{equation} 
R = \frac{-d(d-1)}{L^2}
\end{equation}
which is consistent with our spacetime being a hyperbolic space. Combining this with equation \eqref{ADS.1} we have 
\begin{equation} 
\Lambda = \frac{-(d-1)(d-2)}{2 L^2}.
\end{equation}
From the above metric \eqref{ADS.4} we can see that this space is conformally equivalent to minkowski space. That is to say $g^{ADS}_{\mu \nu} = \Omega^2 g^{Mink}_{\mu \nu}$, where $\Omega$ is some scalar function of the coordinates, albeit for a segment of AdS, known as the Poincare patch. There is a hint towards the location of our conformal boundary in \eqref{ADS.5.1}. For $r \rightarrow \infty$ AdS the time and angular coordinates diverge but the radial coordinate tends to zero. This can be more clearly seen with the change of coordinates given by $r = L\tan(q)$, where $0 \le q < \frac{\pi}{2} $. The metric becomes 
\begin{equation}
ds^2 =  \frac{1}{\cos^{2}(q)}\left( -dt^2 + L^{2} dq^2 + L^{2}\sin^{2}(q)(d\theta^2 + \sin^{2}\theta d\phi^2)\right)
\end{equation}
which at first does not appear to gives us more information as to the structure of the boundary of ADS. Though if we consider a metric conformally related by $\tilde{g}^{\mu \nu} = \cos^{2}(q){g}^{\mu \nu}$ we have
\begin{equation}
d\tilde{s}^2 = -dt^2 + L^{2} dq^2 + L^{2}\sin^{2}(q)(d\theta^2 + \sin^{2}\theta d\phi^2)
\end{equation}
which now includes the point $q= \frac{\pi}{2}$ and at this point we have a hypersurface which has a metric 
\begin{equation}
d\tilde{s}^2 = -dt^2 + L^{2}(d\theta^2 + \sin^{2}\theta d\phi^2)
\end{equation}
which is the \emph{conformal spacial infinity} of AdS spacetime and has the structure of $\mathbb{R}^1 \times S^2$. This establishes that for $r \rightarrow \infty $ there is a conformal boundary with some well-defined structure. With this outlined we can proceed to the further role that AdS spacetime plays in the discussion of holography and specifically geometerising the energy scale. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Geometerising the Energy Scale} \label{Geom_Eng}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

If we take inspiration from one of the coneptual adjustments that is required when moving from classical mechanics to special and general relativity we can better understand the holographic quality of AdS spacetime. The conceptual adjustment I am reffering to is the consideration of time as a local coordinate, and no longer just a parameterisation of the spatial coordinates. This observation gave rise to the progress made by Minkowski and others in understanding the geometric properties of special relativity. Thus considering not merely coordinates $(x(t),y(t),z(t))$ but $(t,x,y,z)$, where these spacetime coordinates can be functions of proper time $\tau$ (or any affine parameter $\lambda$), we are afforded a new insight in to the structure of our physical reality.

Similarly, from the discussion in \S \ref{HoloPrinc} on Holography we can glean a general approach that is arising here; associating Physical quantities with geometric properties. Historically it was not the purpose of the endeavour but seems to arise naturally via the discovery of relationships between geometric and thermodynamical quantities. So what aspect of ADS spacetime are we looking to ascribe a new physical meaning to? To begin with we look at a 2-dimensional dimensionless metric
\begin{equation}
ds^2 = \frac{dx^2 + dy^2}{z^2} \label{ADS.5}
\end{equation}
where here $z$ is some constat with units of length, as do $x$ and $y$. The metric allows for the definition of distances (as well angles) on a manifold, thus in this case the distances $ds^2$ remain unchanged under a different choice of units for $z,x,y$, making it scale invariant. If instead we were to consider the units of $x$ and $y$ to be fixed and varied the dimensions of $z$ we would consider this as some length scale of the metric, i.e. different choices of $z$ corresponding to different measures of distance for the space. If we were to then consider incorporating this change into the geometry of the space it would require a relatively simple adjustment to \eqref{ADS.5}
\begin{equation}
ds^2 = \frac{dx^2 + dy^2 + dz^2}{z^2}. \label{ADS.6}
\end{equation}
which is the metric for the Poincare upper half-space in 3-dimensions, with $z>0$. From this perspective we can consider a flow of the space given by \eqref{ADS.5} at different length scales. 

From here it does not require too much of an intuitive leap to see that if we consider a minkowski metric in the numerator of \eqref{ADS.6}
\begin{equation}
ds^2 = \frac{-dt^2 + dx^2 + dy^2 + dz^2}{z^2}. 
\end{equation}
we arrive at \eqref{ADS.4} which is AdS$_{4}$ spacetime in the Poincare patch, with $L = 1$. This allows us to consider an interpretation of the radial coordinate in the broader topic of gauge/gravity duality, referred to in the literature as the holographic dimension. Note there is a crucial difference here; though this is a nice exposition of the intuition behind the radial coordinate, the flow of $z$ in the above coordinates is not associated exclusively with the flow of length scales, as the AdS metric actually contains $\frac{L^2}{z^2}$. Instead we need to consider the duality involved to interpret the holographic dimension. 

We have only looked at the geometrisation of this scale from the AdS side, but what does this correspond to in our duality. For the field theory side this flow is the flow of energy scales. At the boundary, i.e. where there is weak gravitational curvature and thus, due to our S-duality, strong field theory coupling, we are in the high energy or ultraviolet (UV) range, of the CFT. For small $z$ there is strong gravitational curvature and thus weak coupling in the CFT side, i.e. the infrared (IR) range. Given this understanding of the holographic dimension there is a natural way to think of the flow along the radial coordinate $z$ as a geometrization of renormalisation group flow.

We have explained above an imprecise notion of a foliation of a space in which each hypersurface for constant $z$ has a dual CFT at different energy scales. We can think of the 'holographic' dimension of AdS space as the renormalisation dimension, i.e. the limits of high energy and low energy cutoffs for the dual CFT are contained within this extra dimension and the flow along it is a geometric picture of renomalizition group flow. This understanding was further articulated in [Cite: Iqbal, Liu, 2008] in the context of the universality of the hydrodynamic limit via the membrane paradigm for black holes. The membrane paradigm is a simplifying tool for calculating the thermodynamic effects of the exterior of a blackhole by considering a fictious, thin, clasically radiating fluid that sits just above the event horizon [cite-Thorne et al. 1986]. Iqbal and Liu associated this fluid with the dual quantum field theory (QFT) at weak coupling, motivated by the fact that at sufficiently long length scales QFT's should be described by hydrodynamics. They used this understanding to derive equations governing the evolution of the QFT dual from the horizon to the strongly coupled regime at the boundary, giving a clear presentation of this geometric renormalisation flow. Crucially this also articulated how the behaviour of the dual field theory on the boundary at finite temperature was determined by the horzion's geometry and thermodynamic quantities. In the next section we will discuss the role of thermodynamics and how we can apply the AdS/CFT correspondence to condensed matter systems.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Critical Points and Conformal Symmetry}\label{Hol.Q.M}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A conformal transformation of a space is often described as preserving angles but not distances. More precisely conformal transformations are those transformations of the
metric of  a spacetime $g_{\mu \nu} (x)$ that leave it invariant up to a postive, arbitrary scale factor that can depend on the coordinates of the space time. This means under the transformation $x \mapsto \tilde{x} = f (x)$ the metric becomes
\begin{equation}
g_{\mu \nu}(x) \mapsto \tilde{g}_{\mu \nu} = \left(\Omega(x)\right)^{-2}g_{\mu \nu}(x)
\end{equation}
which can be seen to preseve the causal structure of the space time but not the length of space time intervals. The complete set of conformal transformations in $d > 2$ dimensions are translations, Lorentz transformations, dilations and the special conformal transformation. For an infinitesimal transformation of the coordinates we have, in the order mentioned above,
\begin{equation}
x^{\mu} \mapsto x^{\mu} + a^{\mu} + \omega^{\mu}_{\nu}x^{\nu} + \lambda x^{\mu} + b^{\mu} x^{\nu} x_{\nu} - 2(b^{\nu}x_{\nu})x^{\mu}.
\end{equation}
where the generators corresponding to these quantities are respectively
\begin{align}
P_\mu &= -i\partial_\mu, \\
J_{\mu\nu} &= i(x_\mu\partial_\nu-x_\nu\partial_\mu), \\
D &= -ix_\mu\partial^\mu, \\
K_\mu &= i(x^{\nu}x_{\nu}\partial_\mu-2x_\mu x_\nu\partial^\nu).
\end{align}
For $d=2$ dimensions the number of conformal transformations is infinite. A conformally invariant field theory we have already come across is the massless Klein-Gordon equation in chapter 1 [ref: chpt1]. From equation [eqref: 1.30] we saw that under the conformal transformation to rindler coordinates our equations of motion remained the same. There is another feature of CFT's that we can see from the energy-momentum tensor of this field. For a Klein-Gordon field in two space time dimensions the energy-momentum tensor is
\begin{equation}
T_{\mu \nu } = \partial_{\mu} \phi \partial_{\nu} \phi - \frac{1}{2} g_{\mu \nu}\left(\partial^{\alpha} \phi \partial_{\alpha} \phi \right)
\end{equation}
and taking the trace of this gives
\begin{equation}
g^{\mu \nu} T_{\mu \nu} = 0.
\end{equation}
This is a an essential component of CFT's that conformal symmetry imposes. Their energy momentum-tensors are traceless if they are invariant under scale transformations.

If we look just at dilations, $x^{\mu} \mapsto \lambda x^{\mu}$, a central quality of all CFT's is that they are scale invariant. A feature of most condesed matter systems is that they are not generally scale invariant and thus not described by CFT's. There is a saving grace however, around a quantum critical point there are condensed matter systems, or condensed matters theories (CMT), that exhibit scale invariance. That is to say, when approaching critical points the scale dependent parameters in the model become less and less relevant and the scale invariant quantities donimate. This is where we direct our focus and in using gauge/gravity duality associate our dual CFT with a condensed matter system in the domain where the system exhibits scale invariance. This approach has been used over the last two decades to analyse and provide new universality classes of condensed matter systems. Comprehensive introductions to the use of gauge/gravity duality to these systems, sometimes called the AdS/CMT correspondence, can be found in [Cite: McGreevy 2015, Hartnoll 2018]. 

Scale invariance at a critical point is not only a feature of quantum critical systems but a classical example comes from the theorem of corresponding states. This was first discovered by Johannes van der Waals in 1873 [cite: Van der Waals thesis] when looking at the equation of state that bears his name. This is a modified version of the ideal gas law that takes into account weak interactions between the particles of the gas and the volume the gas itself occupies. The Van der Waals equation of state captures the qualitative behaviour of the phase transition between gas and liquid and thus contains a critical point. To find it we have the equation of state
\begin{equation}
\left(P + \frac{N^2 a}{V^2} \right) \left( V - bN \right) = NRT
\end{equation}
where $N$ is the number of moles of the gas, $b$ is the volume of one mole of the gas, and $a$ is a measure of the average attraction between particles. Simple algebra gives a cubic equation in the volume
\begin{equation}
V^3 - N \left( b+ \frac{RT}{P} \right) V^2 + \frac{N^2 a}{P} V - \frac{N^3 ab}{P} = 0
\end{equation}
which can be written in terms of its roots
\begin{equation}
(V- V_{1})(V-V_{2})(V-V_{3})=0.
\end{equation}
The critical point for the tranisition occurs at $V_{c}=V_1=V_2=V_3$, whereupon subbing $V_{c}$ in to the above and comparing coefficients we find the expressions for the critical volume, pressure and temperature to be
\begin{align}
V_{c} &= 3bN \\
P_{c} &= \frac{a}{27b^2} \\
T_{c} &= \frac{8a}{27 b R}.
\end{align}

These critical values dictate where a phase transition between liquid and gas can and cannot occur, see figure \ref{VDW}.

\begin{figure}[h!]
\centerline{\includegraphics[width=0.6\linewidth]{Images/ADS_CFT/Van_der_Waals_Isotherms}}
\caption{ $P$ - $V$ diagram showing Van der Waals isotherms above and below the critical temperature. We see that above the critical temperature the gas behaves more like an ideal gas without the possibility for condensation. This captures the quality of differing behaviour above and below $T_{c}$ but note that the oscillations where $\partial P / \partial V |_{T} < 0 $ are unphysical and require a modification called a Maxwell construction.}
\label{VDW}
\end{figure}

Defining dimensionless variables using these critical values, known as reduced variables, 
\begin{equation}
V_{r}= \frac{V}{V_{c}}, \quad P_{r} = \frac{P}{P_{c}}, \quad T_{r} = \frac{T}{T_{c}} 
\end{equation}
our equation of state becomes 
\begin{equation}
\left(P_{r} + \frac{3}{V_{r}^2} \right) \left( V_{r} - 1 \right) = 8T_{r}.
\end{equation}
From this equation we see that near the critical point the length scale is not relevant and the gas dependant parameters $a$ and $b$ no longer feature. This is a simple result that satisfies the theorem of corresponding states. Fluids that are described by this equation fall in to a universality class, that is to say they are indistinguishable in their behaviour near the critical point and exhibit scale invariance there. 

A critical point we are interested in analysing is the one that features in the aforementioned Hawking-Page phase transition [cite: Hawking, Page 1983]. As was discussed in \S\ref{Geom_Eng} Iqbal and Liu showed in [Cite: Iqbal,Liu 2008] that the dual strongly coupled field theory on the boundary was determined by the properties of the bulk black hole horizon. The Hawking-Page phase transition only occurs in an asymptotically AdS spacetime. An asymptotically AdS$_{4}$ space time is given by 
\begin{equation}
    ds^{2}=-f^{2}(r)dt^2+\frac{dr^2}{f^2(r)}+r^{2}d\Omega_{k}^2 \label{AsymADS}
\end{equation}
with
\begin{equation}
    f(r)^2 = k-\frac{2\mathcal{M}}{r} + \left( \frac{r}{L} \right)^2.
\end{equation}
and
\begin{equation}
d\Omega_{k}^2 = \left\{\begin{array}{lll}
d\theta^{2} + \sin^{2}(\theta)d\phi^2, &   k= 1 \\
d\theta^{2} + d\phi^2, &  k=0 \\
d\theta^{2} + \sinh^{2}(\theta)d\phi^2, & k= -1 \\ \end{array} \right.
\end{equation}
The $k$'s here determine the geometry of the event horizon at $r=r_{h}$: for $k=1$ the event horizon is a sphere, $k=0$ it is a flat plane, and $k=-1$ is a hyperbolic plane. At the horizon we have 
\begin{equation}
k-\frac{2\mathcal{M}}{r_{h}} + \left( \frac{r_{h}}{L} \right)^2 = 0 \quad \rightarrow \mathcal{M} = \frac{r_{h}}{2} \left( k + \frac{r_{h}^2}{L^2}\right)
\end{equation}
and the temperature for this black hole is given by equation \eqref{Hawk_Rad}
\begin{equation}
T = \frac{|f'(r_{h})|}{4\pi} = \frac{1}{2\pi}\left( \frac{\mathcal{M}}{r_{h}^2} + \frac{r_{h}}{L^2} \right) = \frac{1}{4\pi} \left( \frac{k}{r_{h}} + \frac{3r_{h}}{L^2} \right).
\end{equation}
If we treat $\mathcal{M}$ as the internal energy of the black hole, with the pressure assigned to the cosmological constant and is thus fixed, we can find the heat capacity given by
\begin{equation}
C_{P} = \frac{\partial \mathcal{M}}{\partial T} = \frac{\partial \mathcal{M}}{\partial r_{h}} \left(\frac{\partial T}{\partial r_{h}}\right)^{-1} =  \frac{2\pi r_{h}^2\left(k + 3(r_{h}^2 / L^{2})\right)}{3(r_{h}^2 / L^2) - k}.
\end{equation}
In dimensionless parameters
\begin{equation}
x= \frac{r_{h}}{L}, \quad m=\frac{\mathcal{M}}{L}, \quad t=TL, \quad c_{p}= \frac{C_{p}}{L^2}
\end{equation}
the above expressions for, mass, temperature and heat capacity become
\begin{align}
m=&\frac{x(x^2 +k)}{2}\\
t=&\frac{3x^2+k}{4\pi x}\\
c_{p}=&\frac{2\pi x^2 (3x^2 + k)}{3x^2 -k} \label{cp}
\end{align}
whereupon plotting the heat capacity as a function of the temperature and mass, figures \ref{HP1} and \ref{HP2}, we see clearly the behaviour that is indicitave of a phase transition i.e. when $k=1$ there is a critical temperature $T_{c} = t_{c}/L= \frac{\sqrt{3}}{2\pi L}$ where the heat capacity is diverges.
\begin{figure}[h!]
\centerline{\includegraphics[width=0.8\linewidth]{Images/ADS_CFT/Hawk_Page1}}
\caption{The dimensionless temperature of an AdS black hole as a function of the dimensionless mass for all three values of $k$. We have also here plotted the location of the critical temperature $t_{c} \approx 0.276$.}
\label{HP1}
\end{figure}

\begin{figure}[h!]
\centerline{\includegraphics[width=0.8\linewidth]{Images/ADS_CFT/Hawk_Page2}}
\caption{The dimensionless heat capacity of an AdS black hole as a function of the dimensionless temperature for all three values of $k$. The location of the critical temperature $t_{c}$ and the Hawking-Page phase transition where $C_{p}\rightarrow \infty$, for $k=1$ is the straight magenta line.}
\label{HP2}
\end{figure}
 This behaviour does not occur for the other values of $k$. These figures show that for $t=t_{c}$ the heat capacity diverges and as can be seen from equation \eqref{cp}, the heat capacity is negative in the region of $t<t_{c}$. This indicates that the black hole undergoes a phase transition from a stable state to a unstable one where it radiates away it's energy. This is the essence of the Hawking-Page phase transition. In \S\ref{Results} a nearly identical calculation will follow for an RN-AdS$_{4}$ black hole which will allow us to analyse the behaviour of our dual field theory on the boundary at these critical points. Before this though we will briefly review the prescriptive approach we will be using to obtain our results outlined in [cite:Son,Starinets 2002, Iqbal, Liu, 2009].

\begin{comment}
An appropriate beginning on this topic I feel is to begin with a quote which I feel wonderfully captures the experience of working through the literature on the AdS/CFT correspondence as it is employed in condensed matter, and strongly coupled systems. [Bayntun,et. al] 
\begin{quotation}
Applications of AdS/CFT duality ... to condensed matter physics carry a whiff of a fishing expedition. ... Without a systematic way to derive the magic CFT directly from unerlying electron dynamics one throws theoretical darts into a field space, hoping to find that right 'hyperbolic cow'.
\end{quotation}  
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{ADS/CFT Prescription for Spinors}\label{Holo.Spinors}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As has been noted often in the literature, though the explicit examples of holographic duality require string theory as the starting point [Cite: Maldacena, Ammon and Erdmenger, Hartnoll et.al], the techniques involved are quite general and only require us to use concepts from general relativity and quantum field theory. The list of techniques and presciptions are vast and could not be meaningfully covered in this chapter, we will instead briefly review the prescription outlined in [Cite: Iqbal and Liu 2009] for spinor fields in a background asymptotic AdS$_{4}$ space time with a view towards utilising this approach in \S\ref{Results}. As in equation \eqref{AsymADS} the metric 
\begin{equation}
    ds^{2}=-f^{2}(r)dt^2+\frac{dr^2}{f^2(r)}+r^{2}d\Omega_{k}^2 \label{AsymADS1}
\end{equation} 
has the behaviour near the boundary 
\begin{equation}
g_{tt}, g^{rr}, g_{ii} \approx r^2, \quad r\rightarrow \infty
\end{equation}
where $i$ are the angular components of the metric. For the time being we do not specify the function $f(r)$ in the metric, just that it has the above boundary behaviour. We will be working in Lorentzian signature which does pose subtleties for the boundary counditions for the fermionic field at the horizon but here we will just review the prescription laid out in [Cite: Iqbal, Liu 2009] which was confirmed in [Herzog, Son, 2003].

Given a boundary theory fermionic operator $\mathcal{O}$ that is dual to a spinor field $\psi$ in an AdS background we can compute two point functions for this dual operator just by considering the quadratic part of the action for $\psi$ in the bulk 
\begin{equation}
S[\psi] = \int d^{4}x\sqrt{-g} i \left( \bar{\psi} \Dslash \psi - M \bar{\psi}\psi +  \right) + S_{bd}
\end{equation}
where $S_{bd}$ are boundary terms that ensure a well defined variantional principle for the action [cite: Henneaux arxiv. 9902137]. The dirac operator $\Dslash$ is 
\begin{equation}
\gamma^{\mu}D_{\mu}= \gamma^{a}(e^{-1})^{\mu}_{a}(\partial_{\mu}+\frac{1}{4}\gamma^{bc}(\omega_{bc})_{\mu})
\end{equation}
and $\bar{\psi} = \psi\gamma^t$. The $\gamma$'s are the usual gamma matrices. The $e$'s are components of orthonormal one forms and are related to the metric by 
\begin{equation}
    \eta_{ab}e^{a}_{\mu}e^{b}_{\nu}=g_{\mu\nu}
\end{equation}
where the roman letters denote frame indices while greek letters denote coordinate indices. The $\omega$'s are the matrix elements of spin connection one forms and we can find these using cartan's first structure equation (assuming zero torsion)
\begin{equation}
    de^a= -\omega^{a}{}_{b}\wedge e^{b}.
\end{equation}
as in [ref: Chpt2].

With this the prescription for finding retard greens functions for an operator $\mathcal{O}$ is as follows
\begin{enumerate}
\item Find a solution $\psi = \psi_{+} + \psi_{-}$, to the equations of motion with in-falling boundary conditions at the horizon. With $\psi_{\pm}$ being two component spinors.
\item Expand the solution near the boundary $r \rightarrow \infty$ such that 
\begin{equation}
\psi_{+}= Ar^{-\frac{d}{2} + M} + Br^{-\frac{d}{2} - M -1}, \quad \psi_{-}= Cr^{-\frac{d}{2} + M -1} + Dr^{-\frac{d}{2} - M}.
\end{equation}
plugging this in to dirac equation yields the relationship between the coefficients to be
\begin{equation}
C = \frac{i\gamma^{\mu}k_{\mu}}{2m-1} A, \quad B = \frac{i\gamma^{\mu}k_{\mu}}{2m+1} D
\end{equation}
\end{enumerate}
To begin though we should give a more precise account of equation \eqref{ADSCFT1} that is to say that the relationship between a bulk field in an AdS background and the boundary CFT is given by 
\begin{equation}
\left\langle \exp\left[\int d^dx\;\phi_0 (x) \mathcal{O} (x) \right]\right\rangle_{\mathrm{QFT}} = e^{-S_{\mathrm{grav}}[\phi_0]}
\end{equation}


where one point functions of $\mathcal{O}$ in the presene of the source $\phi_{0}$ can be written as 
\begin{equation}
\langle \mathcal{O}(x) \rangle_{\phi_0} = -\frac{\delta S_{\rm{grav}}}{\delta \phi_0 (x)} = - \lim_{r\to\infty}\Pi_E (r,x)|_{\phi_E}
\end{equation}
and its Fourier transform
\begin{equation}
\langle \mathcal{O}(\omega_E, \vec{k}) \rangle_{\phi_0}  = -\lim_{r\to\infty}\Pi_E (r,\omega_E, \vec{k})|_{ \phi_E} \ .
\end{equation}
and at a linear level one finds that 
\begin{equation}
G_E(\omega_E, \vec{k}) = -\left(\lim_{r\to\infty}\frac{\Pi_E (r,\omega_E, \vec k)|_{ \phi_E}}{\phi_E (r,\omega_E,\vec{k})}\right)
\biggr|_{\phi_0 =0}
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Radial Part - Separation of Variables for the Dirac Equation and Using our Eigenfunctions on the Sphere}\label{Results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The previous section was part of a broader effort to analyse the Dirac equation for an anti-de Sitter blackhole with a magnetic monopole at the centre and a charge on the event-horizon. For the start of the calculations though we will use a more general metric
\begin{equation*}
    ds^{2}=-f^{2}(r)dt^2+\frac{dr^2}{f^2(r)}+r^{2}d\theta^{2}+r^2\sin^2(\theta)d\phi^2.
\end{equation*}
The Dirac operator in a curved space-time as \begin{equation*}
    \Dslash = \gamma^{a}(e^{-1})^{\mu}_{a}D_{\mu}= \gamma^{a}(e^{-1})^{\mu}_{a}(\partial_{\mu}+\Tilde{\lambda}\gamma^{bc}(\omega_{bc})_{\mu}+ \Tilde{\alpha}A_{\mu})
\end{equation*}
where $\Tilde{\lambda}$ and $\Tilde{\alpha}$ are constants and the Roman letters denote frame indices while greek letters denote coordinate indices. The $e$'s are components of orthonormal one-forms and the $\omega$'s are the matrix elements of connection one-forms. The components of the orthonormal one-forms are related to the metric by
\begin{equation*}
    \eta_{ab}e^{a}_{\mu}e^{b}_{\nu}=g_{\mu\nu}
\end{equation*}
the orthonormal one-forms are then
\begin{align*}
    e^{a}&= e^{a}_{\mu}dx^{\mu}\\ 
    e^{0}&= f(r)dt, \ e^{1}= \frac{dr}{f(r)}, \ e^{2}= rd\theta, \ e^{3}= r\sin(\theta)d\phi
\end{align*}
Using Cartan's first structure equation
\begin{equation*}
    de^a= -\omega^{a}{}_{b}\wedge e^{b}
\end{equation*}
(given that we have zero torsion) we can find the connection one-forms. Taking the exterior derivative of the $e$'s above and doing some rearranging gives
\begin{align*}
    de^{0}&= f'(r)e^1\wedge e^0 \\
    de^{1}&= 0\\ 
    de^{2}&= \frac{f(r)}{r}e^1\wedge e^2\\ 
    de^{3}&= \frac{f(r)}{r}e^1\wedge e^3 + \frac{\cot(\theta)}{r}e^2\wedge e^3.\end{align*}
A little work reveals that the connection one-forms are 
\begin{align*}
    \omega^{0}_{\ 1} &= f'(r) e^{0} = f'(r)f(r)dt \\
    \omega^{2}_{\ 1} &= \frac{f(r)}{r} e^{2} = f(r)d\theta  \\
    \omega^{3}_{\ 1} &= \frac{f(r)}{r} e^{3} = f(r)\sin(\theta)d\phi\\
    \omega^{3}_{\ 2} &= \frac{\cot(\theta)}{r} e^{3} = \cos(\theta)d\phi.\\
\intertext{An alternative choice for $\omega^{3}_{\ 2}$ which makes it regular at the north and south pole's is}
    \omega^{3}_{\ 2} &= (\pm1-\cos(\theta))d\phi.
\end{align*}
With these components we can now look at the dirac equation 
\begin{align}
    \Dslash \Psi -m\Psi &= \gamma^{a}(e^{-1})^{\mu}_{a}D_{\mu} \Psi -m\Psi = 0\nonumber \\
    &=\left(\gamma^{0}(e^{-1})^{t}_{0}D_{t} + \gamma^{1}(e^{-1})^{r}_{1}D_{r} + \gamma^{2}(e^{-1})^{\theta}_{2}D_{\theta} + \gamma^{3}(e^{-1})^{\phi}_{3}D_{\phi}\right)\Psi - m\Psi\nonumber \\
    &=\left(\frac{\gamma^{0}}{f(r)}D_{t} + \gamma^{1}f(r)D_{r} + \frac{\gamma^{2}}{r}D_{\theta} + \frac{\gamma^{3}}{r\sin(\theta)}D_{\phi}\right)\Psi - m\Psi\nonumber \\
    &=\left(\frac{\gamma^{0}}{f(r)}D_{t} + \gamma^{1}f(r)D_{r} + \frac{1}{r}D_S \right) \Psi -m\Psi\nonumber \\
\intertext{where $D_S$ is the dirac operator on the unit sphere (which is 
$\frac{1}{\sqrt{2}}$ times that worked out in the previous section). This then gets replaced with the eigenvalues, $\frac{\lambda_S}{2}$, of the Dirac operator on the unit sphere}
  (\Dslash-m)\Psi  &= \left(\frac{\gamma^{0}}{f(r)}D_{t} + \gamma^{1}f(r)D_{r} + 
\frac{i}{\sqrt{2}}\frac{\lambda_S}{r} \mathbb{I}_{2}\otimes \sigma^1 \right) \Psi -m\Psi
\end{align}
Now as there are no connection one-forms with an $r$ index we have $D_r=\partial_r$. We are also going to first consider the static solution which means 
\begin{align*}
    \gamma^{0}D_t &= \gamma^{0}(2\Tilde{\lambda}\gamma^{01}(\omega_{01})_{t}+ \Tilde{\alpha}A_{0})\\
\intertext{With $\gamma^0\gamma^{01}=-2\gamma^1$ and $(\omega_{01})_{t}= -f'(r)f(r)$ we have}
    \gamma^{0}D_t &= 4\Tilde{\lambda}\gamma^{1}f'(r)f(r) + \Tilde{\alpha}\gamma^0A_0.
\end{align*}
The Dirac equation now looks like
\begin{equation*}
    \Dslash \Psi -m\Psi = \left(\gamma^{1}(4\Tilde{\lambda}f'(r) +f(r)\partial_r) + \gamma^0\frac{\Tilde{\alpha}}{f(r)}A_0 + \frac{i}{\sqrt{2}}\frac{\lambda_S}{r} \mathbb{I}_{2}\otimes \sigma^1 \right) \Psi -m\Psi.
 \end{equation*}

Alternatively we cold use a black-brane solution rather than a black hole solution,
in which case the Dirac operator on the sphere is replaced by the Dirac operator in
a plane, \cite{Jellaletal}, and 
$\frac{\lambda_S}{\sqrt{2} r}=\pm\sqrt{\frac{n(n+|m|)} {2}} \frac 1 r $ would be replaced by the $r$-independent eigenvalues in the plane, 
$\lambda_P=\pm \sqrt{|b| n}$.

The constants are $\Tilde{\alpha}=ie$ and $\Tilde{\lambda}=\frac{1}{4}$ and we get four coupled differential equations for the components of the spinor $\Psi$.
Using the gamma matrices
\begin{align*}
    \gamma^0&= \begin{pmatrix} 0 & \mathbb{I}_{2}\\ -\mathbb{I}_{2} & 0 \end{pmatrix}\\
    \gamma^i&= \begin{pmatrix} 0 & \sigma^i\\ \sigma^i & 0 \end{pmatrix}
\end{align*}
;
\begin{align}
    (f'(r)+f(r)\partial_r)\psi_4 + (\frac{\lambda_S}{r}+\frac{ieA_0}{f(r)})\psi_3+m\psi_1&=0\nonumber \\
    (f'(r)+f(r)\partial_r)\psi_3 + (\frac{\lambda_S}{r}+\frac{ieA_0}{f(r)})\psi_4+m\psi_2&=0\nonumber  \\
    (f'(r)+f(r)\partial_r)\psi_2 + (\frac{\lambda_S}{r}-\frac{ieA_0}{f(r)})\psi_1+m\psi_3&=0\label{eq:radial-Dirac-1} \\
    (f'(r)+f(r)\partial_r)\psi_1 + (\frac{\lambda_S}{r}-\frac{ieA_0}{f(r)})\psi_2+m\psi_4&=0.\nonumber
\end{align}
Which we can simplify and partially decouple with a linear combination
\begin{align*}
    &\chi_{1+}= \psi_4+\psi_3, \quad \chi_{2+}= \psi_2+\psi_1\\
    & \chi_{1-}= \psi_4-\psi_3, \quad \chi_{2-}= \psi_2-\psi_1.
\end{align*}
Taking the case of adding the equations we have
\begin{align*}
    (f'(r)+f(r)\partial_r)\chi_{1+} + (\frac{\lambda_S}{r}+\frac{ieA_0}{f(r)})\chi_{1+}+m\chi_{2+}&=0\\
    (f'(r)+f(r)\partial_r)\chi_{2+} + (\frac{\lambda_S}{r}-\frac{ieA_0}{f(r)})\chi_{2+}+m\chi_{1+}&=0.
\end{align*}

\subsection{Comments}

In the above analysis $\gamma^1$ has been associated with the $r$-direction.
This has the disadvantage that the transverse directions on the sphere are associated with $\gamma^2$ and $\gamma^3$, or $\sigma^2$ and $\sigma^3$. We therefore cannot use the form of the eigenspinorss in (\ref{eq:sphere-eigenspinors}), we would have to change the basis. 

An alternative choice of $\gamma$-matrices would be\footnote{This is not quite the same that of Liu et al, \cite{McGreevyetal}, who use ;
\[\gamma^0= \begin{pmatrix} 0 & i \sigma_2\\ i \sigma_2 & 0 \end{pmatrix},
\  \gamma^1 = \begin{pmatrix} 0 & \sigma_1  \\  \sigma_1& 0\end{pmatrix},\
    \gamma^2 = \begin{pmatrix} 0 & \sigma_3\\ \sigma_3 & 0 \end{pmatrix},\ 
\] and associate $\gamma^3$ with the radial direction.
They then set $k_2=0$, so only $\gamma^0$ and $\gamma^1$ are relevant.
In their notation this means that $\gamma^0$ and $\gamma^1$ interchange $y_+$ and
$y_-$ as well as $z_+$ and $z_-$.}
\begin{align*}
    \gamma^0&= \begin{pmatrix} 0 & i \sigma_{3}\\ i \sigma_{3} & 0 \end{pmatrix}
 &  \gamma^1&= \begin{pmatrix} {\mathbf 1} & 0 \\  0 & - {\mathbf 1}\end{pmatrix}\\
    \gamma^2&= \begin{pmatrix} 0 & \sigma_1\\ \sigma_1 & 0 \end{pmatrix} &
 \gamma^3&= \begin{pmatrix} 0 & \sigma_2\\ \sigma_2 & 0 \end{pmatrix}.
\end{align*}
\noindent Now $\gamma^1$ is associated with the $r$-direction and is diagonal while
$\gamma^2$ and $\gamma^3$ ($\sigma_1$ and $\sigma_2$) are associated with the transverse directions on the sphere (or plane) and we can use the eigenspinor in the form
(\ref{eq:sphere-eigenspinors}) (or (\ref{eq:plane-eigenspinors})).  Including an oscillatory time dependence, $\psi \rightarrow e^{-i\omega t}\psi$,
this has the effect of replacing (\ref{eq:radial-Dirac-1}) with
\begin{align}
    \partial_r(f \psi_1) - \Omega_-\psi_3+m\psi_1&=0\nonumber \\
    \partial_r(f \psi_2) + \Omega_+\psi_4+m\psi_2&=0\nonumber  \\
   -\partial_r(f \psi_3) - \Omega_-\psi_1+m\psi_3&=0\label{eq:radial-Dirac-2} \\
   -\partial_r(f \psi_4) + \Omega_+\psi_2+m\psi_4&=0.\nonumber
\end{align}
where 
\begin{equation}
\Omega_\pm(r) = \frac{\omega + e A_0}{f(r)} \pm \frac{\lambda_S}{\sqrt 2 r}.
\end{equation}
Since the eigenspinors on the sphere are 
$\begin{pmatrix}\phi_1(z)\\\phi_2(z) \end{pmatrix}$ we can set
\[\psi_1 = \eta_1(r) \phi_1(z),\quad
\psi_2 = \eta_2(r) \phi_2(z),\quad
\psi_1 = \eta_3(r) \phi_1(z),\quad
\psi_1 = \eta_4(r) \phi_4(z)\]
and all the $z$-dependence factors out,
\begin{align}
    \partial_r(f \eta_1) - \Omega_-\eta_3+m\eta_1&=0\nonumber \\
    \partial_r(f \eta_2) + \Omega_+\eta_4+m\eta_2&=0\nonumber  \\
   -\partial_r(f \eta_3) - \Omega_-\eta_1+m\eta_3&=0\label{eq:radial-Dirac-3} \\
   -\partial_r(f \eta_4) + \Omega_+\eta_2+m\eta_4&=0.\nonumber
\end{align}
For the planar case, using
\[ \Omega_\pm  = \frac{\omega + e A_0}{f(r)} \pm \lambda_P\]
with $\lambda_P=\sqrt{b n}$,
these should be completely equivalent to \cite{McGreevyetal}, albeit in a different basis, with $k= \sqrt{b n}$. Thus the presence of a magnetic field does not affect their analysis.  

We want to repeat their analysis for the spherical case.
This involves analysing the analogue of equations (17) and (18) in 
\cite{McGreevyetal} at large $r$ and extracting the matrix ${\cal S}$ in their equation (19) and solving the differential equations numerically to obtain $G_R$
(their analysis is based on \cite{Iqbal+Liu}).

\bigskip
\subsection{Separation of Variables}
To achieve the separation of variables for the above we apply the method from \cite{Villalba}. This will allow us to isolate the r-dependence in the spinor components.

\medskip

To begin with we review the layout of the dirac equation in our space-time. We are also going to adopt the action used in \cite{McGreevyetal} which looks like 
\begin{equation*}
\textbf{S} = \int d^{d}x\sqrt{-g} i \left( \bar{\Psi} \Dslash \Psi - m \bar{\Psi}\Psi \right).
\end{equation*}
Which gives the following equations of motion
\begin{align*}
    \Dslash \Psi -m\Psi &= \gamma^{a}(e^{-1})^{\mu}_{a}D_{\mu} \Psi -m\Psi = 0\nonumber \\
    &=\left(\gamma^{0}(e^{-1})^{t}_{0}D_{t} + \gamma^{1}(e^{-1})^{r}_{1}D_{r} + \gamma^{2}(e^{-1})^{\theta}_{2}D_{\theta} + \gamma^{3}(e^{-1})^{\phi}_{3}D_{\phi}\right)\Psi - m\Psi\nonumber \\
    &=\left(\frac{\gamma^{0}}{f(r)}D_{t} + \gamma^{1}f(r)D_{r} + \frac{\gamma^{2}}{r}D_{\theta} + \frac{\gamma^{3}}{r\sin(\theta)}D_{\phi}\right)\Psi - m\Psi\nonumber \\
\end{align*}
Each derivative component looks like 
\begin{align*}
       \gamma^{\mu}D_{\mu}=& \gamma^{a}(e^{-1})^{\mu}_{a}(\partial_{\mu}+\frac{1}{4}\gamma^{bc}(\omega_{bc})_{\mu}-iA_{\mu})\\
       \gamma^{t}D_{t}=& \frac{\gamma^{0}}{f(r)}(\partial_{t}+\frac{1}{4}\gamma^{bc}(\omega_{bc})_{t}-iA_{t})
       = \frac{1}{f(r)}\left(-i\gamma^{0}(\omega + A_{t}) + \frac{\gamma^{1}}{2}f'(r)f(r)\right)\\
       \gamma^{r}D_{r}=& \gamma^{1}f(r)\partial_{r}\\
       \gamma^{\theta}D_{\theta}=& \frac{\gamma^{2}}{r}(\partial_{\theta}+\frac{1}{4}\gamma^{bc}(\omega_{bc})_{\theta})= \frac{\gamma^{2}}{r}\partial_{\theta}+\frac{\gamma^{1}}{2r}f(r)\\
       \gamma^{\phi}D_{\phi}=& \frac{\gamma^{3}}{r\sin{\theta}}(\partial_{\phi}+\frac{1}{4}\gamma^{bc}(\omega_{bc})_{\phi}-iA_{\phi})\\
       =&\frac{1}{r\sin{\theta}}\left(\gamma^{3}(\partial_{\phi}-iA_\phi)+\frac{\gamma^{1}}{2}(f(r)\sin{\theta})+\frac{\gamma^{2}}{2}(\pm{1}-\cos{\theta})\right)\\
\end{align*}
Now we can gather the components of the dirac operator according to their gamma matrices. Note that we have replaced the partial derivative $\partial_{t}$ with the frequency $-i\omega$. 

We define \begin{equation*}
     \nabla_{r}:=f(r)\partial_{r}+\frac{f'(r)}{2}+\frac{f(r)}{r}
\end{equation*}
and can then rearrange our dirac equation, giving
\begin{multline}
    r(\Dslash \Psi -m\Psi)= \left(r\gamma^{1}\nabla_{r}-r\frac{i\gamma^{0}}{f(r)}(\omega+A_t)-mr\right)\Psi + \\
    \left(\gamma^{2}\left(\partial_{\theta}+\left(\frac{1}{\sin{\theta}}\frac{(\pm{1}-\cos{\theta})}{2}\right)\right)+\frac{\gamma^{3}}{\sin{\theta}}(\partial_{\phi}-iA_{\phi})\right)\Psi = 0 \label{rD}
\end{multline}
This is in keeping with the method outlined in \cite{Villalba}. To make the dirac equation separable we first have to split it in to two commuting operators, $K_1$ and $K_2$, such that they satisfy
\begin{equation}
    (K_1 + K_2)\Phi = 0. \label{op}
\end{equation}
We have already arranged the dirac equation above \eqref{rD} which has each operator only dependent on either the angular components or the radial components. This allows for the derivatives to commute. Following exactly the approach in \cite{Villalba} we choose  a $\Phi$ which is related to $\Psi$ via a basis change
\begin{equation*}
    \Psi = \gamma^0 \gamma^1 \Phi.
\end{equation*}
which allows the gamma matrices, which form part of each operator, to commute. With commuting operators we know that they share a common eigenvector and thus we can utilise equation \eqref{op} to write  
\begin{align}
    K_1 \Phi=&\left(r\gamma^{1}\nabla_{r}-r\frac{i\gamma^{0}}{f(r)}(\omega+A_t)-mr\right)\gamma^0 \gamma^1 \Phi  =k\Phi \label{op.1} \\
    K_2 \Phi=&\left(\gamma^{2}\left(\partial_{\theta}+\left(\frac{1}{\sin{\theta}}\frac{(\pm{1}-\cos{\theta})}{2}\right)\right)+\frac{\gamma^{3}}{\sin{\theta}}(\partial_{\phi}-iA_{\phi})\right) \gamma^0 \gamma^1 \Phi=-k\Phi \label{op.2}
\end{align}
giving us two equations, one in terms of the angular coordinates and one in terms of the radial. It is not difficult to check that these operators commute. Looking at each equation separately we can find the angular and radial dependence of the spinor. A further step that is made in \cite{Villalba} is to permute the gamma matrices using
\begin{equation*}
    a = \frac{1}{2}(\gamma^1 \gamma^2 - \gamma^1 \gamma^3 + \gamma^2 \gamma^3 + \mathbf{I_4})
\end{equation*}
This matrix commutes with $\gamma^0$ and acts on the other gamma matrices as follows
\begin{align*}
   a \gamma^1 =& \gamma^3 a \\
   a \gamma^3 =& \gamma^2 a \\
   a \gamma^2 =& \gamma^1 a \\
\end{align*}
Thus making another basis change for the spinor
\begin{equation*}
    \Phi = a^{-1} \Bar{\Phi}
\end{equation*}
Changes the equations \eqref{op.1} and \eqref{op.2} to 
\begin{align}
    K_1 \bar{\Phi}=&\left(r{\gamma^{3}}\nabla_{r}-r\frac{i{\gamma^{0}}}{f(r)}(\omega+A_t)-mr\right){\gamma^0 \gamma^3} \Bar{\Phi}  =k\Bar{\Phi} \label{op.3} \\
    K_2 \bar{\Phi}=&\left({\gamma^{1}}\left(\partial_{\theta}+\left(\frac{1}{\sin{\theta}}\frac{(\pm{1}-\cos{\theta})}{2}\right)\right)+\frac{{\gamma^{2}}}{\sin{\theta}}(\partial_{\phi}-iA_{\phi})\right) {\gamma^0 \gamma^3} \Bar{\Phi}=-k\Bar{\Phi} \label{op.4}
\end{align}
To make the equations separable the necessary choice of gamma matrices is
\begin{equation*}
    \gamma^0 = -i\sigma^3 \otimes \mathbf{I}_2 , \quad \gamma^1 = - \sigma^1 \otimes \sigma^2 , \quad \gamma^2 = \sigma^1 \otimes \sigma^1 , \quad \gamma^3 =  \sigma^1 \otimes \sigma^3
\end{equation*}
With 
\begin{equation*}
 \gamma^0 \gamma^3 = \sigma^2 \otimes \sigma^3    
\end{equation*}
\bigskip

Looking at equation \eqref{op.4} first we have 
\begin{align*}
   K_2 \Phi=& \left({-\sigma^1 \otimes \sigma^2}\left(\partial_{\theta}+\left(\frac{1}{\sin{\theta}}\frac{(\pm{1}-\cos{\theta})}{2}\right)\right)+\frac{{\sigma^1 \otimes \sigma^1}}{\sin{\theta}}(\partial_{\phi}-iA_{\phi})\right) {\sigma^2 \otimes \sigma^3} \Bar{\Phi}=-k\Bar{\Phi} \\
   =& \left({\sigma^3 \otimes \sigma^1}\left(\partial_{\theta}+\left(\frac{1}{\sin{\theta}}\frac{(\pm{1}-\cos{\theta})}{2}\right)\right)+\frac{{\sigma^3 \otimes \sigma^2}}{\sin{\theta}}(\partial_{\phi}-iA_{\phi})\right)\Bar{\Phi}=-k\Bar{\Phi}
\end{align*}
Our spinor can then be written as
\begin{equation}
    \Bar{\Phi} = \begin{pmatrix} h_{+}(r)\eta_{+} \\ h_{-}(r)\eta_{-} \end{pmatrix},
\end{equation}
where the $\eta$'s are the eigenspinors on the sphere which we found earlier and are related via
\begin{equation*}
    \sigma^3 \eta_+ = \eta_-
\end{equation*}
The above system of equations then becomes 
\begin{align*}
    \left({\sigma^1}\left(\partial_{\theta}+\left(\frac{1}{\sin{\theta}}\frac{(\pm{1}-\cos{\theta})}{2}\right)\right)+\frac{{\sigma^2}}{\sin{\theta}}(\partial_{\phi}-iA_{\phi})\right)\eta_{+}=&-k\eta_{+} \\
    -\left({\sigma^1}\left(\partial_{\theta}+\left(\frac{1}{\sin{\theta}}\frac{(\pm{1}-\cos{\theta})}{2}\right)\right)+\frac{{\sigma^2}}{\sin{\theta}}(\partial_{\phi}-iA_{\phi})\right)\eta_{-}=&-k\eta_{-}
\end{align*}
Where the operator in front is just the dirac operator on the sphere
\begin{align*}
    \Dslash_{2} \eta_{+} =& -i\lambda \eta_{+} = -k\eta_{+} \\
    -\Dslash_{2} \eta_{-} =& -i\lambda \eta_{-} = -k\eta_{-}
\end{align*}
Where $\lambda_s$ are the eigenvalues worked out in section 3. A thing to note here is that now our $k$'s are not real. Which indicates that our operators $K_1$ and $K_2$ are not hermitian. I'm not sure what problems this causes. 

\newpage
Now looking at the radial part.
With our specific choice of gamma matrices equation \eqref{op.3} becomes 
\begin{align*}
     K_1 \Phi=&\left(r{\sigma^1 \otimes \sigma^3}\nabla_{r}-r\frac{({\sigma^3 \otimes \mathbf{I}_2})}{f(r)}(\omega+A_t)-mr\right){\sigma^2 \otimes \sigma^3} \Bar{\Phi}  =k\Bar{\Phi} \\
     =& \left(r(i{\sigma^3 \otimes \mathbf{I}_2})\nabla_{r}+r\frac{i{\sigma^1 \otimes \sigma^3}}{f(r)}(\omega+A_t)-mr({\sigma^2 \otimes \sigma^3})\right)\Bar{\Phi}  =k\Bar{\Phi} \\
 -\frac{i}{r}K_1    =& \left(({\sigma^3 \otimes \mathbf{I}_2})\nabla_{r}+\frac{{\sigma^1 \otimes \sigma^3}}{f(r)}(\omega+A_t)+m({i\sigma^2 \otimes \sigma^3})\right)\Bar{\Phi}  =-\frac{ik}{r}\Bar{\Phi}.
\end{align*}
Inserting the above form for our spinor this becomes two equations
\begin{align}
    \nabla_{r}(h_{+}(r)\eta_{+})+\left(\frac{{1}}{f(r)}(\omega+A_t)+m\right)({\sigma^3})(h_{-}(r)\eta_{-})  =& \label{eq.3} -\frac{ik}{r}(h_{+}(r)\eta_{+}) \\
    -\nabla_{r}(h_{-}(r)\eta_{-})+\left(\frac{{1}}{f(r)}(\omega+A_t)-m\right)({\sigma^3})(h_{+}(r)\eta_{+})  =& \label{eq.4} -\frac{ik}{r}(h_{-}(r)\eta_{-})
\end{align}
and using the relation between the $\eta$'s we have 
\begin{equation}
    (\nabla_{r} \pm \frac{ik}{r})h_{\pm} = \left(m \mp \frac{(\omega+A_t)}{f(r)}\right)h_{\mp} \label{eq.6}
\end{equation}
%\begin{comment} 
This equation can be further simplified, as in \cite{McGreevyetal}, by substituting 
\begin{equation*}
    h_{\pm}= \frac{g_{\pm}}{r\sqrt{f(r)}}
\end{equation*}
which gives
\begin{equation}
     (\partial_{r} \pm \frac{ik}{rf})g_{\pm} =  \Omega(r) g_{\mp} \label{r.1}
\end{equation}
Where 
\begin{equation*}
    \Omega(r) = \frac{1}{f}\left(m \mp \frac{(\omega+A_t)}{f} \right)
\end{equation*}
Equation \eqref{r.1} could be further simplified by making the substitution
\begin{equation*}
    g_{\pm}= c_{\pm}e^{\mp ik\int^{r}(\frac{d\tilde{r}}{\tilde{r}f(\tilde{r})})} \phi_{\pm}
\end{equation*}
Which turns the above into 
\begin{align*}
   \phi'_{\pm}= \mp \tilde{\Omega}(r) \phi_{\mp}
\end{align*}
with $\tilde{\Omega} = \frac{c_{\mp}}{c_{\pm}}\Omega(r) e^{\pm{2} ik\int^{r}(\frac{d\tilde{r}}{\tilde{r}f})}$. This allows us to decouple the equations fairly nicely giving
\begin{align*}
    \phi''_{\pm}=& \mp(\tilde{\Omega'}\phi_{\mp} + \tilde{\Omega}\phi'_{\mp}) \\
    \phi''_{\pm} =& \frac{\tilde{\Omega'}}{\tilde{\Omega}} \phi'_{\pm} - (\tilde{\Omega})^{2} \phi_{\pm} 
\end{align*} 
which can be rewritten as
\begin{equation*}
    \frac{d}{dr} (\frac{\phi'_{\pm}}{\tilde{\Omega}}) + \tilde{\Omega} \phi_{\pm} = 0
\end{equation*}
Which looks reasonably more workable. What we can actually do here is to redefine
\begin{equation*}
    \frac{\phi'_{\pm}}{\tilde{\Omega}} = \frac{1}{p(r)}
\end{equation*}
and our above equation becomes
\begin{align*}
    \frac{1}{p}\frac{d}{dr}(\frac{1}{p})+ \phi'_{\pm}\phi_{\pm}=& 0 \\
    = \frac{1}{2}\frac{d}{dr}(\frac{1}{p^2}) + \frac{1}{2}\frac{d}{dr}((\phi_{\pm})^2) =& 0 \\
\rightarrow \frac{1}{p^2} + (\phi_{\pm})^2 =& c_1 \\
\intertext{which gives}
    ( \frac{\phi'_{\pm}}{\tilde{\Omega}})^2 + (\phi_{\pm})^2 =& c_1
\intertext{and this has a solution of the form}
\phi_{\pm}= \sqrt{c_1}\cos{(q(r)+\delta)}& 
\end{align*}
Where $\frac{d}{dr}(q(r))= \tilde{\Omega}$, $\delta$ is an arbitrary phase and $c_1$ is a constant.
The full radial functions then look like 
\begin{equation}
    h_{\pm} = \frac{c_{\pm}e^{\mp ik\int^{r}(\frac{d\tilde{r}}{\tilde{r}f(\tilde{r})})}}{r\sqrt{f}}\left(\sqrt{c_1}\cos{(q(r)+\delta)}\right)
\end{equation}
Now we can check this for the case of a flat space time, $f(r)=1$. We will make our life easier by looking only at $h_{+}$. To get out $q(r)$ for this case we need to first simplify $\tilde{\Omega}$ 
\begin{align*}
   \tilde{\Omega} =& \frac{c_{-}}{c_{+}}\left(m - (\omega + \frac{\alpha}{r})\right) e^{ 2ik \int^{r} \frac{d\tilde{r}}{\tilde{r}}}\\
   =& c_0\left(m - (\omega + \frac{\alpha}{r})\right) r^{2ik}
\intertext{Where $c_0 = \frac{c_{-}}{c_{+}} e^{2ikc_2}$, $c_2$ is a constant of integration and $A_t = \frac{\alpha}{r}$}
   q(r) =& c_0 r^{2ik}\left( \frac{(m-\omega)r}{2ik+1} -\frac{\alpha}{2ik}\right) + \text{const}.
\end{align*}
Our radial functions for the flat geometry then are 
\begin{equation}
    h_{+} = \tilde{c_{+}}r^{-ik}\cos\left( c_0 r^{2ik}\left( \frac{(m-\omega)r}{2ik+1} -\frac{\alpha}{2ik}\right)+\delta'\right)
\end{equation}
where we have absorbed integration constants into the $\tilde{c_{+}}$ and $\delta$. We can obtain the functions in a flat geometry without a Coulomb potential by setting $\alpha $ to zero. 
%\end{comment}
\subsection{General solution}
The above solutions are fine given the initial form of the chosen spinor but a more complete set of solutions can be found using
\begin{equation}
\bar{\Phi} =
 \begin{pmatrix}
     G_{+}(r) (\eta_{+}) +  G_{-}(r)( \eta_{-}) \\
     F_{+}(r) (\eta_{+}) +  F_{-}(r)( \eta_{-})
 \end{pmatrix}, \label{eq.1}
\end{equation}
Here we are following the approach found in \cite{itzykson2012quantum} and \cite{bjorken2013relativistic} when looking for  solutions to dirac equation for the hydrogen atom. Given the way in which we have split our Dirac operator in to two parts we are looking for solutions to 
\begin{equation}
    K_1 \bar{\Phi} = -K_2 \bar{\Phi} \label{eq.2}
\end{equation}
whereby we are deviating from the approach in \cite{Villalba}. 

For the right hand side we know that, with our specific choice of gamma matrices, the form of the operator $K_2$ contains the dirac operator on the sphere 
\begin{equation*}
    K_2 = (\sigma_{3} \otimes \Dslash_{2}).
\end{equation*}
Which when acted on \eqref{eq.1} we find 
\begin{align}
  K_2 \bar{\Phi} &=  \begin{pmatrix}
     \Dslash_2(G_{+}(r) (\eta_{+}) +  G_{-}(r)( \eta_{-})) \\
     -\Dslash_2(F_{+}(r) (\eta_{+}) +  F_{-}(r)( \eta_{-}))
 \end{pmatrix} \\
 &= \begin{pmatrix}
     G_{+}(r) (-i\lambda \eta_{+}) +  G_{-}(r)(i\lambda \eta_{-}) \\
     F_{+}(r) (i\lambda \eta_{+}) +  F_{-}(r)(-i\lambda \eta_{-})
     \end{pmatrix} \\
&=  -i\lambda \begin{pmatrix}
     G_{+}(r) (\eta_{+}) -  G_{-}(r)( \eta_{-}) \\
     F_{-}(r) (\eta_{-}) -  F_{+}(r)( \eta_{+})
 \end{pmatrix} \label{eq.5}
\end{align}
Now for the left hand side of equation \eqref{eq.2} we find that we need only substitute in to equation \eqref{eq.3} and \eqref{eq.4} with the components of \eqref{eq.1} above and replacing what is on the other side of the equals with \eqref{eq.5}. 
\begin{align*}
    r\nabla_{r}(G_{+}(r) (\eta_{+}) +  G_{-}(r)( \eta_{-})) + r\Omega_{+}({\sigma^3})(F_{+}(r) (\eta_{+}) +  F_{-}(r)( \eta_{-}))  =& \lambda(G_{+}(r) (\eta_{+}) -  G_{-}(r)( \eta_{-})) \\
   -r\nabla_{r}(F_{+}(r) (\eta_{+}) +  F_{-}(r)( \eta_{-})) + r\Omega_{-}({\sigma^3})(G_{+}(r) (\eta_{+}) +  G_{-}(r)( \eta_{-}))  =& \lambda(F_{-}(r) (\eta_{-}) -  F_{+}(r)( \eta_{+}))
\end{align*}
Where 
\begin{equation}
    \Omega_{\pm} = \left( \frac{\omega + A_t}{f(r)} \pm m\right)
\end{equation}
Noting the relation between the two component spinors on the sphere 
\begin{equation*}
    \sigma^{3}\eta_{\pm} = \eta_{\mp}
\end{equation*}
We find four equations for four radial functions. A linear combination of the above equations can decouple these as follows
\begin{align*}
    r\nabla_{r}(G_{+} (\eta_{+}) +  G_{-}\sigma^{3}( \eta_{+})) + r\Omega_{+}(F_{+} \sigma^{3} (\eta_{+}) +  F_{-}( \eta_{+}))  =& \lambda(G_{+} (\eta_{+}) -  G_{-}\sigma^{3}( \eta_{+})) \\
   -r\nabla_{r}(F_{+} (\eta_{+}) +  F_{-}\sigma^{3}( \eta_{+})) + r\Omega_{-}(G_{+} \sigma^{3}(\eta_{+}) +  G_{-}( \eta_{+}))  =& \lambda(F_{-} \sigma^{3}(\eta_{+}) -  F_{+}( \eta_{+}))
\end{align*}
Which becomes
\begin{align}
    r\nabla_{r}(G_{+} +  G_{-}) + r\Omega_{+}(F_{+} +  F_{-})  =& \lambda(G_{+} -  G_{-}) \\
    r\nabla_{r}(G_{+} - G_{-}) + r\Omega_{+}(F_{-} -  F_{+})  =& \lambda(G_{+} +  G_{-})\\
   -r\nabla_{r}(F_{+} +  F_{-}) + r\Omega_{-}(G_{+} +  G_{-})  =& \lambda(F_{-} -  F_{+}) \\
   -r\nabla_{r}(F_{+} -  F_{-}) + r\Omega_{-}(G_{-} -  G_{+})  =& \lambda(-F_{-} -  F_{+})
\end{align}
It is straightforward to then take linear combinations of these equations to give 
\begin{align}
    (\nabla_{r}-\frac{\lambda}{r})G_{+} + \Omega_{+}(F_{-})  =& 0 \label{eq.7}\\
    (\nabla_{r}+\frac{\lambda}{r})G_{-} + \Omega_{+}(F_{+})  =& 0\\
   (\nabla_{r} - \frac{\lambda}{r})F_{+} - \Omega_{-}(G_{-})  =& 0 \\
   (\nabla_{r} + \frac{\lambda}{r})F_{-} - \Omega_{-}(G_{+})  =& 0. \label{eq.8}
\end{align}
We can see that these functions are coupled to one another in a nearly identical way to equation \eqref{eq.6} whereby if we relabel our $F$'s and $G$'s like so 
\begin{align*}
    G_{+} &= \psi_{+}, \ F_{-} = \psi_{-} \\
    G_{-} &= \varphi_{-}, \ F_{+} = \varphi_{+}
\end{align*}
we have 
\begin{align}
    (\nabla_{r} \mp \frac{\lambda}{r})\psi_{\pm} =& \mp \Omega_{\pm}(\psi_{\mp}) \label{eq.9} \\ 
    (\nabla_{r} \mp \frac{\lambda}{r})\varphi_{\pm} =& \pm \Omega_{\mp}(\varphi_{\mp}). \label{eq.10}
\end{align}
It makes sense that they should decouple in this way given that the initial approach by  Villalba in \cite{Villalba} was to use the fact that $K_1$ and $K_2$ commute, thus making them simultaneously diagonalisable, and to choose a basis whereby 
\begin{equation*}
    K_1 \bar{\Phi} = k \bar{\Phi} \quad \text{ and } \quad K_2 \bar{\Phi} = -k \bar{\Phi}
\end{equation*}
gives solutions of the form 
\begin{align*}
    \bar{\Phi} &= \begin{pmatrix} G_{+} \eta_{+} \\ F_{-}\eta_{-} \end{pmatrix} \\
    \bar{\Phi} &= \begin{pmatrix} G_{-} \eta_{-} \\ F_{+}\eta_{+} \end{pmatrix}.
\end{align*}
The above choice in this subsection is then the most general solution, i.e. a linear combination of these two spinors. 

A way to check that our equations above are correct is to compare them to the well known case of the Dirac equation for the hydrogen atom. We should look for agreement with the equation (2-93) found in \cite{itzykson2012quantum} on p.78. To do so we first must make a substitution 
\begin{equation}
G_{\pm} = \frac{\tilde{G}_{\pm}}{r} \ \text{ and } \ F_{\pm} = \frac{\tilde{F}_{\pm}}{r} 
\end{equation}
as the ansatz made in \cite{itzykson2012quantum} differs from ours above in this way. Then setting $f(r) = 1$ and grouping the $G$'s and $F$'s together, whereby \eqref{eq.7} - \eqref{eq.8} become
\begin{align}
    (\frac{d}{dr} +\frac{1}{r}\mp \frac{\lambda}{r})\frac{\tilde{G}_{\pm}}{r} + \Omega_{+}(\frac{\tilde{F}_{\mp}}{r})  =& 0 \\
   (\frac{d}{dr} +\frac{1}{r} \mp \frac{\lambda}{r})\frac{\tilde{F}_{\pm}}{r} - \Omega_{-}(\frac{\tilde{G}_{\mp}}{r})  =& 0.
\end{align}
Multiplying through by $r$ and differentiating we arrive at 
\begin{align}
    -\frac{d\tilde{G}_{\pm}}{dr} \pm (\lambda)\frac{\tilde{G}_{\pm}}{r} &= (\omega + m + A_t)\tilde{F}_{\mp} \\
   \frac{d\tilde{F}_{\pm}}{dr} \mp (\lambda)\frac{\tilde{F}_{\pm}}{r} &= (\omega -m + A_t)\tilde{G}_{\mp}.
\end{align}
We find that these are the equations found in \cite{itzykson2012quantum}. To see this we send $m \rightarrow -m$ and set 
\begin{equation}
\tilde{G}_{\mp} = F_{lj}  \ \text{ and } \ \tilde{F}_{\pm} = G_{lj}.
\end{equation} Our $\lambda = \pm \sqrt{n(n+|m|)}$ is related to the total angular momentum in \cite{itzykson2012quantum} when we set the magnetic charge $|m|$ (distinct from the above $m$) to zero 
\begin{align*}
    n &= J + \frac{1-|m|}{2}, \quad \text{ from } \eqref{j.1} \\
    m=0 \ \rightarrow \lambda &= \pm n = \pm(J +\frac{1}{2})
\end{align*}
So our equations are consistent with those in \cite{itzykson2012quantum}.

\medskip

To simplify the above equations \eqref{eq.9} and \eqref{eq.10} we follow a similar approach to that found in \cite{McGreevyetal} where we make the substitution
\begin{align*}
    \psi_{\pm} &= \frac{\tilde{\psi}_{\pm}}{r\sqrt{f}} \\
    \varphi_{\pm} &= \frac{\tilde{\varphi}_{\pm}}{r\sqrt{f}},
\end{align*}
which cancels the functions of $r$ found in $\nabla_r$. \eqref{eq.9} and \eqref{eq.10} become 
\begin{align}
    (\partial_{r} \mp \frac{\lambda}{rf(r)})\tilde{\psi}_{\pm} =& \mp \frac{\Omega_{\pm}}{f(r)}(\tilde{\psi}_{\mp}) \\ 
    (\partial_{r} \mp \frac{\lambda}{rf(r)})\tilde{\varphi}_{\pm} =&  \pm \frac{\Omega_{\mp}}{f(r)}(\tilde{\varphi}_{\mp}). 
\end{align}
To decouple these so that we have a set of 2nd order ODE's we need to rearrange the above slightly.
\begin{align}
(\partial_{r} \mp \frac{\lambda}{rf(r)})\tilde{\psi}_{\pm} &= \mp \frac{\Omega_{\pm}}{f(r)}(\tilde{\psi}_{\mp}) \\
(f(r)\partial_{r} \mp \frac{\lambda}{r})\tilde{\psi}_{\pm} &= \mp \Omega_{\pm}(\tilde{\psi}_{\mp}) \label{eq.11} \\
(\mp \Omega_{\pm})^{-1}(f(r)\partial_{r} \mp \frac{\lambda}{r})\tilde{\psi}_{\pm} &= (\tilde{\psi}_{\mp}) \\
(\tilde{\psi}_{\pm}) &= (\pm \Omega_{\mp})^{-1}(f(r)\partial_{r} \pm \frac{\lambda}{r})\tilde{\psi}_{\mp} \label{eq.12}.
\end{align}
Now subbing equation \eqref{eq.12} into \eqref{eq.11} we have
\begin{align*}
    &(f(r)\partial_{r} \mp \frac{\lambda}{r})\left((\pm \Omega_{\mp})^{-1}(f(r)\partial_{r} \pm \frac{\lambda}{r})\tilde{\psi}_{\mp}\right) = \mp \Omega_{\pm}(\tilde{\psi}_{\mp}) \\
    &f(r)\partial_{r} \left((\pm \Omega_{\mp})^{-1}(f(r)\partial_{r} \pm \frac{\lambda}{r})\tilde{\psi}_{\mp}\right) - \frac{\lambda}{r\Omega_{\mp}}(f(r)\partial_{r} \pm \frac{\lambda}{r})\tilde{\psi}_{\mp} = \mp\Omega_{\pm}(\tilde{\psi_{\mp}}) \\
    &f(r)\left[\left(\frac{\mp\Omega_{\mp}'}{(\Omega_{\mp})^{2}}\right)(f(r)\partial_r \pm \frac{\lambda}{r})\tilde{\psi}_{\mp} + (\pm \Omega_{\mp})^{-1}(f'\partial_{r} \mp \frac{\lambda}{r^2})\tilde{\psi}_{\mp} + (\pm \Omega_{\mp})^{-1}(f\partial_{r} \pm \frac{\lambda}{r})\partial_r \tilde{\psi}_{\mp} \right] \\ &- \frac{\lambda}{r\Omega_{\mp}}(f(r)\partial_{r} \pm \frac{\lambda}{r})\tilde{\psi}_{\mp} = \mp\Omega_{\pm}(\tilde{\psi_{\mp}}) \\
    &f(r)\left[\left(\frac{\Omega_{\mp}'}{(\Omega_{\mp})}\right)(f(r)\partial_r \pm \frac{\lambda}{r})\tilde{\psi}_{\mp} - (f'\partial_{r} \mp \frac{\lambda}{r^2})\tilde{\psi}_{\mp} - (f\partial_{r} \pm \frac{\lambda}{r})\partial_r \tilde{\psi}_{\mp} \right]  \pm \frac{\lambda}{r}(f(r)\partial_{r} \pm \frac{\lambda}{r})\tilde{\psi}_{\mp} = \Omega_{\mp}\Omega_{\pm}(\tilde{\psi_{\mp}}) \\
    &f(r)\left[\left(\frac{\Omega_{\mp}'}{(\Omega_{\mp})}\right)(f(r)\partial_r \pm \frac{\lambda}{r})\tilde{\psi}_{\mp} - (f'\partial_{r} \mp \frac{\lambda}{r^2})\tilde{\psi}_{\mp} - f\partial_{r}^{2}\tilde{\psi}_{\mp} \right] + (\frac{\lambda}{r})^{2}\tilde{\psi}_{\mp} = \Omega_{\mp}\Omega_{\pm}(\tilde{\psi_{\mp}})
\end{align*}
multiplying through by a minus, using the definition of $\Omega_{\pm}$, and dropping the $\pm$ from the derivative of $\Omega$ as it doesn't depend on the fermion mass, the final line in the above set of equations becomes

\begin{equation*}
    (f^{2})\partial_{r}^{2}\tilde{\psi}_{\pm} + (f' - \frac{\Omega'}{\Omega_{\pm}}f)(f)\partial_{r}\tilde{\psi}_{\pm} \pm\frac{\lambda }{r}(\frac{\Omega'}{\Omega_{\pm}}f + \frac{f}{r})\tilde{\psi}_{\pm} + \left(\frac{(\omega + A_{t})^{2}}{f^2} -m^2 +(\frac{\lambda}{r})^{2} \right) (\tilde{\psi_{\pm}}) = 0.
\end{equation*}
We want to tidy this further to get a look at the equation we're going to solve numerically. To do this we'll expand out the $\Omega$ functions 
\begin{align}
    \Omega_{\pm} &= \left( \frac{\omega + \frac{qQ_{e}}{r}}{f(r)} \pm m\right) \\
    &= \frac{1}{f}\left( \omega + \frac{qQ_{e}}{r} \pm mf\right)\\
     \Omega' &= \frac{-1}{f^2}\left(\frac{qQ_{e}}{r^2}f + (\omega + \frac{qQ_{e}}{r})f' \right) \\
    \frac{\Omega'}{\Omega_{\pm}} &= \frac{-1}{f}\frac{(\frac{qQ_{e}}{r^2}f + (\omega + \frac{qQ_{e}}{r})f')}{( \omega + \frac{qQ_{e}}{r} \pm mf)}
\end{align}

working with the terms in the O.D.E. that contain $\Omega$'s we have

\begin{align}
    (f'- \frac{\Omega'}{\Omega_{\pm}}f) &= \frac{\frac{qQ_{e}}{r^2}f + 2(\omega + \frac{qQ_{e}}{r})f' + \pm m ff'}{ \omega + \frac{qQ_{e}}{r} \pm mf} \\
    & = \frac{ 2\omega f' + \frac{qQ_{e}}{r}(2f' + \frac{f}{r})  \pm m ff'}{ \omega + \frac{qQ_{e}}{r} \pm mf} \\
    ( \frac{f}{r} + \frac{\Omega'}{\Omega_{\pm}}f) &= \frac{1}{r}\left( \frac{ f(\omega + \frac{qQ_{e}}{r} \pm mf) -r(\frac{qQ_{e}}{r^2}f + (\omega + \frac{qQ_{e}}{r})f')}{ \omega + \frac{qQ_{e}}{r} \pm mf} \right) \\
    &= \frac{1}{r}\left( \frac{\omega(f-rf') - qQ_{e}f' \pm m f^2)}{ \omega + \frac{qQ_{e}}{r} \pm mf} \right)
\end{align}

Calling the denominator of the above two expressions $h(r)$ and denoting derivatives w.r.t. $r$ with primes our O.D.E. becomes

\begin{multline}
    (f^{2})\tilde{\psi}_{\pm}'' + \frac{f}{h}\left(2\omega f' + \frac{qQ_{e}}{r}(2f' + \frac{f}{r})  \pm m ff'\right)\tilde{\psi}_{\pm}' +\\ 
     \left[ \frac{(\omega + \frac{qQ_{e}}{r})^{2}}{f^2} -m^2 +(\frac{\lambda}{r})^{2} \pm\frac{\lambda }{r^2 h}\left(\omega(f-rf') - qQ_{e}f' \pm m f^2\right) \right] (\tilde{\psi_{\pm}}) = 0. \label{eq.13}
\end{multline}

This is the general equation for any space-time with function $f(r)$ and a central potential.

\subsection{Asymptotic ADS}

The function we're interested in so as to exploit the properties of the ADS/CFT correspondence is 
\begin{equation}
    f(r)^2 = k-\frac{2M}{r} + \left(\frac{Q}{r}\right)^2 + \left( \frac{r}{L} \right)^2.
\end{equation}

We have set $G = 1$ and $c=1$. $M$ here is the mass of the black hole. Here $k$ can either be $0$ or $1$, depending on whether we want a planar or spherical event horizon respectively. $Q^2 = Q_{e}^2 + Q_{m}^2$ is the combined charges for the electric and magnetic magnetic fields. It is convenient to write the mass of the black hole in terms of the event horizon radius $r_{h}$

\begin{equation}
    \frac{2M}{r_{h}} = k + \left(\frac{Q}{r_{h}}\right)^2 + \left( \frac{r_{h}}{L} \right)^2
\end{equation}

which gives

\begin{align}
    f(r)^2 &= k(1-\frac{r_{h}}{r}) + Q^2(\frac{1}{r^2} - \frac{1}{r_{h}}r) + \frac{1}{L^2}(r^2 - \frac{r_{h}^3}{r}) \\
    &= k(1-\frac{r_{h}}{r}) + \tilde{Q}^2((\frac{r_{h}}{r})^2 - \frac{r_{h}}{r}) + \frac{r_{h}^2}{L^2}((\frac{r}{r_{h}})^2 - \frac{r_{h}}{r})
\end{align}

Where $\tilde{Q} = \frac{Q}{r_{h}}$. From this we can also calculate the Hawking temperature 
\begin{equation}
    T_{H} = \frac{|(f(r_{h})^2)'|}{4\pi} = \frac{1}{4\pi r_{h}}(k + \frac{3 r_{h}^2}{L^2} - (\tilde{Q})^2)
\end{equation}
which we can see has zero temperature for $\tilde{Q} = \sqrt{k + \frac{3 r_{h}^2}{L^2}}$.
Making the substitution $z = \frac{r_{h}}{r}$ (which puts our horizon $z_{h} = 1$) we have 

\begin{align}
   f(z)^2 &= k(1-z) + \tilde{Q}^2(z^2 - z) + \frac{r_{h}^2}{L^2}((\frac{1}{z^2}) - z) \\
   &= \frac{1}{z^2}\left(k(z^2-z^3) + \tilde{Q}^2(z^4 - z^3) + \frac{r_{h}^2}{L^2}(1 - z^3)\right) \\ 
   &= \frac{1}{z^2}\left(kz^2(1-z) - \tilde{Q}^2 z^3(1 - z) + \frac{r_{h}^2}{L^2}(1 - z)(1+z+z^2)\right)\\
   &= \frac{(1-z)}{z^2}\left(kz^2 - \tilde{Q}^2z^3 + \frac{r_{h}^2}{L^2} (1+z+z^2)\right). \label{eq.25}
\end{align}
This form will make it easier to calculate numerically the functions for the above o.d.e. as our boundary is now at $z=0$. The factor of $\frac{1}{z^2}$ has been taken out as it will be useful for the substitution. We will need to calculate the derivatives with respect to $z$ for the change of variable. We will denote derivatives with respect to $z$ with a dot

\begin{align}
    \tilde{\psi}_{\pm}' &= -(\frac{z^2}{r_h})\dot{\tilde{\psi}}_{\pm} \label{eq.24} \\
    \tilde{\psi}_{\pm}'' &= \frac{z^3}{r_{h}^2}(2\dot{\tilde{\psi}}_{\pm} +z\ddot{\tilde{\psi}}_{\pm}) \\ 
    f' &= -(\frac{z^2}{r_h}) \dot{f}
\end{align}

and putting these expressions in to \eqref{eq.13} we have

\begin{multline}
    (f^{2})\frac{z^3}{r_{h}^2}(2\dot{\tilde{\psi}}_{\pm} +z\ddot{\tilde{\psi}}_{\pm}) - \frac{f}{h}\left(2\omega (-(\frac{z^2}{r_h}) \dot{f}) + \frac{qQ_{e}z}{r_h}(2(-(\frac{z^2}{r_h}) \dot{f}) + \frac{fz}{r_h})  \pm m f(-(\frac{z^2}{r_h}) \dot{f})\right)(\frac{z^2}{r_h})\dot{\tilde{\psi}}_{\pm} +\\ 
     \left[ \frac{(\omega + \frac{qQ_{e}z}{r_h})^{2}}{f^2} -m^2 +(\frac{\lambda z}{r_h})^{2} \pm\frac{\lambda z^2}{r_{h}^2 h}\left(\omega(f-(\frac{r_h}{z})(-(\frac{z^2}{r_h}) \dot{f})) - qQ_{e}(-(\frac{z^2}{r_h}) \dot{f}) \pm m f^2\right) \right] (\tilde{\psi_{\pm}}) = 0
\end{multline}

which we can rearrange a little in to 

\begin{multline}
    (zf)^2(\frac{z}{r_h})^2\ddot{\tilde{\psi}}_{\pm}+ ((zf)^{2}\frac{2z}{r_{h}^2}\dot{\tilde{\psi}}_{\pm})  + \frac{1}{h r_{h}^2}\left(2z\omega (zf)z^2 \dot{f} + \frac{qQ_{e}z^2}{r_h}(2 (zf) z^2 \dot{f} - (zf)^2)  \pm m (zf)^2(z^2 \dot{f})\right)\dot{\tilde{\psi}}_{\pm} +\\ 
     \left[ \frac{(\omega + \frac{qQ_{e}z}{r_h})^{2}}{f^2} -m^2 +(\frac{\lambda z}{r_h})^{2} \pm\frac{\lambda }{r_{h}^2 h}\left(\omega z(zf+ z^2\dot{f}) + \frac{qQ_{e}z^2}{r_h}(z^2 \dot{f}) \pm m z^2 f^2\right) \right] (\tilde{\psi_{\pm}}) = 0. \label{ads.1}
\end{multline}

Recall that 
\begin{align}
    f(z) &= \sqrt{k(1-z) + \tilde{Q}^2(z^2 - z) + \frac{r_{h}^2}{L^2}((\frac{1}{z^2}) - z)} \\
    & = \frac{1}{z} \sqrt{k(z^2-z^3) + \tilde{Q}^2(z^4 - z^3) + \frac{r_{h}^2}{L^2}(1 - z^3)}    
\intertext{labelling the square root function as $\tilde{f}(z)$ such that}
    zf(z)&= \tilde{f}(z)    
\intertext{and looking at the derivative}
    \dot{(f^2)} &= -k + \tilde{Q}^2(2z-1) -(\frac{r_h}{L})^2(\frac{2}{z^3}+1) \\
    &= \frac{1}{z^3}\left(-kz^3 + \tilde{Q}^2(2z^4-z^3) -(\frac{r_h}{L})^2(2+z^3)\right) \\
    &= \frac{g(z)}{z^3}    
\intertext{thus}
    \dot{f} &= \frac{\dot{(f^2)}}{2f} = \frac{g(z)}{2 z^3 f} = \frac{g(z)}{2 z^2 \tilde{f}} \\
    2\tilde{f}z^2\dot{f} &= g(z).
\end{align}
Substituting these in to \eqref{ads.1} we have 

\begin{multline}
    (\tilde{f})^2(\frac{z}{r_h})^2\ddot{\tilde{\psi}}_{\pm}+ ((\tilde{f})^{2}\frac{2z}{r_{h}^2}\dot{\tilde{\psi}}_{\pm})  + \frac{1}{h r_{h}^2}\left(\omega z g(z) + \frac{qQ_{e}z^2}{r_h}(g(z) - (\tilde{f})^2)  \pm m \tilde{f}(\frac{g(z)}{2})\right)\dot{\tilde{\psi}}_{\pm} +\\ 
     \left[ \frac{(\omega z + \frac{qQ_{e}z^2}{r_h})^{2}}{\tilde{f}^2} -m^2 +(\frac{\lambda z}{r_h})^{2} \pm\frac{\lambda }{r_{h}^2 h}\left(\frac{\omega z}{\tilde{f}}(\tilde{f}^2+ \frac{g(z)}{2}) + \frac{qQ_{e}z^2}{r_h}(\frac{g(z)}{2\tilde{f}}) \pm m \tilde{f}^2\right) \right] (\tilde{\psi_{\pm}}) = 0.
\end{multline}
multiplying through with the square of the horizon radius and tidying up the coefficients of the first derivative of $\tilde{\psi}$ with $h(z) = \frac{1}{z}(\omega z + \frac{qQ_{e}z^2}{r_h} + m\tilde{f})$ we get

\begin{multline}
    (\tilde{f})^2z^2\ddot{\tilde{\psi}}_{\pm}  + \frac{1}{h}\left(\omega z(2(\tilde{f})^{2} + g(z)) + \frac{qQ_{e}z^2}{r_h}(g(z) + (\tilde{f})^2)  + m \tilde{f}(2\tilde{f}^{2} \pm \frac{g(z)}{2})\right)\dot{\tilde{\psi}}_{\pm} +\\ 
     \left[ \frac{(\omega zr_h + qQ_{e}z^2)^{2}}{\tilde{f}^2} -(mr_h)^2 +(\lambda z)^{2} \pm\frac{\lambda}{h}\left(\frac{\omega z}{2\tilde{f}}(2\tilde{f}^2 + g(z)) + \frac{qQ_{e}z^2}{r_h}(\frac{g(z)}{2\tilde{f}}) \pm m \tilde{f}^2\right) \right] (\tilde{\psi_{\pm}}) = 0.
\end{multline}

Using the definitions of $\tilde{f}^2 (z)$ and $g(z)$, which are just polynomials in $z$, the combinations of the two which appear in the O.D.E are as follows

\begin{align*}
(z^2)p_{1}(z)&= 2\tilde{f}^2(z) + g(z) = z^2 \left(k(2-3z) +\tilde{Q}^2 (4z^2 -3z) -\left(\frac{r_{h}}{L}\right)^2 (3z)  \right) \\ \label{eq.15}
p_{2}(z)&= \tilde{f}^2 + g = k(z^2 - 2z^3) + \tilde{Q}^2 (3z^4 -2z^3) - \left(\frac{r_{h}}{L}\right)^2 (1+z^3) \\
p_{+}(z)&=2 \tilde{f}^2 + \frac{g}{2} = k(2z^2 - \frac{5}{2}z^3) + \tilde{Q}^2 (3z^4 -\frac{5}{2}z^3) - \left(\frac{r_{h}}{L}\right)^2 (\frac{5}{2}z^3 -1) \\
p_{-}(z)&= 2\tilde{f}^2 - \frac{g}{2} = k(2z^2 - \frac{3}{2}z^3) + \tilde{Q}^2 (3z^4 -\frac{3}{2}z^3) - \left(\frac{r_{h}}{L}\right)^2 (\frac{3}{2}z^3 -3).
\end{align*} 

The factor of $z^2$ in \eqref{eq.15} allows us to divide through this factor and gives

\begin{multline}
    (\tilde{f})^2\ddot{\tilde{\psi}}_{\pm}  + \frac{1}{zh}\left(\omega z^2 (p_{1}(z)) + \frac{qQ_{e}z}{r_h}(p_{2}(z))  + m \tilde{f}\frac{(p_{\pm}(z))}{z}\right)\dot{\tilde{\psi}}_{\pm} +\\ 
     \left[ \frac{(\omega r_h + qQ_{e}z)^{2}}{\tilde{f}^2} -(\frac{mr_h}{z})^2 +(\lambda )^{2} \pm\frac{\lambda}{zh}\left(\frac{\omega z^2}{2\tilde{f}}(p_{1}(z)) + \frac{qQ_{e}z}{r_h}(\frac{g}{2\tilde{f}}) \pm \frac{m \tilde{f}^2}{z}\right) \right] (\tilde{\psi_{\pm}}) = 0.
\end{multline}


\newpage



\subsection{Calculating Greens functions}
The avenue we could try is to follow the approach laid out in \cite{McGreevyetal} whereby we take our equations \eqref{eq.7} - \eqref{eq.8}  and organise them as follows 
\begin{align*}
    (\nabla_{r} \mp \frac{\lambda}{r})G_{\pm} =& - \Omega_{+}(F_{\mp}) \\
    (\nabla_{r} \mp \frac{\lambda}{r})F_{\pm} =& \ \Omega_{-}(G_{\mp}).
\end{align*}
Applying the same substitution as above 
\begin{equation*}
    G_{\pm} = \frac{\tilde{G}_{\pm}}{r\sqrt{f}} \quad \text{ and }
    \quad F_{\pm} = \frac{\tilde{F}_{\pm}}{r\sqrt{f}},
\end{equation*}
and labelling $K = \frac{r(\omega + A_t)}{f(r)}$ we have 
\begin{align}
    (rf(r)\partial_{r} \mp \lambda)\tilde{G}_{\pm} =& - (K + mr)\tilde{F}_{\mp} \label{eq.16} \\
    (rf(r)\partial_{r} \mp \lambda)\tilde{F}_{\pm} =& (K - mr)\tilde{G}_{\mp} \label{eq.17}.
\end{align}
and then introducing the ratios 
\begin{equation}
\chi_+ = \frac{\tilde{G}_{-}}{\tilde{F}_{+}}  \ \text{ and } \ \chi_- = \frac{\tilde{F}_{-}}{\tilde{G}_{+}}.
\end{equation}
we have, by substituting in to \eqref{eq.16} and \eqref{eq.17} and with a little rearranging, the equation 
\begin{align}
    f(r)\partial_{r}\chi_{\pm} &= -2\frac{\lambda}{r}\chi_{\pm} \mp \Omega_{\pm} \mp \Omega_{\mp}(\chi_{\pm})^{2} \\
    rf(r)\partial_{r}\chi_{\pm} &= -2\lambda\chi_{\pm} - (mr \pm K) + (mr \mp K)(\chi_{\pm})^{2}
\end{align}
Which should be easier to tackle numerically. This appears to be fairly close to what \cite{McGreevyetal} call their flow equations (24) with a different choice of potential and $m$ and $\lambda$ switched. 
We can see how these equations relate to those in \cite{McGreevyetal} by taking linear combinations of \eqref{eq.16} and \eqref{eq.17}. Expanding these out will make it easier to see:
\begin{align}
    (rf(r)\partial_{r} - \lambda)\tilde{G}_{+} =& (-K - mr)\tilde{F}_{-} \label{eq.18} \\
    (rf(r)\partial_{r} + \lambda)\tilde{F}_{-} =& (K - mr)\tilde{G}_{+} \label{eq.19}  \\   
    (rf(r)\partial_{r} + \lambda)\tilde{G}_{-} =& (-K - mr)\tilde{F}_{+} \label{eq.20} \\
    (rf(r)\partial_{r} - \lambda)\tilde{F}_{+} =& (K - mr)\tilde{G}_{-} \label{eq.21}     
\end{align}
then taking \eqref{eq.18} $\pm$ \eqref{eq.19} and \eqref{eq.20} $\mp$ \eqref{eq.21}, which gives
\begin{align}
    r(f(r)\partial_{r} + m)(\tilde{G}_{+} + \tilde{F}_{-}) =& (\lambda + K)(\tilde{G}_{+} -\tilde{F}_{-})  \\
    r(f(r)\partial_{r} - m)(\tilde{G}_{+} - \tilde{F}_{-}) =& (\lambda - K)(\tilde{G}_{+} +\tilde{F}_{-})  \\
    r(f(r)\partial_{r} - m)(\tilde{G}_{-} - \tilde{F}_{+}) =& -(\lambda + K)(\tilde{G}_{-} +\tilde{F}_{+})  \\
    r(f(r)\partial_{r} + m)(\tilde{G}_{-} + \tilde{F}_{+}) =& -(\lambda - K)(\tilde{G}_{-} -\tilde{F}_{+}) 
\end{align}
which when grouping the same relative signs of $K$ and $\lambda$ gives 
\begin{align}
    r(f(r)\partial_{r} \mp m)(\tilde{G}_{\pm} \mp \tilde{F}_{\mp}) =& \pm(\lambda - K)(\tilde{G}_{\pm} \pm \tilde{F}_{\mp}) \\
    r(f(r)\partial_{r} \pm m)(\tilde{G}_{\pm} \pm \tilde{F}_{\mp}) =& \pm(\lambda + K)(\tilde{G}_{\pm} \mp \tilde{F}_{\mp}).  
\end{align}
Now identifying $\frac{z_{\mp}}{i} = \tilde{G}_{\pm} \pm \tilde{F}_{\mp}$ and $y_{\pm} = \tilde{G}_{\pm} \mp \tilde{F}_{\mp}$ we have

\begin{align}
    r(f(r)\partial_{r} \mp m)y_{\pm} =& \mp i(\lambda - K)z_{\mp}  \label{eq.22}\\
    r(f(r)\partial_{r} \pm m)z_{\mp} =& \pm i(\lambda + K)y_{\pm}  \label{eq.23}
\end{align}

Which are exactly equations (20) and (21) from \cite{McGreevyetal} with $k_1 = \lambda$ and $u(r)=K(r)$. Then to arrive at what they refer to as their "flow equation" we take ratios of the above functions. 
\begin{equation}
\xi_{+} = \frac{iy_{-}}{z_{+}} = \frac{\tilde{G}_{-} + \tilde{F}_{+}}{\tilde{G}_{-} - \tilde{F}_{+}}, \quad \xi_{-} = \frac{-iz_{-}}{y_{+}} = -\frac{\tilde{G}_{+} + \tilde{F}_{-}}{\tilde{G}_{+} - \tilde{F}_{-}}
\end{equation} 
Which when subbed back in to equations \eqref{eq.22} and \eqref{eq.23} we have.
\begin{equation}
rf(r)\xi_{\pm}' = -2mr\xi_{\pm} \mp (\lambda \mp K) \pm (\lambda \pm K)\xi_{\pm} ^{2}
\end{equation}
Which is equation (24) in \cite{McGreevyetal}, with our notation for the functions in the metric. Now to obtain the boundary conditions we make the substitution, used in section 6.4 above, $z = \frac{r_{h}}{r}$ and noting the derivative with respect to $z$ in equation \eqref{eq.24} we have
\begin{align}
\frac{r_{h}}{z}f(z)(-\frac{z^2}{r_{h}})\dot{\xi}_{\pm}(z) &= -\frac{2mr_{h}}{z}\xi_{\pm}(z) \mp (\lambda \mp K(z)) \pm (\lambda \pm K(z))\xi_{\pm} ^{2}(z) \\
zf(z)\dot{\xi}_{\pm}(z) &= \frac{2mr_{h}}{z}\xi_{\pm}(z) \pm (\lambda \mp K(z)) \mp (\lambda \pm K(z))\xi_{\pm} ^{2}(z) .
\end{align}
Our function $f$ can be written as $f(z)^2 = \frac{\alpha^2 (1-z)}{z^2}h(z)^2$, as in equation \eqref{eq.25}. The function $h^2(z)$ is
\begin{align}
\alpha^2 h^2(z) &= \left(kz^2 - \tilde{Q}^2z^3 + \frac{r_{h}^2}{L^2} (1+z+z^2)\right) \\
h^2(z) &= \left(\frac{kz^2}{\alpha^2} - \frac{\tilde{Q}^2z^3}{\alpha^2} + 1+z+z^2 \right) \\
&= \frac{kz^2}{\alpha^2} - \frac{{Q}^2 z^3}{\alpha^4 L^2} + 1+z+z^2
\end{align}
Where we have introduced the parameter $\alpha = \frac{r_{h}}{L}$. Choosing our potential to match that in \cite{McGreevyetal} (with $q = \mu_{q}$) we have $f(z)K = \frac{r_{h}}{z}(\omega - \frac{q}{r_{h}}(1-z))$. This allows us to write the above as
\begin{align}
zf^2\dot{\xi}_{\pm} &= \frac{2mr_{h}f}{z}\xi_{\pm} \pm (\lambda f \mp fK) \mp (\lambda f \pm fK)\xi_{\pm} ^{2} \\
(1-z)h^2 \dot{\xi}_{\pm} &= \frac{2mL(1-z)^{\frac{1}{2}}}{z}h\xi_{\pm} \pm \frac{\lambda}{\alpha} (1-z)^{\frac{1}{2}}h(1-\xi_{\pm}^2) - (\frac{\omega L}{\alpha} - \frac{q}{\alpha^2}(1-z))(1+\xi_{\pm}^2) \label{eq.26}
\intertext{
where  in the last line we divide through by $\alpha^2 z$. Setting $L=1$ and redefining $\tilde{\omega} = \frac{\omega}{\alpha}$, $\tilde{\lambda} = \frac{\lambda}{\alpha}$ and $\tilde{q} = \frac{q}{\alpha^2}$ we have}
(1-z)h^2 \dot{\xi}_{\pm} &= \frac{2m(1-z)^{\frac{1}{2}}}{z}h\xi_{\pm} \pm \tilde{\lambda} (1-z)^{\frac{1}{2}}h(1-\xi_{\pm}^2) - (\tilde{\omega} - \tilde{q}(1-z))(1+\xi_{\pm}^2)
\end{align}
Now moving close to the horizon $z = 1 - \epsilon^2$, and $h^2(z)$ becomes
\begin{align}
h^2(z) &= \left(\frac{k}{\alpha^2} - \frac{{Q}^2}{\alpha^4} + 3 + \mathcal{O}(\epsilon^2) \right) \\
h^2(z) &= \tilde{h}^2 + \mathcal{O}(\epsilon^2)
\end{align}
Which, to lowest order is realted to the Hawking temperature by
\begin{equation}
\frac{4\pi T_{H}}{r_{h}} = \left(3+ \frac{k}{\alpha^2} - \frac{Q^2}{\alpha^4} \right) = \tilde{h}^2 \quad \rightarrow \quad T_{H} = \frac{\alpha}{4 \pi} \left(3+ \frac{k}{\alpha^2} - \frac{Q^2}{\alpha^4}\right)
\end{equation}
The derivative of $\xi_{\pm}$ become $\dot{\xi}_{\pm} = -\frac{1}{2\epsilon}\frac{\partial\xi_{\pm}}{\partial\epsilon}$ so our ODE looks like
\begin{align}
(-\frac{\epsilon}{2})h^2(z) \frac{\partial \xi_{\pm}}{\partial \epsilon} &= \frac{2m \epsilon}{(1-\epsilon^2)}h\xi_{\pm} \pm \tilde{\lambda} \epsilon h(1-\xi_{\pm}^2) - (\tilde{\omega} + \tilde{A}_{t}(z))(1+\xi_{\pm}^2) \\
-\frac{\epsilon}{2}h^2(z) \frac{\partial \xi_{\pm}}{\partial \epsilon} &= (2m \epsilon)h\xi_{\pm} \pm \tilde{\lambda} \epsilon h(1-\xi_{\pm}^2) - (\tilde{\omega} + \tilde{A}_{t}(z))(1+\xi_{\pm}^2) + \mathcal{O}(\epsilon^2).
\end{align}
Taylor expanding the function $\xi_{\pm}$ we have
\begin{align}
    \xi_{\pm}(1- \epsilon^2) &= \xi_{\pm}(1) + ((1-\epsilon^2) - 1)(\frac{-1}{2\epsilon})\frac{\partial \xi_{\pm}}{\partial \epsilon}(1) + \mathcal{O}(\epsilon^2) \\
    \xi_{\pm}(1- \epsilon^2) &= i + \epsilon\frac{\partial \xi_{\pm}}{\partial \epsilon}(1) + \mathcal{O}(\epsilon^2) \\
    (\xi_{\pm}(1- \epsilon^2))^2 &= -1 + 2i\epsilon\frac{\partial \xi_{\pm}}{\partial \epsilon}(1) + \mathcal{O}(\epsilon^2) \\
    1+(\xi_{\pm}(1- \epsilon^2))^2 &= 2i\epsilon\frac{\partial \xi_{\pm}}{\partial \epsilon}(1) + \mathcal{O}(\epsilon^2) \\
    1- (\xi_{\pm}(1- \epsilon^2))^2 &=  2- 2i\epsilon\frac{\partial \xi_{\pm}}{\partial \epsilon}(1) + \mathcal{O}(\epsilon^2)
\end{align}
with the ingoing boundary conditions at $u=1$, provided $\omega \ne 0$, $\xi_{\pm}(1) = i$. This can be obtained by setting $z = 1$ in equation \eqref{eq.26}. Our potential is $\tilde{A}_{t} = \tilde{q}(1-z)$, which vanishes at the horizon and is of order $\epsilon^2$ in our near horizon coordinates. Thus close to the horizon we have
\begin{align}
(-\frac{\epsilon}{2})\tilde{h}^2(z) \frac{\partial \xi_{\pm}}{\partial \epsilon} &= (2m)\tilde{h}(i\epsilon + \epsilon^2\frac{\partial \xi_{\pm}}{\partial \epsilon}) \pm \tilde{\lambda} \tilde{h}(2\epsilon - 2i\epsilon^2\frac{\partial \xi_{\pm}}{\partial \epsilon}) - (\tilde{\omega} + \tilde{q}\epsilon^2)(2i\epsilon\frac{\partial \xi_{\pm}}{\partial \epsilon}) + \mathcal{O}(\epsilon^3)\\
(-\frac{\epsilon \tilde{h}^2}{2})\frac{\partial \xi_{\pm}}{\partial \epsilon} &= 2\tilde{h} \epsilon (im \pm \tilde{\lambda}) - 2i\tilde{\omega} \epsilon \frac{\partial \xi_{\pm}}{\partial \epsilon} + \mathcal{O}(\epsilon^2)
\end{align}
which when looking at the lowest power of $\epsilon$ gives
\begin{equation}
\frac{\partial \xi_{\pm}}{\partial \epsilon}(1) = \frac{2\tilde{h}(im \pm \tilde{\lambda})}{2i\tilde{\omega} -\frac{\tilde{h}^2}{2}}
\end{equation}
and our boundary condition then is $\xi_{\pm}(1 - \epsilon^2) = i + \epsilon \frac{\partial \xi_{\pm}}{\partial \epsilon}(1)  $ for $\omega \ne 0$. Making $\epsilon$ appropriately small we should be able to get reasonable solutions from our numerical calculations. Which, when we set $m=0$ (to make the functions $\xi_{\pm}$ well behaved at $z=0$) and $k=0$ (as \cite{McGreevyetal} work on a flat event horizon), we find our calculations are in good agreement with results found in \cite{McGreevyetal}. Here we display the results aquired from our numerics which can be checked against their fig.1 and fig.3.

\begin{figure}[h]
\includegraphics[scale=0.27]{Images/ADS_CFT/fig2} 
\includegraphics[scale=0.27]{Images/ADS_CFT/fig3}
\caption{Here we have numerically solved the ODE in equation \eqref{eq.26} above for $z = 1 -(0.001)^2 \rightarrow 10^{-5}$ and saved only the final steps to obtain the greens functions $G_{ii} =\xi_{\pm}(0)$. We have done this for a range of values of the frequency $\omega$ and for fixed values of the planar eigenvalues $\lambda$ (planar as $k=0$, i.e. a flat event horizon).}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[scale=0.27]{Images/ADS_CFT/fig4}
\caption{Here $y1=Re[G_{22}]$ and $y2=Im[G_{22}]$  and we are plotting their behaviour again against $\omega$, but now for $\lambda = 0.9$ which is less than, but quite close to, the value of $\lambda_{f}$. This is what \cite{McGreevyetal} indentify as the value at which we see a fermi surface (hence the subscript f). Again we find consistency in our results with fig.3 from \cite{McGreevyetal}.}
\end{figure}

\newpage
These results afford us reasonable confidence that our numerics will give similarly accurate results when we vary other parameters. For example setting $k=1$ (giving a spherical event horizon) and adjusting the value of the electric charge on the black hole, $Q_{e}$, to ensure the temperature $T_{H} =0$ as in \cite{McGreevyetal} we see that we recover similar behaviour and obtain quasi-particle peaks in the same region of $\omega$ but at higher deviations from the vaccuum, in line with the interpretation of the above results from \cite{McGreevyetal}. This can be seen in the graphs below for the eigenvalues $\lambda = 1.2$ and $\lambda = 3$. 

\begin{figure}[h]
\includegraphics[scale=0.27]{Images/ADS_CFT/fig5} 
\includegraphics[scale=0.27]{Images/ADS_CFT/fig6}
\caption{Again we have numerically solved the ODE in equation \eqref{eq.26} and saved only the final steps to obtain the greens functions $G_{ii} =\xi_{\pm}(0)$. The general behaviour matches with the figures above but the peaks are higher for the same ranges of $\omega$}.
\end{figure}

These calculations are good for the massless case. What do we do if we want to look at the behaviour of these functions with non-zero mass? Well we employ a similar approach as above and delicately examine equation \eqref{eq.26} as we go further out to the boundary at $z=0$. We can't just sub in this value because the term with the mass diverges. If we multiply \eqref{eq.26} through by $z$ and then set it to zero we get

\begin{equation}
\xi_{\pm}(0) = 0
\end{equation}
provided $\dot{\xi}_{\pm}$ is finite at the boundary. This gives us little information about the behaviour of our functions as we appraoch the boundary. If we rearrange equation \eqref{eq.26} by dividing through by the factor infront of the $\dot{\xi}_{\pm}$ we have 
\begin{equation}
\dot{\xi}_{\pm} = \frac{2m}{z(1-z)^{\frac{1}{2}}h(z)}\xi_{\pm} \pm \frac{\tilde{\lambda}}{(1-z)^{\frac{1}{2}}h(z)}(1-\xi_{\pm}^{2}) - \frac{\tilde{\omega} -\tilde{q}(1-z)}{(1-z)h^2(z)}(1-\xi_{\pm}^{2}).
\end{equation}
If we first look at the behaviour of $h^{2}(z)$ close to zero. For $z=\delta$ we have
\begin{align}
h^2(z) &= \frac{kz^2}{\alpha^2} - \frac{{Q}^2 z^3}{\alpha^4 L^2} + 1+z+z^2 \\
&= 1 + \delta + \mathcal{O}(\delta^2) \\
\intertext{so near the boundary at $z=0$ we have}
h^2(z) &\approx 1 + \delta \\
h(z) &= (1+ \delta + \mathcal{O}(\delta^2))^\frac{1}{2} \approx 1 + \frac{\delta}{2} \quad \text{for sufficiently small $\delta$ } \\
(1-\delta)^{\frac{1}{2}} &\approx 1-\frac{\delta}{2}. 
\end{align}
Now we can look at our non-linear ODE near the boundary given these reasonable approximations for small $\delta$. 
\begin{align}
\dot{\xi}_{\pm} &= \frac{2m}{\delta(1-\frac{\delta}{2})(1+\frac{\delta}{2})}\xi_{\pm} \pm \frac{\tilde{\lambda}}{(1-\frac{\delta}{2})(1+\frac{\delta}{2})}(1-\xi_{\pm}^{2}) - \frac{\tilde{\omega} -\tilde{q}(1-\delta)}{(1-\delta)(1+\delta)}(1-\xi_{\pm}^{2})\\
\dot{\xi}_{\pm} &= \frac{2m}{\delta(1-\frac{\delta^2}{4})}\xi_{\pm} \pm \frac{\tilde{\lambda}}{(1-\frac{\delta^2}{4})}(1-\xi_{\pm}^{2}) - \left(\frac{\tilde{\omega}}{1-\delta^2} -\frac{\tilde{q}}{(1+\delta)}\right)(1-\xi_{\pm}^{2}).
\end{align}
Noting that $\xi_{\pm}(\delta)$ is close to zero (and well-behaved) then it seems reasonable to assume that $(\xi_{\pm}(\delta))^2$ would be closer again. So suppressing these terms and terms of order $\delta^2$ we can write our "near boundary" ODE as
\begin{equation}
\dot{\xi}_{\pm} = \frac{2m}{\delta}\xi_{\pm} \pm \tilde{\lambda} - \tilde{\omega} + \frac{\tilde{q}}{1+\delta}.
\end{equation}
Now we can tackle this ODE by treating $\delta$ as the variable, bringing the mass term across the equals and using an integrating factor. This gives 
\begin{equation}
\frac{d}{d\delta}\left(\delta^{-2m}\xi_{\pm}\right)=\left[\pm \tilde{\lambda} - \tilde{\omega} + \frac{\tilde{q}}{1+\delta}\right]\delta^{-2m}
\end{equation} 
Where upon integrating we have
\begin{equation}
\xi_{\pm} = \left(\frac{\pm \tilde{\lambda} - \tilde{\omega}}{1-2m}\right)\delta +\tilde{q}\delta^{2m}\int \frac{d\delta}{(1+\delta)(\delta^{2m})}
\end{equation}
The integral above can be tackled via a series expansion of $\frac{1}{1+\delta} = 1-\delta+\delta^2 -\delta^3 ...$ as $\delta < 1$. The integral becomes
\begin{equation}
\int \frac{d\delta}{(1+\delta)(\delta^{2m})} = \int d\delta \sum_{n=1}^{\infty} (-1)^{n-1}(\delta)^{n-1-2m} = \sum_{n=1}^{\infty} \frac{(-1)^{n-1}(\delta)^{n-2m}}{n-2m} + c_{\pm}
\end{equation} 
which, when multiplied by the factor of $\delta^{2m}$ infront we arrive at
\begin{equation}
\xi_{\pm} = \left(\frac{\pm \tilde{\lambda} - \tilde{\omega} +\tilde{q}}{1-2m}\right)\delta +c_{\pm}\delta^{2m}
\end{equation}
So as $z \rightarrow 0$ we have that $\xi_{\pm}$ must fall off like $z^{2m}$, where $0\leq m < \frac{1}{2}$.

